Investigating the true nature of three hard X-ray sources

Many of the new high energy sources discovered both by INTEGRAL/IBIS and Swift/BAT have been characterised thanks to extensive, multi-band follow-up campaigns, but there are still objects whose nature remains to be asserted. In this paper we investigate the true nature of three high energy sources, IGR J12134-6015, IGR J16058-7253 and Swift J2037.2+4151, employing multiwavelength data from the NIR to the X-rays. Through Gaia and ESO-VLT measurements and through Swift/XRT X-ray spectral analysis, we re-evaluate the classification for IGR J12134-6015, arguing that the source is a Galactic object and in particular a Cataclysmic Variable. We were able to confirm, thanks to NuSTAR observations, that the hard X-ray emission detected by INTEGRAL/IBIS and Swift/BAT from IGR J16058-7253 is coming from two Seyfert 2 galaxies which are both counterparts for this source. Through optical and X-ray spectral analysis of Swift J2037.2+4151 we find that this source is likely part of the rare and peculiar class of Symbiotic X-ray binaries and displays flux and spectral variability as well as interesting spectral features, such as a blending of several emission lines around the iron line complex.

==> biblio.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Created for Manuela Molina at 2021-04-29 17:11:00 +0200 


%% Saved with string encoding Unicode (UTF-8) 

@ARTICLE{landi11a,
       author = {{Landi}, R. and {Bassani}, L. and {Masetti}, N. and {Bazzano}, A. and {Bird}, A.~J.},
        title = "{Swift/XRT follow-up observations of unidentified INTEGRAL sources (1)}",
      journal = {The Astronomer's Telegram},
     keywords = {X-ray, Gamma Ray, Request for Observations, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2011,
        month = apr,
       volume = {3271},
        pages = {1},
archivePrefix = {arXiv},
       eprint = {1003.1214},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ATel.3271....1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tueller06,
       author = {{Tueller}, J. and {Markwardt}, C. and {Ajello}, M. and {Barthelmy}, S. and {Belloni}, T. and {Falcone}, A. and {Gehrels}, N. and {Godet}, O. and {Grupe}, D. and {Holland}, S. and {Kennea}, J. and {Mukai}, K. and {Mushotzky}, R. and {Sambruna}, R. and {Skinner}, G.~K.},
        title = "{Swift BAT Survey Reports 3 New Hard X-ray Sources Near the Galactic Plane}",
      journal = {The Astronomer's Telegram},
     keywords = {X-ray, Gamma Ray, Request for Observations, Transients},
         year = 2006,
        month = jul,
       volume = {853},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ATel..853....1T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fiocchi07,
       author = {{Fiocchi}, Mariateresa and {Bazzano}, Angela and {Ubertini}, Pietro and {Zdziarski}, Andrzej A.},
        title = "{The First Detection of Compton Reflection in the Low-Mass X-Ray Binary 4U 1705-44 with INTEGRAL and BeppoSax}",
      journal = {\apj},
     keywords = {Accretion, Accretion Disks, Gamma Rays: Observations, Radiation Mechanisms: Nonthermal, stars: individual (4U 1705 44), Stars: Neutron, X-Rays: Binaries, Astrophysics},
         year = 2007,
        month = mar,
       volume = {657},
       number = {1},
        pages = {448-452},
          doi = {10.1086/510573},
archivePrefix = {arXiv},
       eprint = {astro-ph/0611050},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...657..448F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{karasev12,
       author = {{Karasev}, D.~I. and {Lutovinov}, A.~A. and {Revnivtsev}, M.~G. and {Krivonos}, R.~A.},
        title = "{Accurate localization and identification of six hard X-ray sources from Chandra and XMM-Newton data}",
      journal = {Astronomy Letters},
     keywords = {X-ray sources, cataclysmic variables, neutron stars, active galactic nuclei, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = oct,
       volume = {38},
       number = {10},
        pages = {629-637},
          doi = {10.1134/S1063773712100039},
archivePrefix = {arXiv},
       eprint = {1209.2945},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012AstL...38..629K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{kormendy13,
       author = {{Kormendy}, John and {Ho}, Luis C.},
        title = "{Coevolution (Or Not) of Supermassive Black Holes and Host Galaxies}",
      journal = {\araa},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = aug,
       volume = {51},
       number = {1},
        pages = {511-653},
          doi = {10.1146/annurev-astro-082708-101811},
archivePrefix = {arXiv},
       eprint = {1304.7762},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ARA&A..51..511K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{demartino20,
       author = {{De Martino}, D. and {Bernardini}, F. and {Mukai}, K. and {Falanga}, M. and {Masetti}, N.},
        title = "{Hard X-ray cataclysmic variables}",
      journal = {Advances in Space Research},
     keywords = {X-Rays: binaries, Stars: cataclysmic variables, Accretion, Accretion discs, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = sep,
       volume = {66},
       number = {5},
        pages = {1209-1225},
          doi = {10.1016/j.asr.2019.09.006},
archivePrefix = {arXiv},
       eprint = {1909.06306},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AdSpR..66.1209D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{barthelmy05,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2005SSRv..120..143B},
	archiveprefix = {arXiv},
	author = {{Barthelmy}, Scott D. and {Barbier}, Louis M. and {Cummings}, Jay R. and {Fenimore}, Ed E. and {Gehrels}, Neil and {Hullinger}, Derek and {Krimm}, Hans A. and {Markwardt}, Craig B. and {Palmer}, David M. and {Parsons}, Ann and {Sato}, Goro and {Suzuki}, Masaya and {Takahashi}, Tadayuki and {Tashiro}, Makota and {Tueller}, Jack},
	date-added = {2021-04-29 17:10:46 +0200},
	date-modified = {2021-04-29 17:10:58 +0200},
	doi = {10.1007/s11214-005-5096-3},
	eprint = {astro-ph/0507410},
	journal = {\ssr},
	keywords = {gamma-ray, GRB, hard X-ray, survey, burst, afterglow, CZT, coded aperture, astrophysics, cosmology, Astrophysics},
	month = oct,
	number = {3-4},
	pages = {143-164},
	primaryclass = {astro-ph},
	title = {{The Burst Alert Telescope (BAT) on the SWIFT Midex Mission}},
	volume = {120},
	year = 2005,
	Bdsk-Url-1 = {https://doi.org/10.1007/s11214-005-5096-3}}

@article{babusieux18,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...616A..10G},
	archiveprefix = {arXiv},
	author = {{Babusiaux}, C. and {van Leeuwen}, F. and {Barstow}, M.~A. and {Jordi}, C. and {Vallenari}, A. and {Bossini}, D. and {Bressan}, A. and {Cantat-Gaudin}, T. and {van Leeuwen}, M. and {Brown}, A.~G.~A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Bailer-Jones}, C.~A.~L. and {Biermann}, M. and {Evans}, D.~W. and {Eyer}, L. and {Jansen}, F. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Siddiqui}, H.~I. and {Soubiran}, C. and {Walton}, N.~A. and {Arenou}, F. and {Bastian}, U. and {Cropper}, M. and {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {Chaoul}, L. and {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and {Guerra}, R. and {Holl}, B. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nienartowicz}, K. and {Panuzzo}, P. and {Portell}, J. and {Riello}, M. and {Seabroke}, G.~M. and {Tanga}, P. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Comoretto}, G. and {Garcia-Reinaldos}, M. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Audard}, M. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Burgess}, P. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Clementini}, G. and {Clotet}, M. and {Creevey}, O. and {Davidson}, M. and {De Ridder}, J. and {Delchambre}, L. and {Dell'Oro}, A. and {Ducourant}, C. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Galluccio}, L. and {Garc{\'\i}a-Torres}, M. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J.~J. and {Gosset}, E. and {Guy}, L.~P. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Hutton}, A. and {Jasniewicz}, G. and {Jean-Antoine-Piccolo}, A. and {Jordan}, S. and {Korn}, A.~J. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {Lebzelter}, T. and {L{\"o}ffler}, W. and {Manteiga}, M. and {Marrese}, P.~M. and {Mart{\'\i}n-Fleitas}, J.~M. and {Moitinho}, A. and {Mora}, A. and {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Richards}, P.~J. and {Rimoldini}, L. and {Robin}, A.~C. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {S{\"u}veges}, M. and {Torra}, J. and {van Reeven}, W. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aerts}, C. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alvarez}, R. and {Alves}, J. and {Anderson}, R.~I. and {Andrei}, A.~H. and {Anglada Varela}, E. and {Antiche}, E. and {Antoja}, T. and {Arcay}, B. and {Astraatmadja}, T.~L. and {Bach}, N. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balm}, P. and {Barache}, C. and {Barata}, C. and {Barbato}, D. and {Barblan}, F. and {Barklem}, P.~S. and {Barrado}, D. and {Barros}, M. and {Bartholom{\'e} Mu{\~n}oz}, L. and {Bassilana}, J. -L. and {Becciani}, U. and {Bellazzini}, M. and {Berihuete}, A. and {Bertone}, S. and {Bianchi}, L. and {Bienaym{\'e}}, O. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Boeche}, C. and {Bombrun}, A. and {Borrachero}, R. and {Bouquillon}, S. and {Bourda}, G. and {Bragaglia}, A. and {Bramante}, L. and {Breddels}, M.~A. and {Brouillet}, N. and {Br{\"u}semeister}, T. and {Brugaletta}, E. and {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {Cannizzaro}, G. and {Carballo}, R. and {Carlucci}, T. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cocozza}, G. and {Costigan}, G. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and {Crowley}, C. and {Cuypers}, J. and {Dafonte}, C. and {Damerdji}, Y. and {Dapergolas}, A. and {David}, P. and {David}, M. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {de Martino}, D. and {de Souza}, R. and {de Torres}, A. and {Debosscher}, J. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Drazinos}, P. and {Dur{\'a}n}, J. and {Edvardsson}, B. and {Enke}, H. and {Eriksson}, K. and {Esquej}, P. and {Eynard Bontemps}, G. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Falc{\~a}o}, A.~J. and {Farr{\`a}s Casas}, M. and {Federici}, L. and {Fedorets}, G. and {Fernique}, P. and {Figueras}, F. and {Filippi}, F. and {Findeisen}, K. and {Fonti}, A. and {Fraile}, E. and {Fraser}, M. and {Fr{\'e}zouls}, B. and {Gai}, M. and {Galleti}, S. and {Garabato}, D. and {Garc{\'\i}a-Sedano}, F. and {Garofalo}, A. and {Garralda}, N. and {Gavel}, A. and {Gavras}, P. and {Gerssen}, J. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Glass}, F. and {Gomes}, M. and {Granvik}, M. and {Gueguen}, A. and {Guerrier}, A. and {Guiraud}, J. and {Guti{\'e}}, R. and {Haigron}, R. and {Hatzidimitriou}, D. and {Hauser}, M. and {Haywood}, M. and {Heiter}, U. and {Helmi}, A. and {Heu}, J. and {Hilger}, T. and {Hobbs}, D. and {Hofmann}, W. and {Holland}, G. and {Huckle}, H.~E. and {Hypki}, A. and {Icardi}, V. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jonker}, P.~G. and {Juh{\'a}sz}, {\'A}. L. and {Julbe}, F. and {Karampelas}, A. and {Kewley}, A. and {Klar}, J. and {Kochoska}, A. and {Kohley}, R. and {Kolenberg}, K. and {Kontizas}, M. and {Kontizas}, E. and {Koposov}, S.~E. and {Kordopatis}, G. and {Kostrzewa-Rutkowska}, Z. and {Koubsky}, P. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Lavigne}, J. -B. and {Le Fustec}, Y. and {Le Poncin-Lafitte}, C. and {Lebreton}, Y. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Lenhardt}, H. and {Leroux}, F. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {L{\'o}pez}, M. and {Managau}, S. and {Mann}, R.~G. and {Mantelet}, G. and {Marchal}, O. and {Marchant}, J.~M. and {Marconi}, M. and {Marinoni}, S. and {Marschalk{\'o}}, G. and {Marshall}, D.~J. and {Martino}, M. and {Marton}, G. and {Mary}, N. and {Massari}, D. and {Matijevi{\v{c}}}, G. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and {Mulone}, A.~F. and {Muraveva}, T. and {Musella}, I. and {Nelemans}, G. and {Nicastro}, L. and {Noval}, L. and {O'Mullane}, W. and {Ord{\'e}novic}, C. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Osborne}, P. and {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and {Palacin}, H. and {Palaversa}, L. and {Panahi}, A. and {Pawlak}, M. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rambaux}, N. and {Ramos-Lerate}, M. and {Regibo}, S. and {Reyl{\'e}}, C. and {Riclet}, F. and {Ripepi}, V. and {Riva}, A. and {Rivard}, A. and {Rixon}, G. and {Roegiers}, T. and {Roelens}, M. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Ruiz-Dern}, L. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Sanna}, N. and {Santana-Ros}, T. and {Sarasso}, M. and {Savietto}, H. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Shih}, I. -C. and {Siltala}, L. and {Silva}, A.~F. and {Smart}, R.~L. and {Smith}, K.~W. and {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {Stoev}, H. and {Suess}, F.~F. and {Surdej}, J. and {Szabados}, L. and {Szegedi-Elek}, E. and {Tapiador}, D. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Terrett}, D. and {Teyssandier}, P. and {Thuillot}, W. and {Titarenko}, A. and {Torra Clotet}, F. and {Turon}, C. and {Ulla}, A. and {Utrilla}, E. and {Uzzi}, S. and {Vaillant}, M. and {Valentini}, G. and {Valette}, V. and {van Elteren}, A. and {Van Hemelryck}, E. and {Vaschetto}, M. and {Vecchiato}, A. and {Veljanoski}, J. and {Viala}, Y. and {Vicente}, D. and {Vogt}, S. and {von Essen}, C. and {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and {Walmsley}, G. and {Weiler}, M. and {Wertz}, O. and {Wevers}, T. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Ziaeepour}, H. and {Zorec}, J. and {Zschocke}, S. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T.},
	date-added = {2021-04-28 11:42:38 +0200},
	date-modified = {2021-04-28 11:43:39 +0200},
	doi = {10.1051/0004-6361/201832843},
	eid = {A10},
	eprint = {1804.09378},
	journal = {\aap},
	keywords = {parallaxes, Hertzsprung-Russell and C-M diagrams, solar neighborhood, stars: evolution, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
	month = aug,
	pages = {A10},
	primaryclass = {astro-ph.SR},
	title = {{Gaia Data Release 2. Observational Hertzsprung-Russell diagrams}},
	volume = {616},
	year = 2018,
	Bdsk-Url-1 = {https://doi.org/10.1051/0004-6361/201832843}}

@ARTICLE{bernardini12,
       author = {{Bernardini}, F. and {de Martino}, D. and {Falanga}, M. and {Mukai}, K. and {Matt}, G. and {Bonnet-Bidaud}, J. -M. and {Masetti}, N. and {Mouchet}, M.},
        title = "{Characterization of new hard X-ray cataclysmic variables}",
      journal = {\aap},
     keywords = {binaries: close, X-rays: binaries, accretion, accretion disks, novae, cataclysmic variables, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = jun,
       volume = {542},
          eid = {A22},
        pages = {A22},
          doi = {10.1051/0004-6361/201219233},
archivePrefix = {arXiv},
       eprint = {1204.3758},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...542A..22B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{chambers16,
       author = {{Chambers}, K.~C. and {Magnier}, E.~A. and {Metcalfe}, N. and {Flewelling}, H.~A. and {Huber}, M.~E. and {Waters}, C.~Z. and {Denneau}, L. and {Draper}, P.~W. and {Farrow}, D. and {Finkbeiner}, D.~P. and {Holmberg}, C. and {Koppenhoefer}, J. and {Price}, P.~A. and {Rest}, A. and {Saglia}, R.~P. and {Schlafly}, E.~F. and {Smartt}, S.~J. and {Sweeney}, W. and {Wainscoat}, R.~J. and {Burgett}, W.~S. and {Chastel}, S. and {Grav}, T. and {Heasley}, J.~N. and {Hodapp}, K.~W. and {Jedicke}, R. and {Kaiser}, N. and {Kudritzki}, R. -P. and {Luppino}, G.~A. and {Lupton}, R.~H. and {Monet}, D.~G. and {Morgan}, J.~S. and {Onaka}, P.~M. and {Shiao}, B. and {Stubbs}, C.~W. and {Tonry}, J.~L. and {White}, R. and {Ba{\~n}ados}, E. and {Bell}, E.~F. and {Bender}, R. and {Bernard}, E.~J. and {Boegner}, M. and {Boffi}, F. and {Botticella}, M.~T. and {Calamida}, A. and {Casertano}, S. and {Chen}, W. -P. and {Chen}, X. and {Cole}, S. and {Deacon}, N. and {Frenk}, C. and {Fitzsimmons}, A. and {Gezari}, S. and {Gibbs}, V. and {Goessl}, C. and {Goggia}, T. and {Gourgue}, R. and {Goldman}, B. and {Grant}, P. and {Grebel}, E.~K. and {Hambly}, N.~C. and {Hasinger}, G. and {Heavens}, A.~F. and {Heckman}, T.~M. and {Henderson}, R. and {Henning}, T. and {Holman}, M. and {Hopp}, U. and {Ip}, W. -H. and {Isani}, S. and {Jackson}, M. and {Keyes}, C.~D. and {Koekemoer}, A.~M. and {Kotak}, R. and {Le}, D. and {Liska}, D. and {Long}, K.~S. and {Lucey}, J.~R. and {Liu}, M. and {Martin}, N.~F. and {Masci}, G. and {McLean}, B. and {Mindel}, E. and {Misra}, P. and {Morganson}, E. and {Murphy}, D.~N.~A. and {Obaika}, A. and {Narayan}, G. and {Nieto-Santisteban}, M.~A. and {Norberg}, P. and {Peacock}, J.~A. and {Pier}, E.~A. and {Postman}, M. and {Primak}, N. and {Rae}, C. and {Rai}, A. and {Riess}, A. and {Riffeser}, A. and {Rix}, H.~W. and {R{\"o}ser}, S. and {Russel}, R. and {Rutz}, L. and {Schilbach}, E. and {Schultz}, A.~S.~B. and {Scolnic}, D. and {Strolger}, L. and {Szalay}, A. and {Seitz}, S. and {Small}, E. and {Smith}, K.~W. and {Soderblom}, D.~R. and {Taylor}, P. and {Thomson}, R. and {Taylor}, A.~N. and {Thakar}, A.~R. and {Thiel}, J. and {Thilker}, D. and {Unger}, D. and {Urata}, Y. and {Valenti}, J. and {Wagner}, J. and {Walder}, T. and {Walter}, F. and {Watters}, S.~P. and {Werner}, S. and {Wood-Vasey}, W.~M. and {Wyse}, R.},
        title = "{The Pan-STARRS1 Surveys}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = dec,
          eid = {arXiv:1612.05560},
        pages = {arXiv:1612.05560},
archivePrefix = {arXiv},
       eprint = {1612.05560},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016arXiv161205560C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{covey07,
       author = {{Covey}, K.~R. and {Ivezi{\'c}}, {\v{Z}}. and {Schlegel}, D. and {Finkbeiner}, D. and {Padmanabhan}, N. and {Lupton}, R.~H. and {Ag{\"u}eros}, M.~A. and {Bochanski}, J.~J. and {Hawley}, S.~L. and {West}, A.~A. and {Seth}, A. and {Kimball}, A. and {Gogarten}, S.~M. and {Claire}, M. and {Haggard}, D. and {Kaib}, N. and {Schneider}, D.~P. and {Sesar}, B.},
        title = "{Stellar SEDs from 0.3 to 2.5 {\ensuremath{\mu}}m: Tracing the Stellar Locus and Searching for Color Outliers in the SDSS and 2MASS}",
      journal = {\aj},
     keywords = {Galaxy: stellar content, infrared: stars, stars: early-type, stars: late-type, surveys, Astrophysics},
         year = 2007,
        month = dec,
       volume = {134},
       number = {6},
        pages = {2398-2417},
          doi = {10.1086/522052},
archivePrefix = {arXiv},
       eprint = {0707.4473},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007AJ....134.2398C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{li16,
       author = {{Li}, Jing and {Smith}, Martin C. and {Zhong}, Jing and {Hou}, Jinliang and {Carlin}, Jeffrey L. and {Newberg}, Heidi Jo and {Liu}, Chao and {Chen}, Li and {Li}, Linlin and {Shao}, Zhengyi and {Small}, Emma and {Tian}, Hao},
        title = "{Selecting M Giants with Infrared Photometry: Distances, Metallicities, and the Sagittarius Stream}",
      journal = {\apj},
     keywords = {galaxies: individual: Sagittarius, Galaxy: halo, Galaxy: structure, stars: abundances, stars: distances, stars: late-type, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = may,
       volume = {823},
       number = {1},
          eid = {59},
        pages = {59},
          doi = {10.3847/0004-637X/823/1/59},
archivePrefix = {arXiv},
       eprint = {1603.00262},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...823...59L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{wang19,
       author = {{Wang}, Shu and {Chen}, Xiaodian},
        title = "{The Optical to Mid-infrared Extinction Law Based on the APOGEE, Gaia DR2, Pan-STARRS1, SDSS, APASS, 2MASS, and WISE Surveys}",
      journal = {\apj},
     keywords = {dust, extinction, infrared: ISM, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = jun,
       volume = {877},
       number = {2},
          eid = {116},
        pages = {116},
          doi = {10.3847/1538-4357/ab1c61},
archivePrefix = {arXiv},
       eprint = {1904.04575},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...877..116W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%@article{demartino19,
%title = {Hard X-ray cataclysmic variables},
%journal = {Advances in Space Research},
%volume = {66},
%number = {5},
%pages = {1209-1225},
%year = {2020},
%note = {Nova Eruptions, Cataclysmic Variables and Related Systems: Challenges in the 2020 Era},
%issn = {0273-1177},
%doi = {https://doi.org/10.1016/j.asr.2019.09.006},
%url = {https://www.sciencedirect.com/science/article/pii/S0273117719306544},
%author = {D. {de Martino} and F. Bernardini and K. Mukai and M. Falanga and N. Masetti},
%keywords = {X-Rays: binaries, Stars: cataclysmic variables, Accretion, Accretion discs},
%}
@article{lusso12,
    author = {Lusso, E. and Comastri, A. and Simmons, B. D. and Mignoli, M. and Zamorani, G. and Vignali, C. and Brusa, M. and Shankar, F. and Lutz, D. and Trump, J. R. and Maiolino, R. and Gilli, R. and Bolzonella, M. and Puccetti, S. and Salvato, M. and Impey, C. D. and Civano, F. and Elvis, M. and Mainieri, V. and Silverman, J. D. and Koekemoer, A. M. and Bongiorno, A. and Merloni, A. and Berta, S. and Le Floc'h, E. and Magnelli, B. and Pozzi, F. and Riguccini, L.},
    title = "{Bolometric luminosities and Eddington ratios of X-ray selected active galactic nuclei in the XMM-COSMOS survey}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {425},
    number = {1},
    pages = {623-640},
    year = {2012},
    month = {09},
    issn = {0035-8711},
    doi = {10.1111/j.1365-2966.2012.21513.x},
    url = {https://doi.org/10.1111/j.1365-2966.2012.21513.x},
    eprint = {https://academic.oup.com/mnras/article-pdf/425/1/623/3222140/425-1-623.pdf},
}

@ARTICLE{brown21,
       author = {{Brown}, A.~G.~A. and {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and {Biermann}, M. and {Creevey}, O.~L. and {Evans}, D.~W. and {Eyer}, L. and {Hutton}, A. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Soubiran}, C. and {Walton}, N.~A. and {Arenou}, F. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Cropper}, M. and {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {van Leeuwen}, F. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {De Angeli}, F. and {Ducourant}, C. and {Fabricius}, C. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Guerra}, R. and {Guerrier}, A. and {Guiraud}, J. and {Jean-Antoine Piccolo}, A. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nicolas}, C. and {Nienartowicz}, K. and {Pailler}, F. and {Panuzzo}, P. and {Riclet}, F. and {Roux}, W. and {Seabroke}, G.~M. and {Sordo}, R. and {Tanga}, P. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Portell}, J. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Brugaletta}, E. and {Burgess}, P.~W. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Cheek}, N. and {Clementini}, G. and {Damerdji}, Y. and {Davidson}, M. and {Delchambre}, L. and {Dell'Oro}, A. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Galluccio}, L. and {Garc{\'\i}a-Lario}, P. and {Garcia-Reinaldos}, M. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gosset}, E. and {Haigron}, R. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hatzidimitriou}, D. and {Heiter}, U. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Holl}, B. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jordan}, S. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {L{\"o}ffler}, W. and {Lorca}, A. and {Manteiga}, M. and {Marchal}, O. and {Marrese}, P.~M. and {Moitinho}, A. and {Mora}, A. and {Muinonen}, K. and {Osborne}, P. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Richards}, P.~J. and {Riello}, M. and {Rimoldini}, L. and {Robin}, A.~C. and {Roegiers}, T. and {Rybizki}, J. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {Ulla}, A. and {Utrilla}, E. and {van Leeuwen}, M. and {van Reeven}, W. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aerts}, C. and {Aguado}, J.~J. and {Ajaj}, M. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {{\'A}lvarez Cid-Fuentes}, J. and {Alves}, J. and {Anderson}, R.~I. and {Anglada Varela}, E. and {Antoja}, T. and {Audard}, M. and {Baines}, D. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balbinot}, E. and {Balog}, Z. and {Barache}, C. and {Barbato}, D. and {Barros}, M. and {Barstow}, M.~A. and {Bartolom{\'e}}, S. and {Bassilana}, J. -L. and {Bauchet}, N. and {Baudesson-Stella}, A. and {Becciani}, U. and {Bellazzini}, M. and {Bernet}, M. and {Bertone}, S. and {Bianchi}, L. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Bombrun}, A. and {Bossini}, D. and {Bouquillon}, S. and {Bragaglia}, A. and {Bramante}, L. and {Breedt}, E. and {Bressan}, A. and {Brouillet}, N. and {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {C{\'a}novas}, H. and {Cantat-Gaudin}, T. and {Carballo}, R. and {Carlucci}, T. and {Carnerero}, M.~I. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Castro Sampol}, P. and {Chaoul}, L. and {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cioni}, M. -R.~L. and {Comoretto}, G. and {Cooper}, W.~J. and {Cornez}, T. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Dapergolas}, A. and {David}, M. and {David}, P. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {De Ridder}, J. and {de Souza}, R. and {de Teodoro}, P. and {de Torres}, A. and {del Peloso}, E.~F. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {Delisle}, J. -B. and {Di Matteo}, P. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Eappachen}, D. and {Edvardsson}, B. and {Enke}, H. and {Esquej}, P. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Fedorets}, G. and {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Fouron}, C. and {Fragkoudi}, F. and {Fraile}, E. and {Franke}, F. and {Gai}, M. and {Garabato}, D. and {Garcia-Gutierrez}, A. and {Garc{\'\i}a-Torres}, M. and {Garofalo}, A. and {Gavras}, P. and {Gerlach}, E. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomel}, R. and {Gomez}, A. and {Gonzalez-Santamaria}, I. and {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Hauser}, M. and {Haywood}, M. and {Helmi}, A. and {Hidalgo}, S.~L. and {Hilger}, T. and {H{\l}adczuk}, N. and {Hobbs}, D. and {Holland}, G. and {Huckle}, H.~E. and {Jasniewicz}, G. and {Jonker}, P.~G. and {Juaristi Campillo}, J. and {Julbe}, F. and {Karbevska}, L. and {Kervella}, P. and {Khanna}, S. and {Kochoska}, A. and {Kontizas}, M. and {Kordopatis}, G. and {Korn}, A.~J. and {Kostrzewa-Rutkowska}, Z. and {Kruszy{\'n}ska}, K. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Le Campion}, J. -F. and {Le Fustec}, Y. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {Madrero Pardo}, P. and {Managau}, S. and {Mann}, R.~G. and {Marchant}, J.~M. and {Marconi}, M. and {Marcos Santos}, M.~M.~S. and {Marinoni}, S. and {Marocco}, F. and {Marshall}, D.~J. and {Martin Polo}, L. and {Mart{\'\i}n-Fleitas}, J.~M. and {Masip}, A. and {Massari}, D. and {Mastrobuono-Battisti}, A. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Mints}, A. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and {Mulone}, A.~F. and {Munoz}, D. and {Muraveva}, T. and {Murphy}, C.~P. and {Musella}, I. and {Noval}, L. and {Ord{\'e}novic}, C. and {Orr{\`u}}, G. and {Osinde}, J. and {Pagani}, C. and {Pagano}, I. and {Palaversa}, L. and {Palicio}, P.~A. and {Panahi}, A. and {Pawlak}, M. and {Pe{\~n}alosa Esteller}, X. and {Penttil{\"a}}, A. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Poretti}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rainer}, M. and {Raiteri}, C.~M. and {Rambaux}, N. and {Ramos}, P. and {Ramos-Lerate}, M. and {Re Fiorentin}, P. and {Regibo}, S. and {Reyl{\'e}}, C. and {Ripepi}, V. and {Riva}, A. and {Rixon}, G. and {Robichon}, N. and {Robin}, C. and {Roelens}, M. and {Rohrbasser}, L. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Rybicki}, K.~A. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, A. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Samaras}, N. and {Sanchez Gimenez}, V. and {Sanna}, N. and {Santove{\~n}a}, R. and {Sarasso}, M. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Semeux}, D. and {Shahaf}, S. and {Siddiqui}, H.~I. and {Siebert}, A. and {Siltala}, L. and {Slezak}, E. and {Smart}, R.~L. and {Solano}, E. and {Solitro}, F. and {Souami}, D. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {S{\"u}veges}, M. and {Szabados}, L. and {Szegedi-Elek}, E. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Thuillot}, W. and {Tonello}, N. and {Torra}, F. and {Torra}, J. and {Turon}, C. and {Unger}, N. and {Vaillant}, M. and {van Dillen}, E. and {Vanel}, O. and {Vecchiato}, A. and {Viala}, Y. and {Vicente}, D. and {Voutsinas}, S. and {Weiler}, M. and {Wevers}, T. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {Yvard}, P. and {Zhao}, H. and {Zorec}, J. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T.},
        title = "{Gaia Early Data Release 3. Summary of the contents and survey properties}",
      journal = {\aap},
     keywords = {catalogs, astrometry, parallaxes, proper motions, techniques: photometric, techniques: radial velocities, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = may,
       volume = {649},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/202039657},
archivePrefix = {arXiv},
       eprint = {2012.01533},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...649A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@article{bar2019,
       author = {{B{\"a}r}, Rudolf E. and {Trakhtenbrot}, Benny and {Oh}, Kyuseok and {Koss}, Michael J. and {Wong}, O. Ivy and {Ricci}, Claudio and {Schawinski}, Kevin and {Weigel}, Anna K. and {Sartori}, Lia F. and {Ichikawa}, Kohei and {Secrest}, Nathan J. and {Stern}, Daniel and {Pacucci}, Fabio and {Mushotzky}, Richard and {Powell}, Meredith C. and {Ricci}, Federica and {Sani}, Eleonora and {Smith}, Krista L. and {Harrison}, Fiona A. and {Lamperti}, Isabella and {Urry}, C. Megan},
        title = "{BAT AGN Spectroscopic Survey - XIII. The nature of the most luminous obscured AGN in the low-redshift universe}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: nuclei, galaxies: Seyfert, radio continuum: galaxies, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = nov,
       volume = {489},
       number = {3},
        pages = {3073-3092},
          doi = {10.1093/mnras/stz2309},
archivePrefix = {arXiv},
       eprint = {1908.07546},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.489.3073B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
     
}


@ARTICLE{onori21,
       author = {{Onori}, F. and {Fiocchi}, M. and {Masetti}, N. and {Rojas}, A.~F. and {Bazzano}, A. and {Bassani}, L. and {Bird}, A.~J.},
        title = "{Multiwavelength observations of the Galactic X-ray binaries IGR J20155+3827 and Swift J1713.4-4219}",
      journal = {\mnras},
     keywords = {radiation mechanisms: non-thermal, stars: individual: IGR J20155+3827, Swift J1713.4-4219, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = may,
       volume = {503},
       number = {1},
        pages = {472-483},
          doi = {10.1093/mnras/stab315},
archivePrefix = {arXiv},
       eprint = {2102.01638},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.503..472O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{hackstein15,
       author = {{Hackstein}, M. and {Fein}, Ch. and {Haas}, M. and {Ramolla}, M. and {Pozo Nu{\~n}ez}, F. and {Barr Dom{\'\i}nguez}, A. and {Kaderhandt}, L. and {Thomsch}, K. and {Niedworok}, N. and {Westhues}, Ch. and {Chini}, R.},
        title = "{The Bochum Survey of the Southern Galactic Disk: II. Follow-up measurements and multi-filter photometry for 1323 square degrees monitored in 2010 - 2015}",
      journal = {Astronomische Nachrichten},
     keywords = {surveys, stars: variables: general, techniques: photometric, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = aug,
       volume = {336},
       number = {6},
        pages = {590-603},
          doi = {10.1002/asna.201512195},
archivePrefix = {arXiv},
       eprint = {1508.01701},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015AN....336..590H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{krivonos12,
       author = {{Krivonos}, R. and {Tsygankov}, S. and {Lutovinov}, A. and {Revnivtsev}, M. and {Churazov}, E. and {Sunyaev}, R.},
        title = "{INTEGRAL/IBIS nine-year Galactic hard X-ray survey}",
      journal = {\aap},
     keywords = {surveys, X-rays: general, catalogs, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = sep,
       volume = {545},
          eid = {A27},
        pages = {A27},
          doi = {10.1051/0004-6361/201219617},
archivePrefix = {arXiv},
       eprint = {1205.3941},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...545A..27K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{paliya19,
       author = {{Paliya}, Vaidehi S. and {Koss}, M. and {Trakhtenbrot}, B. and {Ricci}, C. and {Oh}, K. and {Ajello}, M. and {Stern}, D. and {Powell}, M.~C. and {Urry}, C.~M. and {Harrison}, F. and {Lamperti}, I. and {Mushotzky}, R. and {Marcotulli}, L. and {Mej{\'\i}a-Restrepo}, J. and {Hartmann}, D.},
        title = "{BAT AGN Spectroscopic Survey. XVI. General Physical Characteristics of BAT Blazars}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: jets, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = aug,
       volume = {881},
       number = {2},
          eid = {154},
        pages = {154},
          doi = {10.3847/1538-4357/ab2f8b},
archivePrefix = {arXiv},
       eprint = {1907.01082},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...881..154P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{chen20,
	doi = {10.3847/1538-4365/ab9cae},
	url = {https://doi.org/10.3847/1538-4365/ab9cae},
	year = 2020,
	month = {jul},
	publisher = {American Astronomical Society},
	volume = {249},
	number = {1},
	pages = {18},
	author = {Xiaodian Chen and Shu Wang and Licai Deng and Richard de Grijs and Ming Yang and Hao Tian},
	title = {The Zwicky Transient Facility Catalog of Periodic Variable Stars},
	journal = {\apjs}

}


@ARTICLE{saxton08,
       author = {{Saxton}, R.~D. and {Read}, A.~M. and {Esquej}, P. and {Freyberg}, M.~J. and {Altieri}, B. and {Bermejo}, D.},
        title = "{The first XMM-Newton slew survey catalogue: XMMSL1}",
      journal = {\aap},
     keywords = {X-rays: general, surveys, catalogs, Astrophysics},
         year = 2008,
        month = mar,
       volume = {480},
       number = {2},
        pages = {611-622},
          doi = {10.1051/0004-6361:20079193},
archivePrefix = {arXiv},
       eprint = {0801.3732},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...480..611S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{baumgartner13,
       author = {{Baumgartner}, W.~H. and {Tueller}, J. and {Markwardt}, C.~B. and {Skinner}, G.~K. and {Barthelmy}, S. and {Mushotzky}, R.~F. and {Evans}, P.~A. and {Gehrels}, N.},
        title = "{The 70 Month Swift-BAT All-sky Hard X-Ray Survey}",
      journal = {\apjs},
     keywords = {catalogs, surveys, X-rays: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = aug,
       volume = {207},
       number = {2},
          eid = {19},
        pages = {19},
          doi = {10.1088/0067-0049/207/2/19},
archivePrefix = {arXiv},
       eprint = {1212.3336},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJS..207...19B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oh18,
       author = {{Oh}, Kyuseok and {Koss}, Michael and {Markwardt}, Craig B. and {Schawinski}, Kevin and {Baumgartner}, Wayne H. and {Barthelmy}, Scott D. and {Cenko}, S. Bradley and {Gehrels}, Neil and {Mushotzky}, Richard and {Petulante}, Abigail and {Ricci}, Claudio and {Lien}, Amy and {Trakhtenbrot}, Benny},
        title = "{The 105-Month Swift-BAT All-sky Hard X-Ray Survey}",
      journal = {\apjs},
     keywords = {catalogs, surveys, X-rays: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = mar,
       volume = {235},
       number = {1},
          eid = {4},
        pages = {4},
          doi = {10.3847/1538-4365/aaa7fd},
archivePrefix = {arXiv},
       eprint = {1801.01882},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..235....4O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{predehl95,
       author = {{Predehl}, P. and {Schmitt}, J.~H.~M.~M.},
        title = "{X-raying the interstellar medium: ROSAT observations of dust scattering halos.}",
      journal = {\aap},
     keywords = {INTERSTELLAR MEDIUM: DUST, ISM: CAS A, X-RAYS: ISM},
         year = 1995,
        month = jan,
       volume = {500},
        pages = {459-475},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995A&A...293..889P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{smith07,
       author = {{Smith}, Randall K. and {Bautz}, Mark W. and {Edgar}, Richard J. and {Fujimoto}, Ryuichi and {Hamaguchi}, Kenji and {Hughes}, John P. and {Ishida}, Manabu and {Kelley}, Richard and {Kilbourne}, Caroline A. and {Kuntz}, K.~D. and {McCammon}, Dan and {Miller}, Eric and {Mitsuda}, Kazuhisa and {Mukai}, Koji and {Plucinsky}, Paul P. and {Porter}, F. Scott and {Snowden}, Steve L. and {Takei}, Yoh and {Terada}, Yukikatsu and {Tsuboi}, Yohko and {Yamasaki}, Noriko Y.},
        title = "{Suzaku Observations of the Local and Distant Hot ISM}",
      journal = {\pasj},
     keywords = {ISM: bubbles, plasmas, X-rays: ISM, Astrophysics},
         year = 2007,
        month = jan,
       volume = {59},
        pages = {141-150},
          doi = {10.1093/pasj/59.sp1.S141},
archivePrefix = {arXiv},
       eprint = {astro-ph/0609832},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007PASJ...59S.141S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mukai16,
       author = {{Mukai}, K. and {Luna}, G.~J.~M. and {Cusumano}, G. and {Segreto}, A. and {Munari}, U. and {Sokoloski}, J.~L. and {Lucy}, A.~B. and {Nelson}, T. and {Nu{\~n}ez}, N.~E.},
        title = "{SU Lyncis, a hard X-ray bright M giant: clues point to a large hidden population of symbiotic stars}",
      journal = {\mnras},
     keywords = {binaries: symbiotic, stars: individual: SU Lyn, X-rays: binaries, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = sep,
       volume = {461},
       number = {1},
        pages = {L1-L5},
          doi = {10.1093/mnrasl/slw087},
archivePrefix = {arXiv},
       eprint = {1604.08483},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.461L...1M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{masetti07,
       author = {{Masetti}, N. and {Landi}, R. and {Pretorius}, M.~L. and {Sguera}, V. and {Bird}, A.~J. and {Perri}, M. and {Charles}, P.~A. and {Kennea}, J.~A. and {Malizia}, A. and {Ubertini}, P.},
        title = "{IGR J16194-2810: a new symbiotic X-ray binary}",
      journal = {\aap},
     keywords = {astrometry, stars: binaries: general, X-rays: binaries, stars: neutron, stars: individual: IGR J16194-2810, Astrophysics},
         year = 2007,
        month = jul,
       volume = {470},
       number = {1},
        pages = {331-337},
          doi = {10.1051/0004-6361:20077509},
archivePrefix = {arXiv},
       eprint = {0704.3682},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&A...470..331M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{paizis06,
       author = {{Paizis}, A. and {Farinelli}, R. and {Titarchuk}, L. and {Courvoisier}, T.~J. -L. and {Bazzano}, A. and {Beckmann}, V. and {Frontera}, F. and {Goldoni}, P. and {Kuulkers}, E. and {Mereghetti}, S. and {Rodriguez}, J. and {Vilhu}, O.},
        title = "{Average hard X-ray emission from NS LMXBs: observational evidence of different spectral states in NS LMXBs}",
      journal = {\aap},
     keywords = {X-rays: binaries, binaries: close, stars: neutron, Astrophysics},
         year = 2006,
        month = nov,
       volume = {459},
       number = {1},
        pages = {187-197},
          doi = {10.1051/0004-6361:20065792},
archivePrefix = {arXiv},
       eprint = {astro-ph/0607592},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006A&A...459..187P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{danehkar21,
       author = {{Danehkar}, A. and {Karovska}, M. and {Drake}, J.~J. and {Kashyap}, V.~L.},
        title = "{Long-term X-ray variability of the symbiotic system RT Cru based on Chandra spectroscopy}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, binaries: symbiotic, stars: individual: (RT Cru), Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = feb,
       volume = {500},
       number = {4},
        pages = {4801-4817},
          doi = {10.1093/mnras/staa3554},
archivePrefix = {arXiv},
       eprint = {2011.07390},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.500.4801D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{gualandi01,
       author = {{Gualandi}, R. \& {Merighi}, R.},
        title = "{Bologna Astronomical Observatory Technical Report, v2.0}",
         year = 2001

}


@ARTICLE{vernet11,
       author = {{Vernet}, J. and {Dekker}, H. and {D'Odorico}, S. and {Kaper}, L. and {Kjaergaard}, P. and {Hammer}, F. and {Randich}, S. and {Zerbi}, F. and {Groot}, P.~J. and {Hjorth}, J. and {Guinouard}, I. and {Navarro}, R. and {Adolfse}, T. and {Albers}, P.~W. and {Amans}, J. -P. and {Andersen}, J.~J. and {Andersen}, M.~I. and {Binetruy}, P. and {Bristow}, P. and {Castillo}, R. and {Chemla}, F. and {Christensen}, L. and {Conconi}, P. and {Conzelmann}, R. and {Dam}, J. and {de Caprio}, V. and {de Ugarte Postigo}, A. and {Delabre}, B. and {di Marcantonio}, P. and {Downing}, M. and {Elswijk}, E. and {Finger}, G. and {Fischer}, G. and {Flores}, H. and {Fran{\c{c}}ois}, P. and {Goldoni}, P. and {Guglielmi}, L. and {Haigron}, R. and {Hanenburg}, H. and {Hendriks}, I. and {Horrobin}, M. and {Horville}, D. and {Jessen}, N.~C. and {Kerber}, F. and {Kern}, L. and {Kiekebusch}, M. and {Kleszcz}, P. and {Klougart}, J. and {Kragt}, J. and {Larsen}, H.~H. and {Lizon}, J. -L. and {Lucuix}, C. and {Mainieri}, V. and {Manuputy}, R. and {Martayan}, C. and {Mason}, E. and {Mazzoleni}, R. and {Michaelsen}, N. and {Modigliani}, A. and {Moehler}, S. and {M{\o}ller}, P. and {Norup S{\o}rensen}, A. and {N{\o}rregaard}, P. and {P{\'e}roux}, C. and {Patat}, F. and {Pena}, E. and {Pragt}, J. and {Reinero}, C. and {Rigal}, F. and {Riva}, M. and {Roelfsema}, R. and {Royer}, F. and {Sacco}, G. and {Santin}, P. and {Schoenmaker}, T. and {Spano}, P. and {Sweers}, E. and {Ter Horst}, R. and {Tintori}, M. and {Tromp}, N. and {van Dael}, P. and {van der Vliet}, H. and {Venema}, L. and {Vidali}, M. and {Vinther}, J. and {Vola}, P. and {Winters}, R. and {Wistisen}, D. and {Wulterkens}, G. and {Zacchei}, A.},
        title = "{X-shooter, the new wide band intermediate resolution spectrograph at the ESO Very Large Telescope}",
      journal = {\aap},
     keywords = {instrumentation: spectrographs, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = dec,
       volume = {536},
          eid = {A105},
        pages = {A105},
          doi = {10.1051/0004-6361/201117752},
archivePrefix = {arXiv},
       eprint = {1110.1944},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...536A.105V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{landi09,
       author = {{Landi}, R. and {Bassani}, L. and {Dean}, A.~J. and {Bird}, A.~J. and {Fiocchi}, M. and {Bazzano}, A. and {Nousek}, J.~A. and {Osborne}, J.~P.},
        title = "{INTEGRAL/IBIS and Swift/XRT observations of hard cataclysmic variables}",
      journal = {\mnras},
     keywords = {novae, cataclysmic variables, gamma-rays: observations, X-rays: binaries, Astrophysics},
         year = 2009,
        month = jan,
       volume = {392},
       number = {2},
        pages = {630-640},
          doi = {10.1111/j.1365-2966.2008.14086.x},
archivePrefix = {arXiv},
       eprint = {0810.1844},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.392..630L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@BOOK{lang92,
       author = {{Lang}, Kenneth R.},
        title = "{Astrophysical Data I. Planets and Stars.}",
         year = 1992,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992adps.book.....L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bodaghee12,
       author = {{Bodaghee}, A. and {Tomsick}, J.~A. and {Rodriguez}, J. and {James}, J.~B.},
        title = "{Clustering between High-mass X-Ray Binaries and OB Associations in the Milky Way}",
      journal = {\apj},
     keywords = {Galaxy: stellar content, open clusters and associations: general, stars: massive, stars: neutron, supergiants, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = jan,
       volume = {744},
       number = {2},
          eid = {108},
        pages = {108},
          doi = {10.1088/0004-637X/744/2/108},
archivePrefix = {arXiv},
       eprint = {1109.3466},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...744..108B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{ducati01,
       author = {{Ducati}, Jorge R. and {Bevilacqua}, Claudio M. and {Rembold}, Sandro B. and {Ribeiro}, Daiana},
        title = "{Intrinsic Colors of Stars in the Near-Infrared}",
      journal = {\apj},
     keywords = {Infrared: Stars, Stars: Fundamental Parameters, Techniques: Photometric},
         year = 2001,
        month = sep,
       volume = {558},
       number = {1},
        pages = {309-322},
          doi = {10.1086/322439},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...558..309D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{schlafly11,
       author = {{Schlafly}, Edward F. and {Finkbeiner}, Douglas P.},
        title = "{Measuring Reddening with Sloan Digital Sky Survey Stellar Spectra and Recalibrating SFD}",
      journal = {\apj},
     keywords = {dust, extinction, Galaxy: stellar content, ISM: clouds, Astrophysics - Galaxy Astrophysics},
         year = 2011,
        month = aug,
       volume = {737},
       number = {2},
          eid = {103},
        pages = {103},
          doi = {10.1088/0004-637X/737/2/103},
archivePrefix = {arXiv},
       eprint = {1012.4804},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...737..103S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{skrutskie06,
       author = {{Skrutskie}, M.~F. and {Cutri}, R.~M. and {Stiening}, R. and {Weinberg}, M.~D. and {Schneider}, S. and {Carpenter}, J.~M. and {Beichman}, C. and {Capps}, R. and {Chester}, T. and {Elias}, J. and {Huchra}, J. and {Liebert}, J. and {Lonsdale}, C. and {Monet}, D.~G. and {Price}, S. and {Seitzer}, P. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and {Gizis}, J.~E. and {Howard}, E. and {Evans}, T. and {Fowler}, J. and {Fullmer}, L. and {Hurt}, R. and {Light}, R. and {Kopan}, E.~L. and {Marsh}, K.~A. and {McCallon}, H.~L. and {Tam}, R. and {Van Dyk}, S. and {Wheelock}, S.},
        title = "{The Two Micron All Sky Survey (2MASS)}",
      journal = {\aj},
     keywords = {Catalogs, Infrared: General, Surveys},
         year = 2006,
        month = feb,
       volume = {131},
       number = {2},
        pages = {1163-1183},
          doi = {10.1086/498708},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006AJ....131.1163S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{warner95,
       author = {{Warner}, Brian},
        title = "{Cataclysmic variable stars}",
         year = 1995,
       volume = {28},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995cvs..book.....W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{enoto14,
       author = {{Enoto}, Teruaki and {Sasano}, Makoto and {Yamada}, Shin'ya and {Tamagawa}, Toru and {Makishima}, Kazuo and {Pottschmidt}, Katja and {Marcu}, Diana and {Corbet}, Robin H.~D. and {Fuerst}, Felix and {Wilms}, J{\"o}rn},
        title = "{Spectral and Timing Nature of the Symbiotic X-Ray Binary 4U 1954+319: The Slowest Rotating Neutron Star in an X-Ray Binary System}",
      journal = {\apj},
     keywords = {accretion, accretion disks, binaries: symbiotic, magnetic fields, stars: individual: 3A 1954+319 4U 1954+319, stars: neutron, X-rays : binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = may,
       volume = {786},
       number = {2},
          eid = {127},
        pages = {127},
          doi = {10.1088/0004-637X/786/2/127},
archivePrefix = {arXiv},
       eprint = {1404.0134},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...786..127E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{abril20,
       author = {{Abril}, Javier and {Schmidtobreick}, Linda and {Ederoclite}, Alessandro and {L{\'o}pez-Sanjuan}, Carlos},
        title = "{Disentangling cataclysmic variables in Gaia's HR diagram}",
      journal = {\mnras},
     keywords = {Hertzsprung, Russell and colour, magnitude diagrams, novae, cataclysmic variables, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = feb,
       volume = {492},
       number = {1},
        pages = {L40-L44},
          doi = {10.1093/mnrasl/slz181},
archivePrefix = {arXiv},
       eprint = {1912.01531},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.492L..40A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sazonov20,
       author = {{Sazonov}, S. and {Paizis}, A. and {Bazzano}, A. and {Chelovekov}, I. and {Khabibullin}, I. and {Postnov}, K. and {Mereminskiy}, I. and {Fiocchi}, M. and {B{\'e}langer}, G. and {Bird}, A.~J. and {Bozzo}, E. and {Chenevez}, J. and {Santo}, M. Del and {Falanga}, M. and {Farinelli}, R. and {Ferrigno}, C. and {Grebenev}, S. and {Krivonos}, R. and {Kuulkers}, E. and {Lund}, N. and {Sanchez-Fernandez}, C. and {Tarana}, A. and {Ubertini}, P. and {Wilms}, J.},
        title = "{The Galactic LMXB Population and the Galactic Centre Region}",
      journal = {\nar},
     keywords = {X-ray binaries, INTEGRAL observatory, Accretion, Black holes, Neutron stars, Sgr A*, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = jun,
       volume = {88},
          eid = {101536},
        pages = {101536},
          doi = {10.1016/j.newar.2020.101536},
archivePrefix = {arXiv},
       eprint = {2006.05063},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020NewAR..8801536S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{comeron05,
       author = {{Comer{\'o}n}, F. and {Pasquali}, A.},
        title = "{The ionizing star of the North America and Pelican nebulae}",
      journal = {\aap},
     keywords = {ISM: HII regions, ISM: individual objects: NGC 7000, ISM: individual objects: IC 5070, ISM: individual objects: W80},
         year = 2005,
        month = feb,
       volume = {430},
        pages = {541-548},
          doi = {10.1051/0004-6361:20041788},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...430..541C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{reig16,
       author = {{Reig}, P. and {Milonaki}, F.},
        title = "{Accretion regimes in the X-ray pulsar 4U 1901+03}",
      journal = {\aap},
     keywords = {stars: emission-line, Be, X-rays: binaries, stars: neutron, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = oct,
       volume = {594},
          eid = {A45},
        pages = {A45},
          doi = {10.1051/0004-6361/201629200},
archivePrefix = {arXiv},
       eprint = {1608.06118},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...594A..45R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{negueruela07,
       author = {{Negueruela}, I. and {Schurch}, M.~P.~E.},
        title = "{A search for counterparts to massive X-ray binaries using photometric catalogues}",
      journal = {\aap},
     keywords = {binaries: close, stars: supergiants, X-rays: binaries, stars: emission line, Be, Astrophysics},
         year = 2007,
        month = jan,
       volume = {461},
       number = {2},
        pages = {631-639},
          doi = {10.1051/0004-6361:20066054},
archivePrefix = {arXiv},
       eprint = {astro-ph/0610006},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&A...461..631N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{krivonos21,
       author = {{Krivonos}, Roman A. and {Bird}, Antony J. and {Churazov}, Eugene M. and {Tomsick}, John A. and {Bazzano}, Angela and {Beckmann}, Volker and {B{\'e}langer}, Guillaume and {Bodaghee}, Arash and {Chaty}, Sylvain and {Kuulkers}, Erik and {Lutovinov}, Alexander and {Malizia}, Angela and {Masetti}, Nicola and {Mereminskiy}, Ilya A. and {Sunyaev}, Rashid and {Tsygankov}, Sergey S. and {Ubertini}, Pietro and {Winkler}, Christoph},
        title = "{15 years of galactic surveys and hard X-ray background measurements}",
      journal = {\nar},
     keywords = {X-ray surveys, Cosmic X-ray background, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = jun,
       volume = {92},
          eid = {101612},
        pages = {101612},
          doi = {10.1016/j.newar.2021.101612},
archivePrefix = {arXiv},
       eprint = {2101.09052},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021NewAR..9201612K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{lutovinov20,
       author = {{Lutovinov}, Alexander and {Suleimanov}, Valery and {Manuel Luna}, Gerardo Juan and {Sazonov}, Sergey and {de Martino}, Domitilla and {Ducci}, Lorenzo and {Doroshenko}, Victor and {Falanga}, Maurizio},
        title = "{INTEGRAL View on cataclysmic variables and symbiotic binaries}",
      journal = {\nar},
     keywords = {Cataclysmic variables, Symbiotic stars, X-Ray, White dwarfs, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = dec,
       volume = {91},
          eid = {101547},
        pages = {101547},
          doi = {10.1016/j.newar.2020.101547},
archivePrefix = {arXiv},
       eprint = {2008.10665},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020NewAR..9101547L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{landi17,
       author = {{Landi}, R. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A.~J. and {Fiocchi}, M. and {Malizia}, A. and {Panessa}, F. and {Sguera}, V. and {Ubertini}, P.},
        title = "{Investigating the X-ray counterparts to unidentified sources in the 1000-orbit INTEGRAL/IBIS catalogue}",
      journal = {\mnras},
     keywords = {gamma-rays: general, X-rays: general, Astrophysics - High Energy Astrophysical Phenomena, High Energy Physics - Phenomenology},
         year = 2017,
        month = sep,
       volume = {470},
       number = {1},
        pages = {1107-1120},
          doi = {10.1093/mnras/stx908},
archivePrefix = {arXiv},
       eprint = {1704.03872},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.470.1107L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{malizia20,
       author = {{Malizia}, Angela and {Sazonov}, Sergey and {Bassani}, Loredana and {Pian}, Elena and {Beckmann}, Volker and {Molina}, Manuela and {Mereminskiy}, Ilya and {Belanger}, Guillaume},
        title = "{INTEGRAL view of AGN}",
      journal = {\nar},
     keywords = {INTEGRAL, AGN, Seyferts, Blazars, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = nov,
       volume = {90},
          eid = {101545},
        pages = {101545},
          doi = {10.1016/j.newar.2020.101545},
archivePrefix = {arXiv},
       eprint = {2009.03232},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020NewAR..9001545M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{kretschmar19,
       author = {{Kretschmar}, Peter and {F{\"u}rst}, Felix and {Sidoli}, Lara and {Bozzo}, Enrico and {Alfonso-Garz{\'o}n}, Julia and {Bodaghee}, Arash and {Chaty}, Sylvain and {Chernyakova}, Masha and {Ferrigno}, Carlo and {Manousakis}, Antonios and {Negueruela}, Ignacio and {Postnov}, Konstantin and {Paizis}, Adamantia and {Reig}, Pablo and {Rodes-Roca}, Jos{\'e} Joaqu{\'\i}n and {Tsygankov}, Sergey and {Bird}, Antony J. and {Bissinger n{\'e} K{\"u}hnel}, Matthias and {Blay}, Pere and {Caballero}, Isabel and {Coe}, Malcolm J. and {Domingo}, Albert and {Doroshenko}, Victor and {Ducci}, Lorenzo and {Falanga}, Maurizio and {Grebenev}, Sergei A. and {Grinberg}, Victoria and {Hemphill}, Paul and {Kreykenbohm}, Ingo and {Kreykenbohm n{\'e} Fritz}, Sonja and {Li}, Jian and {Lutovinov}, Alexander A. and {Mart{\'\i}nez-N{\'u}{\~n}ez}, Silvia and {Mas-Hesse}, J. Miguel and {Masetti}, Nicola and {McBride}, Vanessa A. and {Neronov}, Andrii and {Pottschmidt}, Katja and {Rodriguez}, J{\'e}r{\^o}me and {Romano}, Patrizia and {Rothschild}, Richard E. and {Santangelo}, Andrea and {Sguera}, Vito and {Staubert}, R{\"u}diger and {Tomsick}, John A. and {Torrej{\'o}n}, Jos{\'e} Miguel and {Torres}, Diego F. and {Walter}, Roland and {Wilms}, J{\"o}rn and {Wilson-Hodge}, Colleen A. and {Zhang}, Shu},
        title = "{Advances in Understanding High-Mass X-ray Binaries with INTEGRALand Future Directions}",
      journal = {\nar},
     keywords = {X-rays: binaries, accretion, stars: neutron, pulsars: general, gamma rays: observations, INTEGRAL observatory, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = dec,
       volume = {86},
          eid = {101546},
        pages = {101546},
          doi = {10.1016/j.newar.2020.101546},
archivePrefix = {arXiv},
       eprint = {2009.03244},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019NewAR..8601546K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{eyer19,
       author = {{Eyer}, L. and {Rimoldini}, L. and {Audard}, M. and {Anderson}, R.~I. and {Nienartowicz}, K. and {Glass}, F. and {Marchal}, O. and {Grenon}, M. and {Mowlavi}, N. and {Holl}, B. and {Clementini}, G. and {Aerts}, C. and {Mazeh}, T. and {Evans}, D.~W. and {Szabados}, L. and {Brown}, A.~G.~A. and {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and {Bailer-Jones}, C.~A.~L. and {Biermann}, M. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Siddiqui}, H.~I. and {Soubiran}, C. and {van Leeuwen}, F. and {Walton}, N.~A. and {Arenou}, F. and {Bastian}, U. and {Cropper}, M. and {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {Chaoul}, L. and {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and {Guerra}, R. and {Masana}, E. and {Messineo}, R. and {Panuzzo}, P. and {Portell}, J. and {Riello}, M. and {Seabroke}, G.~M. and {Tanga}, P. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Comoretto}, G. and {Garcia-Reinaldos}, M. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Burgess}, P. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Clotet}, M. and {Creevey}, O. and {Davidson}, M. and {De Ridder}, J. and {Delchambre}, L. and {Dell'Oro}, A. and {Ducourant}, C. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Galluccio}, L. and {Garc{\'\i}a-Torres}, M. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J.~J. and {Gosset}, E. and {Guy}, L.~P. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Hutton}, A. and {Jasniewicz}, G. and {Jean-Antoine-Piccolo}, A. and {Jordan}, S. and {Korn}, A.~J. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {Lebzelter}, T. and {L{\"o}ffler}, W. and {Manteiga}, M. and {Marrese}, P.~M. and {Mart{\'\i}n-Fleitas}, J.~M. and {Moitinho}, A. and {Mora}, A. and {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Richards}, P.~J. and {Robin}, A.~C. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {S{\"u}veges}, M. and {Torra}, J. and {van Reeven}, W. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alvarez}, R. and {Alves}, J. and {Andrei}, A.~H. and {Anglada Varela}, E. and {Antiche}, E. and {Antoja}, T. and {Arcay}, B. and {Astraatmadja}, T.~L. and {Bach}, N. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balm}, P. and {Barache}, C. and {Barata}, C. and {Barbato}, D. and {Barblan}, F. and {Barklem}, P.~S. and {Barrado}, D. and {Barros}, M. and {Barstow}, M.~A. and {Bartholom{\'e} Mu{\~n}oz}, S. and {Bassilana}, J. -L. and {Becciani}, U. and {Bellazzini}, M. and {Berihuete}, A. and {Bertone}, S. and {Bianchi}, L. and {Bienaym{\'e}}, O. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Boeche}, C. and {Bombrun}, A. and {Borrachero}, R. and {Bossini}, D. and {Bouquillon}, S. and {Bourda}, G. and {Bragaglia}, A. and {Bramante}, L. and {Breddels}, M.~A. and {Bressan}, A. and {Brouillet}, N. and {Br{\"u}semeister}, T. and {Brugaletta}, E. and {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {Cannizzaro}, G. and {Cantat-Gaudin}, T. and {Carballo}, R. and {Carlucci}, T. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cocozza}, G. and {Costigan}, G. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and {Crowley}, C. and {Cuypers}, J. and {Dafonte}, C. and {Damerdji}, Y. and {Dapergolas}, A. and {David}, P. and {David}, M. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {de Martino}, D. and {de Souza}, R. and {de Torres}, A. and {Debosscher}, J. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Drazinos}, P. and {Dur{\'a}n}, J. and {Edvardsson}, B. and {Enke}, H. and {Eriksson}, K. and {Esquej}, P. and {Eynard Bontemps}, G. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Falc{\~a}o}, A.~J. and {Farr{\`a}s Casas}, M. and {Federici}, L. and {Fedorets}, G. and {Fernique}, P. and {Figueras}, F. and {Filippi}, F. and {Findeisen}, K. and {Fonti}, A. and {Fraile}, E. and {Fraser}, M. and {Fr{\'e}zouls}, B. and {Gai}, M. and {Galleti}, S. and {Garabato}, D. and {Garc{\'\i}a-Sedano}, F. and {Garofalo}, A. and {Garralda}, N. and {Gavel}, A. and {Gavras}, P. and {Gerssen}, J. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomes}, M. and {Granvik}, M. and {Gueguen}, A. and {Guerrier}, A. and {Guiraud}, J. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Haigron}, R. and {Hatzidimitriou}, D. and {Hauser}, M. and {Haywood}, M. and {Heiter}, U. and {Helmi}, A. and {Heu}, J. and {Hilger}, T. and {Hobbs}, D. and {Hofmann}, W. and {Holland}, G. and {Huckle}, H.~E. and {Hypki}, A. and {Icardi}, V. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jonker}, P.~G. and {Juh{\'a}sz}, {\'A}. L. and {Julbe}, F. and {Karampelas}, A. and {Kewley}, A. and {Klar}, J. and {Kochoska}, A. and {Kohley}, R. and {Kolenberg}, K. and {Kontizas}, M. and {Kontizas}, E. and {Koposov}, S.~E. and {Kordopatis}, G. and {Kostrzewa-Rutkowska}, Z. and {Koubsky}, P. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Lavigne}, J. -B. and {Le Fustec}, Y. and {Le Poncin-Lafitte}, C. and {Lebreton}, Y. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Lenhardt}, H. and {Leroux}, F. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {L{\'o}pez}, M. and {Lorenz}, D. and {Managau}, S. and {Mann}, R.~G. and {Mantelet}, G. and {Marchant}, J.~M. and {Marconi}, M. and {Marinoni}, S. and {Marschalk{\'o}}, G. and {Marshall}, D.~J. and {Martino}, M. and {Marton}, G. and {Mary}, N. and {Massari}, D. and {Matijevi{\v{c}}}, G. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morgenthaler}, S. and {Morris}, D. and {Mulone}, A.~F. and {Muraveva}, T. and {Musella}, I. and {Nelemans}, G. and {Nicastro}, L. and {Noval}, L. and {O'Mullane}, W. and {Ord{\'e}novic}, C. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Osborne}, P. and {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and {Palacin}, H. and {Palaversa}, L. and {Panahi}, A. and {Pawlak}, M. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rambaux}, N. and {Ramos-Lerate}, M. and {Regibo}, S. and {Reyl{\'e}}, C. and {Riclet}, F. and {Ripepi}, V. and {Riva}, A. and {Rivard}, A. and {Rixon}, G. and {Roegiers}, T. and {Roelens}, M. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Ruiz-Dern}, L. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Sanna}, N. and {Santana-Ros}, T. and {Sarasso}, M. and {Savietto}, H. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Shih}, I. -C. and {Siltala}, L. and {Silva}, A.~F. and {Smart}, R.~L. and {Smith}, K.~W. and {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {Stoev}, H. and {Suess}, F.~F. and {Surdej}, J. and {Szegedi-Elek}, E. and {Tapiador}, D. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Terrett}, D. and {Teyssandier}, P. and {Thuillot}, W. and {Titarenko}, A. and {Torra Clotet}, F. and {Turon}, C. and {Ulla}, A. and {Utrilla}, E. and {Uzzi}, S. and {Vaillant}, M. and {Valentini}, G. and {Valette}, V. and {van Elteren}, A. and {Van Hemelryck}, E. and {van Leeuwen}, M. and {Vaschetto}, M. and {Vecchiato}, A. and {Veljanoski}, J. and {Viala}, Y. and {Vicente}, D. and {Vogt}, S. and {von Essen}, C. and {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and {Walmsley}, G. and {Weiler}, M. and {Wertz}, O. and {Wevers}, T. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Ziaeepour}, H. and {Zorec}, J. and {Zschocke}, S. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T.},
        title = "{Gaia Data Release 2. Variable stars in the colour-absolute magnitude diagram}",
      journal = {\aap},
     keywords = {stars: general, stars: variables: general, stars: oscillations, binaries: eclipsing, surveys, methods: data analysis, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = mar,
       volume = {623},
          eid = {A110},
        pages = {A110},
          doi = {10.1051/0004-6361/201833304},
archivePrefix = {arXiv},
       eprint = {1804.09382},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...623A.110G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{corbet08,
       author = {{Corbet}, R.~H.~D. and {Sokoloski}, J.~L. and {Mukai}, K. and {Markwardt}, C.~B. and {Tueller}, J.},
        title = "{A Comparison of the Variability of the Symbiotic X-Ray Binaries GX 1+4, 4U 1954+31, and 4U 1700+24 from Swift BAT and RXTE ASM Observations}",
      journal = {\apj},
     keywords = {binaries: symbiotic, stars: individual: GX 1+4 4U 1954+31 4U 1700+24, stars: neutron, X-rays: binaries, Astrophysics},
         year = 2008,
        month = mar,
       volume = {675},
       number = {2},
        pages = {1424-1435},
          doi = {10.1086/526337},
archivePrefix = {arXiv},
       eprint = {0711.1519},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...675.1424C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@inproceedings{landi11,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2011evhe.confE...9L},
	author = {{Landi}, R. and {Bassani}, L. and {Malizia}, A. and {Bazzano}, A. and {Fiocchi}, M. and {Bird}, A.~J.},
	booktitle = {Extreme and Variable High Energy Sky (Extremesky 2011)},
	date-added = {2021-04-28 11:33:31 +0200},
	date-modified = {2021-04-28 11:33:37 +0200},
	eid = {9},
	month = jan,
	pages = {9},
	title = {{Swift/XRT observations of unidentified INTEGRAL/IBIS sources}},
	year = 2011}

@article{westergaard06,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2006ATel..967....1W},
	author = {{Westergaard}, N.~J. and {Budtz-Jorgensen}, C. and {Chenevez}, J. and {Lund}, N. and {Brandt}, S. and {Oxborrow}, C.~A.},
	date-added = {2021-04-28 11:29:17 +0200},
	date-modified = {2021-04-28 11:29:44 +0200},
	journal = {The Astronomer's Telegram},
	keywords = {X-ray, Gamma Ray, Transients},
	month = dec,
	pages = {1},
	title = {{INTEGRAL detection of SWIFT J2037.2+4151}},
	volume = {967},
	year = 2006}

@article{masetti13,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...556A.120M},
	archiveprefix = {arXiv},
	author = {{Masetti}, N. and {Parisi}, P. and {Palazzi}, E. and {Jim{\'e}nez-Bail{\'o}n}, E. and {Chavushyan}, V. and {McBride}, V. and {Rojas}, A.~F. and {Steward}, L. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A.~J. and {Charles}, P.~A. and {Galaz}, G. and {Landi}, R. and {Malizia}, A. and {Mason}, E. and {Minniti}, D. and {Morelli}, L. and {Schiavone}, F. and {Stephen}, J.~B. and {Ubertini}, P.},
	date-added = {2021-04-28 11:28:28 +0200},
	date-modified = {2021-04-28 11:28:37 +0200},
	doi = {10.1051/0004-6361/201322026},
	eid = {A120},
	eprint = {1307.2898},
	journal = {\aap},
	keywords = {galaxies: Seyfert, quasars: emission lines, X-rays: binaries, novae, cataclysmic variables, stars: flare, Astrophysics - High Energy Astrophysical Phenomena},
	month = aug,
	pages = {A120},
	primaryclass = {astro-ph.HE},
	title = {{Unveiling the nature of INTEGRAL objects through optical spectroscopy. X. A new multi-year, multi-observatory campaign}},
	volume = {556},
	year = 2013,
	Bdsk-Url-1 = {https://doi.org/10.1051/0004-6361/201322026}}

@inproceedings{jayasinghe20,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2020AAS...23515403J},
	author = {{Jayasinghe}, T. and {Stanek}, K.~Z. and {Kochanek}, C.~S.},
	booktitle = {American Astronomical Society Meeting Abstracts \#235},
	date-added = {2021-04-28 11:26:14 +0200},
	date-modified = {2021-04-28 11:26:22 +0200},
	eid = {154.03},
	month = jan,
	pages = {154.03},
	series = {American Astronomical Society Meeting Abstracts},
	title = {{The ASAS-SN all-sky catalog of bright variable stars}},
	volume = {235},
	year = 2020}

@article{jayasinghe18,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.477.3145J},
	archiveprefix = {arXiv},
	author = {{Jayasinghe}, T. and {Kochanek}, C.~S. and {Stanek}, K.~Z. and {Shappee}, B.~J. and {Holoien}, T.~W. -S. and {Thompson}, Todd A. and {Prieto}, J.~L. and {Dong}, Subo and {Pawlak}, M. and {Shields}, J.~V. and {Pojmanski}, G. and {Otero}, S. and {Britt}, C.~A. and {Will}, D.},
	date-added = {2021-04-28 11:25:27 +0200},
	date-modified = {2021-04-28 11:25:38 +0200},
	doi = {10.1093/mnras/sty838},
	eprint = {1803.01001},
	journal = {\mnras},
	keywords = {catalogues, surveys, binaries: eclipsing, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics},
	month = jul,
	number = {3},
	pages = {3145-3163},
	primaryclass = {astro-ph.SR},
	title = {{The ASAS-SN catalogue of variable stars I: The Serendipitous Survey}},
	volume = {477},
	year = 2018,
	Bdsk-Url-1 = {https://doi.org/10.1093/mnras/sty838}}

@article{krivonos10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...523A..61K},
	archiveprefix = {arXiv},
	author = {{Krivonos}, R. and {Tsygankov}, S. and {Revnivtsev}, M. and {Grebenev}, S. and {Churazov}, E. and {Sunyaev}, R.},
	date-added = {2021-04-28 11:24:31 +0200},
	date-modified = {2021-04-28 11:24:42 +0200},
	doi = {10.1051/0004-6361/201014935},
	eid = {A61},
	eprint = {1006.4437},
	journal = {\aap},
	keywords = {surveys, X-rays:, general, catalogs, Astrophysics - High Energy Astrophysical Phenomena},
	month = nov,
	pages = {A61},
	primaryclass = {astro-ph.HE},
	title = {{INTEGRAL/IBIS 7-year All-Sky Hard X-Ray Survey. II. Catalog of sources}},
	volume = {523},
	year = 2010,
	Bdsk-Url-1 = {https://doi.org/10.1051/0004-6361/201014935}}

@article{forveille18,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...616E...1F},
	author = {{Forveille}, Thierry and {Kotak}, Rubina and {Shore}, Steve and {Tolstoy}, Eline},
	date-added = {2021-04-22 17:54:58 +0200},
	date-modified = {2021-04-22 17:55:10 +0200},
	doi = {10.1051/0004-6361/201833955},
	eid = {E1},
	journal = {\aap},
	month = aug,
	pages = {E1},
	title = {{Gaia Data Release 2}},
	volume = {616},
	year = 2018,
	Bdsk-Url-1 = {https://doi.org/10.1051/0004-6361/201833955}}

@inproceedings{baumgartner10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2010HEAD...11.1305B},
	author = {{Baumgartner}, Wayne H. and {Tueller}, J. and {Markwardt}, C. and {Skinner}, G.},
	booktitle = {AAS/High Energy Astrophysics Division \#11},
	date-added = {2021-04-22 17:52:28 +0200},
	date-modified = {2021-04-22 17:52:42 +0200},
	eid = {13.05},
	month = mar,
	pages = {13.05},
	series = {AAS/High Energy Astrophysics Division},
	title = {{The Swift-BAT 58 Month Survey}},
	volume = {11},
	year = 2010}

@article{bird16,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJS..223...15B},
	archiveprefix = {arXiv},
	author = {{Bird}, A.~J. and {Bazzano}, A. and {Malizia}, A. and {Fiocchi}, M. and {Sguera}, V. and {Bassani}, L. and {Hill}, A.~B. and {Ubertini}, P. and {Winkler}, C.},
	date-added = {2021-04-22 17:51:31 +0200},
	date-modified = {2021-04-22 17:51:39 +0200},
	doi = {10.3847/0067-0049/223/1/15},
	eid = {15},
	eprint = {1601.06074},
	journal = {\apjs},
	keywords = {Galaxy: general, gamma rays: general, surveys, Astrophysics - High Energy Astrophysical Phenomena},
	month = mar,
	number = {1},
	pages = {15},
	primaryclass = {astro-ph.HE},
	title = {{The IBIS Soft Gamma-Ray Sky after 1000 Integral Orbits}},
	volume = {223},
	year = 2016,
	Bdsk-Url-1 = {https://doi.org/10.3847/0067-0049/223/1/15}}

@article{bailer21,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....161..147B},
	archiveprefix = {arXiv},
	author = {{Bailer-Jones}, C.~A.~L. and {Rybizki}, J. and {Fouesneau}, M. and {Demleitner}, M. and {Andrae}, R.},
	date-added = {2021-04-22 17:47:48 +0200},
	date-modified = {2021-04-22 17:48:04 +0200},
	doi = {10.3847/1538-3881/abd806},
	eid = {147},
	eprint = {2012.05220},
	journal = {\aj},
	keywords = {Catalogs, Galaxy structure, Bayesian statistics, Parallax, Stellar parallax, Photometric parallax, Distance indicators, Astrometry, Markov chain Monte Carlo, Absolute magnitude, 205, 622, 1900, 1197, 1618, 1231, 394, 80, 1889, 10, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
	month = mar,
	number = {3},
	pages = {147},
	primaryclass = {astro-ph.SR},
	title = {{Estimating Distances from Parallaxes. V. Geometric and Photogeometric Distances to 1.47 Billion Stars in Gaia Early Data Release 3}},
	volume = {161},
	year = 2021,
	Bdsk-Url-1 = {https://doi.org/10.3847/1538-3881/abd806}}

@article{molina19,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.484.2735M},
	archiveprefix = {arXiv},
	author = {{Molina}, M. and {Malizia}, A. and {Bassani}, L. and {Ursini}, F. and {Bazzano}, A. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/stz156},
	eprint = {1901.04188},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
	month = apr,
	number = {2},
	pages = {2735-2746},
	primaryclass = {astro-ph.HE},
	title = {{Swift/XRT-NuSTAR spectra of type 1 AGN: confirming INTEGRAL results on the high-energy cut-off}},
	volume = {484},
	year = 2019,
	Bdsk-Url-1 = {https://doi.org/10.1093/mnras/stz156}}

@article{Lubinski_2001,
	author = {Lubinski, P. and Zdziarski, A. A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2001.04481.x},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {May},
	number = {2},
	pages = {L37--L42},
	publisher = {Oxford University Press (OUP)},
	title = {The strength and width of Fe K lines in Seyferts and their correlations with the X-ray slope},
	url = {http://dx.doi.org/10.1046/j.1365-8711.2001.04481.x},
	volume = {323},
	year = {2001},
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2001.04481.x}}

@article{Feng_2014,
	author = {Feng, Hua and Shen, Yue and Li, Hong},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637x/794/1/77},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {Sep},
	number = {1},
	pages = {77},
	publisher = {IOP Publishing},
	title = {SINGLE-EPOCH BLACK HOLE MASS ESTIMATORS FOR BROAD-LINE ACTIVE GALACTIC NUCLEI: RECALIBRATING Hβ WITH A NEW APPROACH},
	url = {http://dx.doi.org/10.1088/0004-637X/794/1/77},
	volume = {794},
	year = {2014},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/794/1/77},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/0004-637x/794/1/77}}

@article{Masetti_2006,
	author = {Masetti, N. and Mason, E. and Bassani, L. and Bird, A. J. and Maiorano, E. and Malizia, A. and Palazzi, E. and Stephen, J. B. and Bazzano, A. and Dean, A. J. and et al.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20054086},
	issn = {1432-0746},
	journal = {Astronomy & Astrophysics},
	month = {Feb},
	number = {2},
	pages = {547--556},
	publisher = {EDP Sciences},
	title = {Unveiling the nature ofINTEGRALobjects through optical spectroscopy},
	url = {http://dx.doi.org/10.1051/0004-6361:20054086},
	volume = {448},
	year = {2006},
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20054086}}

@article{Kaspi_2000,
	author = {Kaspi, Shai and Smith, Paul S. and Netzer, Hagai and Maoz, Dan and Jannuzi, Buell T. and Giveon, Uriel},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/308704},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {Apr},
	number = {2},
	pages = {631--649},
	publisher = {IOP Publishing},
	title = {Reverberation Measurements for 17 Quasars and the Size‐Mass‐Luminosity Relations in Active Galactic Nuclei},
	url = {http://dx.doi.org/10.1086/308704},
	volume = {533},
	year = {2000},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/308704}}

@article{Greene_2005,
	author = {Greene, Jenny E. and Ho, Luis C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/431897},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {Sep},
	number = {1},
	pages = {122--129},
	publisher = {IOP Publishing},
	title = {Estimating Black Hole Masses in Active Galaxies Using the Hα Emission Line},
	url = {http://dx.doi.org/10.1086/431897},
	volume = {630},
	year = {2005},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/431897}}

@article{Grier_2012,
	author = {Grier, C. J. and Peterson, B. M. and Pogge, R. W. and Denney, K. D. and Bentz, M. C. and Martini, Paul and Sergeev, S. G. and Kaspi, S. and Minezaki, T. and Zu, Y. and et al.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637x/755/1/60},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {Jul},
	number = {1},
	pages = {60},
	publisher = {IOP Publishing},
	title = {REVERBERATION MAPPING RESULTS FOR FIVE SEYFERT 1 GALAXIES},
	url = {http://dx.doi.org/10.1088/0004-637X/755/1/60},
	volume = {755},
	year = {2012},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/755/1/60},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/0004-637x/755/1/60}}

@article{Fausnaugh_2017,
	author = {Fausnaugh, M. M. and Grier, C. J. and Bentz, M. C. and Denney, K. D. and Rosa, G. De and Peterson, B. M. and Kochanek, C. S. and Pogge, R. W. and Adams, S. M. and Barth, A. J. and et al.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.3847/1538-4357/aa6d52},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {May},
	number = {2},
	pages = {97},
	publisher = {American Astronomical Society},
	title = {Reverberation Mapping of Optical Emission Lines in Five Active Galaxies},
	url = {http://dx.doi.org/10.3847/1538-4357/aa6d52},
	volume = {840},
	year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.3847/1538-4357/aa6d52}}

@article{Koss_2017,
	author = {Koss, Michael and Trakhtenbrot, Benny and Ricci, Claudio and Lamperti, Isabella and Oh, Kyuseok and Berney, Simon and Schawinski, Kevin and Balokovi{\'c}, Mislav and Baronchelli, Linda and Crenshaw, D. Michael and et al.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.3847/1538-4357/aa8ec9},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {Nov},
	number = {1},
	pages = {74},
	publisher = {American Astronomical Society},
	title = {BAT AGN Spectroscopic Survey. I. Spectral Measurements, Derived Quantities, and AGN Demographics},
	url = {http://dx.doi.org/10.3847/1538-4357/aa8ec9},
	volume = {850},
	year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.3847/1538-4357/aa8ec9}}

@article{Rodriguez_Ardila_2000,
	author = {Rodriguez‐Ardila, Alberto and Pastoriza, Miriani G. and Donzelli, Carlos J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/313293},
	issn = {1538-4365},
	journal = {The Astrophysical Journal Supplement Series},
	month = {Jan},
	number = {1},
	pages = {63--78},
	publisher = {IOP Publishing},
	title = {Visible and Near‐Infrared Spectroscopy of Seyfert 1 and Narrow‐Line Seyfert 1 Galaxies},
	url = {http://dx.doi.org/10.1086/313293},
	volume = {126},
	year = {2000},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/313293}}

@article{Khorunzhev_2012,
	author = {Khorunzhev, G. A. and Sazonov, S. Yu. and Burenin, R. A. and Tkachenko, A. Yu.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1134/s1063773712080026},
	issn = {1562-6873},
	journal = {Astronomy Letters},
	month = {Aug},
	number = {8},
	pages = {475--491},
	publisher = {Pleiades Publishing Ltd},
	title = {Masses and accretion rates of supermassive black holes in active galactic nuclei from the INTEGRAL survey},
	url = {http://dx.doi.org/10.1134/S1063773712080026},
	volume = {38},
	year = {2012},
	Bdsk-Url-1 = {http://dx.doi.org/10.1134/S1063773712080026},
	Bdsk-Url-2 = {http://dx.doi.org/10.1134/s1063773712080026}}

@article{Di_Gesu_2016,
	author = {Di Gesu, L. and Costantini, E.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201628670},
	issn = {1432-0746},
	journal = {Astronomy & Astrophysics},
	month = {Oct},
	pages = {A88},
	publisher = {EDP Sciences},
	title = {The warm absorber in the radio-loud quasar 4C +74.26},
	url = {http://dx.doi.org/10.1051/0004-6361/201628670},
	volume = {594},
	year = {2016},
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201628670}}

@article{Buisson_2018,
	author = {Buisson, D J K and Fabian, A C and Lohfink, A M},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/sty2609},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Sep},
	number = {4},
	pages = {4419--4426},
	publisher = {Oxford University Press (OUP)},
	title = {Coronal temperatures of the AGN ESO 103−035 and IGR 2124.7+5058 from NuSTAR observations},
	url = {http://dx.doi.org/10.1093/mnras/sty2609},
	volume = {481},
	year = {2018},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/sty2609}}

@article{Ricci_2018,
	author = {Ricci, C and Ho, L C and Fabian, A C and Trakhtenbrot, B and Koss, M J and Ueda, Y and Lohfink, A and Shimizu, T and Bauer, F E and Mushotzky, R and et al.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/sty1879},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Jul},
	number = {2},
	pages = {1819--1830},
	publisher = {Oxford University Press (OUP)},
	title = {BAT AGN Spectroscopic Survey -- XII. The relation between coronal properties of active galactic nuclei and the Eddington ratio},
	url = {http://dx.doi.org/10.1093/mnras/sty1879},
	volume = {480},
	year = {2018},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/sty1879}}

@article{Tortosa_2018,
	author = {Tortosa, A. and Bianchi, S. and Marinucci, A. and Matt, G. and Petrucci, P. O.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201732382},
	issn = {1432-0746},
	journal = {Astronomy & Astrophysics},
	month = {Jun},
	pages = {A37},
	publisher = {EDP Sciences},
	title = {A NuSTAR census of coronal parameters in Seyfert galaxies},
	url = {http://dx.doi.org/10.1051/0004-6361/201732382},
	volume = {614},
	year = {2018},
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201732382}}

@article{Kalberla_2005,
	author = {Kalberla, P. M. W. and Burton, W. B. and Hartmann, Dap and Arnal, E. M. and Bajaja, E. and Morras, R. and P{\"o}ppel, W. G. L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20041864},
	issn = {1432-0746},
	journal = {Astronomy & Astrophysics},
	month = {Sep},
	number = {2},
	pages = {775--782},
	publisher = {EDP Sciences},
	title = {The Leiden/Argentine/Bonn (LAB) Survey of Galactic HI},
	url = {http://dx.doi.org/10.1051/0004-6361:20041864},
	volume = {440},
	year = {2005},
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20041864}}

@article{Magdziarz_1995,
	author = {Magdziarz, Pawe{\l} and Zdziarski, Andrzej A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/273.3.837},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Apr},
	number = {3},
	pages = {837--848},
	publisher = {Oxford University Press (OUP)},
	title = {Angle-dependent Compton reflection of X-rays and gamma-rays},
	url = {http://dx.doi.org/10.1093/mnras/273.3.837},
	volume = {273},
	year = {1995},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/273.3.837}}

@article{Lohfink_2017,
	author = {Lohfink, Anne M. and Fabian, Andrew C. and Ballantyne, David R. and Boggs, S. E. and Boorman, Peter and Christensen, F. E. and Craig, W. W. and Farrah, Duncan and Garc{\'\i}a, Javier and Hailey, C. J. and et al.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.3847/1538-4357/aa6d07},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {May},
	number = {2},
	pages = {80},
	publisher = {American Astronomical Society},
	title = {The X-Ray Reflection Spectrum of the Radio-loud Quasar 4C 74.26},
	url = {http://dx.doi.org/10.3847/1538-4357/aa6d07},
	volume = {841},
	year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.3847/1538-4357/aa6d07}}

@article{Ricci_2017,
	author = {Ricci, C. and Trakhtenbrot, B. and Koss, M. J. and Ueda, Y. and Del Vecchio, I. and Treister, E. and Schawinski, K. and Paltani, S. and Oh, K. and Lamperti, I. and et al.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.3847/1538-4365/aa96ad},
	issn = {1538-4365},
	journal = {The Astrophysical Journal Supplement Series},
	month = {Dec},
	number = {2},
	pages = {17},
	publisher = {American Astronomical Society},
	title = {BAT AGN Spectroscopic Survey. V. X-Ray Properties of the Swift/BAT 70-month AGN Catalog},
	url = {http://dx.doi.org/10.3847/1538-4365/aa96ad},
	volume = {233},
	year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.3847/1538-4365/aa96ad}}

@article{Fabian_2017,
	author = {Fabian, A. C. and Lohfink, A. and Belmont, R. and Malzac, J. and Coppi, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/stx221},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Feb},
	number = {3},
	pages = {2566--2570},
	publisher = {Oxford University Press (OUP)},
	title = {Properties of AGN coronae in the NuSTAR era -- II. Hybrid plasma},
	url = {http://dx.doi.org/10.1093/mnras/stx221},
	volume = {467},
	year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stx221}}

@article{Fabian_2015,
	author = {Fabian, A. C. and Lohfink, A. and Kara, E. and Parker, M. L. and Vasudevan, R. and Reynolds, C. S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/stv1218},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Jul},
	number = {4},
	pages = {4375--4383},
	publisher = {Oxford University Press (OUP)},
	title = {Properties of AGN coronae in theNuSTARera},
	url = {http://dx.doi.org/10.1093/mnras/stv1218},
	volume = {451},
	year = {2015},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stv1218}}

@article{Mathur_2000,
	author = {Mathur, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2000.03530.x},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Jun},
	number = {4},
	pages = {L17--L20},
	publisher = {Oxford University Press (OUP)},
	title = {Narrow-line Seyfert 1 galaxies and the evolution of galaxies and active galaxies},
	url = {http://dx.doi.org/10.1046/j.1365-8711.2000.03530.x},
	volume = {314},
	year = {2000},
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2000.03530.x}}

@article{pounds95,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.277L...5P},
	author = {{Pounds}, K.~A. and {Done}, C. and {Osborne}, J.~P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/277.1.L5},
	journal = {\mnras},
	keywords = {ACCRETION, ACCRETION DISCS, GALAXIES: ACTIVE, GALAXIES: INDIVIDUAL: RE 1034+39, GALAXIES: SEYFERT, X-RAYS: GALAXIES},
	month = nov,
	pages = {L5-L10},
	title = {{RE 1034+39: a high-state Seyfert galaxy?}},
	volume = 277,
	year = 1995,
	Bdsk-Url-1 = {https://doi.org/10.1093/mnras/277.1.L5}}

@article{1995,
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/277.1.l5},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Nov},
	publisher = {Oxford University Press (OUP)},
	url = {http://dx.doi.org/10.1093/mnras/277.1.L5},
	year = {1995},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/277.1.L5},
	Bdsk-Url-2 = {http://dx.doi.org/10.1093/mnras/277.1.l5}}

@article{Osterbrock_1985,
	author = {Osterbrock, D. E. and Pogge, R. W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/163513},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {Oct},
	pages = {166},
	publisher = {IOP Publishing},
	title = {The spectra of narrow-line Seyfert 1 galaxies},
	url = {http://dx.doi.org/10.1086/163513},
	volume = {297},
	year = {1985},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/163513}}

@article{Malizia_2012,
	author = {Malizia, A. and Bassani, L. and Bazzano, A. and Bird, A. J. and Masetti, N. and Panessa, F. and Stephen, J. B. and Ubertini, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2012.21755.x},
	issn = {0035-8711},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Oct},
	number = {3},
	pages = {1750--1766},
	publisher = {Oxford University Press (OUP)},
	title = {TheINTEGRAL/IBIS AGN catalogue - I. X-ray absorption properties versus optical classification},
	url = {http://dx.doi.org/10.1111/j.1365-2966.2012.21755.x},
	volume = {426},
	year = {2012},
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2012.21755.x}}

@article{Malizia_2016,
	author = {Malizia, A. and Landi, R. and Molina, M. and Bassani, L. and Bazzano, A. and Bird, A. J. and Ubertini, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/stw972},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Apr},
	number = {1},
	pages = {19--29},
	publisher = {Oxford University Press (OUP)},
	title = {The INTEGRAL/IBISAGN catalogue: an update},
	url = {http://dx.doi.org/10.1093/mnras/stw972},
	volume = {460},
	year = {2016},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stw972}}

@article{tombesi15,
	author = {Tombesi, F. and Mel{\'e}ndez, M. and Veilleux, S. and Reeves, J. N. and Gonz{\'a}lez-Alfonso, E. and Reynolds, C. S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1038/nature14261},
	issn = {1476-4687},
	journal = {Nature},
	month = {Mar},
	number = {7544},
	pages = {436--438},
	publisher = {Springer Nature},
	title = {Wind from the black-hole accretion disk driving a molecular outflow in an active galaxy},
	url = {http://dx.doi.org/10.1038/nature14261},
	volume = {519},
	year = {2015},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature14261}}

@article{tombesi10,
	author = {Tombesi, F. and Cappi, M. and Reeves, J. N. and Palumbo, G. G. C. and Yaqoob, T. and Braito, V. and Dadina, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/200913440},
	issn = {1432-0746},
	journal = {Astronomy and Astrophysics},
	month = {Oct},
	pages = {A57},
	publisher = {EDP Sciences},
	title = {Evidence for ultra-fast outflows in radio-quiet AGNs},
	url = {http://dx.doi.org/10.1051/0004-6361/200913440},
	volume = {521},
	year = {2010},
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200913440}}

@article{marconi04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.351..169M},
	author = {{Marconi}, A. and {Risaliti}, G. and {Gilli}, R. and {Hunt}, L.~K. and {Maiolino}, R. and {Salvati}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2004.07765.x},
	eprint = {astro-ph/0311619},
	journal = {\mnras},
	keywords = {black hole physics, galaxies: active, galaxies: evolution, galaxies: nuclei, quasars: general, cosmology: miscellaneous},
	month = jun,
	pages = {169-185},
	title = {{Local supermassive black holes, relics of active galactic nuclei and the X-ray background}},
	volume = 351,
	year = 2004,
	Bdsk-Url-1 = {https://doi.org/10.1111/j.1365-2966.2004.07765.x}}

@article{lohfink15,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...814...24L},
	archiveprefix = {arXiv},
	author = {{Lohfink}, A.~M. and {Ogle}, P. and {Tombesi}, F. and {Walton}, D. and {Balokovi{\'c}}, M. and {Zoghbi}, A. and {Ballantyne}, D.~R. and {Boggs}, S.~E. and {Christensen}, F.~E. and {Craig}, W.~W. and {Fabian}, A.~C. and {Hailey}, C.~J. and {Harrison}, F.~A. and {King}, A.~L. and {Madejski}, G. and {Matt}, G. and {Reynolds}, C.~S. and {Stern}, D. and {Ursini}, F. and {Zhang}, W.~W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/814/1/24},
	eid = {24},
	eprint = {1510.01333},
	journal = {\apj},
	keywords = {galaxies: active, X-rays: individual: 3C 390.3},
	month = nov,
	pages = {24},
	primaryclass = {astro-ph.HE},
	title = {{The Corona of the Broad-line Radio Galaxy 3C 390.3}},
	volume = 814,
	year = 2015,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/814/1/24}}

@article{brenneman14,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...788...61B},
	archiveprefix = {arXiv},
	author = {{Brenneman}, L.~W. and {Madejski}, G. and {Fuerst}, F. and {Matt}, G. and {Elvis}, M. and {Harrison}, F.~A. and {Ballantyne}, D.~R. and {Boggs}, S.~E. and {Christensen}, F.~E. and {Craig}, W.~W. and {Fabian}, A.~C. and {Grefenstette}, B.~W. and {Hailey}, C.~J. and {Madsen}, K.~K. and {Marinucci}, A. and {Rivers}, E. and {Stern}, D. and {Walton}, D.~J. and {Zhang}, W.~W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/788/1/61},
	eid = {61},
	eprint = {1404.7486},
	journal = {\apj},
	keywords = {accretion, accretion disks, galaxies: active, galaxies: individual: IC 4329A, galaxies: nuclei, galaxies: Seyfert, X-rays: galaxies},
	month = jun,
	pages = {61},
	primaryclass = {astro-ph.HE},
	title = {{The Broad-band X-Ray Spectrum of IC 4329A from a Joint NuSTAR/Suzaku Observation}},
	volume = 788,
	year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/788/1/61}}

@article{titarchuk95,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...450..876T},
	author = {{Titarchuk}, L. and {Lyubarskij}, Y.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/176191},
	journal = {\apj},
	keywords = {PLASMAS, RADIATION MECHANISMS: THERMAL, RADIATIVE TRANSFER, SCATTERING},
	month = sep,
	pages = {876},
	title = {{Power-Law Spectra as a Result of Comptonization of the Soft Radiation in a Plasma Cloud}},
	volume = 450,
	year = 1995,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/176191}}

@article{marinucci15,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.447..160M},
	archiveprefix = {arXiv},
	author = {{Marinucci}, A. and {Matt}, G. and {Bianchi}, S. and {Lu}, T.~N. and {Arevalo}, P. and {Balokovi{\'c}}, M. and {Ballantyne}, D. and {Bauer}, F.~E. and {Boggs}, S.~E. and {Christensen}, F.~E. and {Craig}, W.~W. and {Gandhi}, P. and {Hailey}, C.~J. and {Harrison}, F. and {Puccetti}, S. and {Rivers}, E. and {Walton}, D.~J. and {Stern}, D. and {Zhang}, W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/stu2439},
	eprint = {1411.5151},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: individual: NGC 2110, galaxies: Seyfert},
	month = feb,
	pages = {160-167},
	primaryclass = {astro-ph.HE},
	title = {{The Seyfert 2 galaxy NGC 2110: hard X-ray emission observed by NuSTAR and variability of the iron K{$\alpha$} line}},
	volume = 447,
	year = 2015,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stu2439}}

@article{keek16,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.456.2722K},
	archiveprefix = {arXiv},
	author = {{Keek}, L. and {Ballantyne}, D.~R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/stv2882},
	eprint = {1508.06994},
	journal = {\mnras},
	keywords = {accretion, accretion discs, galaxies: active, galaxies: individual: Mrk 335, galaxies: Seyfert, X-rays: galaxies},
	month = mar,
	pages = {2722-2734},
	primaryclass = {astro-ph.HE},
	title = {{Revealing the accretion disc corona in Mrk 335 with multi-epoch X-ray spectroscopy}},
	volume = 456,
	year = 2016,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stv2882}}

@article{tazaki10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...721.1340T},
	archiveprefix = {arXiv},
	author = {{Tazaki}, F. and {Ueda}, Y. and {Ishino}, Y. and {Eguchi}, S. and {Isobe}, N. and {Terashima}, Y. and {Mushotzky}, R.~F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/721/2/1340},
	eprint = {1008.0722},
	journal = {\apj},
	keywords = {galaxies: active, galaxies: individual: 4C 50.55, X-rays: galaxies},
	month = oct,
	pages = {1340-1347},
	primaryclass = {astro-ph.HE},
	title = {{Suzaku Observation of the Brightest Broad-line Radio Galaxy 4C 50.55 (IGR J21247+5058)}},
	volume = 721,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/721/2/1340}}

@article{sazonov04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...421L..21S},
	author = {{Sazonov}, S.~Y. and {Revnivtsev}, M.~G. and {Lutovinov}, A.~A. and {Sunyaev}, R.~A. and {Grebenev}, S.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20040179},
	eprint = {astro-ph/0405259},
	journal = {\aap},
	keywords = {galaxies: Seyfert, X-rays: general},
	month = jul,
	pages = {L21-L24},
	title = {{Broadband X-ray spectrum of GRS 1734-292, a luminous Seyfert 1 galaxy behind the Galactic Center}},
	volume = 421,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20040179}}

@article{courvoisier03,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411L..53C},
	author = {{Courvoisier}, T.~J.-L. and {Walter}, R. and {Beckmann}, V. and {Dean}, A.~J. and {Dubath}, P. and {Hudec}, R. and {Kretschmar}, P. and {Mereghetti}, S. and {Montmerle}, T. and {Mowlavi}, N. and {Paltani}, S. and {Preite Martinez}, A. and {Produit}, N. and {Staubert}, R. and {Strong}, A.~W. and {Swings}, J.-P. and {Westergaard}, N.~J. and {White}, N. and {Winkler}, C. and {Zdziarski}, A.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20031172},
	eprint = {astro-ph/0308047},
	journal = {\aap},
	keywords = {methods: data analysis, gamma rays: observations},
	month = nov,
	pages = {L53-L57},
	title = {{The INTEGRAL Science Data Centre (ISDC)}},
	volume = 411,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031172}}

@article{Tortosa:2017,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.466.4193T},
	archiveprefix = {arXiv},
	author = {{Tortosa}, A. and {Marinucci}, A. and {Matt}, G. and {Bianchi}, S. and {La Franca}, F. and {Ballantyne}, D.~R. and {Boorman}, P.~G. and {Fabian}, A.~C. and {Farrah}, D. and {Fuerst}, F. and {Gandhi}, P. and {Harrison}, F.~A. and {Koss}, M.~J. and {Ricci}, C. and {Stern}, D. and {Ursini}, F. and {Walton}, D.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/stw3301},
	eprint = {1612.05871},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: individual: GRS 1734-292, galaxies: Seyfert, X-rays: galaxies},
	month = apr,
	pages = {4193-4200},
	primaryclass = {astro-ph.HE},
	title = {{Broad-band X-ray spectral analysis of the Seyfert 1 galaxy GRS 1734-292}},
	volume = 466,
	year = 2017,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stw3301}}

@article{Malizia:2014,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...782L..25M},
	archiveprefix = {arXiv},
	author = {{Malizia}, A. and {Molina}, M. and {Bassani}, L. and {Stephen}, J.~B. and {Bazzano}, A. and {Ubertini}, P. and {Bird}, A.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/2041-8205/782/2/L25},
	eid = {L25},
	eprint = {1401.3647},
	journal = {\apjl},
	keywords = {galaxies: active, gamma rays: galaxies, X-rays: galaxies},
	month = feb,
	pages = {L25},
	primaryclass = {astro-ph.HE},
	title = {{The INTEGRAL High-energy Cut-off Distribution of Type 1 Active Galactic Nuclei}},
	volume = 782,
	year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/782/2/L25}}

@article{tarchi11b,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...532A.125T},
	archiveprefix = {arXiv},
	author = {{Tarchi}, A. and {Castangia}, P. and {Columbano}, A. and {Panessa}, F. and {Braatz}, J.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201117213},
	eid = {A125},
	eprint = {1107.5155},
	journal = {\aap},
	keywords = {masers, galaxies: active, galaxies: nuclei, galaxies: Seyfert, radio lines: galaxies},
	month = aug,
	pages = {A125},
	primaryclass = {astro-ph.CO},
	title = {{Narrow-line Seyfert 1 galaxies: an amasing class of AGN}},
	volume = 532,
	year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201117213}}

@article{tarchi11a,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...525A..91T},
	archiveprefix = {arXiv},
	author = {{Tarchi}, A. and {Castangia}, P. and {Henkel}, C. and {Surcis}, G. and {Menten}, K.~M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201014714},
	eid = {A91},
	eprint = {1008.4253},
	journal = {\aap},
	keywords = {masers, galaxies: active, galaxies: nuclei, galaxies: starburst, radio lines: galaxies},
	month = jan,
	pages = {A91},
	primaryclass = {astro-ph.CO},
	title = {{New H$_{2}$O masers in Seyfert and FIR bright galaxies. IV. Interferometric follow-ups}},
	volume = 525,
	year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201014714}}

@article{ghisellini12,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.424L..26G},
	archiveprefix = {arXiv},
	author = {{Ghisellini}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1745-3933.2012.01280.x},
	eprint = {1205.0549},
	journal = {\mnras},
	keywords = {radiation mechanisms: non-thermal, gamma-ray burst: general, galaxies: active, galaxies: jets, X-rays: general},
	month = jul,
	pages = {L26-L30},
	primaryclass = {astro-ph.HE},
	title = {{Electron-positron pairs in blazar jets and {$\gamma$}-ray loud radio galaxies}},
	volume = 424,
	year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2012.01280.x}}

@article{panessa11,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.417.2426P},
	archiveprefix = {arXiv},
	author = {{Panessa}, F. and {de Rosa}, A. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A. and {Landi}, R. and {Malizia}, A. and {Miniutti}, G. and {Molina}, M. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2011.19268.x},
	eprint = {1106.3023},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: Seyfert, X-rays: galaxies},
	month = nov,
	pages = {2426-2439},
	primaryclass = {astro-ph.HE},
	title = {{Narrow-line Seyfert 1 galaxies at hard X-rays}},
	volume = 417,
	year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.19268.x}}

@article{filippenko03,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...588L..13F},
	author = {{Filippenko}, A.~V. and {Ho}, L.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/375361},
	eprint = {arXiv:astro-ph/0303429},
	journal = {\apjl},
	keywords = {Galaxies: Individual: NGC Number: NGC 4395, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei, Galaxies: Seyfert},
	month = may,
	pages = {L13-L16},
	title = {{A Low-Mass Central Black Hole in the Bulgeless Seyfert 1 Galaxy NGC 4395}},
	volume = 588,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/375361}}

@article{krivonos07,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...475..775K},
	author = {{Krivonos}, R. and {Revnivtsev}, M. and {Lutovinov}, A. and {Sazonov}, S. and {Churazov}, E. and {Sunyaev}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20077191},
	eprint = {arXiv:astro-ph/0701836},
	journal = {\aap},
	keywords = {surveys, X-rays: general, Galaxy: general, galaxies: Seyfert, cosmology: large-scale structure of Universe},
	month = nov,
	pages = {775-784},
	title = {{INTEGRAL/IBIS all-sky survey in hard X-rays}},
	volume = 475,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077191}}

@article{elitzur12,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...747L..33E},
	archiveprefix = {arXiv},
	author = {{Elitzur}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/2041-8205/747/2/L33},
	eid = {L33},
	eprint = {1202.1776},
	journal = {\apjl},
	keywords = {galaxies: active, galaxies: nuclei, galaxies: Seyfert, infrared: galaxies, quasars: general},
	month = mar,
	pages = {L33},
	primaryclass = {astro-ph.CO},
	title = {{On the Unification of Active Galactic Nuclei}},
	volume = 747,
	year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/747/2/L33}}

@article{paturel03,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...412...45P},
	author = {{Paturel}, G. and {Petit}, C. and {Prugniel}, P. and {Theureau}, G. and {Rousseau}, J. and {Brouty}, M. and {Dubois}, P. and {Cambr{\'e}sy}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20031411},
	journal = {\aap},
	keywords = {galaxies: general, catalogs},
	month = dec,
	pages = {45-55},
	title = {{HYPERLEDA. I. Identification and designation of galaxies}},
	volume = 412,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031411}}

@article{mcconnell12,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.422.1527M},
	archiveprefix = {arXiv},
	author = {{McConnell}, D. and {Sadler}, E.~M. and {Murphy}, T. and {Ekers}, R.~D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2012.20726.x},
	eprint = {1202.2625},
	journal = {\mnras},
	keywords = {methods: data analysis, catalogues, surveys, galaxies: active, gamma-rays: galaxies, radio continuum: general},
	month = may,
	pages = {1527-1545},
	primaryclass = {astro-ph.CO},
	title = {{ATPMN: accurate positions and flux densities at 5 and 8 GHz for 8385 sources from the PMN survey}},
	volume = 422,
	year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2012.20726.x}}

@article{landt04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.351...83L},
	author = {{Landt}, H. and {Padovani}, P. and {Perlman}, E.~S. and {Giommi}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2004.07750.x},
	eprint = {arXiv:astro-ph/0402494},
	journal = {\mnras},
	keywords = {galaxies: active, BL Lacertae objects: general, quasars: emission lines},
	month = jun,
	pages = {83-100},
	title = {{A physical classification scheme for blazars}},
	volume = 351,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.07750.x}}


@article{edelson12,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...751...52E},
	archiveprefix = {arXiv},
	author = {{Edelson}, R. and {Malkan}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/751/1/52},
	eid = {52},
	eprint = {1203.1942},
	journal = {\apj},
	keywords = {galaxies: active, galaxies: Seyfert, methods: statistical, quasars: general, surveys},
	month = may,
	pages = {52},
	primaryclass = {astro-ph.CO},
	title = {{Reliable Identifications of Active Galactic Nuclei from the WISE, 2MASS, and ROSAT All-Sky Surveys}},
	volume = 751,
	year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/751/1/52}}

@article{landi10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403..945L},
	archiveprefix = {arXiv},
	author = {{Landi}, R. and {Bassani}, L. and {Malizia}, A. and {Stephen}, J.~B. and {Bazzano}, A. and {Fiocchi}, M. and {Bird}, A.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2010.16183.x},
	eprint = {0912.1519},
	journal = {\mnras},
	keywords = {catalogues, surveys, gamma-rays: observations},
	month = apr,
	pages = {945-959},
	primaryclass = {astro-ph.HE},
	title = {{Swift/XRT observations of unidentified INTEGRAL/IBIS sources}},
	volume = 403,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.16183.x}}

@article{douglas96,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1996AJ....111.1945D},
	author = {{Douglas}, J.~N. and {Bash}, F.~N. and {Bozyan}, F.~A. and {Torrence}, G.~W. and {Wolfe}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/117932},
	journal = {\aj},
	keywords = {SURVEYS, RADIO LINES: GENERAL},
	month = may,
	pages = {1945},
	title = {{The Texas Survey of Radio Sources Covering -35.5 degrees {\lt} declination {\lt} 71.5 degrees at 365 MHz}},
	volume = 111,
	year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/117932}}

@article{wright10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010AJ....140.1868W},
	archiveprefix = {arXiv},
	author = {{Wright}, E.~L. and {Eisenhardt}, P.~R.~M. and {Mainzer}, A.~K. and {Ressler}, M.~E. and {Cutri}, R.~M. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and {Padgett}, D. and {McMillan}, R.~S. and {Skrutskie}, M. and {Stanford}, S.~A. and {Cohen}, M. and {Walker}, R.~G. and {Mather}, J.~C. and {Leisawitz}, D. and {Gautier}, III, T.~N. and {McLean}, I. and {Benford}, D. and {Lonsdale}, C.~J. and {Blain}, A. and {Mendez}, B. and {Irace}, W.~R. and {Duval}, V. and {Liu}, F. and {Royer}, D. and {Heinrichsen}, I. and {Howard}, J. and {Shannon}, M. and {Kendall}, M. and {Walsh}, A.~L. and {Larsen}, M. and {Cardon}, J.~G. and {Schick}, S. and {Schwalm}, M. and {Abid}, M. and {Fabinsky}, B. and {Naes}, L. and {Tsai}, C.-W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-6256/140/6/1868},
	eid = {1868},
	eprint = {1008.0031},
	journal = {\aj},
	keywords = {infrared: general, space vehicles, surveys},
	month = dec,
	pages = {1868-1881},
	primaryclass = {astro-ph.IM},
	title = {{The Wide-field Infrared Survey Explorer (WISE): Mission Description and Initial On-orbit Performance}},
	volume = 140,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/140/6/1868}}

@article{monet03,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003AJ....125..984M},
	author = {{Monet}, D.~G. and {Levine}, S.~E. and {Canzian}, B. and {Ables}, H.~D. and {Bird}, A.~R. and {Dahn}, C.~C. and {Guetter}, H.~H. and {Harris}, H.~C. and {Henden}, A.~A. and {Leggett}, S.~K. and {Levison}, H.~F. and {Luginbuhl}, C.~B. and {Martini}, J. and {Monet}, A.~K.~B. and {Munn}, J.~A. and {Pier}, J.~R. and {Rhodes}, A.~R. and {Riepe}, B. and {Sell}, S. and {Stone}, R.~C. and {Vrba}, F.~J. and {Walker}, R.~L. and {Westerhout}, G. and {Brucato}, R.~J. and {Reid}, I.~N. and {Schoening}, W. and {Hartley}, M. and {Read}, M.~A. and {Tritton}, S.~B.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/345888},
	eprint = {arXiv:astro-ph/0210694},
	journal = {\aj},
	keywords = {Astrometry, Catalogs},
	month = feb,
	pages = {984-993},
	title = {{The USNO-B Catalog}},
	volume = 125,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/345888}}

@article{griffith95,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1995ApJS...97..347G},
	author = {{Griffith}, M.~R. and {Wright}, A.~E. and {Burke}, B.~F. and {Ekers}, R.~D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/192146},
	journal = {\apjs},
	keywords = {ASTRONOMICAL CATALOGS, DATA REDUCTION, EQUATORIAL REGIONS, ERROR ANALYSIS, FLUX DENSITY, RADIO ASTRONOMY, RELIABILITY, SKY SURVEYS (ASTRONOMY), ASTRONOMICAL OBSERVATORIES, CENTIMETER WAVES, SUPERHIGH FREQUENCIES},
	month = apr,
	pages = {347-453},
	title = {{The Parkes-MIT-NRAO (PMN) surveys. 6: Source catalog for the equatorial survey (-9.5 deg less than delta less than +10.0 deg)}},
	volume = 97,
	year = 1995,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/192146}}

@article{bennett86,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1986ApJS...61....1B},
	author = {{Bennett}, C.~L. and {Lawrence}, C.~R. and {Burke}, B.~F. and {Hewitt}, J.~N. and {Mahoney}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/191108},
	journal = {\apjs},
	keywords = {ASTRONOMICAL CATALOGS, RADIO SOURCES (ASTRONOMY), CENTIMETER WAVES, RADIANT FLUX DENSITY, RADIO SPECTRA, RADIO TELESCOPES},
	month = may,
	pages = {1-104},
	title = {{The MIT-Green Bank (MG) 5 GHz survey}},
	volume = 61,
	year = 1986,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/191108}}

@article{vollmer09,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009yCat.8085....0B},
	author = {{Vollmer}, B.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {VizieR Online Data Catalog},
	keywords = {Radio sources, Galaxies: radio, Radio continuum},
	month = jul,
	pages = {0},
	title = {{SPECFIND V2.0 Catalog of radio continuum spectra (Vollmer+ 2009)}},
	volume = 8085,
	year = 2009}

@article{cohen07,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007AJ....134.1245C},
	archiveprefix = {arXiv},
	author = {{Cohen}, A.~S. and {Lane}, W.~M. and {Cotton}, W.~D. and {Kassim}, N.~E. and {Lazio}, T.~J.~W. and {Perley}, R.~A. and {Condon}, J.~J. and {Erickson}, W.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/520719},
	eprint = {0706.1191},
	journal = {\aj},
	keywords = {atmospheric effects, catalogs, radio continuum: general, surveys},
	month = sep,
	pages = {1245-1262},
	title = {{The VLA Low-Frequency Sky Survey}},
	volume = 134,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/520719}}

@article{bock99,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999AJ....117.1578B},
	author = {{Bock}, D.~C.-J. and {Large}, M.~I. and {Sadler}, E.~M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/300786},
	eprint = {arXiv:astro-ph/9812083},
	journal = {\aj},
	keywords = {INSTRUMENTATION: INTERFEROMETERS, RADIO CONTINUUM, SURVEYS},
	month = mar,
	pages = {1578-1593},
	title = {{SUMSS: A Wide-Field Radio Imaging Survey of the Southern Sky. I. Science Goals, Survey Design, and Instrumentation}},
	volume = 117,
	year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/300786}}

@article{Winkler:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411L...1W},
	author = {{Winkler}, C. and {Courvoisier}, T.~J.-L. and {Di Cocco}, G. and {Gehrels}, N. and {Gim{\'e}nez}, A. and {Grebenev}, S. and {Hermsen}, W. and {Mas-Hesse}, J.~M. and {Lebrun}, F. and {Lund}, N. and {Palumbo}, G.~G.~C. and {Paul}, J. and {Roques}, J.-P. and {Schnopper}, H. and {Sch{\"o}nfelder}, V. and {Sunyaev}, R. and {Teegarden}, B. and {Ubertini}, P. and {Vedrenne}, G. and {Dean}, A.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20031288},
	journal = {\aap},
	keywords = {gamma-ray astronomy, space observatory},
	month = nov,
	pages = {L1-L6},
	title = {{The INTEGRAL mission}},
	volume = 411,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031288}}

@article{malizia11,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011ATel.3290....1M},
	author = {{Malizia}, A. and {Landi}, R. and {Bassani}, L. and {Bird}, A.~B.~A.~J. and {Gehrels}, N. and {Kennea}, J.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {The Astronomer's Telegram},
	keywords = {X-ray, Gamma Ray, AGN, Binary},
	month = apr,
	pages = {1},
	title = {{Swift-XRT follow-up of 2 unidentified INTEGRAL sources}},
	volume = 3290,
	year = 2011}

@book{zombeck90,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1990hsaa.book.....Z},
	author = {{Zombeck}, M.~V.},
	booktitle = {Cambridge: University Press, 1990, 2nd ed.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{Zombeck, M.~V.}},
	title = {{Handbook of space astronomy and astrophysics}},
	year = 1990}

@article{wright94,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1994ApJS...91..111W},
	author = {{Wright}, A.~E. and {Griffith}, M.~R. and {Burke}, B.~F. and {Ekers}, R.~D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/191939},
	journal = {\apjs},
	keywords = {ASTRONOMICAL CATALOGS, RADIO ASTRONOMY, RADIO SOURCES (ASTRONOMY), SKY SURVEYS (ASTRONOMY), SOUTHERN SKY, TABLES (DATA), ERROR ANALYSIS, RADIO TELESCOPES},
	month = mar,
	pages = {111-308},
	title = {{The Parkes-MIT-NRAO (PMN) surveys. 2: Source catalog for the southern survey (delta greater than -87.5 deg and less than -37 deg)}},
	volume = 91,
	year = 1994,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/191939}}

@article{white00,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2000yCat.9031....0W},
	author = {{White}, N.~E. and {Giommi}, P. and {Angelini}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {VizieR Online Data Catalog},
	keywords = {X-ray sources, Cross identifications},
	month = jun,
	pages = {0},
	title = {{The WGACAT version of ROSAT sources (White+ 2000)}},
	volume = 9031,
	year = 2000}

@article{stephen05,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...432L..49S},
	author = {{Stephen}, J.~B. and {Bassani}, L. and {Molina}, M. and {Malizia}, A. and {Bazzano}, A. and {Ubertini}, P. and {Dean}, A.~J. and {Bird}, A.~J. and {Lebrun}, F. and {Much}, R. and {Walter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:200500017},
	eprint = {arXiv:astro-ph/0502158},
	journal = {\aap},
	keywords = {catalogues, surveys, gamma-rays: observations},
	month = mar,
	pages = {L49-L52},
	title = {{Using the ROSAT Bright Source Catalogue to find counterparts for IBIS/ISGRI survey sources}},
	volume = 432,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200500017}}

@article{stephen06,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...445..869S},
	author = {{Stephen}, J.~B. and {Bassani}, L. and {Malizia}, A. and {Bazzano}, A. and {Ubertini}, P. and {Bird}, A.~J. and {Dean}, A.~J. and {Lebrun}, F. and {Walter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20053958},
	eprint = {arXiv:astro-ph/0509620},
	journal = {\aap},
	keywords = {catalogs, surveys, gamma-rays: observations},
	month = jan,
	pages = {869-873},
	title = {{Using the ROSAT catalogues to find counterparts for the second IBIS/ISGRI survey sources}},
	volume = 445,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20053958}}

@article{stephen10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.408..422S},
	archiveprefix = {arXiv},
	author = {{Stephen}, J.~B. and {Bassani}, L. and {Landi}, R. and {Malizia}, A. and {Sguera}, V. and {Bazzano}, A. and {Masetti}, N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2010.17123.x},
	eprint = {1004.5232},
	journal = {\mnras},
	keywords = {catalogues, surveys, gamma-rays: general},
	month = oct,
	pages = {422-429},
	primaryclass = {astro-ph.HE},
	title = {{Using the ROSAT catalogue to find counterparts for unidentified objects in the first Fermi/LAT catalogue}},
	volume = 408,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.17123.x}}

@article{souchay09,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...494..799S},
	author = {{Souchay}, J. and {Andrei}, A.~H. and {Barache}, C. and {Bouquillon}, S. and {Gontier}, A.-M. and {Lambert}, S.~B. and {Le Poncin-Lafitte}, C. and {Taris}, F. and {Arias}, E.~F. and {Suchet}, D. and {Baudin}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:200809602},
	journal = {\aap},
	keywords = {reference systems, astrometry, quasars: general, catalogs},
	month = feb,
	pages = {799-815},
	title = {{The construction of the large quasar astrometric catalogue (LQAC)}},
	volume = 494,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200809602}}

@article{murphy10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.402.2403M},
	archiveprefix = {arXiv},
	author = {{Murphy}, T. and {Sadler}, E.~M. and {Ekers}, R.~D. and {Massardi}, M. and {Hancock}, P.~J. and {Mahony}, E. and {Ricci}, R. and {Burke-Spolaor}, S. and {Calabretta}, M. and {Chhetri}, R. and {de Zotti}, G. and {Edwards}, P.~G. and {Ekers}, J.~A. and {Jackson}, C.~A. and {Kesteven}, M.~J. and {Lindley}, E. and {Newton-McGee}, K. and {Phillips}, C. and {Roberts}, P. and {Sault}, R.~J. and {Staveley-Smith}, L. and {Subrahmanyan}, R. and {Walker}, M.~A. and {Wilson}, W.~E.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2009.15961.x},
	eprint = {0911.0002},
	journal = {\mnras},
	keywords = {methods: data analysis, catalogues, surveys, galaxies: active, cosmic microwave background, radio continuum: general},
	month = mar,
	pages = {2403-2423},
	primaryclass = {astro-ph.GA},
	title = {{The Australia Telescope 20 GHz Survey: the source catalogue}},
	volume = 402,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15961.x}}

@inproceedings{mundell99,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999AAS...194.6205M},
	author = {{Mundell}, C.~G. and {Wilson}, A.~S. and {Ulvestad}, J.~S. and {Roy}, A.~L.},
	booktitle = {American Astronomical Society Meeting Abstracts \#194},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	month = may,
	pages = {922},
	series = {Bulletin of the American Astronomical Society},
	title = {{Milli Arc Second Radio Imaging of Seyferts}},
	volume = 31,
	year = 1999}

@article{mauch03,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.342.1117M},
	author = {{Mauch}, T. and {Murphy}, T. and {Buttery}, H.~J. and {Curran}, J. and {Hunstead}, R.~W. and {Piestrzynski}, B. and {Robertson}, J.~G. and {Sadler}, E.~M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2003.06605.x},
	eprint = {arXiv:astro-ph/0303188},
	journal = {\mnras},
	keywords = {methods: data analysis, catalogues, surveys, astrometry, galaxies: statistics, radio continuum: general},
	month = jul,
	pages = {1117-1130},
	title = {{SUMSS: a wide-field radio imaging survey of the southern sky - II. The source catalogue}},
	volume = 342,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2003.06605.x}}

@inproceedings{moretti04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004SPIE.5165..232M},
	author = {{Moretti}, A. and {Campana}, S. and {Tagliaferri}, G. and {Abbey}, A.~F. and {Ambrosi}, R.~M. and {Angelini}, L. and {Beardmore}, A.~P. and {Br{\"a}uninger}, H.~W. and {Burkert}, W. and {Burrows}, D.~N. and {Capalbi}, M. and {Chincarini}, G. and {Citterio}, O. and {Cusumano}, G. and {Freyberg}, M.~J. and {Giommi}, P. and {Hartner}, G.~D. and {Hill}, J.~E. and {Mori}, K. and {Morris}, D.~C. and {Mukerjee}, K. and {Nousek}, J.~A. and {Osborne}, J.~P. and {Short}, A.~D.~T. and {Tamburelli}, F. and {Watson}, D.~J. and {Wells}, A.~A.},
	booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1117/12.504857},
	editor = {{K.~A.~Flanagan \&amp; O.~H.~W.~Siegmund}},
	month = feb,
	pages = {232-240},
	series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
	title = {{SWIFT XRT point spread function measured at the Panter end-to-end tests}},
	volume = 5165,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.504857}}

@article{massaro12,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2012arXiv1203.3801M},
	archiveprefix = {arXiv},
	author = {{Massaro}, F. and {D'Abrusco}, R. and {Tosti}, G. and {Ajello}, M. and {Gasparrini}, A.~P.~D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {1203.3801},
	journal = {ArXiv e-prints},
	keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Galaxy Astrophysics},
	month = mar,
	primaryclass = {astro-ph.HE},
	title = {{Unidentifed gamma-ray sources: hunting gamma-ray blazars}},
	year = 2012}

@article{massaro09,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009yCat..34950691M},
	author = {{Massaro}, E. and {Giommi}, P. and {Leto}, C. and {Marchegiani}, P. and {Maselli}, A. and {Perri}, M. and {Piranomonte}, S. and {Sclavi}, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {VizieR Online Data Catalog},
	keywords = {QSOs, BL Lac objects, Galaxy catalogs, Redshifts, Photometry},
	month = nov,
	pages = {50691},
	title = {{Multifrequency catalogue of blazars, Roma-BZCAT (Massaro+, 2009)}},
	volume = 349,
	year = 2009}

@article{masetti10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...519A..96M},
	archiveprefix = {arXiv},
	author = {{Masetti}, N. and {Parisi}, P. and {Palazzi}, E. and {Jim{\'e}nez-Bail{\'o}n}, E. and {Chavushyan}, V. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A.~J. and {Dean}, A.~J. and {Charles}, P.~A. and {Galaz}, G. and {Landi}, R. and {Malizia}, A. and {Mason}, E. and {McBride}, V.~A. and {Minniti}, D. and {Morelli}, L. and {Schiavone}, F. and {Stephen}, J.~B. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201014852},
	eid = {A96},
	eprint = {1006.4513},
	journal = {\aap},
	keywords = {galaxies: Seyfert, quasars: emission lines, X-rays: binaries, novae, cataclysmic variables, X-rays: general, techniques: spectroscopic},
	month = sep,
	pages = {A96},
	primaryclass = {astro-ph.HE},
	title = {{Unveiling the nature of INTEGRAL objects through optical spectroscopy. VIII. Identification of 44 newly detected hard X-ray sources}},
	volume = 519,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201014852}}

@article{masetti12,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...538A.123M},
	archiveprefix = {arXiv},
	author = {{Masetti}, N. and {Parisi}, P. and {Jim{\'e}nez-Bail{\'o}n}, E. and {Palazzi}, E. and {Chavushyan}, V. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A.~J. and {Dean}, A.~J. and {Galaz}, G. and {Landi}, R. and {Malizia}, A. and {Minniti}, D. and {Morelli}, L. and {Schiavone}, F. and {Stephen}, J.~B. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201118559},
	eid = {A123},
	eprint = {1201.1906},
	journal = {\aap},
	keywords = {X-rays: binaries, galaxies:Seyfert, X-rays: general, novae, cataclysmic variables, quasars: emission lines, stars: flare},
	month = feb,
	pages = {A123},
	primaryclass = {astro-ph.HE},
	title = {{Unveiling the nature of INTEGRAL objects through optical spectroscopy. IX. Twenty two more identifications, and a glance into the far hard X-ray Universe}},
	volume = 538,
	year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201118559}}

@article{kalberla05,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...440..775K},
	author = {{Kalberla}, P.~M.~W. and {Burton}, W.~B. and {Hartmann}, D. and {Arnal}, E.~M. and {Bajaja}, E. and {Morras}, R. and {P{\"o}ppel}, W.~G.~L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20041864},
	eprint = {arXiv:astro-ph/0504140},
	journal = {\aap},
	keywords = {surveys, radio lines: ISM, Galaxy: structure},
	month = sep,
	pages = {775-782},
	title = {{The Leiden/Argentine/Bonn (LAB) Survey of Galactic HI. Final data release of the combined LDS and IAR surveys with improved stray-radiation corrections}},
	volume = 440,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20041864}}

@article{healey07,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..171...61H},
	author = {{Healey}, S.~E. and {Romani}, R.~W. and {Taylor}, G.~B. and {Sadler}, E.~M. and {Ricci}, R. and {Murphy}, T. and {Ulvestad}, J.~S. and {Winn}, J.~N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/513742},
	eprint = {arXiv:astro-ph/0702346},
	journal = {\apjs},
	keywords = {Galaxies: Active, Galaxies: Quasars: General, Surveys},
	month = jul,
	pages = {61-71},
	title = {{CRATES: An All-Sky Survey of Flat-Spectrum Radio Sources}},
	volume = 171,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/513742}}

@article{ghisellini10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.402..497G},
	archiveprefix = {arXiv},
	author = {{Ghisellini}, G. and {Tavecchio}, F. and {Foschini}, L. and {Ghirlanda}, G. and {Maraschi}, L. and {Celotti}, A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2009.15898.x},
	eprint = {0909.0932},
	journal = {\mnras},
	keywords = {radiation mechanisms: non-thermal, BL Lacertae objects: general, quasars: general, gamma-rays: theory, X-rays: general},
	month = feb,
	pages = {497-518},
	primaryclass = {astro-ph.CO},
	title = {{General physical properties of bright Fermi blazars}},
	volume = 402,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15898.x}}

@inproceedings{ghisellini09,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009AIPC.1126..131G},
	archiveprefix = {arXiv},
	author = {{Ghisellini}, G.},
	booktitle = {American Institute of Physics Conference Series},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1063/1.3149394},
	editor = {{J.~Rodriguez \&amp; P.~Ferrando}},
	eprint = {0902.1984},
	keywords = {X-ray, Quasars, Infall, accretion, and accretion disks, Neutrino, muon, pion, and other elementary particles; cosmic rays, Galactic nuclei , circumnuclear matter, and bulges},
	month = may,
	pages = {131-136},
	primaryclass = {astro-ph.CO},
	series = {American Institute of Physics Conference Series},
	title = {{Blazars in Hard X-rays}},
	volume = 1126,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1063/1.3149394}}

@article{gehrels04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...611.1005G},
	author = {{Gehrels}, N. and {Chincarini}, G. and {Giommi}, P. and {Mason}, K.~O. and {Nousek}, J.~A. and {Wells}, A.~A. and {White}, N.~E. and {Barthelmy}, S.~D. and {Burrows}, D.~N. and {Cominsky}, L.~R. and {Hurley}, K.~C. and {Marshall}, F.~E. and {M{\'e}sz{\'a}ros}, P. and {Roming}, P.~W.~A. and {Angelini}, L. and {Barbier}, L.~M. and {Belloni}, T. and {Campana}, S. and {Caraveo}, P.~A. and {Chester}, M.~M. and {Citterio}, O. and {Cline}, T.~L. and {Cropper}, M.~S. and {Cummings}, J.~R. and {Dean}, A.~J. and {Feigelson}, E.~D. and {Fenimore}, E.~E. and {Frail}, D.~A. and {Fruchter}, A.~S. and {Garmire}, G.~P. and {Gendreau}, K. and {Ghisellini}, G. and {Greiner}, J. and {Hill}, J.~E. and {Hunsberger}, S.~D. and {Krimm}, H.~A. and {Kulkarni}, S.~R. and {Kumar}, P. and {Lebrun}, F. and {Lloyd-Ronning}, N.~M. and {Markwardt}, C.~B. and {Mattson}, B.~J. and {Mushotzky}, R.~F. and {Norris}, J.~P. and {Osborne}, J. and {Paczynski}, B. and {Palmer}, D.~M. and {Park}, H.-S. and {Parsons}, A.~M. and {Paul}, J. and {Rees}, M.~J. and {Reynolds}, C.~S. and {Rhoads}, J.~E. and {Sasseen}, T.~P. and {Schaefer}, B.~E. and {Short}, A.~T. and {Smale}, A.~P. and {Smith}, I.~A. and {Stella}, L. and {Tagliaferri}, G. and {Takahashi}, T. and {Tashiro}, M. and {Townsley}, L.~K. and {Tueller}, J. and {Turner}, M.~J.~L. and {Vietri}, M. and {Voges}, W. and {Ward}, M.~J. and {Willingale}, R. and {Zerbi}, F.~M. and {Zhang}, W.~W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/422091},
	journal = {\apj},
	keywords = {Gamma Rays: Bursts, Space Vehicles: Instruments, Telescopes},
	month = aug,
	pages = {1005-1020},
	title = {{The Swift Gamma-Ray Burst Mission}},
	volume = 611,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422091}}

@article{fugmann88,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1988A%26A...205...86F},
	author = {{Fugmann}, W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\aap},
	keywords = {ACTIVE GALACTIC NUCLEI, BL LACERTAE OBJECTS, BLAZARS, EXTRAGALACTIC RADIO SOURCES, OPTICAL POLARIZATION, QUASARS, ASTRONOMICAL CATALOGS, ASTRONOMICAL PHOTOMETRY, RADIO ASTRONOMY},
	month = oct,
	pages = {86-92},
	title = {{Are all flat-spectrum radio sources blazars?}},
	volume = 205,
	year = 1988}

@article{derosa12,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.420.2087D},
	archiveprefix = {arXiv},
	author = {{De Rosa}, A. and {Panessa}, F. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A. and {Landi}, R. and {Malizia}, A. and {Molina}, M. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2011.20167.x},
	eprint = {1111.1946},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: Seyfert, X-rays: galaxies},
	month = mar,
	pages = {2087-2101},
	primaryclass = {astro-ph.CO},
	title = {{Broad-band study of hard X-ray-selected absorbed active galactic nuclei}},
	volume = 420,
	year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.20167.x}}

@article{condon98,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1998AJ....115.1693C},
	author = {{Condon}, J.~J. and {Cotton}, W.~D. and {Greisen}, E.~W. and {Yin}, Q.~F. and {Perley}, R.~A. and {Taylor}, G.~B. and {Broderick}, J.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/300337},
	journal = {\aj},
	keywords = {CATALOGS, METHODS: DATA ANALYSIS, METHODS: OBSERVATIONAL, RADIO CONTINUUM, SURVEYS},
	month = may,
	pages = {1693-1716},
	title = {{The NRAO VLA Sky Survey}},
	volume = 115,
	year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/300337}}

@inproceedings{condon93,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1993ASPC...43...87C},
	author = {{Condon}, J.~J.},
	booktitle = {Sky Surveys. Protostars to Protogalaxies},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{B.~T.~Soifer}},
	month = jan,
	pages = {87},
	series = {Astronomical Society of the Pacific Conference Series},
	title = {{Radio Surveys of AGN}},
	volume = 43,
	year = 1993}

@article{burrows:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005SSRv..120..165B},
	author = {{Burrows}, D.~N. and {Hill}, J.~E. and {Nousek}, J.~A. and {Kennea}, J.~A. and {Wells}, A. and {Osborne}, J.~P. and {Abbey}, A.~F. and {Beardmore}, A. and {Mukerjee}, K. and {Short}, A.~D.~T. and {Chincarini}, G. and {Campana}, S. and {Citterio}, O. and {Moretti}, A. and {Pagani}, C. and {Tagliaferri}, G. and {Giommi}, P. and {Capalbi}, M. and {Tamburelli}, F. and {Angelini}, L. and {Cusumano}, G. and {Br{\"a}uninger}, H.~W. and {Burkert}, W. and {Hartner}, G.~D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1007/s11214-005-5097-2},
	eprint = {arXiv:astro-ph/0508071},
	journal = {\ssr},
	keywords = {gamma-ray burst, X-ray telescope, Swift, X-ray instrumentation, X-ray CCD detector, X-ray mirrors, {$\gamma$}-ray burst},
	month = oct,
	pages = {165-195},
	title = {{The Swift X-Ray Telescope}},
	volume = 120,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s11214-005-5097-2}}

@article{bassani:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...669L...1B},
	archiveprefix = {arXiv},
	author = {{Bassani}, L. and {Landi}, R. and {Malizia}, A. and {Fiocchi}, M.~T. and {Bazzano}, A. and {Bird}, A.~J. and {Dean}, A.~J. and {Gehrels}, N. and {Giommi}, P. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/523757},
	eprint = {0709.3023},
	journal = {\apjl},
	keywords = {Gamma Rays: Observations, quasars: individual (IGR J22517+2218), quasars: individual (MG3 J225155+2217)},
	month = nov,
	pages = {L1-L4},
	title = {{IGR J22517+2218=MG3 J225155+2217: A New Gamma-Ray Lighthouse in the Distant Universe}},
	volume = 669,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/523757}}

@article{polletta11,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...533A..20P},
	archiveprefix = {arXiv},
	author = {{Polletta}, M. and {Nesvadba}, N.~P.~H. and {Neri}, R. and {Omont}, A. and {Berta}, S. and {Bergeron}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201116446},
	eid = {A20},
	eprint = {1107.2129},
	journal = {\aap},
	keywords = {galaxies: high-redshift, galaxies: active, submillimeter: galaxies, submillimeter: ISM, quasars: general, galaxies: evolution},
	month = sep,
	pages = {A20},
	primaryclass = {astro-ph.CO},
	title = {{Disk, merger, or outflow? Molecular gas kinematics in two powerful obscured QSOs at z {\ge} 3.4}},
	volume = 533,
	year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201116446}}

@article{king11,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.415L...6K},
	archiveprefix = {arXiv},
	author = {{King}, A.~R. and {Zubovas}, K. and {Power}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1745-3933.2011.01067.x},
	eprint = {1104.3682},
	journal = {\mnras},
	keywords = {accretion, accretion discs, black hole physics, galaxies: evolution, quasars: general},
	month = jul,
	pages = {L6-L10},
	primaryclass = {astro-ph.GA},
	title = {{Large-scale outflows in galaxies}},
	volume = 415,
	year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2011.01067.x}}

@article{biggs08,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.385..893B},
	archiveprefix = {arXiv},
	author = {{Biggs}, A.~D. and {Ivison}, R.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.12869.x},
	eprint = {0712.3047},
	journal = {\mnras},
	keywords = {instrumentation: interferometers , techniques: interferometric , galaxies: formation , galaxies: starburst , radio continuum: galaxies , submillimetre},
	month = apr,
	pages = {893-904},
	title = {{High-resolution radio observations of submillimetre galaxies}},
	volume = 385,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.12869.x}}

@article{muxlow05,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.358.1159M},
	author = {{Muxlow}, T.~W.~B. and {Richards}, A.~M.~S. and {Garrington}, S.~T. and {Wilkinson}, P.~N. and {Anderson}, B. and {Richards}, E.~A. and {Axon}, D.~J. and {Fomalont}, E.~B. and {Kellermann}, K.~I. and {Partridge}, R.~B. and {Windhorst}, R.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2005.08824.x},
	eprint = {arXiv:astro-ph/0501679},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: evolution, galaxies: starburst, cosmology: observations, radio continuum: galaxies},
	month = apr,
	pages = {1159-1194},
	title = {{High-resolution studies of radio sources in the Hubble Deep and Flanking Fields}},
	volume = 358,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.08824.x}}

@article{clemens08,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...477...95C},
	archiveprefix = {arXiv},
	author = {{Clemens}, M.~S. and {Vega}, O. and {Bressan}, A. and {Granato}, G.~L. and {Silva}, L. and {Panuzzo}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20077224},
	eprint = {0708.0149},
	journal = {\aap},
	keywords = {dust, extinction, galaxies: active, infrared: galaxies, radio continuum: galaxies},
	month = jan,
	pages = {95-104},
	title = {{Modeling the spectral energy distribution of ULIRGs. I. The radio spectra}},
	volume = 477,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077224}}

@article{richards00,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...533..611R},
	author = {{Richards}, E.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/308684},
	eprint = {arXiv:astro-ph/9908313},
	journal = {\apj},
	keywords = {COSMOLOGY: OBSERVATIONS, GALAXIES: ACTIVE, GALAXIES: EVOLUTION, GALAXIES: STARBURST, RADIO CONTINUUM: GALAXIES, SURVEYS},
	month = apr,
	pages = {611-630},
	title = {{The Nature of Radio Emission from Distant Galaxies: The 1.4 GHZ Observations}},
	volume = 533,
	year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/308684}}

@article{donley05,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...634..169D},
	author = {{Donley}, J.~L. and {Rieke}, G.~H. and {Rigby}, J.~R. and {P{\'e}rez-Gonz{\'a}lez}, P.~G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/491668},
	eprint = {arXiv:astro-ph/0507676},
	journal = {\apj},
	keywords = {Galaxies: Active, Radio Continuum: Galaxies, X-Rays: Galaxies},
	month = nov,
	pages = {169-182},
	title = {{Unveiling a Population of AGNs Not Detected in X-Rays}},
	volume = 634,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/491668}}

@book{kellermann74,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1974gegr.book..320K},
	author = {{Kellermann}, K.~I.},
	booktitle = {Galactic and Extra-Galactic Radio Astronomy},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{Verschuur, G.~L., Kellermann, K.~I.; van Brunt, V.}},
	pages = {320},
	publisher = {Springer-Verlag},
	title = {{Radio Galaxies and Quasars}},
	year = 1974}

@article{klein88,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1988A%26A...190...41K},
	author = {{Klein}, U. and {Wielebinski}, R. and {Morsi}, H.~W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\aap},
	keywords = {CONTINUOUS SPECTRA, IRREGULAR GALAXIES, RADIO SOURCES (ASTRONOMY), STAR FORMATION, STARBURST GALAXIES, ASTRONOMICAL MAPS, BRIGHTNESS TEMPERATURE, FAR INFRARED RADIATION, LYMAN SPECTRA, RELATIVISTIC PARTICLES},
	month = jan,
	pages = {41-46},
	title = {{Radio continuum observations of M82}},
	volume = 190,
	year = 1988}

@article{Ferrari:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008SSRv..134...93F},
	archiveprefix = {arXiv},
	author = {{Ferrari}, C. and {Govoni}, F. and {Schindler}, S. and {Bykov}, A.~M. and {Rephaeli}, Y.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1007/s11214-008-9311-x},
	eprint = {0801.0985},
	journal = {\ssr},
	keywords = {Galaxies: clusters: general, Galaxies: intergalactic medium, Radio continuum: general, Radiation mechanisms: non-thermal, Magnetic fields, Acceleration of particles},
	month = feb,
	pages = {93-118},
	title = {{Observations of Extended Radio Emission in Clusters}},
	volume = 134,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s11214-008-9311-x}}

@article{Miley:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26ARv..15...67M},
	archiveprefix = {arXiv},
	author = {{Miley}, G. and {De Breuck}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1007/s00159-007-0008-z},
	eprint = {0802.2770},
	journal = {\aapr},
	keywords = {Radio galaxies, High-redshift, Massive galaxies, Clusters},
	month = feb,
	pages = {67-144},
	title = {{Distant radio galaxies and their environments}},
	volume = 15,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s00159-007-0008-z}}

@article{Jarvis:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.355...20J},
	author = {{Jarvis}, M.~J. and {Cruz}, M.~J. and {Cohen}, A.~S. and {R{\"o}ttgering}, H.~J.~A. and {Kassim}, N.~E.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2004.08278.x},
	eprint = {arXiv:astro-ph/0408082},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: evolution, galaxies: high-redshift, galaxies: nuclei, radio continuum: galaxies},
	month = nov,
	pages = {20-30},
	title = {{Near-infrared K-band imaging of a sample of ultra-steep-spectrum radio sources selected at 74 MHz}},
	volume = 355,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.08278.x}}

@inproceedings{deBreuck:1998,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1998ASSL..226..185D},
	author = {{De Breuck}, C. and {et al.}},
	booktitle = {Observational Cosmology with the New Radio Surveys},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{M.~N.~Bremer, N.~Jackson, \& I.~Perez-Fournon}},
	eprint = {arXiv:astro-ph/9705056},
	pages = {185},
	series = {Astrophysics and Space Science Library},
	title = {{Searches for High Redshift Radio Galaxies}},
	volume = 226,
	year = 1998}

@article{brunner08,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...479..283B},
	archiveprefix = {arXiv},
	author = {{Brunner}, H. and {Cappelluti}, N. and {Hasinger}, G. and {Barcons}, X. and {Fabian}, A.~C. and {Mainieri}, V. and {Szokoly}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20077687},
	eprint = {0711.4822},
	journal = {\aap},
	keywords = {surveys, galaxies: active, galaxies: quasars: general, X-rays: galaxies, X-rays: general},
	month = feb,
	pages = {283-300},
	title = {{XMM-Newton observations of the Lockman Hole: X-ray source catalogue and number counts}},
	volume = 479,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077687}}

@article{magliocchetti08,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.383..479M},
	archiveprefix = {arXiv},
	author = {{Magliocchetti}, M. and {Andreani}, P. and {Zwaan}, M.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2007.12576.x},
	eprint = {0710.2343},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: starburst, cosmology: observations, infrared: galaxies, radio continuum: galaxies},
	month = jan,
	pages = {479-496},
	title = {{The radio properties of optically obscured Spitzer sources}},
	volume = 383,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12576.x}}

@article{ibar09,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.397..281I},
	archiveprefix = {arXiv},
	author = {{Ibar}, E. and {Ivison}, R.~J. and {Biggs}, A.~D. and {Lal}, D.~V. and {Best}, P.~N. and {Green}, D.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2009.14866.x},
	eprint = {0903.3600},
	journal = {\mnras},
	keywords = {techniques: interferometric , galaxies: evolution , galaxies: starburst , radio continuum: galaxies},
	month = jul,
	pages = {281-298},
	primaryclass = {astro-ph.CO},
	title = {{Deep multi-frequency radio imaging in the Lockman Hole using the GMRT and VLA - I. The nature of the sub-mJy radio population}},
	volume = 397,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.14866.x}}

@inproceedings{Paioro:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ASPC..394..397P},
	author = {{Paioro}, L. and {Chiappetti}, L. and {Garilli}, B. and {Franzetti}, P. and {Fumana}, M. and {Scodeggio}, M.},
	booktitle = {Astronomical Data Analysis Software and Systems XVII},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{R.~W.~Argyle, P.~S.~Bunclark, \&amp; J.~R.~Lewis}},
	month = aug,
	pages = {397},
	series = {Astronomical Society of the Pacific Conference Series},
	title = {{DART, a New Solution to Deploy and Access Astronomical Data}},
	volume = 394,
	year = 2008}

@article{Lindner:2011,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737...83L},
	archiveprefix = {arXiv},
	author = {{Lindner}, R.~R. and {Baker}, A.~J. and {Omont}, A. and {Beelen}, A. and {Owen}, F.~N. and {Bertoldi}, F. and {Dole}, H. and {Fiolet}, N. and {Harris}, A.~I. and {Ivison}, R.~J. and {Lonsdale}, C.~J. and {Lutz}, D. and {Polletta}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/737/2/83},
	eprint = {1106.0344},
	journal = {\apj},
	keywords = {galaxies: formation, galaxies: high-redshift, galaxies: starburst, submillimeter: galaxies},
	month = aug,
	pages = {83-+},
	primaryclass = {astro-ph.CO},
	title = {{A Deep 1.2{\nbsp}mm Map of the Lockman Hole North Field}},
	volume = 737,
	year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/737/2/83}}

@article{magdis10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.409...22M},
	archiveprefix = {arXiv},
	author = {{Magdis}, G.~E. and {Elbaz}, D. and {Hwang}, H.~S. and {Amblard}, A. and {Arumugam}, V. and {Aussel}, H. and {Blain}, A. and {Bock}, J. and {Boselli}, A. and {Buat}, V. and {Castro-Rodr{\'{\i}}guez}, N. and {Cava}, A. and {Chanial}, P. and {Clements}, D.~L. and {Conley}, A. and {Conversi}, L. and {Cooray}, A. and {Dowell}, C.~D. and {Dwek}, E. and {Eales}, S. and {Farrah}, D. and {Franceschini}, A. and {Glenn}, J. and {Griffin}, M. and {Halpern}, M. and {Hatziminaoglou}, E. and {Huang}, J. and {Ibar}, E. and {Isaak}, K. and {Le Floc'h}, E. and {Lagache}, G. and {Levenson}, L. and {Lonsdale}, C.~J. and {Lu}, N. and {Madden}, S. and {Maffei}, B. and {Mainetti}, G. and {Marchetti}, L. and {Morrison}, G.~E. and {Nguyen}, H.~T. and {O'Halloran}, B. and {Oliver}, S.~J. and {Omont}, A. and {Owen}, F.~N. and {Page}, M.~J. and {Pannella}, M. and {Panuzzo}, P. and {Papageorgiou}, A. and {Pearson}, C.~P. and {P{\'e}rez-Fournon}, I. and {Pohlen}, M. and {Rigopoulou}, D. and {Rizzo}, D. and {Roseboom}, I.~G. and {Rowan-Robinson}, M. and {Schulz}, B. and {Scott}, D. and {Seymour}, N. and {Shupe}, D.~L. and {Smith}, A.~J. and {Stevens}, J.~A. and {Strazzullo}, V. and {Symeonidis}, M. and {Trichas}, M. and {Tugwell}, K.~E. and {Vaccari}, M. and {Valtchanov}, I. and {Vigroux}, L. and {Wang}, L. and {Wright}, G. and {Xu}, C.~K. and {Zemcov}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2010.17551.x},
	eprint = {1007.4900},
	journal = {\mnras},
	keywords = {galaxies: evolution, galaxies: high-redshift, galaxies: starburst, cosmology: observations, infrared: galaxies, submillimetre: galaxies},
	month = nov,
	pages = {22-28},
	primaryclass = {astro-ph.CO},
	title = {{Herschel reveals a T_{dust}-unbiased selection of z \~{} 2 ultraluminous infrared galaxies}},
	volume = 409,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.17551.x}}

@article{oliver10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518L..21O},
	archiveprefix = {arXiv},
	author = {{Oliver}, S.~J. and {Wang}, L. and {Smith}, A.~J. and {Altieri}, B. and {Amblard}, A. and {Arumugam}, V. and {Auld}, R. and {Aussel}, H. and {Babbedge}, T. and {Blain}, A. and {Bock}, J. and {Boselli}, A. and {Buat}, V. and {Burgarella}, D. and {Castro-Rodr{\'{\i}}guez}, N. and {Cava}, A. and {Chanial}, P. and {Clements}, D.~L. and {Conley}, A. and {Conversi}, L. and {Cooray}, A. and {Dowell}, C.~D. and {Dwek}, E. and {Eales}, S. and {Elbaz}, D. and {Fox}, M. and {Franceschini}, A. and {Gear}, W. and {Glenn}, J. and {Griffin}, M. and {Halpern}, M. and {Hatziminaoglou}, E. and {Ibar}, E. and {Isaak}, K. and {Ivison}, R.~J. and {Lagache}, G. and {Levenson}, L. and {Lu}, N. and {Madden}, S. and {Maffei}, B. and {Mainetti}, G. and {Marchetti}, L. and {Mitchell-Wynne}, K. and {Mortier}, A.~M.~J. and {Nguyen}, H.~T. and {O'Halloran}, B. and {Omont}, A. and {Page}, M.~J. and {Panuzzo}, P. and {Papageorgiou}, A. and {Pearson}, C.~P. and {P{\'e}rez-Fournon}, I. and {Pohlen}, M. and {Rawlings}, J.~I. and {Raymond}, G. and {Rigopoulou}, D. and {Rizzo}, D. and {Roseboom}, I.~G. and {Rowan-Robinson}, M. and {S{\'a}nchez Portal}, M. and {Savage}, R. and {Schulz}, B. and {Scott}, D. and {Seymour}, N. and {Shupe}, D.~L. and {Stevens}, J.~A. and {Symeonidis}, M. and {Trichas}, M. and {Tugwell}, K.~E. and {Vaccari}, M. and {Valiante}, E. and {Valtchanov}, I. and {Vieira}, J.~D. and {Vigroux}, L. and {Ward}, R. and {Wright}, G. and {Xu}, C.~K. and {Zemcov}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201014697},
	eprint = {1005.2184},
	journal = {\aap},
	keywords = {galaxies: evolution, submillimeter: galaxies, surveys},
	month = jul,
	pages = {L21+},
	primaryclass = {astro-ph.CO},
	title = {{HerMES: SPIRE galaxy number counts at 250, 350, and 500 {$\mu$}m}},
	volume = 518,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201014697}}

@article{ibar10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.401L..53I},
	archiveprefix = {arXiv},
	author = {{Ibar}, E. and {Ivison}, R.~J. and {Best}, P.~N. and {Coppin}, K. and {Pope}, A. and {Smail}, I. and {Dunlop}, J.~S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1745-3933.2009.00786.x},
	eprint = {0911.1954},
	journal = {\mnras},
	keywords = {galaxies: evolution , infrared: galaxies , radio continuum: galaxies},
	month = jan,
	pages = {L53-L57},
	primaryclass = {astro-ph.CO},
	title = {{Deep multi-frequency radio imaging in the Lockman Hole - II. The spectral index of submillimetre galaxies}},
	volume = 401,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2009.00786.x}}

@article{granato04,
	adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004ApJ...600..580G&db_key=AST},
	author = {{Granato}, G.~L. and {De Zotti}, G. and {Silva}, L. and {Bressan}, A. and {Danese}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/379875},
	eprint = {arXiv:0307202},
	journal = {\apj},
	month = jan,
	pages = {580-594},
	title = {{A Physical Model for the Coevolution of QSOs and Their Spheroidal Hosts}},
	volume = {600},
	year = {2004},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/379875}}

@article{granato02,
	adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002Ap%26SS.281..497G&db_key=AST},
	author = {{Granato}, G.~L. and {DeZotti}, G. and {Silva}, L. and {Danese}, L. and {Magliocchetti}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\apss},
	pages = {497-500},
	title = {{The Connection between Spheroidal Galaxies and QSOs}},
	volume = {281},
	year = {2002}}

@article{sanders88,
	adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988ApJ...328L..35S&db_key=AST},
	author = {{Sanders}, D.~B. and {Soifer}, B.~T. and {Elias}, J.~H. and {Neugebauer}, G. and {Matthews}, K.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/185155},
	journal = {\apjl},
	month = may,
	pages = {L35-L39},
	title = {{Warm ultraluminous galaxies in the IRAS survey - The transition from galaxy to quasar?}},
	volume = {328},
	year = {1988},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/185155}}

@article{fanti95,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...302..317F},
	author = {{Fanti}, C. and {Fanti}, R. and {Dallacasa}, D. and {Schilizzi}, R.~T. and {Spencer}, R.~E. and {Stanghellini}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\aap},
	keywords = {GALAXIES: ACTIVE, QUASARS: GENERAL, GALAXIES: EVOLUTION, RADIO CONTINUUM: GALAXIES},
	month = oct,
	pages = {317-+},
	title = {{Are compact steep-spectrum sources young?}},
	volume = 302,
	year = 1995}

@article{dimatteo05,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005Natur.433..604D},
	author = {{Di Matteo}, T. and {Springel}, V. and {Hernquist}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1038/nature03335},
	eprint = {arXiv:astro-ph/0502199},
	journal = {\nat},
	month = feb,
	pages = {604-607},
	title = {{Energy input from quasars regulates the growth and activity of black holes and their host galaxies}},
	volume = 433,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature03335}}

@article{cirasuolo03a,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.341..993C},
	author = {{Cirasuolo}, M. and {Magliocchetti}, M. and {Celotti}, A. and {Danese}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2003.06485.x},
	eprint = {arXiv:astro-ph/0301526},
	journal = {\mnras},
	keywords = {galaxies: active, quasars: general, cosmology: observations},
	month = may,
	pages = {993-1004},
	title = {{The radio-loud/radio-quiet dichotomy: news from the 2dF QSO Redshift Survey}},
	volume = 341,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2003.06485.x}}

@article{cirasuolo03b,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.346..447C},
	author = {{Cirasuolo}, M. and {Celotti}, A. and {Magliocchetti}, M. and {Danese}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-2966.2003.07105.x},
	eprint = {arXiv:astro-ph/0306415},
	journal = {\mnras},
	keywords = {galaxies: active, cosmology: observations, radio continuum: general},
	month = dec,
	pages = {447-455},
	title = {{Is there a dichotomy in the radio loudness distribution of quasars?}},
	volume = 346,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-2966.2003.07105.x}}

@article{davies06,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.370.1125D},
	author = {{Davies}, R.~D. and {Dickinson}, C. and {Banday}, A.~J. and {Jaffe}, T.~R. and {G{\'o}rski}, K.~M. and {Davis}, R.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2006.10572.x},
	eprint = {arXiv:astro-ph/0511384},
	journal = {\mnras},
	keywords = {radiation mechanisms: general: cosmic microwave background: cosmology: observations: diffuse radiation: radio continuum: ISM, radiation mechanisms: general, cosmic microwave background, cosmology: observations, diffuse radiation, radio continuum: ISM},
	month = aug,
	pages = {1125-1139},
	title = {{A determination of the spectra of Galactic components observed by the Wilkinson Microwave Anisotropy Probe}},
	volume = 370,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10572.x}}

@article{begelman04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004cbhg.symp..374B},
	author = {{Begelman}, M.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {arXiv:astro-ph/0303040},
	journal = {Coevolution of Black Holes and Galaxies},
	pages = {374-+},
	title = {{AGN Feedback Mechanisms}},
	year = 2004}

@article{shin10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...711..268S},
	archiveprefix = {arXiv},
	author = {{Shin}, M.-S. and {Ostriker}, J.~P. and {Ciotti}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/711/1/268},
	eprint = {0905.4294},
	journal = {\apj},
	keywords = {galaxies: active, galaxies: evolution, galaxies: formation, galaxies: nuclei, methods: numerical},
	month = mar,
	pages = {268-283},
	primaryclass = {astro-ph.GA},
	title = {{Feedback from Central Black Holes in Elliptical Galaxies. II. Can Purely Mechanical Energy Feedback Models Work?}},
	volume = 711,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/711/1/268}}

@article{ciotti09,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...699...89C},
	archiveprefix = {arXiv},
	author = {{Ciotti}, L. and {Ostriker}, J.~P. and {Proga}, D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/699/1/89},
	eprint = {0901.1089},
	journal = {\apj},
	keywords = {accretion, accretion disks, black hole physics, galaxies: active, galaxies: nuclei, galaxies: starburst, quasars: general},
	month = jul,
	pages = {89-104},
	primaryclass = {astro-ph.GA},
	title = {{Feedback from Central Black Holes in Elliptical Galaxies. I. Models with Either Radiative or Mechanical Feedback but not Both}},
	volume = 699,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/699/1/89}}

@article{ciotti07,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...665.1038C},
	author = {{Ciotti}, L. and {Ostriker}, J.~P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/519833},
	eprint = {arXiv:astro-ph/0703057},
	journal = {\apj},
	keywords = {Accretion, Accretion Disks, Black Hole Physics, Galaxies: Active, Galaxies: Nuclei, Galaxies: Starburst, Galaxies: Quasars: General},
	month = aug,
	pages = {1038-1056},
	title = {{Radiative Feedback from Massive Black Holes in Elliptical Galaxies: AGN Flaring and Central Starburst Fueled by Recycled Gas}},
	volume = 665,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/519833}}

@article{condon92,
	adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1992ARA%26A..30..575C},
	author = {{Condon}, J.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1146/annurev.aa.30.090192.003043},
	journal = {\araa},
	pages = {575-611},
	title = {{Radio emission from normal galaxies}},
	volume = {30},
	year = {1992},
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.aa.30.090192.003043}}

@article{nesvadba06,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...650..693N},
	author = {{Nesvadba}, N.~P.~H. and {Lehnert}, M.~D. and {Eisenhauer}, F. and {Gilbert}, A. and {Tecza}, M. and {Abuter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/507266},
	eprint = {arXiv:astro-ph/0606530},
	journal = {\apj},
	keywords = {Cosmology: Observations, Galaxies: Evolution, Galaxies: Kinematics and Dynamics, Infrared: Galaxies},
	month = oct,
	pages = {693-705},
	title = {{Extreme Gas Kinematics in the z=2.2 Powerful Radio Galaxy MRC 1138-262: Evidence for Efficient Active Galactic Nucleus Feedback in the Early Universe?}},
	volume = 650,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/507266}}

@article{murray05,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...618..569M},
	author = {{Murray}, N. and {Quataert}, E. and {Thompson}, T.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/426067},
	eprint = {arXiv:astro-ph/0406070},
	journal = {\apj},
	keywords = {Galaxies: Formation, Galaxies: Fundamental Parameters, Galaxies: General, Galaxies: Starburst, Galaxies: Intergalactic Medium},
	month = jan,
	pages = {569-585},
	title = {{On the Maximum Luminosity of Galaxies and Their Central Black Holes: Feedback from Momentum-driven Winds}},
	volume = 618,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/426067}}

@article{Maiolino:1998,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...338..781M},
	author = {{Maiolino}, R. and {Salvati}, M. and {Bassani}, L. and {Dadina}, M. and {della Ceca}, R. and {Matt}, G. and {Risaliti}, G. and {Zamorani}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {arXiv:astro-ph/9806055},
	journal = {\aap},
	keywords = {X-RAYS: GALAXIES, GALAXIES: SEYFERT, GALAXIES: ACTIVE},
	month = oct,
	pages = {781-794},
	title = {{Heavy obscuration in X-ray weak AGNs}},
	volume = 338,
	year = 1998}

@article{Turner:1997,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...488..164T},
	author = {{Turner}, T.~J. and {George}, I.~M. and {Nandra}, K. and {Mushotzky}, R.~F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/304701},
	eprint = {arXiv:astro-ph/9705087},
	journal = {\apj},
	keywords = {GALAXIES: ACTIVE, GALAXIES: NUCLEI, LINE: FORMATION, X-RAYS: GALAXIES},
	month = oct,
	pages = {164-+},
	title = {{ASCA Observations of Type 2 Seyfert Galaxies. II. The Importance of X-Ray Scattering and Reflection}},
	volume = 488,
	year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/304701}}

@article{Smith:1996,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1996MNRAS.280..355S},
	author = {{Smith}, D.~A. and {Done}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\mnras},
	keywords = {ACCRETION, ACCRETION DISCS, GALAXIES: NUCLEI, GALAXIES: SEYFERT, X-RAYS: GALAXIES},
	month = may,
	pages = {355-377},
	title = {{Unified theories of active galactic nuclei: a hard X-ray sample of Seyfert 2 galaxies}},
	volume = 280,
	year = 1996}

@article{Sajina:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...683..659S},
	author = {{Sajina}, A. and {Yan}, L. and {Lutz}, D. and {Steffen}, A. and {Helou}, G. and {Huynh}, M. and {Frayer}, D. and {Choi}, P. and {Tacconi}, L. and {Dasyra}, K.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/589914},
	journal = {\apj},
	keywords = {Galaxies: Active, Infrared: Galaxies, Galaxies: Quasars: General, Radio Continuum: Galaxies},
	month = aug,
	pages = {659-682},
	title = {{Spitzer Mid-Infrared Spectroscopy of Infrared Luminous Galaxies at z \~{} 2. III. Far-IR to Radio Properties and Optical Spectral Diagnostics}},
	volume = 683,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/589914}}

@article{Kovacs:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...650..592K},
	author = {{Kov{\'a}cs}, A. and {Chapman}, S.~C. and {Dowell}, C.~D. and {Blain}, A.~W. and {Ivison}, R.~J. and {Smail}, I. and {Phillips}, T.~G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/506341},
	eprint = {arXiv:astro-ph/0604591},
	journal = {\apj},
	keywords = {Galaxies: Evolution, Galaxies: High-Redshift, Galaxies: ISM, Galaxies: Photometry, Galaxies: Starburst, Infrared: Galaxies, Submillimeter},
	month = oct,
	pages = {592-603},
	title = {{SHARC-2 350 {$\mu$}m Observations of Distant Submillimeter-selected Galaxies}},
	volume = 650,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/506341}}

@article{Yun:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...554..803Y},
	author = {{Yun}, M.~S. and {Reddy}, N.~A. and {Condon}, J.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/323145},
	eprint = {arXiv:astro-ph/0102154},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Luminosity Function, Mass Function, Galaxies: Starburst, Infrared: Galaxies, Radio Continuum: Galaxies, Surveys},
	month = jun,
	pages = {803-822},
	title = {{Radio Properties of Infrared-selected Galaxies in the IRAS 2 Jy Sample}},
	volume = 554,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/323145}}

@article{Strazzullo:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...714.1305S},
	archiveprefix = {arXiv},
	author = {{Strazzullo}, V. and {Pannella}, M. and {Owen}, F.~N. and {Bender}, R. and {Morrison}, G.~E. and {Wang}, {W.-H.} and {Shupe}, D.~L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/714/2/1305},
	eprint = {1003.4734},
	journal = {\apj},
	keywords = {cosmology: observations, galaxies: active, galaxies: evolution, galaxies: starburst, radio continuum: galaxies},
	month = may,
	pages = {1305-1323},
	primaryclass = {astro-ph.CO},
	title = {{The Deep Swire Field. IV. First Properties of the sub-mJy Galaxy Population: Redshift Distribution, AGN Activity, and Star Formation}},
	volume = 714,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/714/2/1305}}

@article{Ueda:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ApJS..179..124U},
	archiveprefix = {arXiv},
	author = {{Ueda}, Y. and {Watson}, M.~G. and {Stewart}, I.~M. and {Akiyama}, M. and {Schwope}, A.~D. and {Lamer}, G. and {Ebrero}, J. and {Carrera}, F.~J. and {Sekiguchi}, K. and {Yamada}, T. and {Simpson}, C. and {Hasinger}, G. and {Mateos}, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/591083},
	eprint = {0806.2846},
	journal = {\apjs},
	keywords = {Catalogs, Cosmology: Diffuse Radiation, Galaxies: Active, X-Rays: Galaxies, X-Rays: General},
	month = nov,
	pages = {124-141},
	title = {{The Subaru/XMM-Newton Deep Survey (SXDS). III. X-Ray Data}},
	volume = 179,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/591083}}

@article{Simpson:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.372..741S},
	author = {{Simpson}, C. and {Mart{\'{\i}}nez-Sansigre}, A. and {Rawlings}, S. and {Ivison}, R. and {Akiyama}, M. and {Sekiguchi}, K. and {Takata}, T. and {Ueda}, Y. and {Watson}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2006.10907.x},
	eprint = {arXiv:astro-ph/0609529},
	journal = {\mnras},
	keywords = {catalogues, surveys, galaxies: active, radio continuum: galaxies},
	month = oct,
	pages = {741-757},
	title = {{Radio imaging of the Subaru/XMM-Newton Deep Field - I. The 100-{$\mu$}Jy catalogue, optical identifications, and the nature of the faint radio source population}},
	volume = 372,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10907.x}}

@article{Fadda:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004AJ....128....1F},
	author = {{Fadda}, D. and {Jannuzi}, B.~T. and {Ford}, A. and {Storrie-Lombardi}, L.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/421366},
	eprint = {arXiv:astro-ph/0403490},
	journal = {\aj},
	keywords = {Catalogs, Galaxies: Photometry},
	month = jul,
	pages = {1-15},
	title = {{The Spitzer Space Telescope First-Look Survey: KPNO Mosaic-1 R-Band Images and Source Catalogs}},
	volume = 128,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/421366}}

@article{Georgakakis:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.354..127G},
	author = {{Georgakakis}, A. and {Hopkins}, A.~M. and {Afonso}, J. and {Sullivan}, M. and {Mobasher}, B. and {Cram}, L.~E.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2004.08174.x},
	eprint = {arXiv:astro-ph/0407078},
	journal = {\mnras},
	keywords = {surveys, galaxies: general, X-rays: galaxies, X-rays: general},
	month = oct,
	pages = {127-141},
	title = {{The Phoenix Deep Survey: the radio properties of the hard X-ray-selected sample}},
	volume = 354,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.08174.x}}

@article{Ciliegi:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.342..575C},
	author = {{Ciliegi}, P. and {Vignali}, C. and {Comastri}, A. and {Fiore}, F. and {La Franca}, F. and {Perola}, G.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2003.06573.x},
	eprint = {arXiv:astro-ph/0302556},
	journal = {\mnras},
	keywords = {surveys, quasars: general, radio continuum: galaxies},
	month = jun,
	pages = {575-586},
	title = {{The BeppoSAX High Energy Large Area Survey (HELLAS) - VI. The radio properties}},
	volume = 342,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2003.06573.x}}

@article{Barger:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001AJ....122.2177B},
	author = {{Barger}, A.~J. and {Cowie}, L.~L. and {Bautz}, M.~W. and {Brandt}, W.~N. and {Garmire}, G.~P. and {Hornschemeier}, A.~E. and {Ivison}, R.~J. and {Owen}, F.~N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/323454},
	eprint = {arXiv:astro-ph/0106219},
	journal = {\aj},
	keywords = {Cosmology: Observations, Galaxies: Active, Galaxies: Distances and Redshifts, Galaxies: Evolution, Galaxies: Formation},
	month = nov,
	pages = {2177-2189},
	title = {{Supermassive Black Hole Accretion History Inferred from a Large Sample of Chandra Hard X-Ray Sources}},
	volume = 122,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/323454}}

@article{Ibar:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386..953I},
	archiveprefix = {arXiv},
	author = {{Ibar}, E. and {Cirasuolo}, M. and {Ivison}, R. and {Best}, P. and {Smail}, I. and {Biggs}, A. and {Simpson}, C. and {Dunlop}, J. and {Almaini}, O. and {McLure}, R. and {Foucaud}, S. and {Rawlings}, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.13077.x},
	eprint = {0802.2694},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: fundamental parameters, galaxies: high-redshift, galaxies: starburst},
	month = may,
	pages = {953-962},
	title = {{Exploring the infrared/radio correlation at high redshift}},
	volume = 386,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13077.x}}

@article{Garn:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.394..105G},
	archiveprefix = {arXiv},
	author = {{Garn}, T. and {Alexander}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.14296.x},
	eprint = {0812.0281},
	journal = {\mnras},
	keywords = {infrared: galaxies , radio continuum: galaxies},
	month = mar,
	pages = {105-116},
	title = {{Radio source stacking and the infrared/radio correlation at {$\mu$}Jy flux densities}},
	volume = 394,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.14296.x}}

@article{Beswick:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.385.1143B},
	archiveprefix = {arXiv},
	author = {{Beswick}, R.~J. and {Muxlow}, T.~W.~B. and {Thrall}, H. and {Richards}, A.~M.~S. and {Garrington}, S.~T.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.12931.x},
	eprint = {0801.1035},
	journal = {\mnras},
	keywords = {galaxies: high-redshift , galaxies: starburst , infrared: galaxies , radio continuum: galaxies},
	month = apr,
	pages = {1143-1154},
	title = {{An evolution of the infrared-radio correlation at very low flux densities?}},
	volume = 385,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.12931.x}}

@article{ElBouchefry:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.396.2011E},
	archiveprefix = {arXiv},
	author = {{El Bouchefry}, K.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2009.14915.x},
	eprint = {0904.2586},
	journal = {\mnras},
	keywords = {galaxies: active , galaxies: high-redshift , X-rays: diffuse background , X-rays: galaxies},
	month = jul,
	pages = {2011-2037},
	primaryclass = {astro-ph.CO},
	title = {{X-ray identifications of FIRST radio sources in the XBo{\"o}tes field}},
	volume = 396,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.14915.x}}

@article{Brusa:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...409...65B},
	author = {{Brusa}, M. and {Comastri}, A. and {Mignoli}, M. and {Fiore}, F. and {Ciliegi}, P. and {Vignali}, C. and {Severgnini}, P. and {Cocchia}, F. and {La Franca}, F. and {Matt}, G. and {Perola}, G.~C. and {Maiolino}, R. and {Baldi}, A. and {Molendi}, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20031107},
	eprint = {arXiv:astro-ph/0307368},
	journal = {\aap},
	keywords = {surveys, galaxies: active, X-ray: galaxies, X-ray: diffuse background},
	month = oct,
	pages = {65-78},
	title = {{The HELLAS2XMM survey. III. Multiwavelength observations of hard X-ray selected sources in the PKS 0312-77 field}},
	volume = 409,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031107}}

@article{Smolcic:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ApJS..177...14S},
	archiveprefix = {arXiv},
	author = {{Smol{\v c}i{\'c}}, V. and {Schinnerer}, E. and {Scodeggio}, M. and {Franzetti}, P. and {Aussel}, H. and {Bondi}, M. and {Brusa}, M. and {Carilli}, C.~L. and {Capak}, P. and {Charlot}, S. and {Ciliegi}, P. and {Ilbert}, O. and {Ivezi{\'c}}, {\v Z}. and {Jahnke}, K. and {McCracken}, H.~J. and {Obri{\'c}}, M. and {Salvato}, M. and {Sanders}, D.~B. and {Scoville}, N. and {Trump}, J.~R. and {Tremonti}, C. and {Tasca}, L. and {Walcher}, C.~J. and {Zamorani}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/588028},
	eprint = {0803.0997},
	journal = {\apjs},
	keywords = {Cosmology: Observations, Radio Continuum: Galaxies, Surveys},
	month = jul,
	pages = {14-38},
	title = {{A New Method to Separate Star-forming from AGN Galaxies at Intermediate Redshift: The Submillijansky Radio Population in the VLA-COSMOS Survey}},
	volume = 177,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/588028}}

@inproceedings{vanBreugel:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999ldss.work..236V},
	author = {{van Breugel}, W. and {De Breuck}, C. and {R{\"o}ttgering}, H. and {Miley}, G. and {Stanford}, A.},
	booktitle = {Looking Deep in the Southern Sky},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{R.~Morganti; W.~J.~Couch}},
	eprint = {arXiv:astro-ph/9806135},
	pages = {236},
	title = {{Very High Redshift Radio Galaxies}},
	year = 1999}

@article{Lusso:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...512A..34L},
	archiveprefix = {arXiv},
	author = {{Lusso}, E. and {Comastri}, A. and {Vignali}, C. and {Zamorani}, G. and {Brusa}, M. and {Gilli}, R. and {Iwasawa}, K. and {Salvato}, M. and {Civano}, F. and {Elvis}, M. and {Merloni}, A. and {Bongiorno}, A. and {Trump}, J.~R. and {Koekemoer}, A.~M. and {Schinnerer}, E. and {Le Floc'h}, E. and {Cappelluti}, N. and {Jahnke}, K. and {Sargent}, M. and {Silverman}, J. and {Mainieri}, V. and {Fiore}, F. and {Bolzonella}, M. and {Le F{\`e}vre}, O. and {Garilli}, B. and {Iovino}, A. and {Kneib}, J.~P. and {Lamareille}, F. and {Lilly}, S. and {Mignoli}, M. and {Scodeggio}, M. and {Vergani}, D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/200913298},
	eprint = {0912.4166},
	journal = {\aap},
	keywords = {galaxies: active, Galaxy: evolution, quasars: general, methods: statistical},
	month = mar,
	pages = {A34+},
	primaryclass = {astro-ph.CO},
	title = {{The X-ray to optical-UV luminosity ratio of X-ray selected type 1 AGN in XMM-COSMOS}},
	volume = 512,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200913298}}

@article{deBreuck:2000,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2000A%26AS..143..303D},
	author = {{De Breuck}, C. and {van Breugel}, W. and {R{\"o}ttgering}, H.~J.~A. and {Miley}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/aas:2000181},
	eprint = {arXiv:astro-ph/0002297},
	journal = {\aaps},
	keywords = {SURVEYS, GALAXIES: ACTIVE, RADIO CONTINUUM: GALAXIES},
	month = apr,
	pages = {303-333},
	title = {{A sample of 669 ultra steep spectrum radio sources to find high redshift radio galaxies}},
	volume = 143,
	year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/aas:2000181}}

@article{Nesvadba:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...491..407N},
	archiveprefix = {arXiv},
	author = {{Nesvadba}, N.~P.~H. and {Lehnert}, M.~D. and {De Breuck}, C. and {Gilbert}, A.~M. and {van Breugel}, W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:200810346},
	eprint = {0809.5171},
	journal = {\aap},
	keywords = {galaxies: high-redshift, galaxies: formation, galaxies: jets, infrared: galaxies, galaxies: kinematics and dynamics},
	month = nov,
	pages = {407-424},
	title = {{Evidence for powerful AGN winds at high redshift: dynamics of galactic outflows in radio galaxies during the ``Quasar Era''}},
	volume = 491,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200810346}}

@article{Nesvadba:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...475..145N},
	archiveprefix = {arXiv},
	author = {{Nesvadba}, N.~P.~H. and {Lehnert}, M.~D. and {De Breuck}, C. and {Gilbert}, A. and {van Breugel}, W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20078175},
	eprint = {0708.4150},
	journal = {\aap},
	keywords = {galaxies: high-redshift, galaxies: formation, galaxies: kinematics and dynamics, infrared: galaxies, galaxies: jets},
	month = nov,
	pages = {145-153},
	title = {{Compact radio sources and jet-driven AGN feedback in the early universe: constraints from integral-field spectroscopy}},
	volume = 475,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078175}}

@article{Komissarov:1994,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1994A%26A...285...27K},
	author = {{Komissarov}, S.~S. and {Gubanov}, A.~G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\aap},
	keywords = {GALAXIES: CLUSTERS OF, GALAXIES: ACTIVE, RADIATION MECHANISMS: NON THERMAL, RADIO CONTINUUM: GALAXIES},
	month = may,
	pages = {27-43},
	title = {{Relic radio galaxies: evolution of synchrotron spectrum}},
	volume = 285,
	year = 1994}

@article{Murgia:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1011.0567M},
	archiveprefix = {arXiv},
	author = {{Murgia}, M. and {Parma}, P. and {Mack}, {K.~-.} and {de Ruiter}, H.~R. and {Fanti}, R. and {Govoni}, F. and {Tarchi}, A. and {Giacintucci}, S. and {Markevitch}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {1011.0567},
	journal = {ArXiv e-prints},
	keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
	month = nov,
	primaryclass = {astro-ph.CO},
	title = {{Dying Radio Sources in Clusters}},
	year = 2010}

@book{Longair:1992,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1992hea..book.....L},
	author = {{Longair}, M.~S.},
	booktitle = {High Energy Astrophysics, by Malcolm S.~Longair, pp.~436.~ISBN 0521387736.~Cambridge, UK: Cambridge University Press, March 1992.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{Willcox, P.~J.}},
	month = mar,
	title = {{High energy astrophysics. Vol.1: Particles, photons and their detection}},
	year = 1992}

@article{Barger:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002AJ....124.1839B},
	author = {{Barger}, A.~J. and {Cowie}, L.~L. and {Brandt}, W.~N. and {Capak}, P. and {Garmire}, G.~P. and {Hornschemeier}, A.~E. and {Steffen}, A.~T. and {Wehner}, E.~H.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/342448},
	eprint = {arXiv:astro-ph/0206370},
	journal = {\aj},
	keywords = {Cosmology: Observations, Galaxies: Evolution, Galaxies: Formation},
	month = oct,
	pages = {1839-1885},
	title = {{X-Ray, Optical, and Infrared Imaging and Spectral Properties of the 1 Ms Chandra Deep Field North Sources}},
	volume = 124,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/342448}}

@article{Trouille:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...703.2160T},
	archiveprefix = {arXiv},
	author = {{Trouille}, L. and {Barger}, A.~J. and {Cowie}, L.~L. and {Yang}, Y. and {Mushotzky}, R.~F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/703/2/2160},
	eprint = {0908.0002},
	journal = {\apj},
	keywords = {cosmology: observations, galaxies: active},
	month = oct,
	pages = {2160-2170},
	primaryclass = {astro-ph.CO},
	title = {{The OPTX Project. III. X-ray Versus Optical Spectral Type for Active Galactic Nuclei}},
	volume = 703,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/703/2/2160}}

@inproceedings{Panessa:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007AIPC..924..830P},
	author = {{Panessa}, F. and {Barcons}, X. and {Bassani}, L. and {Cappi}, M. and {Carrera}, F.~J. and {Dadina}, M. and {Ho}, L.~C. and {Iwasawa}, K. and {Pellegrini}, S.},
	booktitle = {The Multicolored Landscape of Compact Objects and Their Explosive Origins},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1063/1.2774949},
	editor = {{T.~di Salvo, G.~L.~Israel, L.~Piersant, L.~Burderi, G.~Matt, A.~Tornambe, \&amp; M.~T.~Menna}},
	eprint = {arXiv:astro-ph/0612593},
	keywords = {Active and peculiar galaxies and related systems, X-ray sources; X-ray bursts, Galactic nuclei , circumnuclear matter, and bulges, Magnitudes and colors; luminosities},
	month = aug,
	pages = {830-835},
	series = {American Institute of Physics Conference Series},
	title = {{Multi-wavelength and black hole mass properties of Low Luminosity Active Nuclei}},
	volume = 924,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1063/1.2774949}}

@article{Sikora:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...658..815S},
	author = {{Sikora}, M. and {Stawarz}, {\L}. and {Lasota}, {J.-P.}},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/511972},
	eprint = {arXiv:astro-ph/0604095},
	journal = {\apj},
	keywords = {Galaxies: Jets, Magnetohydrodynamics: MHD, Radiation Mechanisms: Nonthermal},
	month = apr,
	pages = {815-828},
	title = {{Radio Loudness of Active Galactic Nuclei: Observational Facts and Theoretical Implications}},
	volume = 658,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/511972}}

@article{Ho:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...564..120H},
	author = {{Ho}, L.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/324399},
	eprint = {arXiv:astro-ph/0110440},
	journal = {\apj},
	keywords = {Black Hole Physics, Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, Galaxies: Quasars: General, Radio Continuum: Galaxies},
	month = jan,
	pages = {120-132},
	title = {{On the Relationship between Radio Emission and Black Hole Mass in Galactic Nuclei}},
	volume = 564,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/324399}}

@article{Ishibashi:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1010.5591I},
	archiveprefix = {arXiv},
	author = {{Ishibashi}, W. and {Courvoisier}, {T.~J.~-.}},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {1010.5591},
	journal = {ArXiv e-prints},
	keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Galaxy Astrophysics},
	month = oct,
	primaryclass = {astro-ph.HE},
	title = {{Synchrotron radio emission in radio-quiet AGNs}},
	year = 2010}

@article{Ulvestad:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...621..123U},
	author = {{Ulvestad}, J.~S. and {Antonucci}, R.~R.~J. and {Barvainis}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/427426},
	eprint = {arXiv:astro-ph/0411678},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Quasars: General, Radio Continuum: Galaxies},
	month = mar,
	pages = {123-129},
	title = {{VLBA Imaging of Central Engines in Radio-Quiet Quasars}},
	volume = 621,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/427426}}

@article{Debuhr:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1006.3312D},
	archiveprefix = {arXiv},
	author = {{DeBuhr}, J. and {Quataert}, E. and {Ma}, {C.-P.}},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {1006.3312},
	journal = {ArXiv e-prints},
	keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
	month = jun,
	primaryclass = {astro-ph.CO},
	title = {{The Growth of Massive Black Holes in Galaxy Merger Simulations with Feedback by Radiation Pressure}},
	year = 2010}

@article{Wilkes:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009ApJS..185..433W},
	archiveprefix = {arXiv},
	author = {{Wilkes}, B.~J. and {Kilgard}, R. and {Kim}, {D.-W.} and {Kim}, M. and {Polletta}, M. and {Lonsdale}, C. and {Smith}, H.~E. and {Surace}, J. and {Owen}, F.~N. and {Franceschini}, A. and {Siana}, B. and {Shupe}, D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0067-0049/185/2/433},
	eprint = {0910.2675},
	journal = {\apjs},
	keywords = {catalogs, quasars: general, surveys, X-rays: galaxies},
	month = dec,
	pages = {433-450},
	primaryclass = {astro-ph.HE},
	title = {{The SWIRE/Chandra Survey: The X-ray Sources}},
	volume = 185,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/185/2/433}}

@article{Page:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.369..156P},
	author = {{Page}, M.~J. and {Loaring}, N.~S. and {Dwelly}, T. and {Mason}, K.~O. and {McHardy}, I. and {Gunn}, K. and {Moss}, D. and {Sasseen}, T. and {Cordova}, F. and {Kennea}, J. and {Seymour}, N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2006.10278.x},
	eprint = {arXiv:astro-ph/0604015},
	journal = {\mnras},
	keywords = {surveys: galaxies: active: quasars: general: X-rays: galaxies, surveys, galaxies: active, quasars: general, X-rays: galaxies},
	month = jun,
	pages = {156-170},
	title = {{X-ray spectra of sources in the 13^{H} XMM-Newton/Chandra deep field}},
	volume = 369,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10278.x}}

@article{Jamrozy:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.378..581J},
	author = {{Jamrozy}, M. and {Konar}, C. and {Saikia}, D.~J. and {Stawarz}, {\L}. and {Mack}, {K.-H.} and {Siemiginowska}, A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2007.11782.x},
	eprint = {arXiv:astro-ph/0703723},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: individual: 4C29.30, galaxies: nuclei, radio continuum: galaxies},
	month = jun,
	pages = {581-593},
	title = {{Intermittent jet activity in the radio galaxy 4C29.30?}},
	volume = 378,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.11782.x}}

@article{Lal:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.374.1085L},
	author = {{Lal}, D.~V. and {Rao}, A.~P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2006.11225.x},
	eprint = {arXiv:astro-ph/0610678},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: formation, radio continuum: galaxies},
	month = jan,
	pages = {1085-1102},
	title = {{Giant Metrewave Radio Telescope observations of X-shaped radio sources}},
	volume = 374,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.11225.x}}

@article{Jamrozy:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...427...79J},
	author = {{Jamrozy}, M. and {Klein}, U. and {Mack}, {K.-H.} and {Gregorini}, L. and {Parma}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20048056},
	journal = {\aap},
	keywords = {radio continuum: galaxies, galaxies: active, galaxies: individual: B2 0924+30},
	month = nov,
	pages = {79-86},
	title = {{Spectral ageing in the relic radio galaxy B2 0924+30}},
	volume = 427,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20048056}}

@article{Parma:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...470..875P},
	archiveprefix = {arXiv},
	author = {{Parma}, P. and {Murgia}, M. and {de Ruiter}, H.~R. and {Fanti}, R. and {Mack}, {K.-H.} and {Govoni}, F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20077592},
	eprint = {0705.3209},
	journal = {\aap},
	keywords = {radio continuum: galaxies, galaxies: active},
	month = aug,
	pages = {875-888},
	title = {{In search of dying radio sources in the local universe}},
	volume = 470,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077592}}

@article{Fanti:1990,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1990A%26A...231..333F},
	author = {{Fanti}, R. and {Fanti}, C. and {Schilizzi}, R.~T. and {Spencer}, R.~E. and {Nan Rendong} and {Parma}, P. and {van Breugel}, W.~J.~M. and {Venturi}, T.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\aap},
	keywords = {QUASARS, RADIO JETS (ASTRONOMY), RADIO SOURCES (ASTRONOMY), RADIO SPECTRA, COSMOLOGY, VERY LARGE ARRAY (VLA), VERY LONG BASE INTERFEROMETRY},
	month = may,
	pages = {333-346},
	title = {{On the nature of compact steep spectrum radio sources}},
	volume = 231,
	year = 1990}

@article{Tajer:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...467...73T},
	author = {{Tajer}, M. and {Polletta}, M. and {Chiappetti}, L. and {Maraschi}, L. and {Trinchieri}, G. and {Maccagni}, D. and {Andreon}, S. and {Garcet}, O. and {Surdej}, J. and {Pierre}, M. and {Le F{\`e}vre}, O. and {Franceschini}, A. and {Lonsdale}, C.~J. and {Surace}, J.~A. and {Shupe}, D.~L. and {Fang}, F. and {Rowan-Robinson}, M. and {Smith}, H.~E. and {Tresse}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20066667},
	eprint = {arXiv:astro-ph/0703263},
	journal = {\aap},
	keywords = {X-rays: general, surveys, galaxies: active},
	month = may,
	pages = {73-91},
	title = {{Obscured and unobscured AGN populations in a hard-X-ray selected sample of the XMDS survey}},
	volume = 467,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20066667}}

@inproceedings{Prandoni:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009pra..confE..36P},
	author = {{Prandoni}, I. and {Morganti}, R. and {Mignano}, A.},
	booktitle = {Panoramic Radio Astronomy: Wide-field 1-2 GHz Research on Galaxy Evolution},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	title = {{The AGN component in radio deep fields: the First Look Survey}},
	year = 2009}

@article{allen06,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.372...21A},
	author = {{Allen}, S.~W. and {Dunn}, R.~J.~H. and {Fabian}, A.~C. and {Taylor}, G.~B. and {Reynolds}, C.~S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:49:32 +0200},
	doi = {10.1111/j.1365-2966.2006.10778.x},
	eprint = {arXiv:astro-ph/0602549},
	journal = {\mnras},
	keywords = {accretion, accretion discs: black hole physics: galaxies: active: galaxies: jets: X-rays: galaxies, accretion discs, black hole physics, galaxies: active, galaxies: jets, X-rays: galaxies},
	month = oct,
	pages = {21-30},
	title = {{The relation between accretion rate and jet power in X-ray luminous elliptical galaxies}},
	volume = 372,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10778.x}}

@article{Ogle:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...647..161O},
	author = {{Ogle}, P. and {Whysong}, D. and {Antonucci}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/505337},
	eprint = {arXiv:astro-ph/0601485},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Jets, Infrared: Galaxies, Galaxies: Quasars: General},
	month = aug,
	pages = {161-171},
	title = {{Spitzer Reveals Hidden Quasar Nuclei in Some Powerful FR II Radio Galaxies}},
	volume = 647,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/505337}}

@article{Hardcastle:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.396.1929H},
	archiveprefix = {arXiv},
	author = {{Hardcastle}, M.~J. and {Evans}, D.~A. and {Croston}, J.~H.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2009.14887.x},
	eprint = {0904.1323},
	journal = {\mnras},
	keywords = {galaxies: active , X-rays: galaxies},
	month = jul,
	pages = {1929-1952},
	title = {{The active nuclei of z {\lt} 1.0 3CRR radio sources}},
	volume = 396,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.14887.x}}

@article{Hardcastle:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.376.1849H},
	author = {{Hardcastle}, M.~J. and {Evans}, D.~A. and {Croston}, J.~H.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2007.11572.x},
	eprint = {arXiv:astro-ph/0701857},
	journal = {\mnras},
	keywords = {galaxies: active, X-rays: galaxies},
	month = apr,
	pages = {1849-1856},
	title = {{Hot and cold gas accretion and feedback in radio-loud active galaxies}},
	volume = 376,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.11572.x}}

@article{Deyoung:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...710..743D},
	archiveprefix = {arXiv},
	author = {{De Young}, D.~S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/710/1/743},
	eprint = {1001.1178},
	journal = {\apj},
	keywords = {galaxies: active, galaxies: evolution, galaxies: jets, radio continuum: galaxies, turbulence},
	month = feb,
	pages = {743-754},
	title = {{How Does Radio AGN Feedback Feed Back?}},
	volume = 710,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/710/1/743}}

@article{Fabian:2000,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.318L..65F},
	author = {{Fabian}, A.~C. and {Sanders}, J.~S. and {Ettori}, S. and {Taylor}, G.~B. and {Allen}, S.~W. and {Crawford}, C.~S. and {Iwasawa}, K. and {Johnstone}, R.~M. and {Ogle}, P.~M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2000.03904.x},
	eprint = {arXiv:astro-ph/0007456},
	journal = {\mnras},
	keywords = {GALAXIES: CLUSTERS: INDIVIDUAL: PERSEUS, COOLING FLOWS, GALAXIES: INDIVIDUAL: NGC 1275, X-RAYS: GALAXIES},
	month = nov,
	pages = {L65-L68},
	title = {{Chandra imaging of the complex X-ray core of the Perseus cluster}},
	volume = 318,
	year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2000.03904.x}}

@article{Dimatteo:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005Natur.433..604D},
	author = {{Di Matteo}, T. and {Springel}, V. and {Hernquist}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1038/nature03335},
	eprint = {arXiv:astro-ph/0502199},
	journal = {\nat},
	month = feb,
	pages = {604-607},
	title = {{Energy input from quasars regulates the growth and activity of black holes and their host galaxies}},
	volume = 433,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature03335}}

@article{Croton:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.365...11C},
	author = {{Croton}, D.~J. and {Springel}, V. and {White}, S.~D.~M. and {De Lucia}, G. and {Frenk}, C.~S. and {Gao}, L. and {Jenkins}, A. and {Kauffmann}, G. and {Navarro}, J.~F. and {Yoshida}, N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2005.09675.x},
	eprint = {arXiv:astro-ph/0508046},
	journal = {\mnras},
	keywords = {black hole physics, galaxies: active, cooling flows, galaxies: evolution, galaxies: formation, cosmology: theory},
	month = jan,
	pages = {11-28},
	title = {{The many lives of active galactic nuclei: cooling flows, black holes and the luminosities and colours of galaxies}},
	volume = 365,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09675.x}}

@article{Fabian:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.308L..39F},
	author = {{Fabian}, A.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.1999.03017.x},
	eprint = {arXiv:astro-ph/9908064},
	journal = {\mnras},
	month = oct,
	pages = {L39-L43},
	title = {{The obscured growth of massive black holes}},
	volume = 308,
	year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1999.03017.x}}

@article{merloni08,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.388.1011M},
	archiveprefix = {arXiv},
	author = {{Merloni}, A. and {Heinz}, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:48:42 +0200},
	doi = {10.1111/j.1365-2966.2008.13472.x},
	eprint = {0805.2499},
	journal = {\mnras},
	keywords = {accretion, accretion discs , black hole physics , galaxies: active , galaxies: evolution , quasars: general},
	month = aug,
	pages = {1011-1030},
	title = {{A synthesis model for AGN evolution: supermassive black holes growth and feedback modes}},
	volume = 388,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13472.x}}

@article{Hopkins:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...669...67H},
	archiveprefix = {arXiv},
	author = {{Hopkins}, P.~F. and {Hernquist}, L. and {Cox}, T.~J. and {Robertson}, B. and {Krause}, E.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/521601},
	eprint = {0707.4005},
	journal = {\apj},
	keywords = {Cosmology: Theory, Galaxies: Active, Galaxies: Evolution, Galaxies: Quasars: General},
	month = nov,
	pages = {67-73},
	title = {{An Observed Fundamental Plane Relation for Supermassive Black Holes}},
	volume = 669,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/521601}}

@article{Tremaine:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...574..740T},
	author = {{Tremaine}, S. and {Gebhardt}, K. and {Bender}, R. and {Bower}, G. and {Dressler}, A. and {Faber}, S.~M. and {Filippenko}, A.~V. and {Green}, R. and {Grillmair}, C. and {Ho}, L.~C. and {Kormendy}, J. and {Lauer}, T.~R. and {Magorrian}, J. and {Pinkney}, J. and {Richstone}, D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/341002},
	eprint = {arXiv:astro-ph/0203468},
	journal = {\apj},
	keywords = {Black Hole Physics, Galaxies: Bulges, Galaxies: Fundamental Parameters, Galaxies: Nuclei, Galaxy: Bulge, Galaxy: Kinematics and Dynamics},
	month = aug,
	pages = {740-753},
	title = {{The Slope of the Black Hole Mass versus Velocity Dispersion Correlation}},
	volume = 574,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/341002}}

@article{Zakamska:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003AJ....126.2125Z},
	author = {{Zakamska}, N.~L. and {Strauss}, M.~A. and {Krolik}, J.~H. and {Collinge}, M.~J. and {Hall}, P.~B. and {Hao}, L. and {Heckman}, T.~M. and {Ivezi{\'c}}, {\v Z}. and {Richards}, G.~T. and {Schlegel}, D.~J. and {Schneider}, D.~P. and {Strateva}, I. and {Vanden Berk}, D.~E. and {Anderson}, S.~F. and {Brinkmann}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/378610},
	eprint = {arXiv:astro-ph/0309551},
	journal = {\aj},
	keywords = {Galaxies: Active, Galaxies: Quasars: Emission Lines, Galaxies: Quasars: General, Surveys},
	month = nov,
	pages = {2125-2144},
	title = {{Candidate Type II Quasars from the Sloan Digital Sky Survey. I. Selection and Optical Properties of a Sample at 0.3{\lt}Z{\lt}0.83}},
	volume = 126,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/378610}}

@article{Roussel:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...646..841R},
	author = {{Roussel}, H. and {Helou}, G. and {Smith}, J.~D. and {Draine}, B.~T. and {Hollenbach}, D.~J. and {Moustakas}, J. and {Spoon}, H.~W. and {Kennicutt}, R.~C. and {Rieke}, G.~H. and {Walter}, F. and {Armus}, L. and {Dale}, D.~A. and {Sheth}, K. and {Bendo}, G.~J. and {Engelbracht}, C.~W. and {Gordon}, K.~D. and {Meyer}, M.~J. and {Regan}, M.~W. and {Murphy}, E.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/505038},
	eprint = {arXiv:astro-ph/0604267},
	journal = {\apj},
	keywords = {ISM: Dust, Extinction, Galaxies: Evolution, Galaxies: Individual: NGC Number: NGC 1377, Galaxies: ISM, Galaxies: Starburst, Infrared: Galaxies},
	month = aug,
	pages = {841-857},
	title = {{The Opaque Nascent Starburst in NGC 1377: Spitzer SINGS Observations}},
	volume = 646,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/505038}}

@article{Urry:1995,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1995PASP..107..803U},
	author = {{Urry}, C.~M. and {Padovani}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/133630},
	eprint = {arXiv:astro-ph/9506063},
	journal = {\pasp},
	keywords = {GALAXIES: ACTIVE, GALAXIES: FUNDAMENTAL PARAMETERS},
	month = sep,
	pages = {803-+},
	title = {{Unified Schemes for Radio-Loud Active Galactic Nuclei}},
	volume = 107,
	year = 1995,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/133630}}

@inproceedings{Wilson:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003SPIE.4841..451W},
	author = {{Wilson}, J.~C. and {Eikenberry}, S.~S. and {Henderson}, C.~P. and {Hayward}, T.~L. and {Carson}, J.~C. and {Pirger}, B. and {Barry}, D.~J. and {Brandl}, B.~R. and {Houck}, J.~R. and {Fitzgerald}, G.~J. and {Stolberg}, T.~M.},
	booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1117/12.460336},
	editor = {{M.~Iye \& A.~F.~M.~Moorwood}},
	month = mar,
	pages = {451-458},
	series = {Presented at the Society of Photo-Optical Instrumentation Engineers (SPIE) Conference},
	title = {{A Wide-Field Infrared Camera for the Palomar 200-inch Telescope}},
	volume = 4841,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.460336}}

@article{Tueller:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010ApJS..186..378T},
	archiveprefix = {arXiv},
	author = {{Tueller}, J. and {Baumgartner}, W.~H. and {Markwardt}, C.~B. and {Skinner}, G.~K. and {Mushotzky}, R.~F. and {Ajello}, M. and {Barthelmy}, S. and {Beardmore}, A. and {Brandt}, W.~N. and {Burrows}, D. and {Chincarini}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0067-0049/186/2/378},
	eprint = {0903.3037},
	journal = {\apjs},
	keywords = {catalogs, galaxies: active, gamma rays: observations, novae, cataclysmic variables, surveys, X-rays: binaries},
	month = feb,
	pages = {378-405},
	title = {{The 22 Month Swift-BAT All-Sky Hard X-ray Survey}},
	volume = 186,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/186/2/378}}

@article{bird10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010ApJS..186....1B},
	archiveprefix = {arXiv},
	author = {{Bird}, A.~J. and {Bazzano}, A. and {Bassani}, L. and {Capitanio}, F. and {Fiocchi}, M. and {Hill}, A.~B. and {Malizia}, A. and {McBride}, V.~A. and {Scaringi}, S. and {Sguera}, V. and {Stephen}, J.~B. and {Ubertini}, P. and {Dean}, A.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:50:27 +0200},
	doi = {10.1088/0067-0049/186/1/1},
	eprint = {0910.1704},
	journal = {\apjs},
	keywords = {Galaxy: general, gamma rays: observations, surveys},
	month = jan,
	pages = {1-9},
	title = {{The Fourth IBIS/ISGRI Soft Gamma-ray Survey Catalog}},
	volume = 186,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/186/1/1}}

@article{Malizia:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.399..944M},
	archiveprefix = {arXiv},
	author = {{Malizia}, A. and {Stephen}, J.~B. and {Bassani}, L. and {Bird}, A.~J. and {Panessa}, F. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2009.15330.x},
	eprint = {0906.5544},
	journal = {\mnras},
	keywords = {galaxies: active , galaxies: nuclei , X-rays: galaxies},
	month = oct,
	pages = {944-951},
	title = {{The fraction of Compton-thick sources in an INTEGRAL complete AGN sample}},
	volume = 399,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15330.x}}

@article{haardt1991,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...380L..51H},
	author = {{Haardt}, F. and {Maraschi}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:48:31 +0200},
	doi = {10.1086/186171},
	journal = {\apjl},
	keywords = {ACCRETION DISKS, ASTRONOMICAL MODELS, EMISSION SPECTRA, SEYFERT GALAXIES, X RAY SPECTRA, COMPUTATIONAL ASTROPHYSICS, GALACTIC NUCLEI, GRAVITATIONAL EFFECTS, INTERSTELLAR MAGNETIC FIELDS, MAGNETIC FIELD RECONNECTION},
	month = oct,
	pages = {L51-L54},
	title = {{A two-phase model for the X-ray emission from Seyfert galaxies}},
	volume = 380,
	year = 1991,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/186171}}

@article{Hardcastle:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.309..969H},
	author = {{Hardcastle}, M.~J. and {Worrall}, D.~M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.1999.02945.x},
	eprint = {arXiv:astro-ph/9907034},
	journal = {\mnras},
	month = nov,
	pages = {969-990},
	title = {{ROSAT X-ray observations of 3CRR radio sources}},
	volume = 309,
	year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1999.02945.x}}

@article{Ulvestad:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...562L.133U},
	author = {{Ulvestad}, J.~S. and {Ho}, L.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/338254},
	eprint = {arXiv:astro-ph/0110535},
	journal = {\apjl},
	keywords = {Accretion, Accretion Disks, Galaxies: Active, Galaxies: Individual: NGC Number: NGC 3147, Galaxies: Individual: NGC Number: NGC 4203, Galaxies: Individual: NGC Number: NGC 4579, Galaxies: Nuclei, Radio Continuum: Galaxies},
	month = dec,
	pages = {L133-L136},
	title = {{The Origin of Radio Emission in Low-Luminosity Active Galactic Nuclei: Jets, Accretion Flows, or Both?}},
	volume = 562,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/338254}}

@article{Lal:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010AJ....139.1089V},
	archiveprefix = {arXiv},
	author = {{Vir Lal}, D. and {Ho}, L.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-6256/139/3/1089},
	eprint = {1001.1476},
	journal = {\aj},
	keywords = {galaxies: active, galaxies: jets, galaxies: nuclei, galaxies: Seyfert, galaxies: structure, radio continuum: galaxies},
	month = mar,
	pages = {1089-1105},
	title = {{The Radio Properties of Type 2 Quasars}},
	volume = 139,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/139/3/1089}}

@article{Trouille:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ApJS..179....1T},
	archiveprefix = {arXiv},
	author = {{Trouille}, L. and {Barger}, A.~J. and {Cowie}, L.~L. and {Yang}, Y. and {Mushotzky}, R.~F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/591648},
	eprint = {0811.0824},
	journal = {\apjs},
	keywords = {Cosmology: Observations, Galaxies: Active},
	month = nov,
	pages = {1-18},
	title = {{The OPTX Project. I. The Flux and Redshift Catalogs for the CLANS, CLASXS, and CDF-N Fields}},
	volume = 179,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/591648}}

@article{Vollmer:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...489...49V},
	archiveprefix = {arXiv},
	author = {{Vollmer}, B. and {Krichbaum}, T.~P. and {Angelakis}, E. and {Kovalev}, Y.~Y.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20078857},
	eprint = {0806.3694},
	journal = {\aap},
	keywords = {radio continuum: galaxies},
	month = oct,
	pages = {49-55},
	title = {{Quasi-simultaneous multi-frequency observations of inverted-spectrum GPS candidate sources}},
	volume = 489,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078857}}

@article{sopp91,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1991MNRAS.251P..14S},
	author = {{Sopp}, H.~M. and {Alexander}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\mnras},
	keywords = {FAR INFRARED RADIATION, LUMINOSITY, QUASARS, RADIO EMISSION, ACTIVE GALACTIC NUCLEI, RADIO GALAXIES, SEYFERT GALAXIES, STARBURST GALAXIES},
	month = jul,
	pages = {14P-16P},
	title = {{A composite plot of far-infrared versus radio luminosity, and the origin of far-infrared luminosity in quasars}},
	volume = 251,
	year = 1991}

@article{vanBreugel:1998,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...502..614V},
	author = {{van Breugel}, W.~J.~M. and {Stanford}, S.~A. and {Spinrad}, H. and {Stern}, D. and {Graham}, J.~R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/305925},
	eprint = {arXiv:astro-ph/9803019},
	journal = {\apj},
	keywords = {GALAXIES: ACTIVE, GALAXIES: ELLIPTICAL AND LENTICULAR, CD, RADIO CONTINUUM: GALAXIES, GALAXIES: PHOTOMETRY, GALAXIES: STRUCTURE},
	month = aug,
	pages = {614-+},
	title = {{Morphological Evolution in High-Redshift Radio Galaxies and the Formation of Giant Elliptical Galaxies}},
	volume = 502,
	year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/305925}}

@inproceedings{Surace:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005AAS...207.6301S},
	author = {{Surace}, J.~A. and {Shupe}, D.~L. and {Fang}, F. and {Evans}, T. and {Alexov}, A. and {Frayer}, D. and {Lonsdale}, C.~J. and {SWIRE Team}},
	booktitle = {Bulletin of the American Astronomical Society},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	month = dec,
	pages = {1246},
	series = {Bulletin of the American Astronomical Society},
	title = {{Data Processing and Validation of the SWIRE Survey}},
	volume = 37,
	year = 2005}

@article{Lonsdale:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003PASP..115..897L},
	author = {{Lonsdale}, C.~J. and {Smith}, H.~E. and {Rowan-Robinson}, M. and {Surace}, J. and {Shupe}, D. and {Xu}, C. and {Oliver}, S. and {Padgett}, D. and {Fang}, F. and {Conrow}, T. and {Franceschini}, A. and {Gautier}, N. and {Griffin}, M. and {Hacking}, P. and {Masci}, F. and {Morrison}, G. and {O'Linger}, J. and {Owen}, F. and {P{\'e}rez-Fournon}, I. and {Pierre}, M. and {Puetter}, R. and {Stacey}, G. and {Castro}, S. and {Polletta}, M.~d.~C. and {Farrah}, D. and {Jarrett}, T. and {Frayer}, D. and {Siana}, B. and {Babbedge}, T. and {Dye}, S. and {Fox}, M. and {Gonzalez-Solares}, E. and {Salaman}, M. and {Berta}, S. and {Condon}, J.~J. and {Dole}, H. and {Serjeant}, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/376850},
	eprint = {arXiv:astro-ph/0305375},
	journal = {\pasp},
	keywords = {Surveys, Galaxies: Evolution, Galaxies: Active, Cosmology: Large-Scale Structure of Universe, infrared: galaxies},
	month = aug,
	pages = {897-927},
	title = {{SWIRE: The SIRTF Wide-Area Infrared Extragalactic Survey}},
	volume = 115,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/376850}}

@article{Polletta:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...642..673D},
	author = {{Polletta}, M.~d.~C. and {Wilkes}, B.~J. and {Siana}, B. and {Lonsdale}, C.~J. and {Kilgard}, R. and {Smith}, H.~E. and {Kim}, {D.-W.} and {Owen}, F. and {Efstathiou}, A. and {Jarrett}, T. and {Stacey}, G. and {Franceschini}, A. and {Rowan-Robinson}, M. and {Babbedge}, T.~S.~R. and {Berta}, S. and {Fang}, F. and {Farrah}, D. and {Gonz{\'a}lez-Solares}, E. and {Morrison}, G. and {Surace}, J.~A. and {Shupe}, D.~L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/500821},
	eprint = {arXiv:astro-ph/0602228},
	journal = {\apj},
	keywords = {Galaxies: Active, Infrared: Galaxies, quasars: individual (SWIRE J104409.95+585224.8), quasars: individual (SWIRE J104406.30+583954.1), X-Rays: Galaxies},
	month = may,
	pages = {673-693},
	title = {{Chandra and Spitzer Unveil Heavily Obscured Quasars in the Chandra/SWIRE Survey}},
	volume = 642,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/500821}}

@article{McNamara:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...562L.149M},
	author = {{McNamara}, B.~R. and {Wise}, M.~W. and {Nulsen}, P.~E.~J. and {David}, L.~P. and {Carilli}, C.~L. and {Sarazin}, C.~L. and {O'Dea}, C.~P. and {Houck}, J. and {Donahue}, M. and {Baum}, S. and {Voit}, M. and {O'Connell}, R.~W. and {Koekemoer}, A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/338326},
	eprint = {arXiv:astro-ph/0110554},
	journal = {\apjl},
	keywords = {Galaxies: Cooling Flows, Galaxies: Clusters: General, Galaxies: Intergalactic Medium, Radio Continuum: Galaxies, X-Rays: Galaxies: Clusters},
	month = dec,
	pages = {L149-L152},
	title = {{Discovery of Ghost Cavities in the X-Ray Atmosphere of Abell 2597}},
	volume = 562,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/338326}}

@article{Gallimore:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...613..794G},
	author = {{Gallimore}, J.~F. and {Baum}, S.~A. and {O'Dea}, C.~P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/423167},
	eprint = {arXiv:astro-ph/0406062},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Individual: NGC Number: NGC 1068, Galaxies: Nuclei, Galaxies: Seyfert, Radio Continuum: Galaxies},
	month = oct,
	pages = {794-810},
	title = {{The Parsec-Scale Radio Structure of NGC 1068 and the Nature of the Nuclear Radio Source}},
	volume = 613,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/423167}}

@article{Gallimore:1996,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...464..198G},
	author = {{Gallimore}, J.~F. and {Baum}, S.~A. and {O'Dea}, C.~P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/177311},
	journal = {\apj},
	keywords = {GALAXIES: INDIVIDUAL NGC NUMBER: NGC 1068, GALAXIES: JETS, GALAXIES: NUCLEI, GALAXIES: SEYFERT, GALAXIES: STRUCTURE, RADIO CONTINUUM: GALAXIES},
	month = jun,
	pages = {198-+},
	title = {{The Subarcsecond Radio Structure in NGC 1068. II. Implications for the Central Engine and Unifying Schemes}},
	volume = 464,
	year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/177311}}

@article{Roy:1998,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...504..147R},
	author = {{Roy}, A.~L. and {Colbert}, E.~J.~M. and {Wilson}, A.~S. and {Ulvestad}, J.~S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/306071},
	journal = {\apj},
	keywords = {GALAXIES: INDIVIDUAL NGC NUMBER: NGC 1068, GALAXIES: ISM, GALAXIES: JETS, GALAXIES: NUCLEI, GALAXIES: SEYFERT, RADIO CONTINUUM: GALAXIES},
	month = sep,
	pages = {147-+},
	title = {{The Compact Radio Sources in the Nucleus of NGC 1068}},
	volume = 504,
	year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/306071}}

@article{Barvainis:1998,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1998AJ....115..885B},
	author = {{Barvainis}, R. and {Lonsdale}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/300262},
	eprint = {arXiv:astro-ph/9711247},
	journal = {\aj},
	keywords = {GALAXIES: ACTIVE, GALAXIES: ACTIVE},
	month = mar,
	pages = {885-889},
	title = {{Search for Free-Free Absorption Cutoffs from Tori in Three Type 2 Active Galactic Nuclei}},
	volume = 115,
	year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/300262}}

@article{Bassani:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...636L..65B},
	author = {{Bassani}, L. and {Molina}, M. and {Malizia}, A. and {Stephen}, J.~B. and {Bird}, A.~J. and {Bazzano}, A. and {B{\'e}langer}, G. and {Dean}, A.~J. and {De Rosa}, A. and {Laurent}, P. and {Lebrun}, F. and {Ubertini}, P. and {Walter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/500132},
	eprint = {arXiv:astro-ph/0512015},
	journal = {\apjl},
	keywords = {Galaxies: Active, Gamma Rays: Observations, Surveys},
	month = jan,
	pages = {L65-L68},
	title = {{INTEGRAL IBIS Extragalactic Survey: Active Galactic Nuclei Selected at 20-100 keV}},
	volume = 636,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/500132}}

@article{Ulvestad:1986,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1986MNRAS.218..711U},
	author = {{Ulvestad}, J.~S. and {Wilson}, A.~S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\mnras},
	keywords = {ASTRONOMICAL SPECTROSCOPY, EXTRAGALACTIC RADIO SOURCES, GALACTIC NUCLEI, GAMMA RAY SPECTRA, SEYFERT GALAXIES, CENTIMETER WAVES, DIFFUSE RADIATION, EMISSION SPECTRA, GALACTIC STRUCTURE, HIGH RESOLUTION, SPECTRAL RESOLUTION, VISIBLE SPECTRUM},
	month = feb,
	pages = {711-719},
	title = {{The radio source in the very luminous gamma-ray Seyfert galaxy MCG 8-11-11}},
	volume = 218,
	year = 1986}

@article{Ubertini:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411L.131U},
	author = {{Ubertini}, P. and {Lebrun}, F. and {Di Cocco}, G. and {Bazzano}, A. and {Bird}, A.~J. and {Broenstad}, K. and {Goldwurm}, A. and {La Rosa}, G. and {Labanti}, C. and {Laurent}, P. and {Mirabel}, I.~F. and {Quadrini}, E.~M. and {Ramsey}, B. and {Reglero}, V. and {Sabau}, L. and {Sacco}, B. and {Staubert}, R. and {Vigroux}, L. and {Weisskopf}, M.~C. and {Zdziarski}, A.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20031224},
	journal = {\aap},
	keywords = {INTEGRAL, IBIS, gamma-ray imaging},
	month = nov,
	pages = {L131-L139},
	title = {{IBIS: The Imager on-board INTEGRAL}},
	volume = 411,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031224}}

@article{Sambruna:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...665.1030S},
	archiveprefix = {arXiv},
	author = {{Sambruna}, R.~M. and {Reeves}, J.~N. and {Braito}, V.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/519306},
	eprint = {0704.3053},
	journal = {\apj},
	keywords = {Galaxies: Active, X-Rays: Galaxies},
	month = aug,
	pages = {1030-1037},
	title = {{The Remarkable X-Ray Spectrum of the Broad-Line Radio Galaxy 3C 445}},
	volume = 665,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/519306}}

@article{Risaliti:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...386..379R},
	author = {{Risaliti}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20020170},
	eprint = {arXiv:astro-ph/0202392},
	journal = {\aap},
	keywords = {Galaxies: Active, Galaxies: Seyfert, X-rays: Galaxies},
	month = may,
	pages = {379-398},
	title = {{The BeppoSAX view of bright Compton-thin Seyfert 2 galaxies}},
	volume = 386,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20020170}}

@article{Mushotzky:1993,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1993ARA%26A..31..717M},
	author = {{Mushotzky}, R.~F. and {Done}, C. and {Pounds}, K.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1146/annurev.aa.31.090193.003441},
	journal = {\araa},
	keywords = {ACTIVE GALACTIC NUCLEI, POWER SPECTRA, QUASARS, X RAY SPECTRA, SEYFERT GALAXIES, VARIABILITY},
	pages = {717-761},
	title = {{X-ray spectra and time variability of active galactic nuclei}},
	volume = 31,
	year = 1993,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.aa.31.090193.003441}}

@article{Miller:1990,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1990MNRAS.244..207M},
	author = {{Miller}, L. and {Peacock}, J.~A. and {Mead}, A.~R.~G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\mnras},
	keywords = {QUASARS, RADIO ASTRONOMY, RADIO EMISSION, ASTRONOMICAL SPECTROSCOPY, LUMINOSITY, RED SHIFT},
	month = may,
	pages = {207-213},
	title = {{The bimodal radio luminosity function of quasars}},
	volume = 244,
	year = 1990}

@article{Masetti:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...482..113M},
	archiveprefix = {arXiv},
	author = {{Masetti}, N. and {Mason}, E. and {Morelli}, L. and {Cellone}, S.~A. and {McBride}, V.~A. and {Palazzi}, E. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A.~J. and {Charles}, P.~A. and {Dean}, A.~J. and {Galaz}, G. and {Gehrels}, N. and {Landi}, R. and {Malizia}, A. and {Minniti}, D. and {Panessa}, F. and {Romero}, G.~E. and {Stephen}, J.~B. and {Ubertini}, P. and {Walter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20079332},
	eprint = {0802.0988},
	journal = {\aap},
	keywords = {galaxies: Seyfert, X-rays: binaries, stars: novae, , cataclysmic variables, techniques: spectroscopic, X-rays:, general},
	month = apr,
	pages = {113-132},
	title = {{Unveiling the nature of INTEGRAL objects through optical spectroscopy. VI. A multi-observatory identification campaign}},
	volume = 482,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20079332}}

@article{Lewis:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...622..816L},
	author = {{Lewis}, K.~T. and {Eracleous}, M. and {Gliozzi}, M. and {Sambruna}, R.~M. and {Mushotzky}, R.~F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/428380},
	eprint = {arXiv:astro-ph/0412537},
	journal = {\apj},
	keywords = {Accretion, Accretion Disks, Galaxies: Active, Galaxies: Individual: Alphanumeric: 3C 111, Galaxies: Nuclei, X-Rays: Galaxies},
	month = apr,
	pages = {816-829},
	title = {{A Simultaneous RXTE and XMM-Newton Observation of the Broad-Line Radio Galaxy 3C 111}},
	volume = 622,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/428380}}

@article{Larsson:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.388.1037L},
	archiveprefix = {arXiv},
	author = {{Larsson}, J. and {Fabian}, A.~C. and {Ballantyne}, D.~R. and {Miniutti}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.13497.x},
	eprint = {0805.3603},
	journal = {\mnras},
	keywords = {galaxies: active , galaxies: individual: 4C+74.26 , X-rays: galaxies},
	month = aug,
	pages = {1037-1046},
	title = {{Exploring the disc/jet interaction in the radio-loud quasar 4C+74.26 with Suzaku}},
	volume = 388,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13497.x}}

@article{Kharb:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...652..177K},
	author = {{Kharb}, P. and {O'Dea}, C.~P. and {Baum}, S.~A. and {Colbert}, E.~J.~M. and {Xu}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/507945},
	eprint = {arXiv:astro-ph/0607603},
	journal = {\apj},
	keywords = {galaxies: individual (Mrk 6), Galaxies: Seyfert, Radio Continuum: Galaxies},
	month = nov,
	pages = {177-188},
	title = {{A Radio Study of the Seyfert Galaxy Markarian 6: Implications for Seyfert Life Cycles}},
	volume = 652,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/507945}}

@article{Ishwara-Chandra:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.309..100I},
	author = {{Ishwara-Chandra}, C.~H. and {Saikia}, D.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.1999.02835.x},
	eprint = {arXiv:astro-ph/9902252},
	journal = {\mnras},
	month = oct,
	pages = {100-112},
	title = {{Giant radio sources}},
	volume = 309,
	year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1999.02835.x}}

@article{Hardcastle:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.363..649H},
	author = {{Hardcastle}, M.~J. and {Croston}, J.~H.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2005.09469.x},
	eprint = {arXiv:astro-ph/0507694},
	journal = {\mnras},
	keywords = {radiation mechanisms: non-thermal, galaxies: active, galaxies: individual: Pictor A, galaxies: jets, X-rays: galaxies},
	month = oct,
	pages = {649-660},
	title = {{The Chandra view of extended X-ray emission from Pictor A}},
	volume = 363,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09469.x}}

@article{Grandi:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...343...33G},
	author = {{Grandi}, P. and {Guainazzi}, M. and {Haardt}, F. and {Maraschi}, L. and {Massaro}, E. and {Matt}, G. and {Piro}, L. and {Urry}, C.~M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {arXiv:astro-ph/9810450},
	journal = {\aap},
	keywords = {GALAXIES: ACTIVE, GALAXIES: INDIVIDUAL: 3C 390.3, RADIO CONTINUUM: GALAXIES, X-RAYS: GALAXIES},
	month = mar,
	pages = {33-40},
	title = {{Reprocessing and variable cold absorption in the broad-line radio galaxy 3C 390.3}},
	volume = 343,
	year = 1999}

@article{Gliozzi:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...584..176G},
	author = {{Gliozzi}, M. and {Sambruna}, R.~M. and {Eracleous}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/345661},
	eprint = {arXiv:astro-ph/0210300},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Individual: Alphanumeric: 3C 120, Galaxies: Individual: Alphanumeric: 3C 390.3, Galaxies: Nuclei},
	month = feb,
	pages = {176-189},
	title = {{Long-Term Continuous Monitoring of the Broad-Line Radio Galaxies 3C 390.3 and 3C 120 with the Rossi X-Ray Timing Explorer}},
	volume = 584,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/345661}}

@article{Fan:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...407..899F},
	author = {{Fan}, J.~H. and {Zhang}, J.~S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20030896},
	journal = {\aap},
	keywords = {BL Lacertae objects: general, quasars: general, galaxies: Seyfert, galaxies: jets},
	month = sep,
	pages = {899-904},
	title = {{The core dominance parameter of extragalactic radio sources}},
	volume = 407,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20030896}}

@article{Evans:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...642...96E},
	author = {{Evans}, D.~A. and {Worrall}, D.~M. and {Hardcastle}, M.~J. and {Kraft}, R.~P. and {Birkinshaw}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/500658},
	eprint = {arXiv:astro-ph/0512600},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Jets, X-Rays: Galaxies},
	month = may,
	pages = {96-112},
	title = {{Chandra and XMM-Newton Observations of a Sample of Low-Redshift FR I and FR II Radio Galaxy Nuclei}},
	volume = 642,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/500658}}

@article{Dickey:1990,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1990ARA%26A..28..215D},
	author = {{Dickey}, J.~M. and {Lockman}, F.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1146/annurev.aa.28.090190.001243},
	journal = {\araa},
	keywords = {H I REGIONS, MILKY WAY GALAXY, ABSORPTION SPECTRA, LYMAN ALPHA RADIATION, MOLECULAR CLOUDS, RADIO EMISSION, ULTRAVIOLET ASTRONOMY, VERY LONG BASE INTERFEROMETRY},
	pages = {215-261},
	title = {{H I in the Galaxy}},
	volume = 28,
	year = 1990,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.aa.28.090190.001243}}

@article{Derosa:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...483..749D},
	archiveprefix = {arXiv},
	author = {{de Rosa}, A. and {Bassani}, L. and {Ubertini}, P. and {Panessa}, F. and {Malizia}, A. and {Dean}, A.~J. and {Walter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20078319},
	eprint = {0801.4675},
	journal = {\aap},
	keywords = {X-rays: galaxies, galaxies: Seyfert, galaxies: nuclei},
	month = jun,
	pages = {749-758},
	title = {{An X-ray view of absorbed INTEGRAL AGN}},
	volume = 483,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078319}}

@article{de-Bruyn:1989,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...226L..13D},
	author = {{de Bruyn}, A.~G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\aap},
	keywords = {EXTRAGALACTIC RADIO SOURCES, GALACTIC CLUSTERS, QUASARS, RADIO GALAXIES, ASTRONOMICAL SPECTROSCOPY, RADIO ASTRONOMY},
	month = dec,
	pages = {L13-L16},
	title = {{0309 + 411, an Mpc-sized core-dominated radio galaxy/quasar}},
	volume = 226,
	year = 1989}

@article{Ballantyne:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.336..867B},
	author = {{Ballantyne}, D.~R. and {Ross}, R.~R. and {Fabian}, A.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2002.05818.x},
	eprint = {arXiv:astro-ph/0202148},
	journal = {\mnras},
	keywords = {line: formation, radiative transfer, galaxies: active, galaxies: individual: MCG-6-30-15, X-rays: galaxies, X-rays: general},
	month = nov,
	pages = {867-872},
	title = {{Soft X-ray emission lines from photoionized accretion discs: constraints on their strength and width}},
	volume = 336,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2002.05818.x}}

@article{Ballantyne:2005b,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...622L..97B},
	author = {{Ballantyne}, D.~R. and {Fabian}, A.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/429691},
	eprint = {arXiv:astro-ph/0502461},
	journal = {\apjl},
	keywords = {Accretion, Accretion Disks, Galaxies: Active, Galaxies: Individual: Alphanumeric: 4C 74.26, Galaxies: Jets, X-Rays: Galaxies},
	month = apr,
	pages = {L97-L100},
	title = {{Evidence of an Untruncated Accretion Disk in the Broad-Line Radio Galaxy 4C 74.26}},
	volume = 622,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/429691}}

@article{Ballantyne:2005a,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.362.1183B},
	author = {{Ballantyne}, D.~R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2005.09345.x},
	eprint = {arXiv:astro-ph/0506673},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: individual: 4C +74.26, X-rays: galaxies},
	month = oct,
	pages = {1183-1188},
	title = {{A complete view of the broad-line radio galaxy 4C +74.26 with XMM-Newton}},
	volume = 362,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09345.x}}

@article{Brinkmann:2000,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...356..445B},
	author = {{Brinkmann}, W. and {Laurent-Muehleisen}, S.~A. and {Voges}, W. and {Siebert}, J. and {Becker}, R.~H. and {Brotherton}, M.~S. and {White}, R.~L. and {Gregg}, M.~D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\aap},
	keywords = {GALAXIES: ACTIVE, GALAXIES: QUASARS: GENERAL, X-RAYS: GENERAL, RADIO CONTINUUM: GENERAL},
	month = apr,
	pages = {445-462},
	title = {{Radio and X-ray bright AGN: the ROSAT - FIRST correlation}},
	volume = 356,
	year = 2000}

@article{Kellermann:1981,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1981ARA%26A..19..373K},
	author = {{Kellermann}, K.~I. and {Pauliny-Toth}, I.~I.~K.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1146/annurev.aa.19.090181.002105},
	journal = {\araa},
	keywords = {EXTRAGALACTIC RADIO SOURCES, RADIANT FLUX DENSITY, RADIATION DISTRIBUTION, RADIO SPECTRA, SPATIAL DISTRIBUTION, BRIGHTNESS TEMPERATURE, GALACTIC EVOLUTION, QUASARS, RADIO ASTRONOMY, RADIO GALAXIES},
	pages = {373-410},
	title = {{Compact radio sources}},
	volume = 19,
	year = 1981,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.aa.19.090181.002105}}

@article{Jackson:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.304..160J},
	author = {{Jackson}, C.~A. and {Wall}, J.~V.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.1999.02310.x},
	eprint = {arXiv:astro-ph/9808054},
	journal = {\mnras},
	keywords = {GALAXIES: EVOLUTION, GALAXIES: JETS, QUASARS: GENERAL, RADIO CONTINUUM: GALAXIES},
	month = mar,
	pages = {160-174},
	title = {{Extragalactic radio-source evolution under the dual-population unification scheme}},
	volume = 304,
	year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1999.02310.x}}

@article{Seymour:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386.1695S},
	archiveprefix = {arXiv},
	author = {{Seymour}, N. and {Dwelly}, T. and {Moss}, D. and {McHardy}, I. and {Zoghbi}, A. and {Rieke}, G. and {Page}, M. and {Hopkins}, A. and {Loaring}, N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.13166.x},
	eprint = {0802.4105},
	journal = {\mnras},
	keywords = {galaxies: evolution , galaxies: starburst , radio continuum: galaxies},
	month = may,
	pages = {1695-1708},
	title = {{The star formation history of the Universe as revealed by deep radio observations}},
	volume = 386,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13166.x}}

@article{White:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...654...99W},
	author = {{White}, R.~L. and {Helfand}, D.~J. and {Becker}, R.~H. and {Glikman}, E. and {de Vries}, W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/507700},
	eprint = {arXiv:astro-ph/0607335},
	journal = {\apj},
	keywords = {Catalogs, Galaxies: Quasars: Absorption Lines, Galaxies: Quasars: General, Radio Continuum: General, Surveys},
	month = jan,
	pages = {99-114},
	title = {{Signals from the Noise: Image Stacking for Quasars in the FIRST Survey}},
	volume = 654,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/507700}}

@article{Zamfir:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.387..856Z},
	archiveprefix = {arXiv},
	author = {{Zamfir}, S. and {Sulentic}, J.~W. and {Marziani}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.13290.x},
	eprint = {0804.0788},
	journal = {\mnras},
	keywords = {galaxies: active , quasars: emission lines , quasars: general},
	month = jun,
	pages = {856-870},
	title = {{New insights on the QSO radio-loud/radio-quiet dichotomy: SDSS spectra in the context of the 4D eigenvector1 parameter space}},
	volume = 387,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13290.x}}

@article{Kellermann:1989,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1989AJ.....98.1195K},
	author = {{Kellermann}, K.~I. and {Sramek}, R. and {Schmidt}, M. and {Shaffer}, D.~B. and {Green}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/115207},
	journal = {\aj},
	keywords = {ASTRONOMICAL CATALOGS, QUASARS, RADIO SOURCES (ASTRONOMY), VERY LARGE ARRAY (VLA), CENTIMETER WAVES, DATA SAMPLING, LUMINOSITY, RADIANT FLUX DENSITY},
	month = oct,
	pages = {1195-1207},
	title = {{VLA observations of objects in the Palomar Bright Quasar Survey}},
	volume = 98,
	year = 1989,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/115207}}

@article{Wilkes:1987,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1987ApJ...323..243W},
	author = {{Wilkes}, B.~J. and {Elvis}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/165822},
	journal = {\apj},
	keywords = {ASTRONOMICAL SPECTROSCOPY, QUASARS, SPECTRAL ENERGY DISTRIBUTION, X RAY SPECTRA, BL LACERTAE OBJECTS, RADIO SPECTRA, RED SHIFT, STELLAR LUMINOSITY},
	month = dec,
	pages = {243-262},
	title = {{Quasar energy distributions. I - Soft X-ray spectra of quasars}},
	volume = 323,
	year = 1987,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/165822}}

@article{Chiappetti:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...439..413C},
	author = {{Chiappetti}, L. and {Tajer}, M. and {Trinchieri}, G. and {Maccagni}, D. and {Maraschi}, L. and {Paioro}, L. and {Pierre}, M. and {Surdej}, J. and {Garcet}, O. and {Gosset}, E. and {Le F{\`e}vre}, O. and {Bertin}, E. and {McCracken}, H.~J. and {Mellier}, Y. and {Foucaud}, S. and {Radovich}, M. and {Ripepi}, V. and {Arnaboldi}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20042583},
	eprint = {arXiv:astro-ph/0505117},
	journal = {\aap},
	keywords = {X-ray: general, surveys, quasars: general, catalogs},
	month = aug,
	pages = {413-425},
	title = {{The XMM-LSS survey. The XMDS/VVDS 4{$\sigma$} catalogue}},
	volume = 439,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20042583}}

@article{baldi02,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...564..190B},
	author = {{Baldi}, A. and {Molendi}, S. and {Comastri}, A. and {Fiore}, F. and {Matt}, G. and {Vignali}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:50:04 +0200},
	doi = {10.1086/324261},
	eprint = {arXiv:astro-ph/0108514},
	journal = {\apj},
	keywords = {Galaxies: Active, X-Rays: Diffuse Background, X-Rays: Galaxies},
	month = jan,
	pages = {190-195},
	title = {{The HELLAS2XMM Survey. I. The X-Ray Data and the logN-logS Relation}},
	volume = 564,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/324261}}

@article{Rieke:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004ApJS..154...25R},
	author = {{Rieke}, G.~H. and {Young}, E.~T. and {Engelbracht}, C.~W. and {Kelly}, D.~M. and {Low}, F.~J. and {Haller}, E.~E. and {Beeman}, J.~W. and {Gordon}, K.~D. and {Stansberry}, J.~A. and {Misselt}, K.~A. and {Cadien}, J. and {Morrison}, J.~E. and {Rivlis}, G. and {Latter}, W.~B. and {Noriega-Crespo}, A. and {Padgett}, D.~L. and {Stapelfeldt}, K.~R. and {Hines}, D.~C. and {Egami}, E. and {Muzerolle}, J. and {Alonso-Herrero}, A. and {Blaylock}, M. and {Dole}, H. and {Hinz}, J.~L. and {Le Floc'h}, E. and {Papovich}, C. and {P{\'e}rez-Gonz{\'a}lez}, P.~G. and {Smith}, P.~S. and {Su}, K.~Y.~L. and {Bennett}, L. and {Frayer}, D.~T. and {Henderson}, D. and {Lu}, N. and {Masci}, F. and {Pesenson}, M. and {Rebull}, L. and {Rho}, J. and {Keene}, J. and {Stolovy}, S. and {Wachter}, S. and {Wheaton}, W. and {Werner}, M.~W. and {Richards}, P.~L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/422717},
	journal = {\apjs},
	keywords = {Infrared: General, Space Vehicles: Instruments},
	month = sep,
	pages = {25-29},
	title = {{The Multiband Imaging Photometer for Spitzer (MIPS)}},
	volume = 154,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422717}}

@article{Fazio:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004ApJS..154...10F},
	author = {{Fazio}, G.~G. and {Hora}, J.~L. and {Allen}, L.~E. and {Ashby}, M.~L.~N. and {Barmby}, P. and {Deutsch}, L.~K. and {Huang}, {J.-S.} and {Kleiner}, S. and {Marengo}, M. and {Megeath}, S.~T. and {Melnick}, G.~J. and {Pahre}, M.~A. and {Patten}, B.~M. and {Polizotti}, J. and {Smith}, H.~A. and {Taylor}, R.~S. and {Wang}, Z. and {Willner}, S.~P. and {Hoffmann}, W.~F. and {Pipher}, J.~L. and {Forrest}, W.~J. and {McMurty}, C.~W. and {McCreight}, C.~R. and {McKelvey}, M.~E. and {McMurray}, R.~E. and {Koch}, D.~G. and {Moseley}, S.~H. and {Arendt}, R.~G. and {Mentzell}, J.~E. and {Marx}, C.~T. and {Losch}, P. and {Mayman}, P. and {Eichhorn}, W. and {Krebs}, D. and {Jhabvala}, M. and {Gezari}, D.~Y. and {Fixsen}, D.~J. and {Flores}, J. and {Shakoorzadeh}, K. and {Jungo}, R. and {Hakun}, C. and {Workman}, L. and {Karpati}, G. and {Kichak}, R. and {Whitley}, R. and {Mann}, S. and {Tollestrup}, E.~V. and {Eisenhardt}, P. and {Stern}, D. and {Gorjian}, V. and {Bhattacharya}, B. and {Carey}, S. and {Nelson}, B.~O. and {Glaccum}, W.~J. and {Lacy}, M. and {Lowrance}, P.~J. and {Laine}, S. and {Reach}, W.~T. and {Stauffer}, J.~A. and {Surace}, J.~A. and {Wilson}, G. and {Wright}, E.~L. and {Hoffman}, A. and {Domingo}, G. and {Cohen}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/422843},
	eprint = {arXiv:astro-ph/0405616},
	journal = {\apjs},
	keywords = {Infrared: General, Instrumentation: Detectors, Space Vehicles: Instruments},
	month = sep,
	pages = {10-17},
	title = {{The Infrared Array Camera (IRAC) for the Spitzer Space Telescope}},
	volume = 154,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422843}}

@article{Polletta:2000,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...362...75P},
	author = {{Polletta}, M. and {Courvoisier}, {T.~J.-L.} and {Hooper}, E.~J. and {Wilkes}, B.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {arXiv:astro-ph/0006315},
	journal = {\aap},
	keywords = {GALAXIES: QUASARS: GENERAL, INFRARED: GALAXIES, RADIO CONTINUUM: GALAXIES},
	month = oct,
	pages = {75-96},
	title = {{The far-infrared emission of radio loud and radio quiet quasars}},
	volume = 362,
	year = 2000}

@article{Polletta:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...663...81P},
	author = {{Polletta}, M. and {Tajer}, M. and {Maraschi}, L. and {Trinchieri}, G. and {Lonsdale}, C.~J. and {Chiappetti}, L. and {Andreon}, S. and {Pierre}, M. and {Le F{\`e}vre}, O. and {Zamorani}, G. and {Maccagni}, D. and {Garcet}, O. and {Surdej}, J. and {Franceschini}, A. and {Alloin}, D. and {Shupe}, D.~L. and {Surace}, J.~A. and {Fang}, F. and {Rowan-Robinson}, M. and {Smith}, H.~E. and {Tresse}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/518113},
	journal = {\apj},
	keywords = {Galaxies: Active, Infrared: Galaxies, Galaxies: Quasars: General, X-Rays: Galaxies},
	month = jul,
	pages = {81-102},
	title = {{Spectral Energy Distributions of Hard X-Ray Selected Active Galactic Nuclei in the XMM-Newton Medium Deep Survey}},
	volume = 663,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/518113}}

@article{Polletta:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...492...81P},
	archiveprefix = {arXiv},
	author = {{Polletta}, M. and {Omont}, A. and {Berta}, S. and {Bergeron}, J. and {Stalin}, C.~S. and {Petitjean}, P. and {Giorgetti}, M. and {Trinchieri}, G. and {Srianand}, R. and {McCracken}, H.~J. and {Pei}, Y. and {Dannerbauer}, H.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:200810345},
	eprint = {0810.2518},
	journal = {\aap},
	keywords = {galaxies: active, galaxies: evolution, galaxies: high-redshift, quasars: general, infrared: galaxies},
	month = dec,
	pages = {81-92},
	title = {{Obscured and powerful AGN and starburst activities at z \~{} 3.5}},
	volume = 492,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200810345}}

@article{Owen:2009b,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009ApJS..182..625O},
	archiveprefix = {arXiv},
	author = {{Owen}, F.~N. and {Morrison}, G.~E.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0067-0049/182/2/625},
	eprint = {0904.4651},
	journal = {\apjs},
	keywords = {cosmology: observations, galaxies: active, galaxies: starburst, infrared: galaxies},
	month = jun,
	pages = {625-627},
	title = {{The Deep Swire Field. III. Wiyn Spectroscopy}},
	volume = 182,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/182/2/625}}

@article{Owen:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008AJ....136.1889O},
	archiveprefix = {arXiv},
	author = {{Owen}, F.~N. and {Morrison}, G.~E.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-6256/136/5/1889},
	eprint = {0809.0314},
	journal = {\aj},
	keywords = {cosmology: observations, galaxies: evolution, galaxies: starburst, infrared: galaxies},
	month = nov,
	pages = {1889-1900},
	title = {{The Deep Swire Field. I. 20 cm Continuum Radio Observations: A Crowded Sky}},
	volume = 136,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/136/5/1889}}

@article{Owen:2009a,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009AJ....137.4846O},
	archiveprefix = {arXiv},
	author = {{Owen}, F.~N. and {Morrison}, G.~E. and {Klimek}, M.~D. and {Greisen}, E.~W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-6256/137/6/4846},
	eprint = {0904.2011},
	journal = {\aj},
	keywords = {cosmology: observations, galaxies: active, galaxies: evolution, galaxies: general, galaxies: starburst},
	month = jun,
	pages = {4846-4853},
	title = {{The Deep SWIRE Field. II. 90 cm Continuum Observations and 20 cm-90 cm Spectra}},
	volume = 137,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/137/6/4846}}

@inproceedings{Norris:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009ASPC..408..334N},
	author = {{Norris}, R.~P.},
	booktitle = {Astronomical Society of the Pacific Conference Series},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{W.~Wang, Z.~Yang, Z.~Luo, \& Z.~Chen}},
	month = oct,
	pages = {334},
	series = {Astronomical Society of the Pacific Conference Series},
	title = {{Co-Evolution of AGN and Star-Forming Galaxies in the Australia Telescope Large Area Survey}},
	volume = 408,
	year = 2009}

@article{Boyle:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.376.1182B},
	author = {{Boyle}, B.~J. and {Cornwell}, T.~J. and {Middelberg}, E. and {Norris}, R.~P. and {Appleton}, P.~N. and {Smail}, I.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2007.11509.x},
	eprint = {arXiv:astro-ph/0701602},
	journal = {\mnras},
	keywords = {galaxies: starburst , infrared: galaxies , radio continuum: general},
	month = apr,
	pages = {1182-1188},
	title = {{Extending the infrared radio correlation}},
	volume = 376,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.11509.x}}

@article{appleton04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004ApJS..154..147A},
	author = {{Appleton}, P.~N. and {Fadda}, D.~T. and {Marleau}, F.~R. and {Frayer}, D.~T. and {Helou}, G. and {Condon}, J.~J. and {Choi}, P.~I. and {Yan}, L. and {Lacy}, M. and {Wilson}, G. and {Armus}, L. and {Chapman}, S.~C. and {Fang}, F. and {Heinrichson}, I. and {Im}, M. and {Jannuzi}, B.~T. and {Storrie-Lombardi}, L.~J. and {Shupe}, D. and {Soifer}, B.~T. and {Squires}, G. and {Teplitz}, H.~I.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:49:41 +0200},
	doi = {10.1086/422425},
	eprint = {arXiv:astro-ph/0406030},
	journal = {\apjs},
	keywords = {Cosmology: Observations, Galaxies: Evolution, Galaxies: High-Redshift, Infrared: Galaxies},
	month = sep,
	pages = {147-150},
	title = {{The Far- and Mid-Infrared/Radio Correlations in the Spitzer Extragalactic First Look Survey}},
	volume = 154,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422425}}

@article{zdziarski98,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.301..435Z},
	author = {{Zdziarski}, A.~A. and {Poutanen}, J. and {Mikolajewska}, J. and {Gierlinski}, M. and {Ebisawa}, K. and {Johnson}, W.~N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:48:51 +0200},
	doi = {10.1046/j.1365-8711.1998.02021.x},
	eprint = {arXiv:astro-ph/9807300},
	journal = {\mnras},
	keywords = {ACCRETION, ACCRETION DISCS, BINARIES: GENERAL, STARS: INDIVIDUAL: GX 339-4, GAMMA-RAYS: OBSERVATIONS, GAMMA-RAYS: THEORY, X-RAYS: STARS},
	month = dec,
	pages = {435-450},
	title = {{Broad-band X-ray/gamma-ray spectra and binary parameters of GX 339-4 and their astrophysical implications}},
	volume = 301,
	year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1998.02021.x}}

@article{Zdziarski:1990,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1990ApJ...363L...1Z},
	author = {{Zdziarski}, A.~A. and {Ghisellini}, G. and {George}, I.~M. and {Fabian}, A.~C. and {Svensson}, R. and {Done}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/185851},
	journal = {\apjl},
	keywords = {ACTIVE GALACTIC NUCLEI, COMPTON EFFECT, ELECTRON-POSITRON PAIRS, X RAY SPECTRA, ACCRETION DISKS, ASTRONOMICAL SPECTROSCOPY, BACKGROUND RADIATION, GAMMA RAY SPECTRA},
	month = nov,
	pages = {L1-L4},
	title = {{Electron-positron pairs, Compton reflection, and the X-ray spectra of active galactic nuclei}},
	volume = 363,
	year = 1990,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/185851}}

@article{Winter:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...690.1322W},
	archiveprefix = {arXiv},
	author = {{Winter}, L.~M. and {Mushotzky}, R.~F. and {Reynolds}, C.~S. and {Tueller}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/690/2/1322},
	eprint = {0808.0461},
	journal = {\apj},
	keywords = {galaxies: active, surveys, X-rays: galaxies},
	month = jan,
	pages = {1322-1349},
	title = {{X-Ray Spectral Properties of the BAT AGN Sample}},
	volume = 690,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/690/2/1322}}

@article{Winter:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...674..686W},
	archiveprefix = {arXiv},
	author = {{Winter}, L.~M. and {Mushotzky}, R.~F. and {Tueller}, J. and {Markwardt}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/525274},
	eprint = {0711.0019},
	journal = {\apj},
	keywords = {Galaxies: Active, Surveys, X-Rays: Galaxies},
	month = feb,
	pages = {686-710},
	title = {{X-Ray Properties of an Unbiased Hard X-Ray-detected Sample of Active Galactic Nuclei}},
	volume = 674,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/525274}}

@article{Vaughan:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.348.1415V},
	author = {{Vaughan}, S. and {Fabian}, A.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2004.07456.x},
	eprint = {arXiv:astro-ph/0311473},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: individual: MCG, 6-30-15, galaxies: Seyfert, X-rays: galaxies},
	month = mar,
	pages = {1415-1438},
	title = {{A long hard look at MCG-6-30-15 with XMM-Newton- II. Detailed EPIC analysis and modelling}},
	volume = 348,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.07456.x}}

@article{Turner:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...365L.110T},
	author = {{Turner}, M.~J.~L. and {Reeves}, J.~N. and {Ponman}, T.~J. and {Arnaud}, M. and {Barbera}, M. and {Bennie}, P.~J. and {Boer}, M. and {Briel}, U. and {Butler}, I. and {Clavel}, J. and {Dhez}, P. and {Cordova}, F. and {Dos Santos}, S. and {Ferrando}, P. and {Ghizzardi}, S. and {Goodall}, C.~V. and {Griffiths}, R.~G. and {Hochedez}, J.~F. and {Holland}, A.~D. and {Jansen}, F. and {Kendziorra}, E. and {Lagostina}, A. and {Laine}, R. and {La Palombara}, N. and {Lortholary}, M. and {Mason}, K.~O. and {Molendi}, S. and {Pigot}, C. and {Priedhorsky}, W. and {Reppin}, C. and {Rothenflug}, R. and {Salvetat}, P. and {Sauvageot}, J. and {Schmitt}, D. and {Sembay}, S. and {Short}, A. and {Str{\"u}der}, L. and {Trifoglio}, M. and {Tr{\"u}mper}, J. and {Vercellone}, S. and {Vigroux}, L. and {Villa}, G. and {Ward}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20000070},
	eprint = {arXiv:astro-ph/0010612},
	journal = {\aap},
	keywords = {GALAXIES: ACTIVE, GALAXIES: STARBURST, X-RAYS: GALAXIES},
	month = jan,
	pages = {L110-L115},
	title = {{XMM-Newton first-light observations of the Hickson galaxy group 16}},
	volume = 365,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20000070}}

@article{Tueller:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...681..113T},
	archiveprefix = {arXiv},
	author = {{Tueller}, J. and {Mushotzky}, R.~F. and {Barthelmy}, S. and {Cannizzo}, J.~K. and {Gehrels}, N. and {Markwardt}, C.~B. and {Skinner}, G.~K. and {Winter}, L.~M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/588458},
	eprint = {0711.4130},
	journal = {\apj},
	keywords = {Galaxies: Active, Gamma Rays: Observations, Surveys},
	month = jul,
	pages = {113-127},
	title = {{Swift BAT Survey of AGNs}},
	volume = 681,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/588458}}

@article{Treister:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...696..110T},
	archiveprefix = {arXiv},
	author = {{Treister}, E. and {Urry}, C.~M. and {Virani}, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/696/1/110},
	eprint = {0902.0608},
	journal = {\apj},
	keywords = {galaxies: active, galaxies: Seyfert, X-rays: diffuse background, X-rays: galaxies},
	month = may,
	pages = {110-120},
	title = {{The Space Density of Compton-Thick Active Galactic Nucleus and the X-Ray Background}},
	volume = 696,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/696/1/110}}

@article{Struder:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...365L..18S},
	author = {{Str{\"u}der}, L. and {Briel}, U. and {Dennerl}, K. and {Hartmann}, R. and {Kendziorra}, E. and {Meidinger}, N. and {Pfeffermann}, E. and {Reppin}, C. and {Aschenbach}, B. and {Bornemann}, W. and {Br{\"a}uninger}, H. and {Burkert}, W. and {Elender}, M. and {Freyberg}, M. and {Haberl}, F. and {Hartner}, G. and {Heuschmann}, F. and {Hippmann}, H. and {Kastelic}, E. and {Kemmer}, S. and {Kettenring}, G. and {Kink}, W. and {Krause}, N. and {M{\"u}ller}, S. and {Oppitz}, A. and {Pietsch}, W. and {Popp}, M. and {Predehl}, P. and {Read}, A. and {Stephan}, K.~H. and {St{\"o}tter}, D. and {Tr{\"u}mper}, J. and {Holl}, P. and {Kemmer}, J. and {Soltau}, H. and {St{\"o}tter}, R. and {Weber}, U. and {Weichert}, U. and {von Zanthier}, C. and {Carathanassis}, D. and {Lutz}, G. and {Richter}, R.~H. and {Solc}, P. and {B{\"o}ttcher}, H. and {Kuster}, M. and {Staubert}, R. and {Abbey}, A. and {Holland}, A. and {Turner}, M. and {Balasini}, M. and {Bignami}, G.~F. and {La Palombara}, N. and {Villa}, G. and {Buttler}, W. and {Gianini}, F. and {Lain{\'e}}, R. and {Lumb}, D. and {Dhez}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20000066},
	journal = {\aap},
	keywords = {XMM-NEWTON, BACK ILLUMINATED PN-CCDS, RADIATION HARDNESS, ENERGY RESOLUTION, QUANTUM EFFICIENCY, PARTICLE AND FLOURESCENCE BACKGROUND},
	month = jan,
	pages = {L18-L26},
	title = {{The European Photon Imaging Camera on XMM-Newton: The pn-CCD camera}},
	volume = 365,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20000066}}

@article{Spergel:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003ApJS..148..175S},
	author = {{Spergel}, D.~N. and {Verde}, L. and {Peiris}, H.~V. and {Komatsu}, E. and {Nolta}, M.~R. and {Bennett}, C.~L. and {Halpern}, M. and {Hinshaw}, G. and {Jarosik}, N. and {Kogut}, A. and {Limon}, M. and {Meyer}, S.~S. and {Page}, L. and {Tucker}, G.~S. and {Weiland}, J.~L. and {Wollack}, E. and {Wright}, E.~L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/377226},
	eprint = {arXiv:astro-ph/0302209},
	journal = {\apjs},
	keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Cosmological Parameters- Cosmology: Observations, Cosmology: Early Universe},
	month = sep,
	pages = {175-194},
	title = {{First-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Determination of Cosmological Parameters}},
	volume = 148,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/377226}}

@article{Sazonov:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...482..517S},
	archiveprefix = {arXiv},
	author = {{Sazonov}, S. and {Krivonos}, R. and {Revnivtsev}, M. and {Churazov}, E. and {Sunyaev}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20078537},
	eprint = {0708.3215},
	journal = {\aap},
	keywords = {surveys, galaxies: active, galaxies: evolution, galaxies: Seyfert, X-rays: diffuse background},
	month = may,
	pages = {517-527},
	title = {{Cumulative hard X-ray spectrum of local AGN: a link to the cosmic X-ray background}},
	volume = 482,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078537}}

@article{Sambruna:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...526...60S},
	author = {{Sambruna}, R.~M. and {Eracleous}, M. and {Mushotzky}, R.~F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/307981},
	eprint = {arXiv:astro-ph/9905365},
	journal = {\apj},
	keywords = {GALAXIES: ACTIVE, RADIATION MECHANISMS: NONTHERMAL, SURVEYS, X-RAYS: GALAXIES},
	month = nov,
	pages = {60-96},
	title = {{An X-Ray Spectral Survey of Radio-loud Active Galactic Nuclei with ASCA}},
	volume = 526,
	year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/307981}}

@article{Reeves:2000,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.316..234R},
	author = {{Reeves}, J.~N. and {Turner}, M.~J.~L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2000.03510.x},
	eprint = {arXiv:astro-ph/0003080},
	journal = {\mnras},
	keywords = {SURVEYS, GALAXIES: ACTIVE, QUASARS: GENERAL, X-RAYS: GENERAL},
	month = aug,
	pages = {234-248},
	title = {{X-ray spectra of a large sample of quasars with ASCA}},
	volume = 316,
	year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2000.03510.x}}

@article{Piro:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999AN....320..236P},
	author = {{Piro}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {Astronomische Nachrichten},
	pages = {236-+},
	title = {{Probing the AGN environment with X-ray measurements}},
	volume = 320,
	year = 1999}

@article{Piconcelli:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...432..835P},
	author = {{Piconcelli}, E. and {Guainazzi}, M. and {Cappi}, M. and {Jimenez-Bailon}, E. and {Schartel}, N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20041804},
	eprint = {arXiv:astro-ph/0412360},
	journal = {\aap},
	keywords = {galaxies: individual: RX J1343.4+0001, galaxies: active, galaxies: quasars: general, X-ray: galaxies},
	month = mar,
	pages = {835-839},
	title = {{The XMM-Newton spectrum of the high-z optically-obscured QSO RX J1343.4+0001: a classic radio quiet QSO}},
	volume = 432,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20041804}}

@article{Petrucci:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...556..716P},
	author = {{Petrucci}, P.~O. and {Haardt}, F. and {Maraschi}, L. and {Grandi}, P. and {Malzac}, J. and {Matt}, G. and {Nicastro}, F. and {Piro}, L. and {Perola}, G.~C. and {De Rosa}, A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/321629},
	eprint = {arXiv:astro-ph/0101219},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Seyfert, X-Rays: Galaxies},
	month = aug,
	pages = {716-726},
	title = {{Testing Comptonization Models Using BeppoSAX Observations of Seyfert 1 Galaxies}},
	volume = 556,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/321629}}

@article{Perola:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...389..802P},
	author = {{Perola}, G.~C. and {Matt}, G. and {Cappi}, M. and {Fiore}, F. and {Guainazzi}, M. and {Maraschi}, L. and {Petrucci}, P.~O. and {Piro}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20020658},
	eprint = {arXiv:astro-ph/0205045},
	journal = {\aap},
	keywords = {galaxies: Seyfert, X-rays: galaxies},
	month = jul,
	pages = {802-811},
	title = {{Compton reflection and iron fluorescence in BeppoSAX observations of Seyfert type 1 galaxies}},
	volume = 389,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20020658}}

@article{Panessa:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...483..151P},
	archiveprefix = {arXiv},
	author = {{Panessa}, F. and {Bassani}, L. and {de Rosa}, A. and {Bird}, A.~J. and {Dean}, A.~J. and {Fiocchi}, M. and {Malizia}, A. and {Molina}, M. and {Ubertini}, P. and {Walter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20078657},
	eprint = {0803.0896},
	journal = {\aap},
	keywords = {galaxies: Seyfert, X-rays: galaxies},
	month = may,
	pages = {151-160},
	title = {{The broad-band XMM-Newton and INTEGRAL spectra of bright type 1 Seyfert galaxies}},
	volume = 483,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078657}}

@article{Mushotzky:1984,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1984AdSpR...3..157M},
	author = {{Mushotzky}, R.~F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1016/0273-1177(84)90081-4},
	journal = {Advances in Space Research},
	keywords = {ACTIVE GALACTIC NUCLEI, HEAO, PERIODIC VARIATIONS, X RAY SOURCES, X RAY SPECTRA, ASTRONOMICAL MODELS, BL LACERTAE OBJECTS, QUASARS, RADIO GALAXIES, SEYFERT GALAXIES, SPECTRAL ENERGY DISTRIBUTION, SPECTRAL LINE WIDTH},
	pages = {157-165},
	title = {{X-ray spectra and time variability of active galactic nuclei}},
	volume = 3,
	year = 1984,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/0273-1177(84)90081-4}}

@article{Molina:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.371..821M},
	author = {{Molina}, M. and {Malizia}, A. and {Bassani}, L. and {Bird}, A.~J. and {Dean}, A.~J. and {Landi}, R. and {de Rosa}, A. and {Walter}, R. and {Barlow}, E.~J. and {Clark}, D.~J. and {Hill}, A.~B. and {Sguera}, V.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2006.10715.x},
	eprint = {arXiv:astro-ph/0606488},
	journal = {\mnras},
	keywords = {galaxies: active: galaxies: Seyfert, galaxies: active, galaxies: Seyfert},
	month = sep,
	pages = {821-828},
	title = {{INTEGRAL observations of active galactic nuclei obscured by the Galactic plane}},
	volume = 371,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10715.x}}

@article{Molina:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.382..937M},
	archiveprefix = {arXiv},
	author = {{Molina}, M. and {Giroletti}, M. and {Malizia}, A. and {Landi}, R. and {Bassani}, L. and {Bird}, A.~J. and {Dean}, A.~J. and {de Rosa}, A. and {Fiocchi}, M. and {Panessa}, F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2007.12464.x},
	eprint = {0709.1895},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: Seyfert, X-rays: galaxies},
	month = dec,
	pages = {937-943},
	title = {{Broad-band X-ray spectrum of the newly discovered broad-line radio galaxy IGR J21247+5058}},
	volume = 382,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12464.x}}

@article{Molina:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.390.1217M},
	archiveprefix = {arXiv},
	author = {{Molina}, M. and {Bassani}, L. and {Malizia}, A. and {Bird}, A.~J. and {Dean}, A.~J. and {Fiocchi}, M. and {Panessa}, F. and {de Rosa}, A. and {Landi}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.13824.x},
	eprint = {0809.0255},
	journal = {\mnras},
	keywords = {galaxies: active , X-rays: galaxies},
	month = nov,
	pages = {1217-1228},
	title = {{A broad-band spectral analysis of eight radio-loud type 1 active galactic nuclei selected in the hard X-ray band}},
	volume = 390,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13824.x}}

@article{Molina:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.399.1293M},
	archiveprefix = {arXiv},
	author = {{Molina}, M. and {Bassani}, L. and {Malizia}, A. and {Stephen}, J.~B. and {Bird}, A.~J. and {Dean}, A.~J. and {Panessa}, F. and {de Rosa}, A. and {Landi}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2009.15257.x},
	eprint = {0906.2909},
	journal = {\mnras},
	keywords = {galaxies: active , gamma-rays: observations , X-rays: galaxies},
	month = nov,
	pages = {1293-1306},
	title = {{The INTEGRAL complete sample of type 1 AGN}},
	volume = 399,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15257.x}}

@article{Miniutti:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007PASJ...59S.315M},
	author = {{Miniutti}, G. and {Fabian}, A.~C. and {Anabuki}, N. and {Crummy}, J. and {Fukazawa}, Y. and {Gallo}, L. and {Haba}, Y. and {Hayashida}, K. and {Holt}, S. and {Kunieda}, H. and {Larsson}, J. and {Markowitz}, A. and {Matsumoto}, C. and {Ohno}, M. and {Reeves}, J.~N. and {Takahashi}, T. and {Tanaka}, Y. and {Terashima}, Y. and {Torii}, K. and {Ueda}, Y. and {Ushio}, M. and {Watanabe}, S. and {Yamauchi}, M. and {Yaqoob}, T.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {arXiv:astro-ph/0609521},
	journal = {\pasj},
	keywords = {galaxies: active, galaxies: individual (MCG -6-30-15), galaxies: Seyfert, X-rays: galaxies},
	month = jan,
	pages = {315-325},
	title = {{Suzaku Observations of the Hard X-Ray Variability of MCG -6-30-15: the Effects of Strong Gravity around a Kerr Black Hole}},
	volume = 59,
	year = 2007}

@article{Miniutti:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.349.1435M},
	author = {{Miniutti}, G. and {Fabian}, A.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2004.07611.x},
	eprint = {arXiv:astro-ph/0309064},
	journal = {\mnras},
	keywords = {accretion, accretion discs, black hole physics, relativity, galaxies: active, X-rays: galaxies, X-rays: stars},
	month = apr,
	pages = {1435-1448},
	title = {{A light bending model for the X-ray temporal and spectral properties of accreting black holes}},
	volume = 349,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.07611.x}}

@article{Merloni:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.370.1699M},
	author = {{Merloni}, A. and {Malzac}, J. and {Fabian}, A.~C. and {Ross}, R.~R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2006.10676.x},
	eprint = {arXiv:astro-ph/0606262},
	journal = {\mnras},
	keywords = {accretion, accretion discs: black hole physics, accretion discs, black hole physics},
	month = aug,
	pages = {1699-1712},
	title = {{On the X-ray spectra of luminous, inhomogeneous accretion flows}},
	volume = 370,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10676.x}}

@article{Mattson:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...664..101M},
	archiveprefix = {arXiv},
	author = {{Mattson}, B.~J. and {Weaver}, K.~A. and {Reynolds}, C.~S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/518783},
	eprint = {0704.1587},
	journal = {\apj},
	keywords = {Galaxies: Seyfert, X-Rays: Galaxies},
	month = jul,
	pages = {101-105},
	title = {{Possible X-Ray Diagnostic for Jet/Disk Dominance in Type 1 AGNs}},
	volume = 664,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/518783}}

@article{Matt:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...445..451M},
	author = {{Matt}, G. and {Bianchi}, S. and {de Rosa}, A. and {Grandi}, P. and {Perola}, G.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20054013},
	eprint = {arXiv:astro-ph/0509017},
	journal = {\aap},
	keywords = {galaxies: active, X-rays: galaxies, galaxies: individual: MCG+8-11-11},
	month = jan,
	pages = {451-456},
	title = {{XMM-Newton observation of the bright Seyfert 1 galaxy, MCG+8-11-11}},
	volume = 445,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20054013}}

@inproceedings{Matt:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001AIPC..599..209M},
	author = {{Matt}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1063/1.1434634},
	eprint = {arXiv:astro-ph/0007105},
	journal = {X-ray Astronomy: Stellar Endpoints, AGN, and the Diffuse X-ray Background},
	keywords = {Active and peculiar galaxies and related systems, X-ray sources; X-ray bursts},
	month = dec,
	pages = {209-218},
	title = {{The broad band spectrum and variability of Seyfert 1}},
	volume = 599,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1063/1.1434634}}

@article{Masetti:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...470..331M},
	archiveprefix = {arXiv},
	author = {{Masetti}, N. and {Landi}, R. and {Pretorius}, M.~L. and {Sguera}, V. and {Bird}, A.~J. and {Perri}, M. and {Charles}, P.~A. and {Kennea}, J.~A. and {Malizia}, A. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20077509},
	eprint = {0704.3682},
	journal = {\aap},
	keywords = {astrometry, stars: binaries: general, X-rays: binaries, stars: neutron, stars: individual: IGR J16194-2810},
	month = jul,
	pages = {331-337},
	title = {{IGR J16194-2810: a new symbiotic X-ray binary}},
	volume = 470,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077509}}

@article{Markowitz:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...646..783M},
	author = {{Markowitz}, A. and {Reeves}, J.~N. and {Braito}, V.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/505107},
	eprint = {arXiv:astro-ph/0604353},
	journal = {\apj},
	keywords = {Galaxies: Active, galaxies: individual (IC 4329a), Galaxies: Seyfert, X-Rays: Galaxies},
	month = aug,
	pages = {783-800},
	title = {{Fe K Emission and Absorption in the XMM-EPIC Spectrum of the Seyfert Galaxy IC 4329a}},
	volume = 646,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/505107}}

@inproceedings{Maraschi:1997,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1997ASPC..121..101M},
	author = {{Maraschi}, L. and {Haardt}, F.},
	booktitle = {IAU Colloq. 163: Accretion Phenomena and Related Outflows},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{D.~T.~Wickramasinghe, G.~V.~Bicknell, \& L.~Ferrario}},
	pages = {101-+},
	series = {Astronomical Society of the Pacific Conference Series},
	title = {{Disk-Corona Models and X-Ray Emission from Seyfert Galaxies}},
	volume = 121,
	year = 1997}

@article{malzac02,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.336.1209M},
	author = {{Malzac}, J. and {Petrucci}, {P.-O.}},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:49:08 +0200},
	doi = {10.1046/j.1365-8711.2002.05851.x},
	eprint = {arXiv:astro-ph/0109339},
	journal = {\mnras},
	keywords = {accretion, accretion discs, black hole physics, radiative transfer, galaxies: Seyfert, gamma-rays: theory, X-rays: general},
	month = nov,
	pages = {1209-1216},
	title = {{Reflection at large distance from the central engine in Seyferts}},
	volume = 336,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2002.05851.x}}

@article{Malzac:2001a,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.326..417M},
	author = {{Malzac}, J. and {Beloborodov}, A.~M. and {Poutanen}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2001.04450.x},
	eprint = {arXiv:astro-ph/0102490},
	journal = {\mnras},
	keywords = {ACCRETION, ACCRETION DISCS, RADIATIVE TRANSFER, STARS: INDIVIDUAL: CYG X-1, GALAXIES: SEYFERT, GAMMA-RAYS: THEORY, X-RAYS: GENERAL},
	month = sep,
	pages = {417-427},
	title = {{X-ray spectra of accretion discs with dynamic coronae}},
	volume = 326,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2001.04450.x}}

@article{malzac01b,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.325.1625M},
	author = {{Malzac}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:49:00 +0200},
	doi = {10.1046/j.1365-8711.2001.04567.x},
	eprint = {arXiv:astro-ph/0104273},
	journal = {\mnras},
	keywords = {ACCRETION, ACCRETION DISCS, BLACK HOLE PHYSICS, RADIATIVE TRANSFER, GALAXIES: SEYFERT, GAMMA-RAYS: THEORY, X-RAYS: GENERAL},
	month = aug,
	pages = {1625-1636},
	title = {{A quasi-spherical inner accretion flow in Seyfert galaxies?}},
	volume = 325,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2001.04567.x}}

@article{Malizia:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.389.1360M},
	archiveprefix = {arXiv},
	author = {{Malizia}, A. and {Bassani}, L. and {Bird}, A.~J. and {Landi}, R. and {Masetti}, N. and {de Rosa}, A. and {Panessa}, F. and {Molina}, M. and {Dean}, A.~J. and {Perri}, M. and {Tueller}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.13657.x},
	eprint = {0806.4824},
	journal = {\mnras},
	keywords = {galaxies: active , galaxies: Seyfert , X-rays: galaxies},
	month = sep,
	pages = {1360-1366},
	title = {{First high-energy observations of narrow-line Seyfert 1s with INTEGRAL/IBIS}},
	volume = 389,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13657.x}}

@article{Malizia:2003a,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...406..105M},
	author = {{Malizia}, A. and {Bassani}, L. and {Capalbi}, M. and {Fabian}, A.~C. and {Fiore}, F. and {Nicastro}, F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20030743},
	eprint = {arXiv:astro-ph/0305329},
	journal = {\aap},
	keywords = {X-rays: galaxies, galaxies: Seyfert, galaxies: individual: MKN6},
	month = jul,
	pages = {105-109},
	title = {{A BeppoSAX observation of MKN6}},
	volume = 406,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20030743}}

@article{Malizia:2003b,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...589L..17M},
	author = {{Malizia}, A. and {Bassani}, L. and {Stephen}, J.~B. and {Di Cocco}, G. and {Fiore}, F. and {Dean}, A.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/375712},
	eprint = {arXiv:astro-ph/0304133},
	journal = {\apjl},
	keywords = {Galaxies: Active, Galaxies: Seyfert},
	month = may,
	pages = {L17-L20},
	title = {{BeppoSAX Average Spectra of Seyfert Galaxies}},
	volume = 589,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/375712}}

@article{Lebrun:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411L.141L},
	author = {{Lebrun}, F. and {Leray}, J.~P. and {Lavocat}, P. and {Cr{\'e}tolle}, J. and {Arqu{\`e}s}, M. and {Blondel}, C. and {Bonnin}, C. and {Bou{\`e}re}, A. and {Cara}, C. and {Chaleil}, T. and {Daly}, F. and {Desages}, F. and {Dzitko}, H. and {Horeau}, B. and {Laurent}, P. and {Limousin}, O. and {Mathy}, F. and {Mauguen}, V. and {Meignier}, F. and {Molini{\'e}}, F. and {Poindron}, E. and {Rouger}, M. and {Sauvageon}, A. and {Tourrette}, T.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20031367},
	eprint = {arXiv:astro-ph/0310362},
	journal = {\aap},
	keywords = {space telescope, cadmium telluride detectors, gamma-ray astronomy, calibration, INTEGRAL},
	month = nov,
	pages = {L141-L148},
	title = {{ISGRI: The INTEGRAL Soft Gamma-Ray Imager}},
	volume = 411,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031367}}

@article{Landi:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.380..926L},
	archiveprefix = {arXiv},
	author = {{Landi}, R. and {de Rosa}, A. and {Dean}, A.~J. and {Bassani}, L. and {Ubertini}, P. and {Bird}, A.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2007.12168.x},
	eprint = {0707.0832},
	journal = {\mnras},
	keywords = {gamma-rays: observations, X-rays: individual: PSR J1617-5055},
	month = sep,
	pages = {926-932},
	title = {{HESS J1616-508: likely to be powered by PSR J1617-5055}},
	volume = 380,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12168.x}}

@inproceedings{Hill:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004SPIE.5165..217H},
	author = {{Hill}, J.~E. and {Burrows}, D.~N. and {Nousek}, J.~A. and {Abbey}, A.~F. and {Ambrosi}, R.~M. and {Br{\"a}uninger}, H.~W. and {Burkert}, W. and {Campana}, S. and {Cheruvu}, C. and {Cusumano}, G. and {Freyberg}, M.~J. and {Hartner}, G.~D. and {Klar}, R. and {Mangels}, C. and {Moretti}, A. and {Mori}, K. and {Morris}, D.~C. and {Short}, A.~D.~T. and {Tagliaferri}, G. and {Watson}, D.~J. and {Wood}, P. and {Wells}, A.~A.},
	booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1117/12.505728},
	editor = {{K.~A.~Flanagan \& O.~H.~W.~Siegmund}},
	month = feb,
	pages = {217-231},
	series = {Presented at the Society of Photo-Optical Instrumentation Engineers (SPIE) Conference},
	title = {{Readout modes and automated operation of the Swift X-ray Telescope}},
	volume = 5165,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.505728}}

@article{Hickox:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...645...95H},
	author = {{Hickox}, R.~C. and {Markevitch}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/504070},
	eprint = {arXiv:astro-ph/0512542},
	journal = {\apj},
	keywords = {Galaxies: Active, Methods: Data Analysis, X-Rays: Diffuse Background, X-Rays: Galaxies},
	month = jul,
	pages = {95-114},
	title = {{Absolute Measurement of the Unresolved Cosmic X-Ray Background in the 0.5-8 keV Band with Chandra}},
	volume = 645,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/504070}}

@article{Guainazzi:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006AN....327.1032G},
	author = {{Guainazzi}, M. and {Bianchi}, S. and {Dov{\v c}iak}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1002/asna.200610687},
	eprint = {arXiv:astro-ph/0610151},
	journal = {Astronomische Nachrichten},
	keywords = {quasars: emission lines, galaxies: nuclei, galaxies: active, X-ray: galaxies, line: profiles},
	pages = {1032-+},
	title = {{Statistics of relativistically broadened Fe K{$\alpha$} lines in AGN}},
	volume = 327,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1002/asna.200610687}}

@article{Guainazzi:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...346..407G},
	author = {{Guainazzi}, M. and {Perola}, G.~C. and {Matt}, G. and {Nicastro}, F. and {Bassani}, L. and {Fiore}, F. and {dal Fiume}, D. and {Piro}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {arXiv:astro-ph/9903449},
	journal = {\aap},
	keywords = {GALAXIES: INDIVIDUAL: NGC 4593, GALAXIES: NUCLEI, GALAXIES: SEYFERT, X-RAYS: GALAXIES},
	month = jun,
	pages = {407-414},
	title = {{The complex 0.1-200 keV spectrum of the Seyfert 1 Galaxy NGC 4593}},
	volume = 346,
	year = 1999}

@article{Gruber:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...520..124G},
	author = {{Gruber}, D.~E. and {Matteson}, J.~L. and {Peterson}, L.~E. and {Jung}, G.~V.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/307450},
	eprint = {arXiv:astro-ph/9903492},
	journal = {\apj},
	keywords = {COSMOLOGY: DIFFUSE RADIATION, INSTRUMENTATION: DETECTORS, X-RAYS: GENERAL},
	month = jul,
	pages = {124-129},
	title = {{The Spectrum of Diffuse Cosmic Hard X-Rays Measured with HEAO 1}},
	volume = 520,
	year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/307450}}

@article{Grandi:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...642..113G},
	author = {{Grandi}, P. and {Malaguti}, G. and {Fiocchi}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/500100},
	eprint = {arXiv:astro-ph/0511784},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Nuclei, Surveys, X-Rays: Galaxies},
	month = may,
	pages = {113-125},
	title = {{BeppoSAX View of Radio-loud Active Galactic Nuclei}},
	volume = 642,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/500100}}

@article{Goldwurm:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411L.223G},
	author = {{Goldwurm}, A. and {David}, P. and {Foschini}, L. and {Gros}, A. and {Laurent}, P. and {Sauvageon}, A. and {Bird}, A.~J. and {Lerusse}, L. and {Produit}, N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20031395},
	eprint = {arXiv:astro-ph/0311172},
	journal = {\aap},
	keywords = {coded masks, imaging, gamma-rays},
	month = nov,
	pages = {L223-L229},
	title = {{The INTEGRAL/IBIS scientific data analysis}},
	volume = 411,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031395}}

@article{Gilli:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...463...79G},
	author = {{Gilli}, R. and {Comastri}, A. and {Hasinger}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20066334},
	eprint = {arXiv:astro-ph/0610939},
	journal = {\aap},
	keywords = {X-rays: galaxies, galaxies: active, X-rays: general, cosmology: diffuse radiation, X-rays: diffuse background},
	month = feb,
	pages = {79-96},
	title = {{The synthesis of the cosmic X-ray background in the Chandra and XMM-Newton era}},
	volume = 463,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20066334}}

@article{Gandhi:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.382.1005G},
	archiveprefix = {arXiv},
	author = {{Gandhi}, P. and {Fabian}, A.~C. and {Suebsuwong}, T. and {Malzac}, J. and {Miniutti}, G. and {Wilman}, R.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2007.12462.x},
	eprint = {0709.1984},
	journal = {\mnras},
	keywords = {galaxies: active, X-rays: galaxies},
	month = dec,
	pages = {1005-1018},
	title = {{Constraints on light bending and reflection from the hard X-ray background}},
	volume = 382,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12462.x}}

@article{Fabian:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.335L...1F},
	author = {{Fabian}, A.~C. and {Vaughan}, S. and {Nandra}, K. and {Iwasawa}, K. and {Ballantyne}, D.~R. and {Lee}, J.~C. and {De Rosa}, A. and {Turner}, A. and {Young}, A.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2002.05740.x},
	eprint = {arXiv:astro-ph/0206095},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: general, galaxies: individual: MCG, 6-30-15, galaxies: Seyfert, X-rays: galaxies},
	month = sep,
	pages = {L1-L5},
	title = {{A long hard look at MCG-6-30-15 with XMM-Newton}},
	volume = 335,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2002.05740.x}}

@article{Fabian:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.353.1071F},
	author = {{Fabian}, A.~C. and {Miniutti}, G. and {Gallo}, L. and {Boller}, T. and {Tanaka}, Y. and {Vaughan}, S. and {Ross}, R.~R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2004.08036.x},
	eprint = {arXiv:astro-ph/0405160},
	journal = {\mnras},
	keywords = {line: formation, galaxies: active, galaxies: individual: 1H 0707-495, X-rays: galaxies, X-rays: general},
	month = oct,
	pages = {1071-1077},
	title = {{X-ray reflection in the narrow-line Seyfert 1 galaxy 1H 0707-495}},
	volume = 353,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.08036.x}}

@article{Fabian:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.361..795F},
	author = {{Fabian}, A.~C. and {Miniutti}, G. and {Iwasawa}, K. and {Ross}, R.~R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2005.09148.x},
	eprint = {arXiv:astro-ph/0504472},
	journal = {\mnras},
	keywords = {line: formation, galaxies: active, galaxies: individual: 1H 0419-577, X-rays: galaxies, X-rays: general},
	month = aug,
	pages = {795-802},
	title = {{X-ray reflection in the Seyfert galaxy 1H 0419-577 revealing strong relativistic effects in the vicinity of a Kerr black hole}},
	volume = 361,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09148.x}}

@article{Elitzur:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...648L.101E},
	author = {{Elitzur}, M. and {Shlosman}, I.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/508158},
	eprint = {arXiv:astro-ph/0605686},
	journal = {\apjl},
	keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, Infrared: Galaxies, Galaxies: Quasars: General},
	month = sep,
	pages = {L101-L104},
	title = {{The AGN-obscuring Torus: The End of the ``Doughnut'' Paradigm?}},
	volume = 648,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/508158}}

@article{Derosa:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...387..838D},
	author = {{De Rosa}, A. and {Piro}, L. and {Fiore}, F. and {Grandi}, P. and {Maraschi}, L. and {Matt}, G. and {Nicastro}, F. and {Petrucci}, P.~O.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20020444},
	eprint = {arXiv:astro-ph/0203344},
	journal = {\aap},
	keywords = {galaxies: individual: NGC 3783, galaxies: Seyfert, X-rays: galaxies},
	month = jun,
	pages = {838-849},
	title = {{The BeppoSAX broad-band spectrum and variability of the Seyfert 1 NGC 3783}},
	volume = 387,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20020444}}

@article{Derosa:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...463..903D},
	author = {{de Rosa}, A. and {Piro}, L. and {Perola}, G.~C. and {Capalbi}, M. and {Cappi}, M. and {Grandi}, P. and {Maraschi}, L. and {Petrucci}, P.~O.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20065028},
	eprint = {arXiv:astro-ph/0611470},
	journal = {\aap},
	keywords = {galaxies: Seyfert, X-rays: galaxies, galaxies: individual: NGC 4151},
	month = mar,
	pages = {903-912},
	title = {{The broad band spectrum and variability of NGC 4151 observed by BeppoSAX}},
	volume = 463,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20065028}}

@article{Dadina:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...485..417D},
	archiveprefix = {arXiv},
	author = {{Dadina}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20077569},
	eprint = {0801.4338},
	journal = {\aap},
	keywords = {X-rays: galaxies, galaxies: Seyfert:, galaxies: active},
	month = jul,
	pages = {417-424},
	title = {{Seyfert galaxies in the local Universe (z {\le} 0.1): the average X-ray spectrum as seen by BeppoSAX}},
	volume = 485,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077569}}

@article{Dadina:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...461.1209D},
	author = {{Dadina}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20065734},
	journal = {\aap},
	keywords = {catalogs, galaxies: active, galaxies: Seyfert, X-ray: galaxies},
	month = jan,
	pages = {1209-1252},
	title = {{BeppoSAX observations in the 2-100 keV band of the nearby Seyfert galaxies: an atlas of spectra}},
	volume = 461,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20065734}}

@article{Comastri:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007PThPS.169..274C},
	archiveprefix = {arXiv},
	author = {{Comastri}, A. and {Gilli}, R. and {Vignali}, C. and {Matt}, G. and {Fiore}, F. and {Iwasawa}, K.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {0704.1253},
	journal = {Progress of Theoretical Physics Supplement},
	pages = {274-277},
	title = {{Compton Thick AGN in the Suzaku Era}},
	volume = 169,
	year = 2007}

@article{Comastri:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005ExA....20...41C},
	author = {{Comastri}, A. and {Gilli}, R. and {Hasinger}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1007/s10686-006-9041-6},
	eprint = {arXiv:astro-ph/0604523},
	journal = {Experimental Astronomy},
	keywords = {X-rays, Background radiation, AGN},
	month = dec,
	pages = {41-47},
	title = {{Rolling down from the 30 keV peak: Modelling the Hard X-Ray and {$\gamma$}-Ray Backgrounds}},
	volume = 20,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10686-006-9041-6}}

@article{Comastri:1995,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...296....1C},
	author = {{Comastri}, A. and {Setti}, G. and {Zamorani}, G. and {Hasinger}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {arXiv:astro-ph/9409067},
	journal = {\aap},
	keywords = {X-RAYS: GENERAL, X-RAYS: GALAXIES, COSMOLOGY: DIFFUSE RADIATION, GALAXIES:NUCLEI, QUASARS:GENERAL},
	month = apr,
	pages = {1-+},
	title = {{The contribution of AGNs to the X-ray background.}},
	volume = 296,
	year = 1995}

@article{Cappi:1996,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...458..149C},
	author = {{Cappi}, M. and {Mihara}, T. and {Matsuoka}, M. and {Hayashida}, K. and {Weaver}, K.~A. and {Otani}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/176799},
	eprint = {arXiv:astro-ph/9510065},
	journal = {\apj},
	keywords = {GALAXIES: INDIVIDUAL ALPHANUMERIC: IC 4329A, GALAXIES: SEYFERT, X-RAYS: GALAXIES},
	month = feb,
	pages = {149-+},
	title = {{Warm Absorber, Reflection, and Fe K Line in the X-Ray Spectrum of IC 4329A}},
	volume = 458,
	year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/176799}}

@article{bird04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...607L..33B},
	author = {{Bird}, A.~J. and {Barlow}, E.~J. and {Bassani}, L. and {Bazzano}, A. and {Bodaghee}, A. and {Capitanio}, F. and {Cocchi}, M. and {Del Santo}, M. and {Dean}, A.~J. and {Hill}, A.~B. and {Lebrun}, F. and {Malaguti}, G. and {Malizia}, A. and {Much}, R. and {Shaw}, S.~E. and {Stephen}, J.~B. and {Terrier}, R. and {Ubertini}, P. and {Walter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:50:36 +0200},
	doi = {10.1086/421772},
	journal = {\apjl},
	keywords = {Galaxy: General, Gamma Rays: Observations, Surveys},
	month = may,
	pages = {L33-L37},
	title = {{The First IBIS/ISGRI Soft Gamma-Ray Galactic Plane Survey Catalog}},
	volume = 607,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/421772}}

@article{bird06,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...636..765B},
	author = {{Bird}, A.~J. and {Barlow}, E.~J. and {Bassani}, L. and {Bazzano}, A. and {B{\'e}langer}, G. and {Bodaghee}, A. and {Capitanio}, F. and {Dean}, A.~J. and {Fiocchi}, M. and {Hill}, A.~B. and {Lebrun}, F. and {Malizia}, A. and {Mas-Hesse}, J.~M. and {Molina}, M. and {Moran}, L. and {Renaud}, M. and {Sguera}, V. and {Shaw}, S.~E. and {Stephen}, J.~B. and {Terrier}, R. and {Ubertini}, P. and {Walter}, R. and {Willis}, D.~R. and {Winkler}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:50:53 +0200},
	doi = {10.1086/498090},
	journal = {\apj},
	keywords = {Galaxy: General, Gamma Rays: Observations, Surveys},
	month = jan,
	pages = {765-776},
	title = {{The Second IBIS/ISGRI Soft Gamma-Ray Survey Catalog}},
	volume = 636,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/498090}}

@article{bird07,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..170..175B},
	author = {{Bird}, A.~J. and {Malizia}, A. and {Bazzano}, A. and {Barlow}, E.~J. and {Bassani}, L. and {Hill}, A.~B. and {B{\'e}langer}, G. and {Capitanio}, F. and {Clark}, D.~J. and {Dean}, A.~J. and {Fiocchi}, M. and {G{\"o}tz}, D. and {Lebrun}, F. and {Molina}, M. and {Produit}, N. and {Renaud}, M. and {Sguera}, V. and {Stephen}, J.~B. and {Terrier}, R. and {Ubertini}, P. and {Walter}, R. and {Winkler}, C. and {Zurita}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:50:44 +0200},
	doi = {10.1086/513148},
	eprint = {arXiv:astro-ph/0611493},
	journal = {\apjs},
	keywords = {Galaxy: General, Gamma Rays: Observations, Surveys},
	month = may,
	pages = {175-186},
	title = {{The Third IBIS/ISGRI Soft Gamma-Ray Survey Catalog}},
	volume = 170,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/513148}}

@article{Bianchi:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...495..421B},
	archiveprefix = {arXiv},
	author = {{Bianchi}, S. and {Guainazzi}, M. and {Matt}, G. and {Fonseca Bonilla}, N. and {Ponti}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:200810620},
	eprint = {0811.1126},
	journal = {\aap},
	keywords = {galaxies: active, galaxies: Seyfert, quasars: general, X-rays: general},
	month = feb,
	pages = {421-430},
	title = {{CAIXA: a catalogue of AGN in the XMM-Newton archive. I. Spectral analysis}},
	volume = 495,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200810620}}

@article{Bianchi:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...467L..19B},
	author = {{Bianchi}, S. and {Guainazzi}, M. and {Matt}, G. and {Fonseca Bonilla}, N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20077331},
	eprint = {arXiv:astro-ph/0703433},
	journal = {\aap},
	keywords = {galaxies: active, galaxies: Seyfert, quasars: general, X-rays: general},
	month = may,
	pages = {L19-L22},
	title = {{On the Iwasawa-Taniguchi effect of radio-quiet AGN}},
	volume = 467,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077331}}

@article{Beckmann:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...475..827B},
	author = {{Beckmann}, V. and {Barthelmy}, S.~D. and {Courvoisier}, {T.~J.-L.} and {Gehrels}, N. and {Soldi}, S. and {Tueller}, J. and {Wendt}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20078355},
	journal = {\aap},
	keywords = {galaxies: active, galaxies: Seyfert , X-rays:, galaxies, surveys},
	month = dec,
	pages = {827-835},
	title = {{Hard X-ray variability of active galactic nuclei}},
	volume = 475,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078355}}

@article{baumgartner08,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ATel.1429....1B},
	author = {{Baumgartner}, W. and {Tueller}, J. and {Mushotzky}, R. and {Barthelmy}, S. and {Cannizzo}, J. and {Gehrels}, N. and {Markwardt}, C. and {Skinner}, G. and {Winter}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:50:16 +0200},
	journal = {The Astronomer's Telegram},
	keywords = {X-ray, Gamma Ray, AGN, Black Holes, Quasars},
	month = mar,
	pages = {1-+},
	title = {{Swift/BAT teams announces website with catalog of AGN from the first 9}},
	volume = 1429,
	year = 2008}

@article{Barger:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005AJ....129..578B},
	author = {{Barger}, A.~J. and {Cowie}, L.~L. and {Mushotzky}, R.~F. and {Yang}, Y. and {Wang}, {W.-H.} and {Steffen}, A.~T. and {Capak}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/426915},
	eprint = {arXiv:astro-ph/0410527},
	journal = {\aj},
	keywords = {Cosmology: Observations, Galaxies: Active, Galaxies: Distances and Redshifts, Galaxies: Evolution, Galaxies: Formation},
	month = feb,
	pages = {578-609},
	title = {{The Cosmic Evolution of Hard X-Ray-selected Active Galactic Nuclei}},
	volume = 129,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/426915}}

@article{Avni:1980,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1980ApJ...235..694A},
	author = {{Avni}, Y. and {Bahcall}, J.~N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/157673},
	journal = {\apj},
	keywords = {COSMOLOGY, DATA SAMPLING, QUASARS, STELLAR EVOLUTION, ASTROPHYSICS, POISSON DENSITY FUNCTIONS, STELLAR LUMINOSITY},
	month = feb,
	pages = {694-716},
	title = {{On the simultaneous analysis of several complete samples - The V/Vmax and Ve/Va variables, with applications to quasars}},
	volume = 235,
	year = 1980,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/157673}}

@inproceedings{arnaud96,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1996ASPC..101...17A},
	author = {{Arnaud}, K.~A.},
	booktitle = {Astronomical Data Analysis Software and Systems V},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:49:53 +0200},
	editor = {{G.~H.~Jacoby \& J.~Barnes}},
	pages = {17},
	series = {Astronomical Society of the Pacific Conference Series},
	title = {{XSPEC: The First Ten Years}},
	volume = 101,
	year = 1996}

@article{ajello08,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...673...96A},
	archiveprefix = {arXiv},
	author = {{Ajello}, M. and {Rau}, A. and {Greiner}, J. and {Kanbach}, G. and {Salvato}, M. and {Strong}, A.~W. and {Barthelmy}, S.~D. and {Gehrels}, N. and {Markwardt}, C.~B. and {Tueller}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:49:24 +0200},
	doi = {10.1086/524104},
	eprint = {0709.4333},
	journal = {\apj},
	keywords = {Galaxies: Active, Surveys, X-Rays: Binaries, X-Rays: Galaxies},
	month = jan,
	pages = {96-113},
	title = {{The Swift BAT X-Ray Survey. III. X-Ray Spectra and Statistical Properties}},
	volume = 673,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/524104}}

@article{croton06a,
	adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006MNRAS.369.1808C&db_key=AST},
	author = {{Croton}, D.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2006.10429.x},
	eprint = {arXiv:0512375},
	journal = {\mnras},
	month = jul,
	pages = {1808-1812},
	title = {{Evolution in the black hole mass-bulge mass relation: a theoretical perspective}},
	volume = {369},
	year = {2006},
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10429.x}}

@article{norris11,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...736...55N},
	archiveprefix = {arXiv},
	author = {{Norris}, R.~P. and {Afonso}, J. and {Cava}, A. and {Farrah}, D. and {Huynh}, M.~T. and {Ivison}, R.~J. and {Jarvis}, M. and {Lacy}, M. and {Mao}, M. and {Maraston}, C. and {Mauduit}, J.-C. and {Middelberg}, E. and {Oliver}, S. and {Seymour}, N. and {Surace}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/736/1/55},
	eprint = {1105.0960},
	journal = {\apj},
	keywords = {galaxies: evolution, galaxies: formation, galaxies: starburst},
	month = jul,
	pages = {55-+},
	primaryclass = {astro-ph.CO},
	title = {{Deep Spitzer Observations of Infrared-faint Radio Sources: High-redshift Radio-loud Active Galactic Nuclei?}},
	volume = 736,
	year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/736/1/55}}

@article{sikora07,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...658..815S},
	author = {{Sikora}, M. and {Stawarz}, {\L}. and {Lasota}, J.-P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/511972},
	eprint = {arXiv:astro-ph/0604095},
	journal = {\apj},
	keywords = {Galaxies: Jets, Magnetohydrodynamics: MHD, Radiation Mechanisms: Nonthermal},
	month = apr,
	pages = {815-828},
	title = {{Radio Loudness of Active Galactic Nuclei: Observational Facts and Theoretical Implications}},
	volume = 658,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/511972}}

@article{best06,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.368L..67B},
	author = {{Best}, P.~N. and {Kaiser}, C.~R. and {Heckman}, T.~M. and {Kauffmann}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1745-3933.2006.00159.x},
	eprint = {arXiv:astro-ph/0602171},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: evolution, galaxies: stellar content, accretion, radio continuum: galaxies},
	month = may,
	pages = {L67-L71},
	title = {{AGN-controlled cooling in elliptical galaxies}},
	volume = 368,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2006.00159.x}}

@article{clemens10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.405..887C},
	archiveprefix = {arXiv},
	author = {{Clemens}, M.~S. and {Scaife}, A. and {Vega}, O. and {Bressan}, A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2010.16534.x},
	eprint = {1002.3334},
	journal = {\mnras},
	keywords = {galaxies: active, infrared: galaxies, radio continuum: galaxies},
	month = jun,
	pages = {887-897},
	primaryclass = {astro-ph.GA},
	title = {{Starburst evolution: free-free absorption in the radio spectra of luminous IRAS galaxies}},
	volume = 405,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.16534.x}}


==> biblio_copy.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Created for Manuela Molina at 2021-04-29 17:11:00 +0200 


%% Saved with string encoding Unicode (UTF-8) 

@ARTICLE{landi11a,
       author = {{Landi}, R. and {Bassani}, L. and {Masetti}, N. and {Bazzano}, A. and {Bird}, A.~J.},
        title = "{Swift/XRT follow-up observations of unidentified INTEGRAL sources (1)}",
      journal = {The Astronomer's Telegram},
     keywords = {X-ray, Gamma Ray, Request for Observations, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2011,
        month = apr,
       volume = {3271},
        pages = {1},
archivePrefix = {arXiv},
       eprint = {1003.1214},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ATel.3271....1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tueller06,
       author = {{Tueller}, J. and {Markwardt}, C. and {Ajello}, M. and {Barthelmy}, S. and {Belloni}, T. and {Falcone}, A. and {Gehrels}, N. and {Godet}, O. and {Grupe}, D. and {Holland}, S. and {Kennea}, J. and {Mukai}, K. and {Mushotzky}, R. and {Sambruna}, R. and {Skinner}, G.~K.},
        title = "{Swift BAT Survey Reports 3 New Hard X-ray Sources Near the Galactic Plane}",
      journal = {The Astronomer's Telegram},
     keywords = {X-ray, Gamma Ray, Request for Observations, Transients},
         year = 2006,
        month = jul,
       volume = {853},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ATel..853....1T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fiocchi07,
       author = {{Fiocchi}, Mariateresa and {Bazzano}, Angela and {Ubertini}, Pietro and {Zdziarski}, Andrzej A.},
        title = "{The First Detection of Compton Reflection in the Low-Mass X-Ray Binary 4U 1705-44 with INTEGRAL and BeppoSax}",
      journal = {\apj},
     keywords = {Accretion, Accretion Disks, Gamma Rays: Observations, Radiation Mechanisms: Nonthermal, stars: individual (4U 1705 44), Stars: Neutron, X-Rays: Binaries, Astrophysics},
         year = 2007,
        month = mar,
       volume = {657},
       number = {1},
        pages = {448-452},
          doi = {10.1086/510573},
archivePrefix = {arXiv},
       eprint = {astro-ph/0611050},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...657..448F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{karasev12,
       author = {{Karasev}, D.~I. and {Lutovinov}, A.~A. and {Revnivtsev}, M.~G. and {Krivonos}, R.~A.},
        title = "{Accurate localization and identification of six hard X-ray sources from Chandra and XMM-Newton data}",
      journal = {Astronomy Letters},
     keywords = {X-ray sources, cataclysmic variables, neutron stars, active galactic nuclei, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = oct,
       volume = {38},
       number = {10},
        pages = {629-637},
          doi = {10.1134/S1063773712100039},
archivePrefix = {arXiv},
       eprint = {1209.2945},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012AstL...38..629K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{kormendy13,
       author = {{Kormendy}, John and {Ho}, Luis C.},
        title = "{Coevolution (Or Not) of Supermassive Black Holes and Host Galaxies}",
      journal = {\araa},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = aug,
       volume = {51},
       number = {1},
        pages = {511-653},
          doi = {10.1146/annurev-astro-082708-101811},
archivePrefix = {arXiv},
       eprint = {1304.7762},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ARA&A..51..511K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{demartino20,
       author = {{De Martino}, D. and {Bernardini}, F. and {Mukai}, K. and {Falanga}, M. and {Masetti}, N.},
        title = "{Hard X-ray cataclysmic variables}",
      journal = {Advances in Space Research},
     keywords = {X-Rays: binaries, Stars: cataclysmic variables, Accretion, Accretion discs, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = sep,
       volume = {66},
       number = {5},
        pages = {1209-1225},
          doi = {10.1016/j.asr.2019.09.006},
archivePrefix = {arXiv},
       eprint = {1909.06306},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AdSpR..66.1209D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{barthelmy05,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2005SSRv..120..143B},
	archiveprefix = {arXiv},
	author = {{Barthelmy}, Scott D. and {Barbier}, Louis M. and {Cummings}, Jay R. and {Fenimore}, Ed E. and {Gehrels}, Neil and {Hullinger}, Derek and {Krimm}, Hans A. and {Markwardt}, Craig B. and {Palmer}, David M. and {Parsons}, Ann and {Sato}, Goro and {Suzuki}, Masaya and {Takahashi}, Tadayuki and {Tashiro}, Makota and {Tueller}, Jack},
	date-added = {2021-04-29 17:10:46 +0200},
	date-modified = {2021-04-29 17:10:58 +0200},
	doi = {10.1007/s11214-005-5096-3},
	eprint = {astro-ph/0507410},
	journal = {\ssr},
	keywords = {gamma-ray, GRB, hard X-ray, survey, burst, afterglow, CZT, coded aperture, astrophysics, cosmology, Astrophysics},
	month = oct,
	number = {3-4},
	pages = {143-164},
	primaryclass = {astro-ph},
	title = {{The Burst Alert Telescope (BAT) on the SWIFT Midex Mission}},
	volume = {120},
	year = 2005,
	Bdsk-Url-1 = {https://doi.org/10.1007/s11214-005-5096-3}}

@article{babusieux18,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...616A..10G},
	archiveprefix = {arXiv},
	author = {{Babusiaux}, C. and {van Leeuwen}, F. and {Barstow}, M.~A. and {Jordi}, C. and {Vallenari}, A. and {Bossini}, D. and {Bressan}, A. and {Cantat-Gaudin}, T. and {van Leeuwen}, M. and {Brown}, A.~G.~A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Bailer-Jones}, C.~A.~L. and {Biermann}, M. and {Evans}, D.~W. and {Eyer}, L. and {Jansen}, F. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Siddiqui}, H.~I. and {Soubiran}, C. and {Walton}, N.~A. and {Arenou}, F. and {Bastian}, U. and {Cropper}, M. and {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {Chaoul}, L. and {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and {Guerra}, R. and {Holl}, B. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nienartowicz}, K. and {Panuzzo}, P. and {Portell}, J. and {Riello}, M. and {Seabroke}, G.~M. and {Tanga}, P. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Comoretto}, G. and {Garcia-Reinaldos}, M. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Audard}, M. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Burgess}, P. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Clementini}, G. and {Clotet}, M. and {Creevey}, O. and {Davidson}, M. and {De Ridder}, J. and {Delchambre}, L. and {Dell'Oro}, A. and {Ducourant}, C. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Galluccio}, L. and {Garc{\'\i}a-Torres}, M. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J.~J. and {Gosset}, E. and {Guy}, L.~P. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Hutton}, A. and {Jasniewicz}, G. and {Jean-Antoine-Piccolo}, A. and {Jordan}, S. and {Korn}, A.~J. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {Lebzelter}, T. and {L{\"o}ffler}, W. and {Manteiga}, M. and {Marrese}, P.~M. and {Mart{\'\i}n-Fleitas}, J.~M. and {Moitinho}, A. and {Mora}, A. and {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Richards}, P.~J. and {Rimoldini}, L. and {Robin}, A.~C. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {S{\"u}veges}, M. and {Torra}, J. and {van Reeven}, W. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aerts}, C. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alvarez}, R. and {Alves}, J. and {Anderson}, R.~I. and {Andrei}, A.~H. and {Anglada Varela}, E. and {Antiche}, E. and {Antoja}, T. and {Arcay}, B. and {Astraatmadja}, T.~L. and {Bach}, N. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balm}, P. and {Barache}, C. and {Barata}, C. and {Barbato}, D. and {Barblan}, F. and {Barklem}, P.~S. and {Barrado}, D. and {Barros}, M. and {Bartholom{\'e} Mu{\~n}oz}, L. and {Bassilana}, J. -L. and {Becciani}, U. and {Bellazzini}, M. and {Berihuete}, A. and {Bertone}, S. and {Bianchi}, L. and {Bienaym{\'e}}, O. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Boeche}, C. and {Bombrun}, A. and {Borrachero}, R. and {Bouquillon}, S. and {Bourda}, G. and {Bragaglia}, A. and {Bramante}, L. and {Breddels}, M.~A. and {Brouillet}, N. and {Br{\"u}semeister}, T. and {Brugaletta}, E. and {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {Cannizzaro}, G. and {Carballo}, R. and {Carlucci}, T. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cocozza}, G. and {Costigan}, G. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and {Crowley}, C. and {Cuypers}, J. and {Dafonte}, C. and {Damerdji}, Y. and {Dapergolas}, A. and {David}, P. and {David}, M. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {de Martino}, D. and {de Souza}, R. and {de Torres}, A. and {Debosscher}, J. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Drazinos}, P. and {Dur{\'a}n}, J. and {Edvardsson}, B. and {Enke}, H. and {Eriksson}, K. and {Esquej}, P. and {Eynard Bontemps}, G. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Falc{\~a}o}, A.~J. and {Farr{\`a}s Casas}, M. and {Federici}, L. and {Fedorets}, G. and {Fernique}, P. and {Figueras}, F. and {Filippi}, F. and {Findeisen}, K. and {Fonti}, A. and {Fraile}, E. and {Fraser}, M. and {Fr{\'e}zouls}, B. and {Gai}, M. and {Galleti}, S. and {Garabato}, D. and {Garc{\'\i}a-Sedano}, F. and {Garofalo}, A. and {Garralda}, N. and {Gavel}, A. and {Gavras}, P. and {Gerssen}, J. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Glass}, F. and {Gomes}, M. and {Granvik}, M. and {Gueguen}, A. and {Guerrier}, A. and {Guiraud}, J. and {Guti{\'e}}, R. and {Haigron}, R. and {Hatzidimitriou}, D. and {Hauser}, M. and {Haywood}, M. and {Heiter}, U. and {Helmi}, A. and {Heu}, J. and {Hilger}, T. and {Hobbs}, D. and {Hofmann}, W. and {Holland}, G. and {Huckle}, H.~E. and {Hypki}, A. and {Icardi}, V. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jonker}, P.~G. and {Juh{\'a}sz}, {\'A}. L. and {Julbe}, F. and {Karampelas}, A. and {Kewley}, A. and {Klar}, J. and {Kochoska}, A. and {Kohley}, R. and {Kolenberg}, K. and {Kontizas}, M. and {Kontizas}, E. and {Koposov}, S.~E. and {Kordopatis}, G. and {Kostrzewa-Rutkowska}, Z. and {Koubsky}, P. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Lavigne}, J. -B. and {Le Fustec}, Y. and {Le Poncin-Lafitte}, C. and {Lebreton}, Y. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Lenhardt}, H. and {Leroux}, F. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {L{\'o}pez}, M. and {Managau}, S. and {Mann}, R.~G. and {Mantelet}, G. and {Marchal}, O. and {Marchant}, J.~M. and {Marconi}, M. and {Marinoni}, S. and {Marschalk{\'o}}, G. and {Marshall}, D.~J. and {Martino}, M. and {Marton}, G. and {Mary}, N. and {Massari}, D. and {Matijevi{\v{c}}}, G. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and {Mulone}, A.~F. and {Muraveva}, T. and {Musella}, I. and {Nelemans}, G. and {Nicastro}, L. and {Noval}, L. and {O'Mullane}, W. and {Ord{\'e}novic}, C. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Osborne}, P. and {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and {Palacin}, H. and {Palaversa}, L. and {Panahi}, A. and {Pawlak}, M. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rambaux}, N. and {Ramos-Lerate}, M. and {Regibo}, S. and {Reyl{\'e}}, C. and {Riclet}, F. and {Ripepi}, V. and {Riva}, A. and {Rivard}, A. and {Rixon}, G. and {Roegiers}, T. and {Roelens}, M. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Ruiz-Dern}, L. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Sanna}, N. and {Santana-Ros}, T. and {Sarasso}, M. and {Savietto}, H. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Shih}, I. -C. and {Siltala}, L. and {Silva}, A.~F. and {Smart}, R.~L. and {Smith}, K.~W. and {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {Stoev}, H. and {Suess}, F.~F. and {Surdej}, J. and {Szabados}, L. and {Szegedi-Elek}, E. and {Tapiador}, D. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Terrett}, D. and {Teyssandier}, P. and {Thuillot}, W. and {Titarenko}, A. and {Torra Clotet}, F. and {Turon}, C. and {Ulla}, A. and {Utrilla}, E. and {Uzzi}, S. and {Vaillant}, M. and {Valentini}, G. and {Valette}, V. and {van Elteren}, A. and {Van Hemelryck}, E. and {Vaschetto}, M. and {Vecchiato}, A. and {Veljanoski}, J. and {Viala}, Y. and {Vicente}, D. and {Vogt}, S. and {von Essen}, C. and {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and {Walmsley}, G. and {Weiler}, M. and {Wertz}, O. and {Wevers}, T. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Ziaeepour}, H. and {Zorec}, J. and {Zschocke}, S. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T.},
	date-added = {2021-04-28 11:42:38 +0200},
	date-modified = {2021-04-28 11:43:39 +0200},
	doi = {10.1051/0004-6361/201832843},
	eid = {A10},
	eprint = {1804.09378},
	journal = {\aap},
	keywords = {parallaxes, Hertzsprung-Russell and C-M diagrams, solar neighborhood, stars: evolution, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
	month = aug,
	pages = {A10},
	primaryclass = {astro-ph.SR},
	title = {{Gaia Data Release 2. Observational Hertzsprung-Russell diagrams}},
	volume = {616},
	year = 2018,
	Bdsk-Url-1 = {https://doi.org/10.1051/0004-6361/201832843}}

@ARTICLE{bernardini12,
       author = {{Bernardini}, F. and {de Martino}, D. and {Falanga}, M. and {Mukai}, K. and {Matt}, G. and {Bonnet-Bidaud}, J. -M. and {Masetti}, N. and {Mouchet}, M.},
        title = "{Characterization of new hard X-ray cataclysmic variables}",
      journal = {\aap},
     keywords = {binaries: close, X-rays: binaries, accretion, accretion disks, novae, cataclysmic variables, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = jun,
       volume = {542},
          eid = {A22},
        pages = {A22},
          doi = {10.1051/0004-6361/201219233},
archivePrefix = {arXiv},
       eprint = {1204.3758},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...542A..22B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{chambers16,
       author = {{Chambers}, K.~C. and {Magnier}, E.~A. and {Metcalfe}, N. and {Flewelling}, H.~A. and {Huber}, M.~E. and {Waters}, C.~Z. and {Denneau}, L. and {Draper}, P.~W. and {Farrow}, D. and {Finkbeiner}, D.~P. and {Holmberg}, C. and {Koppenhoefer}, J. and {Price}, P.~A. and {Rest}, A. and {Saglia}, R.~P. and {Schlafly}, E.~F. and {Smartt}, S.~J. and {Sweeney}, W. and {Wainscoat}, R.~J. and {Burgett}, W.~S. and {Chastel}, S. and {Grav}, T. and {Heasley}, J.~N. and {Hodapp}, K.~W. and {Jedicke}, R. and {Kaiser}, N. and {Kudritzki}, R. -P. and {Luppino}, G.~A. and {Lupton}, R.~H. and {Monet}, D.~G. and {Morgan}, J.~S. and {Onaka}, P.~M. and {Shiao}, B. and {Stubbs}, C.~W. and {Tonry}, J.~L. and {White}, R. and {Ba{\~n}ados}, E. and {Bell}, E.~F. and {Bender}, R. and {Bernard}, E.~J. and {Boegner}, M. and {Boffi}, F. and {Botticella}, M.~T. and {Calamida}, A. and {Casertano}, S. and {Chen}, W. -P. and {Chen}, X. and {Cole}, S. and {Deacon}, N. and {Frenk}, C. and {Fitzsimmons}, A. and {Gezari}, S. and {Gibbs}, V. and {Goessl}, C. and {Goggia}, T. and {Gourgue}, R. and {Goldman}, B. and {Grant}, P. and {Grebel}, E.~K. and {Hambly}, N.~C. and {Hasinger}, G. and {Heavens}, A.~F. and {Heckman}, T.~M. and {Henderson}, R. and {Henning}, T. and {Holman}, M. and {Hopp}, U. and {Ip}, W. -H. and {Isani}, S. and {Jackson}, M. and {Keyes}, C.~D. and {Koekemoer}, A.~M. and {Kotak}, R. and {Le}, D. and {Liska}, D. and {Long}, K.~S. and {Lucey}, J.~R. and {Liu}, M. and {Martin}, N.~F. and {Masci}, G. and {McLean}, B. and {Mindel}, E. and {Misra}, P. and {Morganson}, E. and {Murphy}, D.~N.~A. and {Obaika}, A. and {Narayan}, G. and {Nieto-Santisteban}, M.~A. and {Norberg}, P. and {Peacock}, J.~A. and {Pier}, E.~A. and {Postman}, M. and {Primak}, N. and {Rae}, C. and {Rai}, A. and {Riess}, A. and {Riffeser}, A. and {Rix}, H.~W. and {R{\"o}ser}, S. and {Russel}, R. and {Rutz}, L. and {Schilbach}, E. and {Schultz}, A.~S.~B. and {Scolnic}, D. and {Strolger}, L. and {Szalay}, A. and {Seitz}, S. and {Small}, E. and {Smith}, K.~W. and {Soderblom}, D.~R. and {Taylor}, P. and {Thomson}, R. and {Taylor}, A.~N. and {Thakar}, A.~R. and {Thiel}, J. and {Thilker}, D. and {Unger}, D. and {Urata}, Y. and {Valenti}, J. and {Wagner}, J. and {Walder}, T. and {Walter}, F. and {Watters}, S.~P. and {Werner}, S. and {Wood-Vasey}, W.~M. and {Wyse}, R.},
        title = "{The Pan-STARRS1 Surveys}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = dec,
          eid = {arXiv:1612.05560},
        pages = {arXiv:1612.05560},
archivePrefix = {arXiv},
       eprint = {1612.05560},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016arXiv161205560C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{covey07,
       author = {{Covey}, K.~R. and {Ivezi{\'c}}, {\v{Z}}. and {Schlegel}, D. and {Finkbeiner}, D. and {Padmanabhan}, N. and {Lupton}, R.~H. and {Ag{\"u}eros}, M.~A. and {Bochanski}, J.~J. and {Hawley}, S.~L. and {West}, A.~A. and {Seth}, A. and {Kimball}, A. and {Gogarten}, S.~M. and {Claire}, M. and {Haggard}, D. and {Kaib}, N. and {Schneider}, D.~P. and {Sesar}, B.},
        title = "{Stellar SEDs from 0.3 to 2.5 {\ensuremath{\mu}}m: Tracing the Stellar Locus and Searching for Color Outliers in the SDSS and 2MASS}",
      journal = {\aj},
     keywords = {Galaxy: stellar content, infrared: stars, stars: early-type, stars: late-type, surveys, Astrophysics},
         year = 2007,
        month = dec,
       volume = {134},
       number = {6},
        pages = {2398-2417},
          doi = {10.1086/522052},
archivePrefix = {arXiv},
       eprint = {0707.4473},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007AJ....134.2398C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{li16,
       author = {{Li}, Jing and {Smith}, Martin C. and {Zhong}, Jing and {Hou}, Jinliang and {Carlin}, Jeffrey L. and {Newberg}, Heidi Jo and {Liu}, Chao and {Chen}, Li and {Li}, Linlin and {Shao}, Zhengyi and {Small}, Emma and {Tian}, Hao},
        title = "{Selecting M Giants with Infrared Photometry: Distances, Metallicities, and the Sagittarius Stream}",
      journal = {\apj},
     keywords = {galaxies: individual: Sagittarius, Galaxy: halo, Galaxy: structure, stars: abundances, stars: distances, stars: late-type, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = may,
       volume = {823},
       number = {1},
          eid = {59},
        pages = {59},
          doi = {10.3847/0004-637X/823/1/59},
archivePrefix = {arXiv},
       eprint = {1603.00262},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...823...59L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{wang19,
       author = {{Wang}, Shu and {Chen}, Xiaodian},
        title = "{The Optical to Mid-infrared Extinction Law Based on the APOGEE, Gaia DR2, Pan-STARRS1, SDSS, APASS, 2MASS, and WISE Surveys}",
      journal = {\apj},
     keywords = {dust, extinction, infrared: ISM, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = jun,
       volume = {877},
       number = {2},
          eid = {116},
        pages = {116},
          doi = {10.3847/1538-4357/ab1c61},
archivePrefix = {arXiv},
       eprint = {1904.04575},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...877..116W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%@article{demartino19,
%title = {Hard X-ray cataclysmic variables},
%journal = {Advances in Space Research},
%volume = {66},
%number = {5},
%pages = {1209-1225},
%year = {2020},
%note = {Nova Eruptions, Cataclysmic Variables and Related Systems: Challenges in the 2020 Era},
%issn = {0273-1177},
%doi = {https://doi.org/10.1016/j.asr.2019.09.006},
%url = {https://www.sciencedirect.com/science/article/pii/S0273117719306544},
%author = {D. {de Martino} and F. Bernardini and K. Mukai and M. Falanga and N. Masetti},
%keywords = {X-Rays: binaries, Stars: cataclysmic variables, Accretion, Accretion discs},
%}
@article{lusso12,
    author = {Lusso, E. and Comastri, A. and Simmons, B. D. and Mignoli, M. and Zamorani, G. and Vignali, C. and Brusa, M. and Shankar, F. and Lutz, D. and Trump, J. R. and Maiolino, R. and Gilli, R. and Bolzonella, M. and Puccetti, S. and Salvato, M. and Impey, C. D. and Civano, F. and Elvis, M. and Mainieri, V. and Silverman, J. D. and Koekemoer, A. M. and Bongiorno, A. and Merloni, A. and Berta, S. and Le Floc'h, E. and Magnelli, B. and Pozzi, F. and Riguccini, L.},
    title = "{Bolometric luminosities and Eddington ratios of X-ray selected active galactic nuclei in the XMM-COSMOS survey}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {425},
    number = {1},
    pages = {623-640},
    year = {2012},
    month = {09},
    issn = {0035-8711},
    doi = {10.1111/j.1365-2966.2012.21513.x},
    url = {https://doi.org/10.1111/j.1365-2966.2012.21513.x},
    eprint = {https://academic.oup.com/mnras/article-pdf/425/1/623/3222140/425-1-623.pdf},
}

@ARTICLE{brown21,
       author = {{Brown}, A.~G.~A. and {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and {Biermann}, M. and {Creevey}, O.~L. and {Evans}, D.~W. and {Eyer}, L. and {Hutton}, A. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Soubiran}, C. and {Walton}, N.~A. and {Arenou}, F. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Cropper}, M. and {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {van Leeuwen}, F. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {De Angeli}, F. and {Ducourant}, C. and {Fabricius}, C. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Guerra}, R. and {Guerrier}, A. and {Guiraud}, J. and {Jean-Antoine Piccolo}, A. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nicolas}, C. and {Nienartowicz}, K. and {Pailler}, F. and {Panuzzo}, P. and {Riclet}, F. and {Roux}, W. and {Seabroke}, G.~M. and {Sordo}, R. and {Tanga}, P. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Portell}, J. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Brugaletta}, E. and {Burgess}, P.~W. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Cheek}, N. and {Clementini}, G. and {Damerdji}, Y. and {Davidson}, M. and {Delchambre}, L. and {Dell'Oro}, A. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Galluccio}, L. and {Garc{\'\i}a-Lario}, P. and {Garcia-Reinaldos}, M. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gosset}, E. and {Haigron}, R. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hatzidimitriou}, D. and {Heiter}, U. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Holl}, B. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jordan}, S. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {L{\"o}ffler}, W. and {Lorca}, A. and {Manteiga}, M. and {Marchal}, O. and {Marrese}, P.~M. and {Moitinho}, A. and {Mora}, A. and {Muinonen}, K. and {Osborne}, P. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Richards}, P.~J. and {Riello}, M. and {Rimoldini}, L. and {Robin}, A.~C. and {Roegiers}, T. and {Rybizki}, J. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {Ulla}, A. and {Utrilla}, E. and {van Leeuwen}, M. and {van Reeven}, W. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aerts}, C. and {Aguado}, J.~J. and {Ajaj}, M. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {{\'A}lvarez Cid-Fuentes}, J. and {Alves}, J. and {Anderson}, R.~I. and {Anglada Varela}, E. and {Antoja}, T. and {Audard}, M. and {Baines}, D. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balbinot}, E. and {Balog}, Z. and {Barache}, C. and {Barbato}, D. and {Barros}, M. and {Barstow}, M.~A. and {Bartolom{\'e}}, S. and {Bassilana}, J. -L. and {Bauchet}, N. and {Baudesson-Stella}, A. and {Becciani}, U. and {Bellazzini}, M. and {Bernet}, M. and {Bertone}, S. and {Bianchi}, L. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Bombrun}, A. and {Bossini}, D. and {Bouquillon}, S. and {Bragaglia}, A. and {Bramante}, L. and {Breedt}, E. and {Bressan}, A. and {Brouillet}, N. and {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {C{\'a}novas}, H. and {Cantat-Gaudin}, T. and {Carballo}, R. and {Carlucci}, T. and {Carnerero}, M.~I. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Castro Sampol}, P. and {Chaoul}, L. and {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cioni}, M. -R.~L. and {Comoretto}, G. and {Cooper}, W.~J. and {Cornez}, T. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Dapergolas}, A. and {David}, M. and {David}, P. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {De Ridder}, J. and {de Souza}, R. and {de Teodoro}, P. and {de Torres}, A. and {del Peloso}, E.~F. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {Delisle}, J. -B. and {Di Matteo}, P. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Eappachen}, D. and {Edvardsson}, B. and {Enke}, H. and {Esquej}, P. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Fedorets}, G. and {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Fouron}, C. and {Fragkoudi}, F. and {Fraile}, E. and {Franke}, F. and {Gai}, M. and {Garabato}, D. and {Garcia-Gutierrez}, A. and {Garc{\'\i}a-Torres}, M. and {Garofalo}, A. and {Gavras}, P. and {Gerlach}, E. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomel}, R. and {Gomez}, A. and {Gonzalez-Santamaria}, I. and {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Hauser}, M. and {Haywood}, M. and {Helmi}, A. and {Hidalgo}, S.~L. and {Hilger}, T. and {H{\l}adczuk}, N. and {Hobbs}, D. and {Holland}, G. and {Huckle}, H.~E. and {Jasniewicz}, G. and {Jonker}, P.~G. and {Juaristi Campillo}, J. and {Julbe}, F. and {Karbevska}, L. and {Kervella}, P. and {Khanna}, S. and {Kochoska}, A. and {Kontizas}, M. and {Kordopatis}, G. and {Korn}, A.~J. and {Kostrzewa-Rutkowska}, Z. and {Kruszy{\'n}ska}, K. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Le Campion}, J. -F. and {Le Fustec}, Y. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {Madrero Pardo}, P. and {Managau}, S. and {Mann}, R.~G. and {Marchant}, J.~M. and {Marconi}, M. and {Marcos Santos}, M.~M.~S. and {Marinoni}, S. and {Marocco}, F. and {Marshall}, D.~J. and {Martin Polo}, L. and {Mart{\'\i}n-Fleitas}, J.~M. and {Masip}, A. and {Massari}, D. and {Mastrobuono-Battisti}, A. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Mints}, A. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and {Mulone}, A.~F. and {Munoz}, D. and {Muraveva}, T. and {Murphy}, C.~P. and {Musella}, I. and {Noval}, L. and {Ord{\'e}novic}, C. and {Orr{\`u}}, G. and {Osinde}, J. and {Pagani}, C. and {Pagano}, I. and {Palaversa}, L. and {Palicio}, P.~A. and {Panahi}, A. and {Pawlak}, M. and {Pe{\~n}alosa Esteller}, X. and {Penttil{\"a}}, A. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Poretti}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rainer}, M. and {Raiteri}, C.~M. and {Rambaux}, N. and {Ramos}, P. and {Ramos-Lerate}, M. and {Re Fiorentin}, P. and {Regibo}, S. and {Reyl{\'e}}, C. and {Ripepi}, V. and {Riva}, A. and {Rixon}, G. and {Robichon}, N. and {Robin}, C. and {Roelens}, M. and {Rohrbasser}, L. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Rybicki}, K.~A. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, A. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Samaras}, N. and {Sanchez Gimenez}, V. and {Sanna}, N. and {Santove{\~n}a}, R. and {Sarasso}, M. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Semeux}, D. and {Shahaf}, S. and {Siddiqui}, H.~I. and {Siebert}, A. and {Siltala}, L. and {Slezak}, E. and {Smart}, R.~L. and {Solano}, E. and {Solitro}, F. and {Souami}, D. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {S{\"u}veges}, M. and {Szabados}, L. and {Szegedi-Elek}, E. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Thuillot}, W. and {Tonello}, N. and {Torra}, F. and {Torra}, J. and {Turon}, C. and {Unger}, N. and {Vaillant}, M. and {van Dillen}, E. and {Vanel}, O. and {Vecchiato}, A. and {Viala}, Y. and {Vicente}, D. and {Voutsinas}, S. and {Weiler}, M. and {Wevers}, T. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {Yvard}, P. and {Zhao}, H. and {Zorec}, J. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T.},
        title = "{Gaia Early Data Release 3. Summary of the contents and survey properties}",
      journal = {\aap},
     keywords = {catalogs, astrometry, parallaxes, proper motions, techniques: photometric, techniques: radial velocities, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = may,
       volume = {649},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/202039657},
archivePrefix = {arXiv},
       eprint = {2012.01533},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...649A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@article{bar2019,
       author = {{B{\"a}r}, Rudolf E. and {Trakhtenbrot}, Benny and {Oh}, Kyuseok and {Koss}, Michael J. and {Wong}, O. Ivy and {Ricci}, Claudio and {Schawinski}, Kevin and {Weigel}, Anna K. and {Sartori}, Lia F. and {Ichikawa}, Kohei and {Secrest}, Nathan J. and {Stern}, Daniel and {Pacucci}, Fabio and {Mushotzky}, Richard and {Powell}, Meredith C. and {Ricci}, Federica and {Sani}, Eleonora and {Smith}, Krista L. and {Harrison}, Fiona A. and {Lamperti}, Isabella and {Urry}, C. Megan},
        title = "{BAT AGN Spectroscopic Survey - XIII. The nature of the most luminous obscured AGN in the low-redshift universe}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: nuclei, galaxies: Seyfert, radio continuum: galaxies, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = nov,
       volume = {489},
       number = {3},
        pages = {3073-3092},
          doi = {10.1093/mnras/stz2309},
archivePrefix = {arXiv},
       eprint = {1908.07546},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.489.3073B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
     
}


@ARTICLE{onori21,
       author = {{Onori}, F. and {Fiocchi}, M. and {Masetti}, N. and {Rojas}, A.~F. and {Bazzano}, A. and {Bassani}, L. and {Bird}, A.~J.},
        title = "{Multiwavelength observations of the Galactic X-ray binaries IGR J20155+3827 and Swift J1713.4-4219}",
      journal = {\mnras},
     keywords = {radiation mechanisms: non-thermal, stars: individual: IGR J20155+3827, Swift J1713.4-4219, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = may,
       volume = {503},
       number = {1},
        pages = {472-483},
          doi = {10.1093/mnras/stab315},
archivePrefix = {arXiv},
       eprint = {2102.01638},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.503..472O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{hackstein15,
       author = {{Hackstein}, M. and {Fein}, Ch. and {Haas}, M. and {Ramolla}, M. and {Pozo Nu{\~n}ez}, F. and {Barr Dom{\'\i}nguez}, A. and {Kaderhandt}, L. and {Thomsch}, K. and {Niedworok}, N. and {Westhues}, Ch. and {Chini}, R.},
        title = "{The Bochum Survey of the Southern Galactic Disk: II. Follow-up measurements and multi-filter photometry for 1323 square degrees monitored in 2010 - 2015}",
      journal = {Astronomische Nachrichten},
     keywords = {surveys, stars: variables: general, techniques: photometric, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = aug,
       volume = {336},
       number = {6},
        pages = {590-603},
          doi = {10.1002/asna.201512195},
archivePrefix = {arXiv},
       eprint = {1508.01701},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015AN....336..590H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{krivonos12,
       author = {{Krivonos}, R. and {Tsygankov}, S. and {Lutovinov}, A. and {Revnivtsev}, M. and {Churazov}, E. and {Sunyaev}, R.},
        title = "{INTEGRAL/IBIS nine-year Galactic hard X-ray survey}",
      journal = {\aap},
     keywords = {surveys, X-rays: general, catalogs, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = sep,
       volume = {545},
          eid = {A27},
        pages = {A27},
          doi = {10.1051/0004-6361/201219617},
archivePrefix = {arXiv},
       eprint = {1205.3941},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...545A..27K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{paliya19,
       author = {{Paliya}, Vaidehi S. and {Koss}, M. and {Trakhtenbrot}, B. and {Ricci}, C. and {Oh}, K. and {Ajello}, M. and {Stern}, D. and {Powell}, M.~C. and {Urry}, C.~M. and {Harrison}, F. and {Lamperti}, I. and {Mushotzky}, R. and {Marcotulli}, L. and {Mej{\'\i}a-Restrepo}, J. and {Hartmann}, D.},
        title = "{BAT AGN Spectroscopic Survey. XVI. General Physical Characteristics of BAT Blazars}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: jets, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = aug,
       volume = {881},
       number = {2},
          eid = {154},
        pages = {154},
          doi = {10.3847/1538-4357/ab2f8b},
archivePrefix = {arXiv},
       eprint = {1907.01082},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...881..154P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{chen20,
	doi = {10.3847/1538-4365/ab9cae},
	url = {https://doi.org/10.3847/1538-4365/ab9cae},
	year = 2020,
	month = {jul},
	publisher = {American Astronomical Society},
	volume = {249},
	number = {1},
	pages = {18},
	author = {Xiaodian Chen and Shu Wang and Licai Deng and Richard de Grijs and Ming Yang and Hao Tian},
	title = {The Zwicky Transient Facility Catalog of Periodic Variable Stars},
	journal = {\apjs}

}


@ARTICLE{saxton08,
       author = {{Saxton}, R.~D. and {Read}, A.~M. and {Esquej}, P. and {Freyberg}, M.~J. and {Altieri}, B. and {Bermejo}, D.},
        title = "{The first XMM-Newton slew survey catalogue: XMMSL1}",
      journal = {\aap},
     keywords = {X-rays: general, surveys, catalogs, Astrophysics},
         year = 2008,
        month = mar,
       volume = {480},
       number = {2},
        pages = {611-622},
          doi = {10.1051/0004-6361:20079193},
archivePrefix = {arXiv},
       eprint = {0801.3732},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...480..611S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{baumgartner13,
       author = {{Baumgartner}, W.~H. and {Tueller}, J. and {Markwardt}, C.~B. and {Skinner}, G.~K. and {Barthelmy}, S. and {Mushotzky}, R.~F. and {Evans}, P.~A. and {Gehrels}, N.},
        title = "{The 70 Month Swift-BAT All-sky Hard X-Ray Survey}",
      journal = {\apjs},
     keywords = {catalogs, surveys, X-rays: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = aug,
       volume = {207},
       number = {2},
          eid = {19},
        pages = {19},
          doi = {10.1088/0067-0049/207/2/19},
archivePrefix = {arXiv},
       eprint = {1212.3336},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJS..207...19B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oh18,
       author = {{Oh}, Kyuseok and {Koss}, Michael and {Markwardt}, Craig B. and {Schawinski}, Kevin and {Baumgartner}, Wayne H. and {Barthelmy}, Scott D. and {Cenko}, S. Bradley and {Gehrels}, Neil and {Mushotzky}, Richard and {Petulante}, Abigail and {Ricci}, Claudio and {Lien}, Amy and {Trakhtenbrot}, Benny},
        title = "{The 105-Month Swift-BAT All-sky Hard X-Ray Survey}",
      journal = {\apjs},
     keywords = {catalogs, surveys, X-rays: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = mar,
       volume = {235},
       number = {1},
          eid = {4},
        pages = {4},
          doi = {10.3847/1538-4365/aaa7fd},
archivePrefix = {arXiv},
       eprint = {1801.01882},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..235....4O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{predehl95,
       author = {{Predehl}, P. and {Schmitt}, J.~H.~M.~M.},
        title = "{X-raying the interstellar medium: ROSAT observations of dust scattering halos.}",
      journal = {\aap},
     keywords = {INTERSTELLAR MEDIUM: DUST, ISM: CAS A, X-RAYS: ISM},
         year = 1995,
        month = jan,
       volume = {500},
        pages = {459-475},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995A&A...293..889P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{smith07,
       author = {{Smith}, Randall K. and {Bautz}, Mark W. and {Edgar}, Richard J. and {Fujimoto}, Ryuichi and {Hamaguchi}, Kenji and {Hughes}, John P. and {Ishida}, Manabu and {Kelley}, Richard and {Kilbourne}, Caroline A. and {Kuntz}, K.~D. and {McCammon}, Dan and {Miller}, Eric and {Mitsuda}, Kazuhisa and {Mukai}, Koji and {Plucinsky}, Paul P. and {Porter}, F. Scott and {Snowden}, Steve L. and {Takei}, Yoh and {Terada}, Yukikatsu and {Tsuboi}, Yohko and {Yamasaki}, Noriko Y.},
        title = "{Suzaku Observations of the Local and Distant Hot ISM}",
      journal = {\pasj},
     keywords = {ISM: bubbles, plasmas, X-rays: ISM, Astrophysics},
         year = 2007,
        month = jan,
       volume = {59},
        pages = {141-150},
          doi = {10.1093/pasj/59.sp1.S141},
archivePrefix = {arXiv},
       eprint = {astro-ph/0609832},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007PASJ...59S.141S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mukai16,
       author = {{Mukai}, K. and {Luna}, G.~J.~M. and {Cusumano}, G. and {Segreto}, A. and {Munari}, U. and {Sokoloski}, J.~L. and {Lucy}, A.~B. and {Nelson}, T. and {Nu{\~n}ez}, N.~E.},
        title = "{SU Lyncis, a hard X-ray bright M giant: clues point to a large hidden population of symbiotic stars}",
      journal = {\mnras},
     keywords = {binaries: symbiotic, stars: individual: SU Lyn, X-rays: binaries, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = sep,
       volume = {461},
       number = {1},
        pages = {L1-L5},
          doi = {10.1093/mnrasl/slw087},
archivePrefix = {arXiv},
       eprint = {1604.08483},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.461L...1M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{masetti07,
       author = {{Masetti}, N. and {Landi}, R. and {Pretorius}, M.~L. and {Sguera}, V. and {Bird}, A.~J. and {Perri}, M. and {Charles}, P.~A. and {Kennea}, J.~A. and {Malizia}, A. and {Ubertini}, P.},
        title = "{IGR J16194-2810: a new symbiotic X-ray binary}",
      journal = {\aap},
     keywords = {astrometry, stars: binaries: general, X-rays: binaries, stars: neutron, stars: individual: IGR J16194-2810, Astrophysics},
         year = 2007,
        month = jul,
       volume = {470},
       number = {1},
        pages = {331-337},
          doi = {10.1051/0004-6361:20077509},
archivePrefix = {arXiv},
       eprint = {0704.3682},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&A...470..331M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{paizis06,
       author = {{Paizis}, A. and {Farinelli}, R. and {Titarchuk}, L. and {Courvoisier}, T.~J. -L. and {Bazzano}, A. and {Beckmann}, V. and {Frontera}, F. and {Goldoni}, P. and {Kuulkers}, E. and {Mereghetti}, S. and {Rodriguez}, J. and {Vilhu}, O.},
        title = "{Average hard X-ray emission from NS LMXBs: observational evidence of different spectral states in NS LMXBs}",
      journal = {\aap},
     keywords = {X-rays: binaries, binaries: close, stars: neutron, Astrophysics},
         year = 2006,
        month = nov,
       volume = {459},
       number = {1},
        pages = {187-197},
          doi = {10.1051/0004-6361:20065792},
archivePrefix = {arXiv},
       eprint = {astro-ph/0607592},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006A&A...459..187P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{danehkar21,
       author = {{Danehkar}, A. and {Karovska}, M. and {Drake}, J.~J. and {Kashyap}, V.~L.},
        title = "{Long-term X-ray variability of the symbiotic system RT Cru based on Chandra spectroscopy}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, binaries: symbiotic, stars: individual: (RT Cru), Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = feb,
       volume = {500},
       number = {4},
        pages = {4801-4817},
          doi = {10.1093/mnras/staa3554},
archivePrefix = {arXiv},
       eprint = {2011.07390},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.500.4801D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{gualandi01,
       author = {{Gualandi}, R. \& {Merighi}, R.},
        title = "{Bologna Astronomical Observatory Technical Report, v2.0}",
         year = 2001

}


@ARTICLE{vernet11,
       author = {{Vernet}, J. and {Dekker}, H. and {D'Odorico}, S. and {Kaper}, L. and {Kjaergaard}, P. and {Hammer}, F. and {Randich}, S. and {Zerbi}, F. and {Groot}, P.~J. and {Hjorth}, J. and {Guinouard}, I. and {Navarro}, R. and {Adolfse}, T. and {Albers}, P.~W. and {Amans}, J. -P. and {Andersen}, J.~J. and {Andersen}, M.~I. and {Binetruy}, P. and {Bristow}, P. and {Castillo}, R. and {Chemla}, F. and {Christensen}, L. and {Conconi}, P. and {Conzelmann}, R. and {Dam}, J. and {de Caprio}, V. and {de Ugarte Postigo}, A. and {Delabre}, B. and {di Marcantonio}, P. and {Downing}, M. and {Elswijk}, E. and {Finger}, G. and {Fischer}, G. and {Flores}, H. and {Fran{\c{c}}ois}, P. and {Goldoni}, P. and {Guglielmi}, L. and {Haigron}, R. and {Hanenburg}, H. and {Hendriks}, I. and {Horrobin}, M. and {Horville}, D. and {Jessen}, N.~C. and {Kerber}, F. and {Kern}, L. and {Kiekebusch}, M. and {Kleszcz}, P. and {Klougart}, J. and {Kragt}, J. and {Larsen}, H.~H. and {Lizon}, J. -L. and {Lucuix}, C. and {Mainieri}, V. and {Manuputy}, R. and {Martayan}, C. and {Mason}, E. and {Mazzoleni}, R. and {Michaelsen}, N. and {Modigliani}, A. and {Moehler}, S. and {M{\o}ller}, P. and {Norup S{\o}rensen}, A. and {N{\o}rregaard}, P. and {P{\'e}roux}, C. and {Patat}, F. and {Pena}, E. and {Pragt}, J. and {Reinero}, C. and {Rigal}, F. and {Riva}, M. and {Roelfsema}, R. and {Royer}, F. and {Sacco}, G. and {Santin}, P. and {Schoenmaker}, T. and {Spano}, P. and {Sweers}, E. and {Ter Horst}, R. and {Tintori}, M. and {Tromp}, N. and {van Dael}, P. and {van der Vliet}, H. and {Venema}, L. and {Vidali}, M. and {Vinther}, J. and {Vola}, P. and {Winters}, R. and {Wistisen}, D. and {Wulterkens}, G. and {Zacchei}, A.},
        title = "{X-shooter, the new wide band intermediate resolution spectrograph at the ESO Very Large Telescope}",
      journal = {\aap},
     keywords = {instrumentation: spectrographs, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = dec,
       volume = {536},
          eid = {A105},
        pages = {A105},
          doi = {10.1051/0004-6361/201117752},
archivePrefix = {arXiv},
       eprint = {1110.1944},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...536A.105V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{landi09,
       author = {{Landi}, R. and {Bassani}, L. and {Dean}, A.~J. and {Bird}, A.~J. and {Fiocchi}, M. and {Bazzano}, A. and {Nousek}, J.~A. and {Osborne}, J.~P.},
        title = "{INTEGRAL/IBIS and Swift/XRT observations of hard cataclysmic variables}",
      journal = {\mnras},
     keywords = {novae, cataclysmic variables, gamma-rays: observations, X-rays: binaries, Astrophysics},
         year = 2009,
        month = jan,
       volume = {392},
       number = {2},
        pages = {630-640},
          doi = {10.1111/j.1365-2966.2008.14086.x},
archivePrefix = {arXiv},
       eprint = {0810.1844},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.392..630L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@BOOK{lang92,
       author = {{Lang}, Kenneth R.},
        title = "{Astrophysical Data I. Planets and Stars.}",
         year = 1992,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992adps.book.....L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bodaghee12,
       author = {{Bodaghee}, A. and {Tomsick}, J.~A. and {Rodriguez}, J. and {James}, J.~B.},
        title = "{Clustering between High-mass X-Ray Binaries and OB Associations in the Milky Way}",
      journal = {\apj},
     keywords = {Galaxy: stellar content, open clusters and associations: general, stars: massive, stars: neutron, supergiants, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = jan,
       volume = {744},
       number = {2},
          eid = {108},
        pages = {108},
          doi = {10.1088/0004-637X/744/2/108},
archivePrefix = {arXiv},
       eprint = {1109.3466},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...744..108B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{ducati01,
       author = {{Ducati}, Jorge R. and {Bevilacqua}, Claudio M. and {Rembold}, Sandro B. and {Ribeiro}, Daiana},
        title = "{Intrinsic Colors of Stars in the Near-Infrared}",
      journal = {\apj},
     keywords = {Infrared: Stars, Stars: Fundamental Parameters, Techniques: Photometric},
         year = 2001,
        month = sep,
       volume = {558},
       number = {1},
        pages = {309-322},
          doi = {10.1086/322439},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...558..309D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{schlafly11,
       author = {{Schlafly}, Edward F. and {Finkbeiner}, Douglas P.},
        title = "{Measuring Reddening with Sloan Digital Sky Survey Stellar Spectra and Recalibrating SFD}",
      journal = {\apj},
     keywords = {dust, extinction, Galaxy: stellar content, ISM: clouds, Astrophysics - Galaxy Astrophysics},
         year = 2011,
        month = aug,
       volume = {737},
       number = {2},
          eid = {103},
        pages = {103},
          doi = {10.1088/0004-637X/737/2/103},
archivePrefix = {arXiv},
       eprint = {1012.4804},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...737..103S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{skrutskie06,
       author = {{Skrutskie}, M.~F. and {Cutri}, R.~M. and {Stiening}, R. and {Weinberg}, M.~D. and {Schneider}, S. and {Carpenter}, J.~M. and {Beichman}, C. and {Capps}, R. and {Chester}, T. and {Elias}, J. and {Huchra}, J. and {Liebert}, J. and {Lonsdale}, C. and {Monet}, D.~G. and {Price}, S. and {Seitzer}, P. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and {Gizis}, J.~E. and {Howard}, E. and {Evans}, T. and {Fowler}, J. and {Fullmer}, L. and {Hurt}, R. and {Light}, R. and {Kopan}, E.~L. and {Marsh}, K.~A. and {McCallon}, H.~L. and {Tam}, R. and {Van Dyk}, S. and {Wheelock}, S.},
        title = "{The Two Micron All Sky Survey (2MASS)}",
      journal = {\aj},
     keywords = {Catalogs, Infrared: General, Surveys},
         year = 2006,
        month = feb,
       volume = {131},
       number = {2},
        pages = {1163-1183},
          doi = {10.1086/498708},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006AJ....131.1163S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{warner95,
       author = {{Warner}, Brian},
        title = "{Cataclysmic variable stars}",
         year = 1995,
       volume = {28},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995cvs..book.....W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{enoto14,
       author = {{Enoto}, Teruaki and {Sasano}, Makoto and {Yamada}, Shin'ya and {Tamagawa}, Toru and {Makishima}, Kazuo and {Pottschmidt}, Katja and {Marcu}, Diana and {Corbet}, Robin H.~D. and {Fuerst}, Felix and {Wilms}, J{\"o}rn},
        title = "{Spectral and Timing Nature of the Symbiotic X-Ray Binary 4U 1954+319: The Slowest Rotating Neutron Star in an X-Ray Binary System}",
      journal = {\apj},
     keywords = {accretion, accretion disks, binaries: symbiotic, magnetic fields, stars: individual: 3A 1954+319 4U 1954+319, stars: neutron, X-rays : binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = may,
       volume = {786},
       number = {2},
          eid = {127},
        pages = {127},
          doi = {10.1088/0004-637X/786/2/127},
archivePrefix = {arXiv},
       eprint = {1404.0134},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...786..127E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{abril20,
       author = {{Abril}, Javier and {Schmidtobreick}, Linda and {Ederoclite}, Alessandro and {L{\'o}pez-Sanjuan}, Carlos},
        title = "{Disentangling cataclysmic variables in Gaia's HR diagram}",
      journal = {\mnras},
     keywords = {Hertzsprung, Russell and colour, magnitude diagrams, novae, cataclysmic variables, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = feb,
       volume = {492},
       number = {1},
        pages = {L40-L44},
          doi = {10.1093/mnrasl/slz181},
archivePrefix = {arXiv},
       eprint = {1912.01531},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.492L..40A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sazonov20,
       author = {{Sazonov}, S. and {Paizis}, A. and {Bazzano}, A. and {Chelovekov}, I. and {Khabibullin}, I. and {Postnov}, K. and {Mereminskiy}, I. and {Fiocchi}, M. and {B{\'e}langer}, G. and {Bird}, A.~J. and {Bozzo}, E. and {Chenevez}, J. and {Santo}, M. Del and {Falanga}, M. and {Farinelli}, R. and {Ferrigno}, C. and {Grebenev}, S. and {Krivonos}, R. and {Kuulkers}, E. and {Lund}, N. and {Sanchez-Fernandez}, C. and {Tarana}, A. and {Ubertini}, P. and {Wilms}, J.},
        title = "{The Galactic LMXB Population and the Galactic Centre Region}",
      journal = {\nar},
     keywords = {X-ray binaries, INTEGRAL observatory, Accretion, Black holes, Neutron stars, Sgr A*, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = jun,
       volume = {88},
          eid = {101536},
        pages = {101536},
          doi = {10.1016/j.newar.2020.101536},
archivePrefix = {arXiv},
       eprint = {2006.05063},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020NewAR..8801536S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{comeron05,
       author = {{Comer{\'o}n}, F. and {Pasquali}, A.},
        title = "{The ionizing star of the North America and Pelican nebulae}",
      journal = {\aap},
     keywords = {ISM: HII regions, ISM: individual objects: NGC 7000, ISM: individual objects: IC 5070, ISM: individual objects: W80},
         year = 2005,
        month = feb,
       volume = {430},
        pages = {541-548},
          doi = {10.1051/0004-6361:20041788},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...430..541C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{reig16,
       author = {{Reig}, P. and {Milonaki}, F.},
        title = "{Accretion regimes in the X-ray pulsar 4U 1901+03}",
      journal = {\aap},
     keywords = {stars: emission-line, Be, X-rays: binaries, stars: neutron, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = oct,
       volume = {594},
          eid = {A45},
        pages = {A45},
          doi = {10.1051/0004-6361/201629200},
archivePrefix = {arXiv},
       eprint = {1608.06118},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...594A..45R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{negueruela07,
       author = {{Negueruela}, I. and {Schurch}, M.~P.~E.},
        title = "{A search for counterparts to massive X-ray binaries using photometric catalogues}",
      journal = {\aap},
     keywords = {binaries: close, stars: supergiants, X-rays: binaries, stars: emission line, Be, Astrophysics},
         year = 2007,
        month = jan,
       volume = {461},
       number = {2},
        pages = {631-639},
          doi = {10.1051/0004-6361:20066054},
archivePrefix = {arXiv},
       eprint = {astro-ph/0610006},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&A...461..631N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{krivonos21,
       author = {{Krivonos}, Roman A. and {Bird}, Antony J. and {Churazov}, Eugene M. and {Tomsick}, John A. and {Bazzano}, Angela and {Beckmann}, Volker and {B{\'e}langer}, Guillaume and {Bodaghee}, Arash and {Chaty}, Sylvain and {Kuulkers}, Erik and {Lutovinov}, Alexander and {Malizia}, Angela and {Masetti}, Nicola and {Mereminskiy}, Ilya A. and {Sunyaev}, Rashid and {Tsygankov}, Sergey S. and {Ubertini}, Pietro and {Winkler}, Christoph},
        title = "{15 years of galactic surveys and hard X-ray background measurements}",
      journal = {\nar},
     keywords = {X-ray surveys, Cosmic X-ray background, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = jun,
       volume = {92},
          eid = {101612},
        pages = {101612},
          doi = {10.1016/j.newar.2021.101612},
archivePrefix = {arXiv},
       eprint = {2101.09052},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021NewAR..9201612K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{lutovinov20,
       author = {{Lutovinov}, Alexander and {Suleimanov}, Valery and {Manuel Luna}, Gerardo Juan and {Sazonov}, Sergey and {de Martino}, Domitilla and {Ducci}, Lorenzo and {Doroshenko}, Victor and {Falanga}, Maurizio},
        title = "{INTEGRAL View on cataclysmic variables and symbiotic binaries}",
      journal = {\nar},
     keywords = {Cataclysmic variables, Symbiotic stars, X-Ray, White dwarfs, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = dec,
       volume = {91},
          eid = {101547},
        pages = {101547},
          doi = {10.1016/j.newar.2020.101547},
archivePrefix = {arXiv},
       eprint = {2008.10665},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020NewAR..9101547L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{landi17,
       author = {{Landi}, R. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A.~J. and {Fiocchi}, M. and {Malizia}, A. and {Panessa}, F. and {Sguera}, V. and {Ubertini}, P.},
        title = "{Investigating the X-ray counterparts to unidentified sources in the 1000-orbit INTEGRAL/IBIS catalogue}",
      journal = {\mnras},
     keywords = {gamma-rays: general, X-rays: general, Astrophysics - High Energy Astrophysical Phenomena, High Energy Physics - Phenomenology},
         year = 2017,
        month = sep,
       volume = {470},
       number = {1},
        pages = {1107-1120},
          doi = {10.1093/mnras/stx908},
archivePrefix = {arXiv},
       eprint = {1704.03872},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.470.1107L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{malizia20,
       author = {{Malizia}, Angela and {Sazonov}, Sergey and {Bassani}, Loredana and {Pian}, Elena and {Beckmann}, Volker and {Molina}, Manuela and {Mereminskiy}, Ilya and {Belanger}, Guillaume},
        title = "{INTEGRAL view of AGN}",
      journal = {\nar},
     keywords = {INTEGRAL, AGN, Seyferts, Blazars, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = nov,
       volume = {90},
          eid = {101545},
        pages = {101545},
          doi = {10.1016/j.newar.2020.101545},
archivePrefix = {arXiv},
       eprint = {2009.03232},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020NewAR..9001545M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{kretschmar19,
       author = {{Kretschmar}, Peter and {F{\"u}rst}, Felix and {Sidoli}, Lara and {Bozzo}, Enrico and {Alfonso-Garz{\'o}n}, Julia and {Bodaghee}, Arash and {Chaty}, Sylvain and {Chernyakova}, Masha and {Ferrigno}, Carlo and {Manousakis}, Antonios and {Negueruela}, Ignacio and {Postnov}, Konstantin and {Paizis}, Adamantia and {Reig}, Pablo and {Rodes-Roca}, Jos{\'e} Joaqu{\'\i}n and {Tsygankov}, Sergey and {Bird}, Antony J. and {Bissinger n{\'e} K{\"u}hnel}, Matthias and {Blay}, Pere and {Caballero}, Isabel and {Coe}, Malcolm J. and {Domingo}, Albert and {Doroshenko}, Victor and {Ducci}, Lorenzo and {Falanga}, Maurizio and {Grebenev}, Sergei A. and {Grinberg}, Victoria and {Hemphill}, Paul and {Kreykenbohm}, Ingo and {Kreykenbohm n{\'e} Fritz}, Sonja and {Li}, Jian and {Lutovinov}, Alexander A. and {Mart{\'\i}nez-N{\'u}{\~n}ez}, Silvia and {Mas-Hesse}, J. Miguel and {Masetti}, Nicola and {McBride}, Vanessa A. and {Neronov}, Andrii and {Pottschmidt}, Katja and {Rodriguez}, J{\'e}r{\^o}me and {Romano}, Patrizia and {Rothschild}, Richard E. and {Santangelo}, Andrea and {Sguera}, Vito and {Staubert}, R{\"u}diger and {Tomsick}, John A. and {Torrej{\'o}n}, Jos{\'e} Miguel and {Torres}, Diego F. and {Walter}, Roland and {Wilms}, J{\"o}rn and {Wilson-Hodge}, Colleen A. and {Zhang}, Shu},
        title = "{Advances in Understanding High-Mass X-ray Binaries with INTEGRALand Future Directions}",
      journal = {\nar},
     keywords = {X-rays: binaries, accretion, stars: neutron, pulsars: general, gamma rays: observations, INTEGRAL observatory, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = dec,
       volume = {86},
          eid = {101546},
        pages = {101546},
          doi = {10.1016/j.newar.2020.101546},
archivePrefix = {arXiv},
       eprint = {2009.03244},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019NewAR..8601546K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{eyer19,
       author = {{Eyer}, L. and {Rimoldini}, L. and {Audard}, M. and {Anderson}, R.~I. and {Nienartowicz}, K. and {Glass}, F. and {Marchal}, O. and {Grenon}, M. and {Mowlavi}, N. and {Holl}, B. and {Clementini}, G. and {Aerts}, C. and {Mazeh}, T. and {Evans}, D.~W. and {Szabados}, L. and {Brown}, A.~G.~A. and {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and {Bailer-Jones}, C.~A.~L. and {Biermann}, M. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Siddiqui}, H.~I. and {Soubiran}, C. and {van Leeuwen}, F. and {Walton}, N.~A. and {Arenou}, F. and {Bastian}, U. and {Cropper}, M. and {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {Chaoul}, L. and {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and {Guerra}, R. and {Masana}, E. and {Messineo}, R. and {Panuzzo}, P. and {Portell}, J. and {Riello}, M. and {Seabroke}, G.~M. and {Tanga}, P. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Comoretto}, G. and {Garcia-Reinaldos}, M. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Burgess}, P. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Clotet}, M. and {Creevey}, O. and {Davidson}, M. and {De Ridder}, J. and {Delchambre}, L. and {Dell'Oro}, A. and {Ducourant}, C. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Galluccio}, L. and {Garc{\'\i}a-Torres}, M. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J.~J. and {Gosset}, E. and {Guy}, L.~P. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Hutton}, A. and {Jasniewicz}, G. and {Jean-Antoine-Piccolo}, A. and {Jordan}, S. and {Korn}, A.~J. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {Lebzelter}, T. and {L{\"o}ffler}, W. and {Manteiga}, M. and {Marrese}, P.~M. and {Mart{\'\i}n-Fleitas}, J.~M. and {Moitinho}, A. and {Mora}, A. and {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Richards}, P.~J. and {Robin}, A.~C. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {S{\"u}veges}, M. and {Torra}, J. and {van Reeven}, W. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alvarez}, R. and {Alves}, J. and {Andrei}, A.~H. and {Anglada Varela}, E. and {Antiche}, E. and {Antoja}, T. and {Arcay}, B. and {Astraatmadja}, T.~L. and {Bach}, N. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balm}, P. and {Barache}, C. and {Barata}, C. and {Barbato}, D. and {Barblan}, F. and {Barklem}, P.~S. and {Barrado}, D. and {Barros}, M. and {Barstow}, M.~A. and {Bartholom{\'e} Mu{\~n}oz}, S. and {Bassilana}, J. -L. and {Becciani}, U. and {Bellazzini}, M. and {Berihuete}, A. and {Bertone}, S. and {Bianchi}, L. and {Bienaym{\'e}}, O. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Boeche}, C. and {Bombrun}, A. and {Borrachero}, R. and {Bossini}, D. and {Bouquillon}, S. and {Bourda}, G. and {Bragaglia}, A. and {Bramante}, L. and {Breddels}, M.~A. and {Bressan}, A. and {Brouillet}, N. and {Br{\"u}semeister}, T. and {Brugaletta}, E. and {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {Cannizzaro}, G. and {Cantat-Gaudin}, T. and {Carballo}, R. and {Carlucci}, T. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cocozza}, G. and {Costigan}, G. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and {Crowley}, C. and {Cuypers}, J. and {Dafonte}, C. and {Damerdji}, Y. and {Dapergolas}, A. and {David}, P. and {David}, M. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {de Martino}, D. and {de Souza}, R. and {de Torres}, A. and {Debosscher}, J. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Drazinos}, P. and {Dur{\'a}n}, J. and {Edvardsson}, B. and {Enke}, H. and {Eriksson}, K. and {Esquej}, P. and {Eynard Bontemps}, G. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Falc{\~a}o}, A.~J. and {Farr{\`a}s Casas}, M. and {Federici}, L. and {Fedorets}, G. and {Fernique}, P. and {Figueras}, F. and {Filippi}, F. and {Findeisen}, K. and {Fonti}, A. and {Fraile}, E. and {Fraser}, M. and {Fr{\'e}zouls}, B. and {Gai}, M. and {Galleti}, S. and {Garabato}, D. and {Garc{\'\i}a-Sedano}, F. and {Garofalo}, A. and {Garralda}, N. and {Gavel}, A. and {Gavras}, P. and {Gerssen}, J. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomes}, M. and {Granvik}, M. and {Gueguen}, A. and {Guerrier}, A. and {Guiraud}, J. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Haigron}, R. and {Hatzidimitriou}, D. and {Hauser}, M. and {Haywood}, M. and {Heiter}, U. and {Helmi}, A. and {Heu}, J. and {Hilger}, T. and {Hobbs}, D. and {Hofmann}, W. and {Holland}, G. and {Huckle}, H.~E. and {Hypki}, A. and {Icardi}, V. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jonker}, P.~G. and {Juh{\'a}sz}, {\'A}. L. and {Julbe}, F. and {Karampelas}, A. and {Kewley}, A. and {Klar}, J. and {Kochoska}, A. and {Kohley}, R. and {Kolenberg}, K. and {Kontizas}, M. and {Kontizas}, E. and {Koposov}, S.~E. and {Kordopatis}, G. and {Kostrzewa-Rutkowska}, Z. and {Koubsky}, P. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Lavigne}, J. -B. and {Le Fustec}, Y. and {Le Poncin-Lafitte}, C. and {Lebreton}, Y. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Lenhardt}, H. and {Leroux}, F. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {L{\'o}pez}, M. and {Lorenz}, D. and {Managau}, S. and {Mann}, R.~G. and {Mantelet}, G. and {Marchant}, J.~M. and {Marconi}, M. and {Marinoni}, S. and {Marschalk{\'o}}, G. and {Marshall}, D.~J. and {Martino}, M. and {Marton}, G. and {Mary}, N. and {Massari}, D. and {Matijevi{\v{c}}}, G. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morgenthaler}, S. and {Morris}, D. and {Mulone}, A.~F. and {Muraveva}, T. and {Musella}, I. and {Nelemans}, G. and {Nicastro}, L. and {Noval}, L. and {O'Mullane}, W. and {Ord{\'e}novic}, C. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Osborne}, P. and {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and {Palacin}, H. and {Palaversa}, L. and {Panahi}, A. and {Pawlak}, M. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rambaux}, N. and {Ramos-Lerate}, M. and {Regibo}, S. and {Reyl{\'e}}, C. and {Riclet}, F. and {Ripepi}, V. and {Riva}, A. and {Rivard}, A. and {Rixon}, G. and {Roegiers}, T. and {Roelens}, M. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Ruiz-Dern}, L. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Sanna}, N. and {Santana-Ros}, T. and {Sarasso}, M. and {Savietto}, H. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Shih}, I. -C. and {Siltala}, L. and {Silva}, A.~F. and {Smart}, R.~L. and {Smith}, K.~W. and {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {Stoev}, H. and {Suess}, F.~F. and {Surdej}, J. and {Szegedi-Elek}, E. and {Tapiador}, D. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Terrett}, D. and {Teyssandier}, P. and {Thuillot}, W. and {Titarenko}, A. and {Torra Clotet}, F. and {Turon}, C. and {Ulla}, A. and {Utrilla}, E. and {Uzzi}, S. and {Vaillant}, M. and {Valentini}, G. and {Valette}, V. and {van Elteren}, A. and {Van Hemelryck}, E. and {van Leeuwen}, M. and {Vaschetto}, M. and {Vecchiato}, A. and {Veljanoski}, J. and {Viala}, Y. and {Vicente}, D. and {Vogt}, S. and {von Essen}, C. and {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and {Walmsley}, G. and {Weiler}, M. and {Wertz}, O. and {Wevers}, T. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Ziaeepour}, H. and {Zorec}, J. and {Zschocke}, S. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T.},
        title = "{Gaia Data Release 2. Variable stars in the colour-absolute magnitude diagram}",
      journal = {\aap},
     keywords = {stars: general, stars: variables: general, stars: oscillations, binaries: eclipsing, surveys, methods: data analysis, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = mar,
       volume = {623},
          eid = {A110},
        pages = {A110},
          doi = {10.1051/0004-6361/201833304},
archivePrefix = {arXiv},
       eprint = {1804.09382},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...623A.110G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{corbet08,
       author = {{Corbet}, R.~H.~D. and {Sokoloski}, J.~L. and {Mukai}, K. and {Markwardt}, C.~B. and {Tueller}, J.},
        title = "{A Comparison of the Variability of the Symbiotic X-Ray Binaries GX 1+4, 4U 1954+31, and 4U 1700+24 from Swift BAT and RXTE ASM Observations}",
      journal = {\apj},
     keywords = {binaries: symbiotic, stars: individual: GX 1+4 4U 1954+31 4U 1700+24, stars: neutron, X-rays: binaries, Astrophysics},
         year = 2008,
        month = mar,
       volume = {675},
       number = {2},
        pages = {1424-1435},
          doi = {10.1086/526337},
archivePrefix = {arXiv},
       eprint = {0711.1519},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...675.1424C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@inproceedings{landi11,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2011evhe.confE...9L},
	author = {{Landi}, R. and {Bassani}, L. and {Malizia}, A. and {Bazzano}, A. and {Fiocchi}, M. and {Bird}, A.~J.},
	booktitle = {Extreme and Variable High Energy Sky (Extremesky 2011)},
	date-added = {2021-04-28 11:33:31 +0200},
	date-modified = {2021-04-28 11:33:37 +0200},
	eid = {9},
	month = jan,
	pages = {9},
	title = {{Swift/XRT observations of unidentified INTEGRAL/IBIS sources}},
	year = 2011}

@article{westergaard06,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2006ATel..967....1W},
	author = {{Westergaard}, N.~J. and {Budtz-Jorgensen}, C. and {Chenevez}, J. and {Lund}, N. and {Brandt}, S. and {Oxborrow}, C.~A.},
	date-added = {2021-04-28 11:29:17 +0200},
	date-modified = {2021-04-28 11:29:44 +0200},
	journal = {The Astronomer's Telegram},
	keywords = {X-ray, Gamma Ray, Transients},
	month = dec,
	pages = {1},
	title = {{INTEGRAL detection of SWIFT J2037.2+4151}},
	volume = {967},
	year = 2006}

@article{masetti13,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...556A.120M},
	archiveprefix = {arXiv},
	author = {{Masetti}, N. and {Parisi}, P. and {Palazzi}, E. and {Jim{\'e}nez-Bail{\'o}n}, E. and {Chavushyan}, V. and {McBride}, V. and {Rojas}, A.~F. and {Steward}, L. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A.~J. and {Charles}, P.~A. and {Galaz}, G. and {Landi}, R. and {Malizia}, A. and {Mason}, E. and {Minniti}, D. and {Morelli}, L. and {Schiavone}, F. and {Stephen}, J.~B. and {Ubertini}, P.},
	date-added = {2021-04-28 11:28:28 +0200},
	date-modified = {2021-04-28 11:28:37 +0200},
	doi = {10.1051/0004-6361/201322026},
	eid = {A120},
	eprint = {1307.2898},
	journal = {\aap},
	keywords = {galaxies: Seyfert, quasars: emission lines, X-rays: binaries, novae, cataclysmic variables, stars: flare, Astrophysics - High Energy Astrophysical Phenomena},
	month = aug,
	pages = {A120},
	primaryclass = {astro-ph.HE},
	title = {{Unveiling the nature of INTEGRAL objects through optical spectroscopy. X. A new multi-year, multi-observatory campaign}},
	volume = {556},
	year = 2013,
	Bdsk-Url-1 = {https://doi.org/10.1051/0004-6361/201322026}}

@inproceedings{jayasinghe20,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2020AAS...23515403J},
	author = {{Jayasinghe}, T. and {Stanek}, K.~Z. and {Kochanek}, C.~S.},
	booktitle = {American Astronomical Society Meeting Abstracts \#235},
	date-added = {2021-04-28 11:26:14 +0200},
	date-modified = {2021-04-28 11:26:22 +0200},
	eid = {154.03},
	month = jan,
	pages = {154.03},
	series = {American Astronomical Society Meeting Abstracts},
	title = {{The ASAS-SN all-sky catalog of bright variable stars}},
	volume = {235},
	year = 2020}

@article{jayasinghe18,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.477.3145J},
	archiveprefix = {arXiv},
	author = {{Jayasinghe}, T. and {Kochanek}, C.~S. and {Stanek}, K.~Z. and {Shappee}, B.~J. and {Holoien}, T.~W. -S. and {Thompson}, Todd A. and {Prieto}, J.~L. and {Dong}, Subo and {Pawlak}, M. and {Shields}, J.~V. and {Pojmanski}, G. and {Otero}, S. and {Britt}, C.~A. and {Will}, D.},
	date-added = {2021-04-28 11:25:27 +0200},
	date-modified = {2021-04-28 11:25:38 +0200},
	doi = {10.1093/mnras/sty838},
	eprint = {1803.01001},
	journal = {\mnras},
	keywords = {catalogues, surveys, binaries: eclipsing, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics},
	month = jul,
	number = {3},
	pages = {3145-3163},
	primaryclass = {astro-ph.SR},
	title = {{The ASAS-SN catalogue of variable stars I: The Serendipitous Survey}},
	volume = {477},
	year = 2018,
	Bdsk-Url-1 = {https://doi.org/10.1093/mnras/sty838}}

@article{krivonos10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...523A..61K},
	archiveprefix = {arXiv},
	author = {{Krivonos}, R. and {Tsygankov}, S. and {Revnivtsev}, M. and {Grebenev}, S. and {Churazov}, E. and {Sunyaev}, R.},
	date-added = {2021-04-28 11:24:31 +0200},
	date-modified = {2021-04-28 11:24:42 +0200},
	doi = {10.1051/0004-6361/201014935},
	eid = {A61},
	eprint = {1006.4437},
	journal = {\aap},
	keywords = {surveys, X-rays:, general, catalogs, Astrophysics - High Energy Astrophysical Phenomena},
	month = nov,
	pages = {A61},
	primaryclass = {astro-ph.HE},
	title = {{INTEGRAL/IBIS 7-year All-Sky Hard X-Ray Survey. II. Catalog of sources}},
	volume = {523},
	year = 2010,
	Bdsk-Url-1 = {https://doi.org/10.1051/0004-6361/201014935}}

@article{forveille18,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...616E...1F},
	author = {{Forveille}, Thierry and {Kotak}, Rubina and {Shore}, Steve and {Tolstoy}, Eline},
	date-added = {2021-04-22 17:54:58 +0200},
	date-modified = {2021-04-22 17:55:10 +0200},
	doi = {10.1051/0004-6361/201833955},
	eid = {E1},
	journal = {\aap},
	month = aug,
	pages = {E1},
	title = {{Gaia Data Release 2}},
	volume = {616},
	year = 2018,
	Bdsk-Url-1 = {https://doi.org/10.1051/0004-6361/201833955}}

@inproceedings{baumgartner10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2010HEAD...11.1305B},
	author = {{Baumgartner}, Wayne H. and {Tueller}, J. and {Markwardt}, C. and {Skinner}, G.},
	booktitle = {AAS/High Energy Astrophysics Division \#11},
	date-added = {2021-04-22 17:52:28 +0200},
	date-modified = {2021-04-22 17:52:42 +0200},
	eid = {13.05},
	month = mar,
	pages = {13.05},
	series = {AAS/High Energy Astrophysics Division},
	title = {{The Swift-BAT 58 Month Survey}},
	volume = {11},
	year = 2010}

@article{bird16,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJS..223...15B},
	archiveprefix = {arXiv},
	author = {{Bird}, A.~J. and {Bazzano}, A. and {Malizia}, A. and {Fiocchi}, M. and {Sguera}, V. and {Bassani}, L. and {Hill}, A.~B. and {Ubertini}, P. and {Winkler}, C.},
	date-added = {2021-04-22 17:51:31 +0200},
	date-modified = {2021-04-22 17:51:39 +0200},
	doi = {10.3847/0067-0049/223/1/15},
	eid = {15},
	eprint = {1601.06074},
	journal = {\apjs},
	keywords = {Galaxy: general, gamma rays: general, surveys, Astrophysics - High Energy Astrophysical Phenomena},
	month = mar,
	number = {1},
	pages = {15},
	primaryclass = {astro-ph.HE},
	title = {{The IBIS Soft Gamma-Ray Sky after 1000 Integral Orbits}},
	volume = {223},
	year = 2016,
	Bdsk-Url-1 = {https://doi.org/10.3847/0067-0049/223/1/15}}

@article{bailer21,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....161..147B},
	archiveprefix = {arXiv},
	author = {{Bailer-Jones}, C.~A.~L. and {Rybizki}, J. and {Fouesneau}, M. and {Demleitner}, M. and {Andrae}, R.},
	date-added = {2021-04-22 17:47:48 +0200},
	date-modified = {2021-04-22 17:48:04 +0200},
	doi = {10.3847/1538-3881/abd806},
	eid = {147},
	eprint = {2012.05220},
	journal = {\aj},
	keywords = {Catalogs, Galaxy structure, Bayesian statistics, Parallax, Stellar parallax, Photometric parallax, Distance indicators, Astrometry, Markov chain Monte Carlo, Absolute magnitude, 205, 622, 1900, 1197, 1618, 1231, 394, 80, 1889, 10, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
	month = mar,
	number = {3},
	pages = {147},
	primaryclass = {astro-ph.SR},
	title = {{Estimating Distances from Parallaxes. V. Geometric and Photogeometric Distances to 1.47 Billion Stars in Gaia Early Data Release 3}},
	volume = {161},
	year = 2021,
	Bdsk-Url-1 = {https://doi.org/10.3847/1538-3881/abd806}}

@article{molina19,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.484.2735M},
	archiveprefix = {arXiv},
	author = {{Molina}, M. and {Malizia}, A. and {Bassani}, L. and {Ursini}, F. and {Bazzano}, A. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/stz156},
	eprint = {1901.04188},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
	month = apr,
	number = {2},
	pages = {2735-2746},
	primaryclass = {astro-ph.HE},
	title = {{Swift/XRT-NuSTAR spectra of type 1 AGN: confirming INTEGRAL results on the high-energy cut-off}},
	volume = {484},
	year = 2019,
	Bdsk-Url-1 = {https://doi.org/10.1093/mnras/stz156}}

@article{Lubinski_2001,
	author = {Lubinski, P. and Zdziarski, A. A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2001.04481.x},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {May},
	number = {2},
	pages = {L37--L42},
	publisher = {Oxford University Press (OUP)},
	title = {The strength and width of Fe K lines in Seyferts and their correlations with the X-ray slope},
	url = {http://dx.doi.org/10.1046/j.1365-8711.2001.04481.x},
	volume = {323},
	year = {2001},
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2001.04481.x}}

@article{Feng_2014,
	author = {Feng, Hua and Shen, Yue and Li, Hong},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637x/794/1/77},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {Sep},
	number = {1},
	pages = {77},
	publisher = {IOP Publishing},
	title = {SINGLE-EPOCH BLACK HOLE MASS ESTIMATORS FOR BROAD-LINE ACTIVE GALACTIC NUCLEI: RECALIBRATING Hβ WITH A NEW APPROACH},
	url = {http://dx.doi.org/10.1088/0004-637X/794/1/77},
	volume = {794},
	year = {2014},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/794/1/77},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/0004-637x/794/1/77}}

@article{Masetti_2006,
	author = {Masetti, N. and Mason, E. and Bassani, L. and Bird, A. J. and Maiorano, E. and Malizia, A. and Palazzi, E. and Stephen, J. B. and Bazzano, A. and Dean, A. J. and et al.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20054086},
	issn = {1432-0746},
	journal = {Astronomy & Astrophysics},
	month = {Feb},
	number = {2},
	pages = {547--556},
	publisher = {EDP Sciences},
	title = {Unveiling the nature ofINTEGRALobjects through optical spectroscopy},
	url = {http://dx.doi.org/10.1051/0004-6361:20054086},
	volume = {448},
	year = {2006},
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20054086}}

@article{Kaspi_2000,
	author = {Kaspi, Shai and Smith, Paul S. and Netzer, Hagai and Maoz, Dan and Jannuzi, Buell T. and Giveon, Uriel},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/308704},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {Apr},
	number = {2},
	pages = {631--649},
	publisher = {IOP Publishing},
	title = {Reverberation Measurements for 17 Quasars and the Size‐Mass‐Luminosity Relations in Active Galactic Nuclei},
	url = {http://dx.doi.org/10.1086/308704},
	volume = {533},
	year = {2000},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/308704}}

@article{Greene_2005,
	author = {Greene, Jenny E. and Ho, Luis C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/431897},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {Sep},
	number = {1},
	pages = {122--129},
	publisher = {IOP Publishing},
	title = {Estimating Black Hole Masses in Active Galaxies Using the Hα Emission Line},
	url = {http://dx.doi.org/10.1086/431897},
	volume = {630},
	year = {2005},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/431897}}

@article{Grier_2012,
	author = {Grier, C. J. and Peterson, B. M. and Pogge, R. W. and Denney, K. D. and Bentz, M. C. and Martini, Paul and Sergeev, S. G. and Kaspi, S. and Minezaki, T. and Zu, Y. and et al.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637x/755/1/60},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {Jul},
	number = {1},
	pages = {60},
	publisher = {IOP Publishing},
	title = {REVERBERATION MAPPING RESULTS FOR FIVE SEYFERT 1 GALAXIES},
	url = {http://dx.doi.org/10.1088/0004-637X/755/1/60},
	volume = {755},
	year = {2012},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/755/1/60},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/0004-637x/755/1/60}}

@article{Fausnaugh_2017,
	author = {Fausnaugh, M. M. and Grier, C. J. and Bentz, M. C. and Denney, K. D. and Rosa, G. De and Peterson, B. M. and Kochanek, C. S. and Pogge, R. W. and Adams, S. M. and Barth, A. J. and et al.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.3847/1538-4357/aa6d52},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {May},
	number = {2},
	pages = {97},
	publisher = {American Astronomical Society},
	title = {Reverberation Mapping of Optical Emission Lines in Five Active Galaxies},
	url = {http://dx.doi.org/10.3847/1538-4357/aa6d52},
	volume = {840},
	year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.3847/1538-4357/aa6d52}}

@article{Koss_2017,
	author = {Koss, Michael and Trakhtenbrot, Benny and Ricci, Claudio and Lamperti, Isabella and Oh, Kyuseok and Berney, Simon and Schawinski, Kevin and Balokovi{\'c}, Mislav and Baronchelli, Linda and Crenshaw, D. Michael and et al.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.3847/1538-4357/aa8ec9},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {Nov},
	number = {1},
	pages = {74},
	publisher = {American Astronomical Society},
	title = {BAT AGN Spectroscopic Survey. I. Spectral Measurements, Derived Quantities, and AGN Demographics},
	url = {http://dx.doi.org/10.3847/1538-4357/aa8ec9},
	volume = {850},
	year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.3847/1538-4357/aa8ec9}}

@article{Rodriguez_Ardila_2000,
	author = {Rodriguez‐Ardila, Alberto and Pastoriza, Miriani G. and Donzelli, Carlos J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/313293},
	issn = {1538-4365},
	journal = {The Astrophysical Journal Supplement Series},
	month = {Jan},
	number = {1},
	pages = {63--78},
	publisher = {IOP Publishing},
	title = {Visible and Near‐Infrared Spectroscopy of Seyfert 1 and Narrow‐Line Seyfert 1 Galaxies},
	url = {http://dx.doi.org/10.1086/313293},
	volume = {126},
	year = {2000},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/313293}}

@article{Khorunzhev_2012,
	author = {Khorunzhev, G. A. and Sazonov, S. Yu. and Burenin, R. A. and Tkachenko, A. Yu.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1134/s1063773712080026},
	issn = {1562-6873},
	journal = {Astronomy Letters},
	month = {Aug},
	number = {8},
	pages = {475--491},
	publisher = {Pleiades Publishing Ltd},
	title = {Masses and accretion rates of supermassive black holes in active galactic nuclei from the INTEGRAL survey},
	url = {http://dx.doi.org/10.1134/S1063773712080026},
	volume = {38},
	year = {2012},
	Bdsk-Url-1 = {http://dx.doi.org/10.1134/S1063773712080026},
	Bdsk-Url-2 = {http://dx.doi.org/10.1134/s1063773712080026}}

@article{Di_Gesu_2016,
	author = {Di Gesu, L. and Costantini, E.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201628670},
	issn = {1432-0746},
	journal = {Astronomy & Astrophysics},
	month = {Oct},
	pages = {A88},
	publisher = {EDP Sciences},
	title = {The warm absorber in the radio-loud quasar 4C +74.26},
	url = {http://dx.doi.org/10.1051/0004-6361/201628670},
	volume = {594},
	year = {2016},
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201628670}}

@article{Buisson_2018,
	author = {Buisson, D J K and Fabian, A C and Lohfink, A M},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/sty2609},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Sep},
	number = {4},
	pages = {4419--4426},
	publisher = {Oxford University Press (OUP)},
	title = {Coronal temperatures of the AGN ESO 103−035 and IGR 2124.7+5058 from NuSTAR observations},
	url = {http://dx.doi.org/10.1093/mnras/sty2609},
	volume = {481},
	year = {2018},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/sty2609}}

@article{Ricci_2018,
	author = {Ricci, C and Ho, L C and Fabian, A C and Trakhtenbrot, B and Koss, M J and Ueda, Y and Lohfink, A and Shimizu, T and Bauer, F E and Mushotzky, R and et al.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/sty1879},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Jul},
	number = {2},
	pages = {1819--1830},
	publisher = {Oxford University Press (OUP)},
	title = {BAT AGN Spectroscopic Survey -- XII. The relation between coronal properties of active galactic nuclei and the Eddington ratio},
	url = {http://dx.doi.org/10.1093/mnras/sty1879},
	volume = {480},
	year = {2018},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/sty1879}}

@article{Tortosa_2018,
	author = {Tortosa, A. and Bianchi, S. and Marinucci, A. and Matt, G. and Petrucci, P. O.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201732382},
	issn = {1432-0746},
	journal = {Astronomy & Astrophysics},
	month = {Jun},
	pages = {A37},
	publisher = {EDP Sciences},
	title = {A NuSTAR census of coronal parameters in Seyfert galaxies},
	url = {http://dx.doi.org/10.1051/0004-6361/201732382},
	volume = {614},
	year = {2018},
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201732382}}

@article{Kalberla_2005,
	author = {Kalberla, P. M. W. and Burton, W. B. and Hartmann, Dap and Arnal, E. M. and Bajaja, E. and Morras, R. and P{\"o}ppel, W. G. L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20041864},
	issn = {1432-0746},
	journal = {Astronomy & Astrophysics},
	month = {Sep},
	number = {2},
	pages = {775--782},
	publisher = {EDP Sciences},
	title = {The Leiden/Argentine/Bonn (LAB) Survey of Galactic HI},
	url = {http://dx.doi.org/10.1051/0004-6361:20041864},
	volume = {440},
	year = {2005},
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20041864}}

@article{Magdziarz_1995,
	author = {Magdziarz, Pawe{\l} and Zdziarski, Andrzej A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/273.3.837},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Apr},
	number = {3},
	pages = {837--848},
	publisher = {Oxford University Press (OUP)},
	title = {Angle-dependent Compton reflection of X-rays and gamma-rays},
	url = {http://dx.doi.org/10.1093/mnras/273.3.837},
	volume = {273},
	year = {1995},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/273.3.837}}

@article{Lohfink_2017,
	author = {Lohfink, Anne M. and Fabian, Andrew C. and Ballantyne, David R. and Boggs, S. E. and Boorman, Peter and Christensen, F. E. and Craig, W. W. and Farrah, Duncan and Garc{\'\i}a, Javier and Hailey, C. J. and et al.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.3847/1538-4357/aa6d07},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {May},
	number = {2},
	pages = {80},
	publisher = {American Astronomical Society},
	title = {The X-Ray Reflection Spectrum of the Radio-loud Quasar 4C 74.26},
	url = {http://dx.doi.org/10.3847/1538-4357/aa6d07},
	volume = {841},
	year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.3847/1538-4357/aa6d07}}

@article{Ricci_2017,
	author = {Ricci, C. and Trakhtenbrot, B. and Koss, M. J. and Ueda, Y. and Del Vecchio, I. and Treister, E. and Schawinski, K. and Paltani, S. and Oh, K. and Lamperti, I. and et al.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.3847/1538-4365/aa96ad},
	issn = {1538-4365},
	journal = {The Astrophysical Journal Supplement Series},
	month = {Dec},
	number = {2},
	pages = {17},
	publisher = {American Astronomical Society},
	title = {BAT AGN Spectroscopic Survey. V. X-Ray Properties of the Swift/BAT 70-month AGN Catalog},
	url = {http://dx.doi.org/10.3847/1538-4365/aa96ad},
	volume = {233},
	year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.3847/1538-4365/aa96ad}}

@article{Fabian_2017,
	author = {Fabian, A. C. and Lohfink, A. and Belmont, R. and Malzac, J. and Coppi, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/stx221},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Feb},
	number = {3},
	pages = {2566--2570},
	publisher = {Oxford University Press (OUP)},
	title = {Properties of AGN coronae in the NuSTAR era -- II. Hybrid plasma},
	url = {http://dx.doi.org/10.1093/mnras/stx221},
	volume = {467},
	year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stx221}}

@article{Fabian_2015,
	author = {Fabian, A. C. and Lohfink, A. and Kara, E. and Parker, M. L. and Vasudevan, R. and Reynolds, C. S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/stv1218},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Jul},
	number = {4},
	pages = {4375--4383},
	publisher = {Oxford University Press (OUP)},
	title = {Properties of AGN coronae in theNuSTARera},
	url = {http://dx.doi.org/10.1093/mnras/stv1218},
	volume = {451},
	year = {2015},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stv1218}}

@article{Mathur_2000,
	author = {Mathur, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2000.03530.x},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Jun},
	number = {4},
	pages = {L17--L20},
	publisher = {Oxford University Press (OUP)},
	title = {Narrow-line Seyfert 1 galaxies and the evolution of galaxies and active galaxies},
	url = {http://dx.doi.org/10.1046/j.1365-8711.2000.03530.x},
	volume = {314},
	year = {2000},
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2000.03530.x}}

@article{pounds95,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.277L...5P},
	author = {{Pounds}, K.~A. and {Done}, C. and {Osborne}, J.~P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/277.1.L5},
	journal = {\mnras},
	keywords = {ACCRETION, ACCRETION DISCS, GALAXIES: ACTIVE, GALAXIES: INDIVIDUAL: RE 1034+39, GALAXIES: SEYFERT, X-RAYS: GALAXIES},
	month = nov,
	pages = {L5-L10},
	title = {{RE 1034+39: a high-state Seyfert galaxy?}},
	volume = 277,
	year = 1995,
	Bdsk-Url-1 = {https://doi.org/10.1093/mnras/277.1.L5}}

@article{1995,
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/277.1.l5},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Nov},
	publisher = {Oxford University Press (OUP)},
	url = {http://dx.doi.org/10.1093/mnras/277.1.L5},
	year = {1995},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/277.1.L5},
	Bdsk-Url-2 = {http://dx.doi.org/10.1093/mnras/277.1.l5}}

@article{Osterbrock_1985,
	author = {Osterbrock, D. E. and Pogge, R. W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/163513},
	issn = {1538-4357},
	journal = {The Astrophysical Journal},
	month = {Oct},
	pages = {166},
	publisher = {IOP Publishing},
	title = {The spectra of narrow-line Seyfert 1 galaxies},
	url = {http://dx.doi.org/10.1086/163513},
	volume = {297},
	year = {1985},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/163513}}

@article{Malizia_2012,
	author = {Malizia, A. and Bassani, L. and Bazzano, A. and Bird, A. J. and Masetti, N. and Panessa, F. and Stephen, J. B. and Ubertini, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2012.21755.x},
	issn = {0035-8711},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Oct},
	number = {3},
	pages = {1750--1766},
	publisher = {Oxford University Press (OUP)},
	title = {TheINTEGRAL/IBIS AGN catalogue - I. X-ray absorption properties versus optical classification},
	url = {http://dx.doi.org/10.1111/j.1365-2966.2012.21755.x},
	volume = {426},
	year = {2012},
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2012.21755.x}}

@article{Malizia_2016,
	author = {Malizia, A. and Landi, R. and Molina, M. and Bassani, L. and Bazzano, A. and Bird, A. J. and Ubertini, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/stw972},
	issn = {1365-2966},
	journal = {Monthly Notices of the Royal Astronomical Society},
	month = {Apr},
	number = {1},
	pages = {19--29},
	publisher = {Oxford University Press (OUP)},
	title = {The INTEGRAL/IBISAGN catalogue: an update},
	url = {http://dx.doi.org/10.1093/mnras/stw972},
	volume = {460},
	year = {2016},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stw972}}

@article{tombesi15,
	author = {Tombesi, F. and Mel{\'e}ndez, M. and Veilleux, S. and Reeves, J. N. and Gonz{\'a}lez-Alfonso, E. and Reynolds, C. S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1038/nature14261},
	issn = {1476-4687},
	journal = {Nature},
	month = {Mar},
	number = {7544},
	pages = {436--438},
	publisher = {Springer Nature},
	title = {Wind from the black-hole accretion disk driving a molecular outflow in an active galaxy},
	url = {http://dx.doi.org/10.1038/nature14261},
	volume = {519},
	year = {2015},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature14261}}

@article{tombesi10,
	author = {Tombesi, F. and Cappi, M. and Reeves, J. N. and Palumbo, G. G. C. and Yaqoob, T. and Braito, V. and Dadina, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/200913440},
	issn = {1432-0746},
	journal = {Astronomy and Astrophysics},
	month = {Oct},
	pages = {A57},
	publisher = {EDP Sciences},
	title = {Evidence for ultra-fast outflows in radio-quiet AGNs},
	url = {http://dx.doi.org/10.1051/0004-6361/200913440},
	volume = {521},
	year = {2010},
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200913440}}

@article{marconi04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.351..169M},
	author = {{Marconi}, A. and {Risaliti}, G. and {Gilli}, R. and {Hunt}, L.~K. and {Maiolino}, R. and {Salvati}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2004.07765.x},
	eprint = {astro-ph/0311619},
	journal = {\mnras},
	keywords = {black hole physics, galaxies: active, galaxies: evolution, galaxies: nuclei, quasars: general, cosmology: miscellaneous},
	month = jun,
	pages = {169-185},
	title = {{Local supermassive black holes, relics of active galactic nuclei and the X-ray background}},
	volume = 351,
	year = 2004,
	Bdsk-Url-1 = {https://doi.org/10.1111/j.1365-2966.2004.07765.x}}

@article{lohfink15,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...814...24L},
	archiveprefix = {arXiv},
	author = {{Lohfink}, A.~M. and {Ogle}, P. and {Tombesi}, F. and {Walton}, D. and {Balokovi{\'c}}, M. and {Zoghbi}, A. and {Ballantyne}, D.~R. and {Boggs}, S.~E. and {Christensen}, F.~E. and {Craig}, W.~W. and {Fabian}, A.~C. and {Hailey}, C.~J. and {Harrison}, F.~A. and {King}, A.~L. and {Madejski}, G. and {Matt}, G. and {Reynolds}, C.~S. and {Stern}, D. and {Ursini}, F. and {Zhang}, W.~W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/814/1/24},
	eid = {24},
	eprint = {1510.01333},
	journal = {\apj},
	keywords = {galaxies: active, X-rays: individual: 3C 390.3},
	month = nov,
	pages = {24},
	primaryclass = {astro-ph.HE},
	title = {{The Corona of the Broad-line Radio Galaxy 3C 390.3}},
	volume = 814,
	year = 2015,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/814/1/24}}

@article{brenneman14,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...788...61B},
	archiveprefix = {arXiv},
	author = {{Brenneman}, L.~W. and {Madejski}, G. and {Fuerst}, F. and {Matt}, G. and {Elvis}, M. and {Harrison}, F.~A. and {Ballantyne}, D.~R. and {Boggs}, S.~E. and {Christensen}, F.~E. and {Craig}, W.~W. and {Fabian}, A.~C. and {Grefenstette}, B.~W. and {Hailey}, C.~J. and {Madsen}, K.~K. and {Marinucci}, A. and {Rivers}, E. and {Stern}, D. and {Walton}, D.~J. and {Zhang}, W.~W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/788/1/61},
	eid = {61},
	eprint = {1404.7486},
	journal = {\apj},
	keywords = {accretion, accretion disks, galaxies: active, galaxies: individual: IC 4329A, galaxies: nuclei, galaxies: Seyfert, X-rays: galaxies},
	month = jun,
	pages = {61},
	primaryclass = {astro-ph.HE},
	title = {{The Broad-band X-Ray Spectrum of IC 4329A from a Joint NuSTAR/Suzaku Observation}},
	volume = 788,
	year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/788/1/61}}

@article{titarchuk95,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...450..876T},
	author = {{Titarchuk}, L. and {Lyubarskij}, Y.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/176191},
	journal = {\apj},
	keywords = {PLASMAS, RADIATION MECHANISMS: THERMAL, RADIATIVE TRANSFER, SCATTERING},
	month = sep,
	pages = {876},
	title = {{Power-Law Spectra as a Result of Comptonization of the Soft Radiation in a Plasma Cloud}},
	volume = 450,
	year = 1995,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/176191}}

@article{marinucci15,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.447..160M},
	archiveprefix = {arXiv},
	author = {{Marinucci}, A. and {Matt}, G. and {Bianchi}, S. and {Lu}, T.~N. and {Arevalo}, P. and {Balokovi{\'c}}, M. and {Ballantyne}, D. and {Bauer}, F.~E. and {Boggs}, S.~E. and {Christensen}, F.~E. and {Craig}, W.~W. and {Gandhi}, P. and {Hailey}, C.~J. and {Harrison}, F. and {Puccetti}, S. and {Rivers}, E. and {Walton}, D.~J. and {Stern}, D. and {Zhang}, W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/stu2439},
	eprint = {1411.5151},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: individual: NGC 2110, galaxies: Seyfert},
	month = feb,
	pages = {160-167},
	primaryclass = {astro-ph.HE},
	title = {{The Seyfert 2 galaxy NGC 2110: hard X-ray emission observed by NuSTAR and variability of the iron K{$\alpha$} line}},
	volume = 447,
	year = 2015,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stu2439}}

@article{keek16,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.456.2722K},
	archiveprefix = {arXiv},
	author = {{Keek}, L. and {Ballantyne}, D.~R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/stv2882},
	eprint = {1508.06994},
	journal = {\mnras},
	keywords = {accretion, accretion discs, galaxies: active, galaxies: individual: Mrk 335, galaxies: Seyfert, X-rays: galaxies},
	month = mar,
	pages = {2722-2734},
	primaryclass = {astro-ph.HE},
	title = {{Revealing the accretion disc corona in Mrk 335 with multi-epoch X-ray spectroscopy}},
	volume = 456,
	year = 2016,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stv2882}}

@article{tazaki10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...721.1340T},
	archiveprefix = {arXiv},
	author = {{Tazaki}, F. and {Ueda}, Y. and {Ishino}, Y. and {Eguchi}, S. and {Isobe}, N. and {Terashima}, Y. and {Mushotzky}, R.~F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/721/2/1340},
	eprint = {1008.0722},
	journal = {\apj},
	keywords = {galaxies: active, galaxies: individual: 4C 50.55, X-rays: galaxies},
	month = oct,
	pages = {1340-1347},
	primaryclass = {astro-ph.HE},
	title = {{Suzaku Observation of the Brightest Broad-line Radio Galaxy 4C 50.55 (IGR J21247+5058)}},
	volume = 721,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/721/2/1340}}

@article{sazonov04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...421L..21S},
	author = {{Sazonov}, S.~Y. and {Revnivtsev}, M.~G. and {Lutovinov}, A.~A. and {Sunyaev}, R.~A. and {Grebenev}, S.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20040179},
	eprint = {astro-ph/0405259},
	journal = {\aap},
	keywords = {galaxies: Seyfert, X-rays: general},
	month = jul,
	pages = {L21-L24},
	title = {{Broadband X-ray spectrum of GRS 1734-292, a luminous Seyfert 1 galaxy behind the Galactic Center}},
	volume = 421,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20040179}}

@article{courvoisier03,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411L..53C},
	author = {{Courvoisier}, T.~J.-L. and {Walter}, R. and {Beckmann}, V. and {Dean}, A.~J. and {Dubath}, P. and {Hudec}, R. and {Kretschmar}, P. and {Mereghetti}, S. and {Montmerle}, T. and {Mowlavi}, N. and {Paltani}, S. and {Preite Martinez}, A. and {Produit}, N. and {Staubert}, R. and {Strong}, A.~W. and {Swings}, J.-P. and {Westergaard}, N.~J. and {White}, N. and {Winkler}, C. and {Zdziarski}, A.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20031172},
	eprint = {astro-ph/0308047},
	journal = {\aap},
	keywords = {methods: data analysis, gamma rays: observations},
	month = nov,
	pages = {L53-L57},
	title = {{The INTEGRAL Science Data Centre (ISDC)}},
	volume = 411,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031172}}

@article{Tortosa:2017,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.466.4193T},
	archiveprefix = {arXiv},
	author = {{Tortosa}, A. and {Marinucci}, A. and {Matt}, G. and {Bianchi}, S. and {La Franca}, F. and {Ballantyne}, D.~R. and {Boorman}, P.~G. and {Fabian}, A.~C. and {Farrah}, D. and {Fuerst}, F. and {Gandhi}, P. and {Harrison}, F.~A. and {Koss}, M.~J. and {Ricci}, C. and {Stern}, D. and {Ursini}, F. and {Walton}, D.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1093/mnras/stw3301},
	eprint = {1612.05871},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: individual: GRS 1734-292, galaxies: Seyfert, X-rays: galaxies},
	month = apr,
	pages = {4193-4200},
	primaryclass = {astro-ph.HE},
	title = {{Broad-band X-ray spectral analysis of the Seyfert 1 galaxy GRS 1734-292}},
	volume = 466,
	year = 2017,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stw3301}}

@article{Malizia:2014,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...782L..25M},
	archiveprefix = {arXiv},
	author = {{Malizia}, A. and {Molina}, M. and {Bassani}, L. and {Stephen}, J.~B. and {Bazzano}, A. and {Ubertini}, P. and {Bird}, A.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/2041-8205/782/2/L25},
	eid = {L25},
	eprint = {1401.3647},
	journal = {\apjl},
	keywords = {galaxies: active, gamma rays: galaxies, X-rays: galaxies},
	month = feb,
	pages = {L25},
	primaryclass = {astro-ph.HE},
	title = {{The INTEGRAL High-energy Cut-off Distribution of Type 1 Active Galactic Nuclei}},
	volume = 782,
	year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/782/2/L25}}

@article{tarchi11b,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...532A.125T},
	archiveprefix = {arXiv},
	author = {{Tarchi}, A. and {Castangia}, P. and {Columbano}, A. and {Panessa}, F. and {Braatz}, J.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201117213},
	eid = {A125},
	eprint = {1107.5155},
	journal = {\aap},
	keywords = {masers, galaxies: active, galaxies: nuclei, galaxies: Seyfert, radio lines: galaxies},
	month = aug,
	pages = {A125},
	primaryclass = {astro-ph.CO},
	title = {{Narrow-line Seyfert 1 galaxies: an amasing class of AGN}},
	volume = 532,
	year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201117213}}

@article{tarchi11a,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...525A..91T},
	archiveprefix = {arXiv},
	author = {{Tarchi}, A. and {Castangia}, P. and {Henkel}, C. and {Surcis}, G. and {Menten}, K.~M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201014714},
	eid = {A91},
	eprint = {1008.4253},
	journal = {\aap},
	keywords = {masers, galaxies: active, galaxies: nuclei, galaxies: starburst, radio lines: galaxies},
	month = jan,
	pages = {A91},
	primaryclass = {astro-ph.CO},
	title = {{New H$_{2}$O masers in Seyfert and FIR bright galaxies. IV. Interferometric follow-ups}},
	volume = 525,
	year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201014714}}

@article{ghisellini12,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.424L..26G},
	archiveprefix = {arXiv},
	author = {{Ghisellini}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1745-3933.2012.01280.x},
	eprint = {1205.0549},
	journal = {\mnras},
	keywords = {radiation mechanisms: non-thermal, gamma-ray burst: general, galaxies: active, galaxies: jets, X-rays: general},
	month = jul,
	pages = {L26-L30},
	primaryclass = {astro-ph.HE},
	title = {{Electron-positron pairs in blazar jets and {$\gamma$}-ray loud radio galaxies}},
	volume = 424,
	year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2012.01280.x}}

@article{panessa11,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.417.2426P},
	archiveprefix = {arXiv},
	author = {{Panessa}, F. and {de Rosa}, A. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A. and {Landi}, R. and {Malizia}, A. and {Miniutti}, G. and {Molina}, M. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2011.19268.x},
	eprint = {1106.3023},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: Seyfert, X-rays: galaxies},
	month = nov,
	pages = {2426-2439},
	primaryclass = {astro-ph.HE},
	title = {{Narrow-line Seyfert 1 galaxies at hard X-rays}},
	volume = 417,
	year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.19268.x}}

@article{filippenko03,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...588L..13F},
	author = {{Filippenko}, A.~V. and {Ho}, L.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/375361},
	eprint = {arXiv:astro-ph/0303429},
	journal = {\apjl},
	keywords = {Galaxies: Individual: NGC Number: NGC 4395, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei, Galaxies: Seyfert},
	month = may,
	pages = {L13-L16},
	title = {{A Low-Mass Central Black Hole in the Bulgeless Seyfert 1 Galaxy NGC 4395}},
	volume = 588,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/375361}}

@article{krivonos07,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...475..775K},
	author = {{Krivonos}, R. and {Revnivtsev}, M. and {Lutovinov}, A. and {Sazonov}, S. and {Churazov}, E. and {Sunyaev}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20077191},
	eprint = {arXiv:astro-ph/0701836},
	journal = {\aap},
	keywords = {surveys, X-rays: general, Galaxy: general, galaxies: Seyfert, cosmology: large-scale structure of Universe},
	month = nov,
	pages = {775-784},
	title = {{INTEGRAL/IBIS all-sky survey in hard X-rays}},
	volume = 475,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077191}}

@article{elitzur12,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...747L..33E},
	archiveprefix = {arXiv},
	author = {{Elitzur}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/2041-8205/747/2/L33},
	eid = {L33},
	eprint = {1202.1776},
	journal = {\apjl},
	keywords = {galaxies: active, galaxies: nuclei, galaxies: Seyfert, infrared: galaxies, quasars: general},
	month = mar,
	pages = {L33},
	primaryclass = {astro-ph.CO},
	title = {{On the Unification of Active Galactic Nuclei}},
	volume = 747,
	year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/747/2/L33}}

@article{paturel03,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...412...45P},
	author = {{Paturel}, G. and {Petit}, C. and {Prugniel}, P. and {Theureau}, G. and {Rousseau}, J. and {Brouty}, M. and {Dubois}, P. and {Cambr{\'e}sy}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20031411},
	journal = {\aap},
	keywords = {galaxies: general, catalogs},
	month = dec,
	pages = {45-55},
	title = {{HYPERLEDA. I. Identification and designation of galaxies}},
	volume = 412,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031411}}

@article{mcconnell12,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.422.1527M},
	archiveprefix = {arXiv},
	author = {{McConnell}, D. and {Sadler}, E.~M. and {Murphy}, T. and {Ekers}, R.~D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2012.20726.x},
	eprint = {1202.2625},
	journal = {\mnras},
	keywords = {methods: data analysis, catalogues, surveys, galaxies: active, gamma-rays: galaxies, radio continuum: general},
	month = may,
	pages = {1527-1545},
	primaryclass = {astro-ph.CO},
	title = {{ATPMN: accurate positions and flux densities at 5 and 8 GHz for 8385 sources from the PMN survey}},
	volume = 422,
	year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2012.20726.x}}

@article{landt04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.351...83L},
	author = {{Landt}, H. and {Padovani}, P. and {Perlman}, E.~S. and {Giommi}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2004.07750.x},
	eprint = {arXiv:astro-ph/0402494},
	journal = {\mnras},
	keywords = {galaxies: active, BL Lacertae objects: general, quasars: emission lines},
	month = jun,
	pages = {83-100},
	title = {{A physical classification scheme for blazars}},
	volume = 351,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.07750.x}}


@article{edelson12,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...751...52E},
	archiveprefix = {arXiv},
	author = {{Edelson}, R. and {Malkan}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/751/1/52},
	eid = {52},
	eprint = {1203.1942},
	journal = {\apj},
	keywords = {galaxies: active, galaxies: Seyfert, methods: statistical, quasars: general, surveys},
	month = may,
	pages = {52},
	primaryclass = {astro-ph.CO},
	title = {{Reliable Identifications of Active Galactic Nuclei from the WISE, 2MASS, and ROSAT All-Sky Surveys}},
	volume = 751,
	year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/751/1/52}}

@article{landi10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403..945L},
	archiveprefix = {arXiv},
	author = {{Landi}, R. and {Bassani}, L. and {Malizia}, A. and {Stephen}, J.~B. and {Bazzano}, A. and {Fiocchi}, M. and {Bird}, A.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2010.16183.x},
	eprint = {0912.1519},
	journal = {\mnras},
	keywords = {catalogues, surveys, gamma-rays: observations},
	month = apr,
	pages = {945-959},
	primaryclass = {astro-ph.HE},
	title = {{Swift/XRT observations of unidentified INTEGRAL/IBIS sources}},
	volume = 403,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.16183.x}}

@article{douglas96,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1996AJ....111.1945D},
	author = {{Douglas}, J.~N. and {Bash}, F.~N. and {Bozyan}, F.~A. and {Torrence}, G.~W. and {Wolfe}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/117932},
	journal = {\aj},
	keywords = {SURVEYS, RADIO LINES: GENERAL},
	month = may,
	pages = {1945},
	title = {{The Texas Survey of Radio Sources Covering -35.5 degrees {\lt} declination {\lt} 71.5 degrees at 365 MHz}},
	volume = 111,
	year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/117932}}

@article{wright10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010AJ....140.1868W},
	archiveprefix = {arXiv},
	author = {{Wright}, E.~L. and {Eisenhardt}, P.~R.~M. and {Mainzer}, A.~K. and {Ressler}, M.~E. and {Cutri}, R.~M. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and {Padgett}, D. and {McMillan}, R.~S. and {Skrutskie}, M. and {Stanford}, S.~A. and {Cohen}, M. and {Walker}, R.~G. and {Mather}, J.~C. and {Leisawitz}, D. and {Gautier}, III, T.~N. and {McLean}, I. and {Benford}, D. and {Lonsdale}, C.~J. and {Blain}, A. and {Mendez}, B. and {Irace}, W.~R. and {Duval}, V. and {Liu}, F. and {Royer}, D. and {Heinrichsen}, I. and {Howard}, J. and {Shannon}, M. and {Kendall}, M. and {Walsh}, A.~L. and {Larsen}, M. and {Cardon}, J.~G. and {Schick}, S. and {Schwalm}, M. and {Abid}, M. and {Fabinsky}, B. and {Naes}, L. and {Tsai}, C.-W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-6256/140/6/1868},
	eid = {1868},
	eprint = {1008.0031},
	journal = {\aj},
	keywords = {infrared: general, space vehicles, surveys},
	month = dec,
	pages = {1868-1881},
	primaryclass = {astro-ph.IM},
	title = {{The Wide-field Infrared Survey Explorer (WISE): Mission Description and Initial On-orbit Performance}},
	volume = 140,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/140/6/1868}}

@article{monet03,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003AJ....125..984M},
	author = {{Monet}, D.~G. and {Levine}, S.~E. and {Canzian}, B. and {Ables}, H.~D. and {Bird}, A.~R. and {Dahn}, C.~C. and {Guetter}, H.~H. and {Harris}, H.~C. and {Henden}, A.~A. and {Leggett}, S.~K. and {Levison}, H.~F. and {Luginbuhl}, C.~B. and {Martini}, J. and {Monet}, A.~K.~B. and {Munn}, J.~A. and {Pier}, J.~R. and {Rhodes}, A.~R. and {Riepe}, B. and {Sell}, S. and {Stone}, R.~C. and {Vrba}, F.~J. and {Walker}, R.~L. and {Westerhout}, G. and {Brucato}, R.~J. and {Reid}, I.~N. and {Schoening}, W. and {Hartley}, M. and {Read}, M.~A. and {Tritton}, S.~B.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/345888},
	eprint = {arXiv:astro-ph/0210694},
	journal = {\aj},
	keywords = {Astrometry, Catalogs},
	month = feb,
	pages = {984-993},
	title = {{The USNO-B Catalog}},
	volume = 125,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/345888}}

@article{griffith95,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1995ApJS...97..347G},
	author = {{Griffith}, M.~R. and {Wright}, A.~E. and {Burke}, B.~F. and {Ekers}, R.~D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/192146},
	journal = {\apjs},
	keywords = {ASTRONOMICAL CATALOGS, DATA REDUCTION, EQUATORIAL REGIONS, ERROR ANALYSIS, FLUX DENSITY, RADIO ASTRONOMY, RELIABILITY, SKY SURVEYS (ASTRONOMY), ASTRONOMICAL OBSERVATORIES, CENTIMETER WAVES, SUPERHIGH FREQUENCIES},
	month = apr,
	pages = {347-453},
	title = {{The Parkes-MIT-NRAO (PMN) surveys. 6: Source catalog for the equatorial survey (-9.5 deg less than delta less than +10.0 deg)}},
	volume = 97,
	year = 1995,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/192146}}

@article{bennett86,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1986ApJS...61....1B},
	author = {{Bennett}, C.~L. and {Lawrence}, C.~R. and {Burke}, B.~F. and {Hewitt}, J.~N. and {Mahoney}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/191108},
	journal = {\apjs},
	keywords = {ASTRONOMICAL CATALOGS, RADIO SOURCES (ASTRONOMY), CENTIMETER WAVES, RADIANT FLUX DENSITY, RADIO SPECTRA, RADIO TELESCOPES},
	month = may,
	pages = {1-104},
	title = {{The MIT-Green Bank (MG) 5 GHz survey}},
	volume = 61,
	year = 1986,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/191108}}

@article{vollmer09,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009yCat.8085....0B},
	author = {{Vollmer}, B.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {VizieR Online Data Catalog},
	keywords = {Radio sources, Galaxies: radio, Radio continuum},
	month = jul,
	pages = {0},
	title = {{SPECFIND V2.0 Catalog of radio continuum spectra (Vollmer+ 2009)}},
	volume = 8085,
	year = 2009}

@article{cohen07,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007AJ....134.1245C},
	archiveprefix = {arXiv},
	author = {{Cohen}, A.~S. and {Lane}, W.~M. and {Cotton}, W.~D. and {Kassim}, N.~E. and {Lazio}, T.~J.~W. and {Perley}, R.~A. and {Condon}, J.~J. and {Erickson}, W.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/520719},
	eprint = {0706.1191},
	journal = {\aj},
	keywords = {atmospheric effects, catalogs, radio continuum: general, surveys},
	month = sep,
	pages = {1245-1262},
	title = {{The VLA Low-Frequency Sky Survey}},
	volume = 134,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/520719}}

@article{bock99,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999AJ....117.1578B},
	author = {{Bock}, D.~C.-J. and {Large}, M.~I. and {Sadler}, E.~M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/300786},
	eprint = {arXiv:astro-ph/9812083},
	journal = {\aj},
	keywords = {INSTRUMENTATION: INTERFEROMETERS, RADIO CONTINUUM, SURVEYS},
	month = mar,
	pages = {1578-1593},
	title = {{SUMSS: A Wide-Field Radio Imaging Survey of the Southern Sky. I. Science Goals, Survey Design, and Instrumentation}},
	volume = 117,
	year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/300786}}

@article{Winkler:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411L...1W},
	author = {{Winkler}, C. and {Courvoisier}, T.~J.-L. and {Di Cocco}, G. and {Gehrels}, N. and {Gim{\'e}nez}, A. and {Grebenev}, S. and {Hermsen}, W. and {Mas-Hesse}, J.~M. and {Lebrun}, F. and {Lund}, N. and {Palumbo}, G.~G.~C. and {Paul}, J. and {Roques}, J.-P. and {Schnopper}, H. and {Sch{\"o}nfelder}, V. and {Sunyaev}, R. and {Teegarden}, B. and {Ubertini}, P. and {Vedrenne}, G. and {Dean}, A.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20031288},
	journal = {\aap},
	keywords = {gamma-ray astronomy, space observatory},
	month = nov,
	pages = {L1-L6},
	title = {{The INTEGRAL mission}},
	volume = 411,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031288}}

@article{malizia11,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011ATel.3290....1M},
	author = {{Malizia}, A. and {Landi}, R. and {Bassani}, L. and {Bird}, A.~B.~A.~J. and {Gehrels}, N. and {Kennea}, J.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {The Astronomer's Telegram},
	keywords = {X-ray, Gamma Ray, AGN, Binary},
	month = apr,
	pages = {1},
	title = {{Swift-XRT follow-up of 2 unidentified INTEGRAL sources}},
	volume = 3290,
	year = 2011}

@book{zombeck90,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1990hsaa.book.....Z},
	author = {{Zombeck}, M.~V.},
	booktitle = {Cambridge: University Press, 1990, 2nd ed.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{Zombeck, M.~V.}},
	title = {{Handbook of space astronomy and astrophysics}},
	year = 1990}

@article{wright94,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1994ApJS...91..111W},
	author = {{Wright}, A.~E. and {Griffith}, M.~R. and {Burke}, B.~F. and {Ekers}, R.~D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/191939},
	journal = {\apjs},
	keywords = {ASTRONOMICAL CATALOGS, RADIO ASTRONOMY, RADIO SOURCES (ASTRONOMY), SKY SURVEYS (ASTRONOMY), SOUTHERN SKY, TABLES (DATA), ERROR ANALYSIS, RADIO TELESCOPES},
	month = mar,
	pages = {111-308},
	title = {{The Parkes-MIT-NRAO (PMN) surveys. 2: Source catalog for the southern survey (delta greater than -87.5 deg and less than -37 deg)}},
	volume = 91,
	year = 1994,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/191939}}

@article{white00,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2000yCat.9031....0W},
	author = {{White}, N.~E. and {Giommi}, P. and {Angelini}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {VizieR Online Data Catalog},
	keywords = {X-ray sources, Cross identifications},
	month = jun,
	pages = {0},
	title = {{The WGACAT version of ROSAT sources (White+ 2000)}},
	volume = 9031,
	year = 2000}

@article{stephen05,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...432L..49S},
	author = {{Stephen}, J.~B. and {Bassani}, L. and {Molina}, M. and {Malizia}, A. and {Bazzano}, A. and {Ubertini}, P. and {Dean}, A.~J. and {Bird}, A.~J. and {Lebrun}, F. and {Much}, R. and {Walter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:200500017},
	eprint = {arXiv:astro-ph/0502158},
	journal = {\aap},
	keywords = {catalogues, surveys, gamma-rays: observations},
	month = mar,
	pages = {L49-L52},
	title = {{Using the ROSAT Bright Source Catalogue to find counterparts for IBIS/ISGRI survey sources}},
	volume = 432,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200500017}}

@article{stephen06,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...445..869S},
	author = {{Stephen}, J.~B. and {Bassani}, L. and {Malizia}, A. and {Bazzano}, A. and {Ubertini}, P. and {Bird}, A.~J. and {Dean}, A.~J. and {Lebrun}, F. and {Walter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20053958},
	eprint = {arXiv:astro-ph/0509620},
	journal = {\aap},
	keywords = {catalogs, surveys, gamma-rays: observations},
	month = jan,
	pages = {869-873},
	title = {{Using the ROSAT catalogues to find counterparts for the second IBIS/ISGRI survey sources}},
	volume = 445,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20053958}}

@article{stephen10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.408..422S},
	archiveprefix = {arXiv},
	author = {{Stephen}, J.~B. and {Bassani}, L. and {Landi}, R. and {Malizia}, A. and {Sguera}, V. and {Bazzano}, A. and {Masetti}, N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2010.17123.x},
	eprint = {1004.5232},
	journal = {\mnras},
	keywords = {catalogues, surveys, gamma-rays: general},
	month = oct,
	pages = {422-429},
	primaryclass = {astro-ph.HE},
	title = {{Using the ROSAT catalogue to find counterparts for unidentified objects in the first Fermi/LAT catalogue}},
	volume = 408,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.17123.x}}

@article{souchay09,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...494..799S},
	author = {{Souchay}, J. and {Andrei}, A.~H. and {Barache}, C. and {Bouquillon}, S. and {Gontier}, A.-M. and {Lambert}, S.~B. and {Le Poncin-Lafitte}, C. and {Taris}, F. and {Arias}, E.~F. and {Suchet}, D. and {Baudin}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:200809602},
	journal = {\aap},
	keywords = {reference systems, astrometry, quasars: general, catalogs},
	month = feb,
	pages = {799-815},
	title = {{The construction of the large quasar astrometric catalogue (LQAC)}},
	volume = 494,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200809602}}

@article{murphy10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.402.2403M},
	archiveprefix = {arXiv},
	author = {{Murphy}, T. and {Sadler}, E.~M. and {Ekers}, R.~D. and {Massardi}, M. and {Hancock}, P.~J. and {Mahony}, E. and {Ricci}, R. and {Burke-Spolaor}, S. and {Calabretta}, M. and {Chhetri}, R. and {de Zotti}, G. and {Edwards}, P.~G. and {Ekers}, J.~A. and {Jackson}, C.~A. and {Kesteven}, M.~J. and {Lindley}, E. and {Newton-McGee}, K. and {Phillips}, C. and {Roberts}, P. and {Sault}, R.~J. and {Staveley-Smith}, L. and {Subrahmanyan}, R. and {Walker}, M.~A. and {Wilson}, W.~E.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2009.15961.x},
	eprint = {0911.0002},
	journal = {\mnras},
	keywords = {methods: data analysis, catalogues, surveys, galaxies: active, cosmic microwave background, radio continuum: general},
	month = mar,
	pages = {2403-2423},
	primaryclass = {astro-ph.GA},
	title = {{The Australia Telescope 20 GHz Survey: the source catalogue}},
	volume = 402,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15961.x}}

@inproceedings{mundell99,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999AAS...194.6205M},
	author = {{Mundell}, C.~G. and {Wilson}, A.~S. and {Ulvestad}, J.~S. and {Roy}, A.~L.},
	booktitle = {American Astronomical Society Meeting Abstracts \#194},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	month = may,
	pages = {922},
	series = {Bulletin of the American Astronomical Society},
	title = {{Milli Arc Second Radio Imaging of Seyferts}},
	volume = 31,
	year = 1999}

@article{mauch03,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.342.1117M},
	author = {{Mauch}, T. and {Murphy}, T. and {Buttery}, H.~J. and {Curran}, J. and {Hunstead}, R.~W. and {Piestrzynski}, B. and {Robertson}, J.~G. and {Sadler}, E.~M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2003.06605.x},
	eprint = {arXiv:astro-ph/0303188},
	journal = {\mnras},
	keywords = {methods: data analysis, catalogues, surveys, astrometry, galaxies: statistics, radio continuum: general},
	month = jul,
	pages = {1117-1130},
	title = {{SUMSS: a wide-field radio imaging survey of the southern sky - II. The source catalogue}},
	volume = 342,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2003.06605.x}}

@inproceedings{moretti04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004SPIE.5165..232M},
	author = {{Moretti}, A. and {Campana}, S. and {Tagliaferri}, G. and {Abbey}, A.~F. and {Ambrosi}, R.~M. and {Angelini}, L. and {Beardmore}, A.~P. and {Br{\"a}uninger}, H.~W. and {Burkert}, W. and {Burrows}, D.~N. and {Capalbi}, M. and {Chincarini}, G. and {Citterio}, O. and {Cusumano}, G. and {Freyberg}, M.~J. and {Giommi}, P. and {Hartner}, G.~D. and {Hill}, J.~E. and {Mori}, K. and {Morris}, D.~C. and {Mukerjee}, K. and {Nousek}, J.~A. and {Osborne}, J.~P. and {Short}, A.~D.~T. and {Tamburelli}, F. and {Watson}, D.~J. and {Wells}, A.~A.},
	booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1117/12.504857},
	editor = {{K.~A.~Flanagan \&amp; O.~H.~W.~Siegmund}},
	month = feb,
	pages = {232-240},
	series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
	title = {{SWIFT XRT point spread function measured at the Panter end-to-end tests}},
	volume = 5165,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.504857}}

@article{massaro12,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2012arXiv1203.3801M},
	archiveprefix = {arXiv},
	author = {{Massaro}, F. and {D'Abrusco}, R. and {Tosti}, G. and {Ajello}, M. and {Gasparrini}, A.~P.~D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {1203.3801},
	journal = {ArXiv e-prints},
	keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Galaxy Astrophysics},
	month = mar,
	primaryclass = {astro-ph.HE},
	title = {{Unidentifed gamma-ray sources: hunting gamma-ray blazars}},
	year = 2012}

@article{massaro09,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009yCat..34950691M},
	author = {{Massaro}, E. and {Giommi}, P. and {Leto}, C. and {Marchegiani}, P. and {Maselli}, A. and {Perri}, M. and {Piranomonte}, S. and {Sclavi}, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {VizieR Online Data Catalog},
	keywords = {QSOs, BL Lac objects, Galaxy catalogs, Redshifts, Photometry},
	month = nov,
	pages = {50691},
	title = {{Multifrequency catalogue of blazars, Roma-BZCAT (Massaro+, 2009)}},
	volume = 349,
	year = 2009}

@article{masetti10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...519A..96M},
	archiveprefix = {arXiv},
	author = {{Masetti}, N. and {Parisi}, P. and {Palazzi}, E. and {Jim{\'e}nez-Bail{\'o}n}, E. and {Chavushyan}, V. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A.~J. and {Dean}, A.~J. and {Charles}, P.~A. and {Galaz}, G. and {Landi}, R. and {Malizia}, A. and {Mason}, E. and {McBride}, V.~A. and {Minniti}, D. and {Morelli}, L. and {Schiavone}, F. and {Stephen}, J.~B. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201014852},
	eid = {A96},
	eprint = {1006.4513},
	journal = {\aap},
	keywords = {galaxies: Seyfert, quasars: emission lines, X-rays: binaries, novae, cataclysmic variables, X-rays: general, techniques: spectroscopic},
	month = sep,
	pages = {A96},
	primaryclass = {astro-ph.HE},
	title = {{Unveiling the nature of INTEGRAL objects through optical spectroscopy. VIII. Identification of 44 newly detected hard X-ray sources}},
	volume = 519,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201014852}}

@article{masetti12,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...538A.123M},
	archiveprefix = {arXiv},
	author = {{Masetti}, N. and {Parisi}, P. and {Jim{\'e}nez-Bail{\'o}n}, E. and {Palazzi}, E. and {Chavushyan}, V. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A.~J. and {Dean}, A.~J. and {Galaz}, G. and {Landi}, R. and {Malizia}, A. and {Minniti}, D. and {Morelli}, L. and {Schiavone}, F. and {Stephen}, J.~B. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201118559},
	eid = {A123},
	eprint = {1201.1906},
	journal = {\aap},
	keywords = {X-rays: binaries, galaxies:Seyfert, X-rays: general, novae, cataclysmic variables, quasars: emission lines, stars: flare},
	month = feb,
	pages = {A123},
	primaryclass = {astro-ph.HE},
	title = {{Unveiling the nature of INTEGRAL objects through optical spectroscopy. IX. Twenty two more identifications, and a glance into the far hard X-ray Universe}},
	volume = 538,
	year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201118559}}

@article{kalberla05,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...440..775K},
	author = {{Kalberla}, P.~M.~W. and {Burton}, W.~B. and {Hartmann}, D. and {Arnal}, E.~M. and {Bajaja}, E. and {Morras}, R. and {P{\"o}ppel}, W.~G.~L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20041864},
	eprint = {arXiv:astro-ph/0504140},
	journal = {\aap},
	keywords = {surveys, radio lines: ISM, Galaxy: structure},
	month = sep,
	pages = {775-782},
	title = {{The Leiden/Argentine/Bonn (LAB) Survey of Galactic HI. Final data release of the combined LDS and IAR surveys with improved stray-radiation corrections}},
	volume = 440,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20041864}}

@article{healey07,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..171...61H},
	author = {{Healey}, S.~E. and {Romani}, R.~W. and {Taylor}, G.~B. and {Sadler}, E.~M. and {Ricci}, R. and {Murphy}, T. and {Ulvestad}, J.~S. and {Winn}, J.~N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/513742},
	eprint = {arXiv:astro-ph/0702346},
	journal = {\apjs},
	keywords = {Galaxies: Active, Galaxies: Quasars: General, Surveys},
	month = jul,
	pages = {61-71},
	title = {{CRATES: An All-Sky Survey of Flat-Spectrum Radio Sources}},
	volume = 171,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/513742}}

@article{ghisellini10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.402..497G},
	archiveprefix = {arXiv},
	author = {{Ghisellini}, G. and {Tavecchio}, F. and {Foschini}, L. and {Ghirlanda}, G. and {Maraschi}, L. and {Celotti}, A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2009.15898.x},
	eprint = {0909.0932},
	journal = {\mnras},
	keywords = {radiation mechanisms: non-thermal, BL Lacertae objects: general, quasars: general, gamma-rays: theory, X-rays: general},
	month = feb,
	pages = {497-518},
	primaryclass = {astro-ph.CO},
	title = {{General physical properties of bright Fermi blazars}},
	volume = 402,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15898.x}}

@inproceedings{ghisellini09,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009AIPC.1126..131G},
	archiveprefix = {arXiv},
	author = {{Ghisellini}, G.},
	booktitle = {American Institute of Physics Conference Series},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1063/1.3149394},
	editor = {{J.~Rodriguez \&amp; P.~Ferrando}},
	eprint = {0902.1984},
	keywords = {X-ray, Quasars, Infall, accretion, and accretion disks, Neutrino, muon, pion, and other elementary particles; cosmic rays, Galactic nuclei , circumnuclear matter, and bulges},
	month = may,
	pages = {131-136},
	primaryclass = {astro-ph.CO},
	series = {American Institute of Physics Conference Series},
	title = {{Blazars in Hard X-rays}},
	volume = 1126,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1063/1.3149394}}

@article{gehrels04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...611.1005G},
	author = {{Gehrels}, N. and {Chincarini}, G. and {Giommi}, P. and {Mason}, K.~O. and {Nousek}, J.~A. and {Wells}, A.~A. and {White}, N.~E. and {Barthelmy}, S.~D. and {Burrows}, D.~N. and {Cominsky}, L.~R. and {Hurley}, K.~C. and {Marshall}, F.~E. and {M{\'e}sz{\'a}ros}, P. and {Roming}, P.~W.~A. and {Angelini}, L. and {Barbier}, L.~M. and {Belloni}, T. and {Campana}, S. and {Caraveo}, P.~A. and {Chester}, M.~M. and {Citterio}, O. and {Cline}, T.~L. and {Cropper}, M.~S. and {Cummings}, J.~R. and {Dean}, A.~J. and {Feigelson}, E.~D. and {Fenimore}, E.~E. and {Frail}, D.~A. and {Fruchter}, A.~S. and {Garmire}, G.~P. and {Gendreau}, K. and {Ghisellini}, G. and {Greiner}, J. and {Hill}, J.~E. and {Hunsberger}, S.~D. and {Krimm}, H.~A. and {Kulkarni}, S.~R. and {Kumar}, P. and {Lebrun}, F. and {Lloyd-Ronning}, N.~M. and {Markwardt}, C.~B. and {Mattson}, B.~J. and {Mushotzky}, R.~F. and {Norris}, J.~P. and {Osborne}, J. and {Paczynski}, B. and {Palmer}, D.~M. and {Park}, H.-S. and {Parsons}, A.~M. and {Paul}, J. and {Rees}, M.~J. and {Reynolds}, C.~S. and {Rhoads}, J.~E. and {Sasseen}, T.~P. and {Schaefer}, B.~E. and {Short}, A.~T. and {Smale}, A.~P. and {Smith}, I.~A. and {Stella}, L. and {Tagliaferri}, G. and {Takahashi}, T. and {Tashiro}, M. and {Townsley}, L.~K. and {Tueller}, J. and {Turner}, M.~J.~L. and {Vietri}, M. and {Voges}, W. and {Ward}, M.~J. and {Willingale}, R. and {Zerbi}, F.~M. and {Zhang}, W.~W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/422091},
	journal = {\apj},
	keywords = {Gamma Rays: Bursts, Space Vehicles: Instruments, Telescopes},
	month = aug,
	pages = {1005-1020},
	title = {{The Swift Gamma-Ray Burst Mission}},
	volume = 611,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422091}}

@article{fugmann88,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1988A%26A...205...86F},
	author = {{Fugmann}, W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\aap},
	keywords = {ACTIVE GALACTIC NUCLEI, BL LACERTAE OBJECTS, BLAZARS, EXTRAGALACTIC RADIO SOURCES, OPTICAL POLARIZATION, QUASARS, ASTRONOMICAL CATALOGS, ASTRONOMICAL PHOTOMETRY, RADIO ASTRONOMY},
	month = oct,
	pages = {86-92},
	title = {{Are all flat-spectrum radio sources blazars?}},
	volume = 205,
	year = 1988}

@article{derosa12,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.420.2087D},
	archiveprefix = {arXiv},
	author = {{De Rosa}, A. and {Panessa}, F. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A. and {Landi}, R. and {Malizia}, A. and {Molina}, M. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2011.20167.x},
	eprint = {1111.1946},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: Seyfert, X-rays: galaxies},
	month = mar,
	pages = {2087-2101},
	primaryclass = {astro-ph.CO},
	title = {{Broad-band study of hard X-ray-selected absorbed active galactic nuclei}},
	volume = 420,
	year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.20167.x}}

@article{condon98,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1998AJ....115.1693C},
	author = {{Condon}, J.~J. and {Cotton}, W.~D. and {Greisen}, E.~W. and {Yin}, Q.~F. and {Perley}, R.~A. and {Taylor}, G.~B. and {Broderick}, J.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/300337},
	journal = {\aj},
	keywords = {CATALOGS, METHODS: DATA ANALYSIS, METHODS: OBSERVATIONAL, RADIO CONTINUUM, SURVEYS},
	month = may,
	pages = {1693-1716},
	title = {{The NRAO VLA Sky Survey}},
	volume = 115,
	year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/300337}}

@inproceedings{condon93,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1993ASPC...43...87C},
	author = {{Condon}, J.~J.},
	booktitle = {Sky Surveys. Protostars to Protogalaxies},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{B.~T.~Soifer}},
	month = jan,
	pages = {87},
	series = {Astronomical Society of the Pacific Conference Series},
	title = {{Radio Surveys of AGN}},
	volume = 43,
	year = 1993}

@article{burrows:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005SSRv..120..165B},
	author = {{Burrows}, D.~N. and {Hill}, J.~E. and {Nousek}, J.~A. and {Kennea}, J.~A. and {Wells}, A. and {Osborne}, J.~P. and {Abbey}, A.~F. and {Beardmore}, A. and {Mukerjee}, K. and {Short}, A.~D.~T. and {Chincarini}, G. and {Campana}, S. and {Citterio}, O. and {Moretti}, A. and {Pagani}, C. and {Tagliaferri}, G. and {Giommi}, P. and {Capalbi}, M. and {Tamburelli}, F. and {Angelini}, L. and {Cusumano}, G. and {Br{\"a}uninger}, H.~W. and {Burkert}, W. and {Hartner}, G.~D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1007/s11214-005-5097-2},
	eprint = {arXiv:astro-ph/0508071},
	journal = {\ssr},
	keywords = {gamma-ray burst, X-ray telescope, Swift, X-ray instrumentation, X-ray CCD detector, X-ray mirrors, {$\gamma$}-ray burst},
	month = oct,
	pages = {165-195},
	title = {{The Swift X-Ray Telescope}},
	volume = 120,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s11214-005-5097-2}}

@article{bassani:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...669L...1B},
	archiveprefix = {arXiv},
	author = {{Bassani}, L. and {Landi}, R. and {Malizia}, A. and {Fiocchi}, M.~T. and {Bazzano}, A. and {Bird}, A.~J. and {Dean}, A.~J. and {Gehrels}, N. and {Giommi}, P. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/523757},
	eprint = {0709.3023},
	journal = {\apjl},
	keywords = {Gamma Rays: Observations, quasars: individual (IGR J22517+2218), quasars: individual (MG3 J225155+2217)},
	month = nov,
	pages = {L1-L4},
	title = {{IGR J22517+2218=MG3 J225155+2217: A New Gamma-Ray Lighthouse in the Distant Universe}},
	volume = 669,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/523757}}

@article{polletta11,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...533A..20P},
	archiveprefix = {arXiv},
	author = {{Polletta}, M. and {Nesvadba}, N.~P.~H. and {Neri}, R. and {Omont}, A. and {Berta}, S. and {Bergeron}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201116446},
	eid = {A20},
	eprint = {1107.2129},
	journal = {\aap},
	keywords = {galaxies: high-redshift, galaxies: active, submillimeter: galaxies, submillimeter: ISM, quasars: general, galaxies: evolution},
	month = sep,
	pages = {A20},
	primaryclass = {astro-ph.CO},
	title = {{Disk, merger, or outflow? Molecular gas kinematics in two powerful obscured QSOs at z {\ge} 3.4}},
	volume = 533,
	year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201116446}}

@article{king11,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.415L...6K},
	archiveprefix = {arXiv},
	author = {{King}, A.~R. and {Zubovas}, K. and {Power}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1745-3933.2011.01067.x},
	eprint = {1104.3682},
	journal = {\mnras},
	keywords = {accretion, accretion discs, black hole physics, galaxies: evolution, quasars: general},
	month = jul,
	pages = {L6-L10},
	primaryclass = {astro-ph.GA},
	title = {{Large-scale outflows in galaxies}},
	volume = 415,
	year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2011.01067.x}}

@article{biggs08,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.385..893B},
	archiveprefix = {arXiv},
	author = {{Biggs}, A.~D. and {Ivison}, R.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.12869.x},
	eprint = {0712.3047},
	journal = {\mnras},
	keywords = {instrumentation: interferometers , techniques: interferometric , galaxies: formation , galaxies: starburst , radio continuum: galaxies , submillimetre},
	month = apr,
	pages = {893-904},
	title = {{High-resolution radio observations of submillimetre galaxies}},
	volume = 385,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.12869.x}}

@article{muxlow05,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.358.1159M},
	author = {{Muxlow}, T.~W.~B. and {Richards}, A.~M.~S. and {Garrington}, S.~T. and {Wilkinson}, P.~N. and {Anderson}, B. and {Richards}, E.~A. and {Axon}, D.~J. and {Fomalont}, E.~B. and {Kellermann}, K.~I. and {Partridge}, R.~B. and {Windhorst}, R.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2005.08824.x},
	eprint = {arXiv:astro-ph/0501679},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: evolution, galaxies: starburst, cosmology: observations, radio continuum: galaxies},
	month = apr,
	pages = {1159-1194},
	title = {{High-resolution studies of radio sources in the Hubble Deep and Flanking Fields}},
	volume = 358,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.08824.x}}

@article{clemens08,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...477...95C},
	archiveprefix = {arXiv},
	author = {{Clemens}, M.~S. and {Vega}, O. and {Bressan}, A. and {Granato}, G.~L. and {Silva}, L. and {Panuzzo}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20077224},
	eprint = {0708.0149},
	journal = {\aap},
	keywords = {dust, extinction, galaxies: active, infrared: galaxies, radio continuum: galaxies},
	month = jan,
	pages = {95-104},
	title = {{Modeling the spectral energy distribution of ULIRGs. I. The radio spectra}},
	volume = 477,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077224}}

@article{richards00,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...533..611R},
	author = {{Richards}, E.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/308684},
	eprint = {arXiv:astro-ph/9908313},
	journal = {\apj},
	keywords = {COSMOLOGY: OBSERVATIONS, GALAXIES: ACTIVE, GALAXIES: EVOLUTION, GALAXIES: STARBURST, RADIO CONTINUUM: GALAXIES, SURVEYS},
	month = apr,
	pages = {611-630},
	title = {{The Nature of Radio Emission from Distant Galaxies: The 1.4 GHZ Observations}},
	volume = 533,
	year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/308684}}

@article{donley05,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...634..169D},
	author = {{Donley}, J.~L. and {Rieke}, G.~H. and {Rigby}, J.~R. and {P{\'e}rez-Gonz{\'a}lez}, P.~G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/491668},
	eprint = {arXiv:astro-ph/0507676},
	journal = {\apj},
	keywords = {Galaxies: Active, Radio Continuum: Galaxies, X-Rays: Galaxies},
	month = nov,
	pages = {169-182},
	title = {{Unveiling a Population of AGNs Not Detected in X-Rays}},
	volume = 634,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/491668}}

@book{kellermann74,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1974gegr.book..320K},
	author = {{Kellermann}, K.~I.},
	booktitle = {Galactic and Extra-Galactic Radio Astronomy},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{Verschuur, G.~L., Kellermann, K.~I.; van Brunt, V.}},
	pages = {320},
	publisher = {Springer-Verlag},
	title = {{Radio Galaxies and Quasars}},
	year = 1974}

@article{klein88,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1988A%26A...190...41K},
	author = {{Klein}, U. and {Wielebinski}, R. and {Morsi}, H.~W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\aap},
	keywords = {CONTINUOUS SPECTRA, IRREGULAR GALAXIES, RADIO SOURCES (ASTRONOMY), STAR FORMATION, STARBURST GALAXIES, ASTRONOMICAL MAPS, BRIGHTNESS TEMPERATURE, FAR INFRARED RADIATION, LYMAN SPECTRA, RELATIVISTIC PARTICLES},
	month = jan,
	pages = {41-46},
	title = {{Radio continuum observations of M82}},
	volume = 190,
	year = 1988}

@article{Ferrari:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008SSRv..134...93F},
	archiveprefix = {arXiv},
	author = {{Ferrari}, C. and {Govoni}, F. and {Schindler}, S. and {Bykov}, A.~M. and {Rephaeli}, Y.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1007/s11214-008-9311-x},
	eprint = {0801.0985},
	journal = {\ssr},
	keywords = {Galaxies: clusters: general, Galaxies: intergalactic medium, Radio continuum: general, Radiation mechanisms: non-thermal, Magnetic fields, Acceleration of particles},
	month = feb,
	pages = {93-118},
	title = {{Observations of Extended Radio Emission in Clusters}},
	volume = 134,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s11214-008-9311-x}}

@article{Miley:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26ARv..15...67M},
	archiveprefix = {arXiv},
	author = {{Miley}, G. and {De Breuck}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1007/s00159-007-0008-z},
	eprint = {0802.2770},
	journal = {\aapr},
	keywords = {Radio galaxies, High-redshift, Massive galaxies, Clusters},
	month = feb,
	pages = {67-144},
	title = {{Distant radio galaxies and their environments}},
	volume = 15,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s00159-007-0008-z}}

@article{Jarvis:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.355...20J},
	author = {{Jarvis}, M.~J. and {Cruz}, M.~J. and {Cohen}, A.~S. and {R{\"o}ttgering}, H.~J.~A. and {Kassim}, N.~E.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2004.08278.x},
	eprint = {arXiv:astro-ph/0408082},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: evolution, galaxies: high-redshift, galaxies: nuclei, radio continuum: galaxies},
	month = nov,
	pages = {20-30},
	title = {{Near-infrared K-band imaging of a sample of ultra-steep-spectrum radio sources selected at 74 MHz}},
	volume = 355,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.08278.x}}

@inproceedings{deBreuck:1998,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1998ASSL..226..185D},
	author = {{De Breuck}, C. and {et al.}},
	booktitle = {Observational Cosmology with the New Radio Surveys},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{M.~N.~Bremer, N.~Jackson, \& I.~Perez-Fournon}},
	eprint = {arXiv:astro-ph/9705056},
	pages = {185},
	series = {Astrophysics and Space Science Library},
	title = {{Searches for High Redshift Radio Galaxies}},
	volume = 226,
	year = 1998}

@article{brunner08,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...479..283B},
	archiveprefix = {arXiv},
	author = {{Brunner}, H. and {Cappelluti}, N. and {Hasinger}, G. and {Barcons}, X. and {Fabian}, A.~C. and {Mainieri}, V. and {Szokoly}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20077687},
	eprint = {0711.4822},
	journal = {\aap},
	keywords = {surveys, galaxies: active, galaxies: quasars: general, X-rays: galaxies, X-rays: general},
	month = feb,
	pages = {283-300},
	title = {{XMM-Newton observations of the Lockman Hole: X-ray source catalogue and number counts}},
	volume = 479,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077687}}

@article{magliocchetti08,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.383..479M},
	archiveprefix = {arXiv},
	author = {{Magliocchetti}, M. and {Andreani}, P. and {Zwaan}, M.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2007.12576.x},
	eprint = {0710.2343},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: starburst, cosmology: observations, infrared: galaxies, radio continuum: galaxies},
	month = jan,
	pages = {479-496},
	title = {{The radio properties of optically obscured Spitzer sources}},
	volume = 383,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12576.x}}

@article{ibar09,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.397..281I},
	archiveprefix = {arXiv},
	author = {{Ibar}, E. and {Ivison}, R.~J. and {Biggs}, A.~D. and {Lal}, D.~V. and {Best}, P.~N. and {Green}, D.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2009.14866.x},
	eprint = {0903.3600},
	journal = {\mnras},
	keywords = {techniques: interferometric , galaxies: evolution , galaxies: starburst , radio continuum: galaxies},
	month = jul,
	pages = {281-298},
	primaryclass = {astro-ph.CO},
	title = {{Deep multi-frequency radio imaging in the Lockman Hole using the GMRT and VLA - I. The nature of the sub-mJy radio population}},
	volume = 397,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.14866.x}}

@inproceedings{Paioro:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ASPC..394..397P},
	author = {{Paioro}, L. and {Chiappetti}, L. and {Garilli}, B. and {Franzetti}, P. and {Fumana}, M. and {Scodeggio}, M.},
	booktitle = {Astronomical Data Analysis Software and Systems XVII},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{R.~W.~Argyle, P.~S.~Bunclark, \&amp; J.~R.~Lewis}},
	month = aug,
	pages = {397},
	series = {Astronomical Society of the Pacific Conference Series},
	title = {{DART, a New Solution to Deploy and Access Astronomical Data}},
	volume = 394,
	year = 2008}

@article{Lindner:2011,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737...83L},
	archiveprefix = {arXiv},
	author = {{Lindner}, R.~R. and {Baker}, A.~J. and {Omont}, A. and {Beelen}, A. and {Owen}, F.~N. and {Bertoldi}, F. and {Dole}, H. and {Fiolet}, N. and {Harris}, A.~I. and {Ivison}, R.~J. and {Lonsdale}, C.~J. and {Lutz}, D. and {Polletta}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/737/2/83},
	eprint = {1106.0344},
	journal = {\apj},
	keywords = {galaxies: formation, galaxies: high-redshift, galaxies: starburst, submillimeter: galaxies},
	month = aug,
	pages = {83-+},
	primaryclass = {astro-ph.CO},
	title = {{A Deep 1.2{\nbsp}mm Map of the Lockman Hole North Field}},
	volume = 737,
	year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/737/2/83}}

@article{magdis10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.409...22M},
	archiveprefix = {arXiv},
	author = {{Magdis}, G.~E. and {Elbaz}, D. and {Hwang}, H.~S. and {Amblard}, A. and {Arumugam}, V. and {Aussel}, H. and {Blain}, A. and {Bock}, J. and {Boselli}, A. and {Buat}, V. and {Castro-Rodr{\'{\i}}guez}, N. and {Cava}, A. and {Chanial}, P. and {Clements}, D.~L. and {Conley}, A. and {Conversi}, L. and {Cooray}, A. and {Dowell}, C.~D. and {Dwek}, E. and {Eales}, S. and {Farrah}, D. and {Franceschini}, A. and {Glenn}, J. and {Griffin}, M. and {Halpern}, M. and {Hatziminaoglou}, E. and {Huang}, J. and {Ibar}, E. and {Isaak}, K. and {Le Floc'h}, E. and {Lagache}, G. and {Levenson}, L. and {Lonsdale}, C.~J. and {Lu}, N. and {Madden}, S. and {Maffei}, B. and {Mainetti}, G. and {Marchetti}, L. and {Morrison}, G.~E. and {Nguyen}, H.~T. and {O'Halloran}, B. and {Oliver}, S.~J. and {Omont}, A. and {Owen}, F.~N. and {Page}, M.~J. and {Pannella}, M. and {Panuzzo}, P. and {Papageorgiou}, A. and {Pearson}, C.~P. and {P{\'e}rez-Fournon}, I. and {Pohlen}, M. and {Rigopoulou}, D. and {Rizzo}, D. and {Roseboom}, I.~G. and {Rowan-Robinson}, M. and {Schulz}, B. and {Scott}, D. and {Seymour}, N. and {Shupe}, D.~L. and {Smith}, A.~J. and {Stevens}, J.~A. and {Strazzullo}, V. and {Symeonidis}, M. and {Trichas}, M. and {Tugwell}, K.~E. and {Vaccari}, M. and {Valtchanov}, I. and {Vigroux}, L. and {Wang}, L. and {Wright}, G. and {Xu}, C.~K. and {Zemcov}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2010.17551.x},
	eprint = {1007.4900},
	journal = {\mnras},
	keywords = {galaxies: evolution, galaxies: high-redshift, galaxies: starburst, cosmology: observations, infrared: galaxies, submillimetre: galaxies},
	month = nov,
	pages = {22-28},
	primaryclass = {astro-ph.CO},
	title = {{Herschel reveals a T_{dust}-unbiased selection of z \~{} 2 ultraluminous infrared galaxies}},
	volume = 409,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.17551.x}}

@article{oliver10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518L..21O},
	archiveprefix = {arXiv},
	author = {{Oliver}, S.~J. and {Wang}, L. and {Smith}, A.~J. and {Altieri}, B. and {Amblard}, A. and {Arumugam}, V. and {Auld}, R. and {Aussel}, H. and {Babbedge}, T. and {Blain}, A. and {Bock}, J. and {Boselli}, A. and {Buat}, V. and {Burgarella}, D. and {Castro-Rodr{\'{\i}}guez}, N. and {Cava}, A. and {Chanial}, P. and {Clements}, D.~L. and {Conley}, A. and {Conversi}, L. and {Cooray}, A. and {Dowell}, C.~D. and {Dwek}, E. and {Eales}, S. and {Elbaz}, D. and {Fox}, M. and {Franceschini}, A. and {Gear}, W. and {Glenn}, J. and {Griffin}, M. and {Halpern}, M. and {Hatziminaoglou}, E. and {Ibar}, E. and {Isaak}, K. and {Ivison}, R.~J. and {Lagache}, G. and {Levenson}, L. and {Lu}, N. and {Madden}, S. and {Maffei}, B. and {Mainetti}, G. and {Marchetti}, L. and {Mitchell-Wynne}, K. and {Mortier}, A.~M.~J. and {Nguyen}, H.~T. and {O'Halloran}, B. and {Omont}, A. and {Page}, M.~J. and {Panuzzo}, P. and {Papageorgiou}, A. and {Pearson}, C.~P. and {P{\'e}rez-Fournon}, I. and {Pohlen}, M. and {Rawlings}, J.~I. and {Raymond}, G. and {Rigopoulou}, D. and {Rizzo}, D. and {Roseboom}, I.~G. and {Rowan-Robinson}, M. and {S{\'a}nchez Portal}, M. and {Savage}, R. and {Schulz}, B. and {Scott}, D. and {Seymour}, N. and {Shupe}, D.~L. and {Stevens}, J.~A. and {Symeonidis}, M. and {Trichas}, M. and {Tugwell}, K.~E. and {Vaccari}, M. and {Valiante}, E. and {Valtchanov}, I. and {Vieira}, J.~D. and {Vigroux}, L. and {Ward}, R. and {Wright}, G. and {Xu}, C.~K. and {Zemcov}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/201014697},
	eprint = {1005.2184},
	journal = {\aap},
	keywords = {galaxies: evolution, submillimeter: galaxies, surveys},
	month = jul,
	pages = {L21+},
	primaryclass = {astro-ph.CO},
	title = {{HerMES: SPIRE galaxy number counts at 250, 350, and 500 {$\mu$}m}},
	volume = 518,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201014697}}

@article{ibar10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.401L..53I},
	archiveprefix = {arXiv},
	author = {{Ibar}, E. and {Ivison}, R.~J. and {Best}, P.~N. and {Coppin}, K. and {Pope}, A. and {Smail}, I. and {Dunlop}, J.~S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1745-3933.2009.00786.x},
	eprint = {0911.1954},
	journal = {\mnras},
	keywords = {galaxies: evolution , infrared: galaxies , radio continuum: galaxies},
	month = jan,
	pages = {L53-L57},
	primaryclass = {astro-ph.CO},
	title = {{Deep multi-frequency radio imaging in the Lockman Hole - II. The spectral index of submillimetre galaxies}},
	volume = 401,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2009.00786.x}}

@article{granato04,
	adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004ApJ...600..580G&db_key=AST},
	author = {{Granato}, G.~L. and {De Zotti}, G. and {Silva}, L. and {Bressan}, A. and {Danese}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/379875},
	eprint = {arXiv:0307202},
	journal = {\apj},
	month = jan,
	pages = {580-594},
	title = {{A Physical Model for the Coevolution of QSOs and Their Spheroidal Hosts}},
	volume = {600},
	year = {2004},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/379875}}

@article{granato02,
	adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002Ap%26SS.281..497G&db_key=AST},
	author = {{Granato}, G.~L. and {DeZotti}, G. and {Silva}, L. and {Danese}, L. and {Magliocchetti}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\apss},
	pages = {497-500},
	title = {{The Connection between Spheroidal Galaxies and QSOs}},
	volume = {281},
	year = {2002}}

@article{sanders88,
	adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988ApJ...328L..35S&db_key=AST},
	author = {{Sanders}, D.~B. and {Soifer}, B.~T. and {Elias}, J.~H. and {Neugebauer}, G. and {Matthews}, K.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/185155},
	journal = {\apjl},
	month = may,
	pages = {L35-L39},
	title = {{Warm ultraluminous galaxies in the IRAS survey - The transition from galaxy to quasar?}},
	volume = {328},
	year = {1988},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/185155}}

@article{fanti95,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...302..317F},
	author = {{Fanti}, C. and {Fanti}, R. and {Dallacasa}, D. and {Schilizzi}, R.~T. and {Spencer}, R.~E. and {Stanghellini}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\aap},
	keywords = {GALAXIES: ACTIVE, QUASARS: GENERAL, GALAXIES: EVOLUTION, RADIO CONTINUUM: GALAXIES},
	month = oct,
	pages = {317-+},
	title = {{Are compact steep-spectrum sources young?}},
	volume = 302,
	year = 1995}

@article{dimatteo05,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005Natur.433..604D},
	author = {{Di Matteo}, T. and {Springel}, V. and {Hernquist}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1038/nature03335},
	eprint = {arXiv:astro-ph/0502199},
	journal = {\nat},
	month = feb,
	pages = {604-607},
	title = {{Energy input from quasars regulates the growth and activity of black holes and their host galaxies}},
	volume = 433,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature03335}}

@article{cirasuolo03a,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.341..993C},
	author = {{Cirasuolo}, M. and {Magliocchetti}, M. and {Celotti}, A. and {Danese}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2003.06485.x},
	eprint = {arXiv:astro-ph/0301526},
	journal = {\mnras},
	keywords = {galaxies: active, quasars: general, cosmology: observations},
	month = may,
	pages = {993-1004},
	title = {{The radio-loud/radio-quiet dichotomy: news from the 2dF QSO Redshift Survey}},
	volume = 341,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2003.06485.x}}

@article{cirasuolo03b,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.346..447C},
	author = {{Cirasuolo}, M. and {Celotti}, A. and {Magliocchetti}, M. and {Danese}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-2966.2003.07105.x},
	eprint = {arXiv:astro-ph/0306415},
	journal = {\mnras},
	keywords = {galaxies: active, cosmology: observations, radio continuum: general},
	month = dec,
	pages = {447-455},
	title = {{Is there a dichotomy in the radio loudness distribution of quasars?}},
	volume = 346,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-2966.2003.07105.x}}

@article{davies06,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.370.1125D},
	author = {{Davies}, R.~D. and {Dickinson}, C. and {Banday}, A.~J. and {Jaffe}, T.~R. and {G{\'o}rski}, K.~M. and {Davis}, R.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2006.10572.x},
	eprint = {arXiv:astro-ph/0511384},
	journal = {\mnras},
	keywords = {radiation mechanisms: general: cosmic microwave background: cosmology: observations: diffuse radiation: radio continuum: ISM, radiation mechanisms: general, cosmic microwave background, cosmology: observations, diffuse radiation, radio continuum: ISM},
	month = aug,
	pages = {1125-1139},
	title = {{A determination of the spectra of Galactic components observed by the Wilkinson Microwave Anisotropy Probe}},
	volume = 370,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10572.x}}

@article{begelman04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004cbhg.symp..374B},
	author = {{Begelman}, M.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {arXiv:astro-ph/0303040},
	journal = {Coevolution of Black Holes and Galaxies},
	pages = {374-+},
	title = {{AGN Feedback Mechanisms}},
	year = 2004}

@article{shin10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...711..268S},
	archiveprefix = {arXiv},
	author = {{Shin}, M.-S. and {Ostriker}, J.~P. and {Ciotti}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/711/1/268},
	eprint = {0905.4294},
	journal = {\apj},
	keywords = {galaxies: active, galaxies: evolution, galaxies: formation, galaxies: nuclei, methods: numerical},
	month = mar,
	pages = {268-283},
	primaryclass = {astro-ph.GA},
	title = {{Feedback from Central Black Holes in Elliptical Galaxies. II. Can Purely Mechanical Energy Feedback Models Work?}},
	volume = 711,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/711/1/268}}

@article{ciotti09,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...699...89C},
	archiveprefix = {arXiv},
	author = {{Ciotti}, L. and {Ostriker}, J.~P. and {Proga}, D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/699/1/89},
	eprint = {0901.1089},
	journal = {\apj},
	keywords = {accretion, accretion disks, black hole physics, galaxies: active, galaxies: nuclei, galaxies: starburst, quasars: general},
	month = jul,
	pages = {89-104},
	primaryclass = {astro-ph.GA},
	title = {{Feedback from Central Black Holes in Elliptical Galaxies. I. Models with Either Radiative or Mechanical Feedback but not Both}},
	volume = 699,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/699/1/89}}

@article{ciotti07,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...665.1038C},
	author = {{Ciotti}, L. and {Ostriker}, J.~P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/519833},
	eprint = {arXiv:astro-ph/0703057},
	journal = {\apj},
	keywords = {Accretion, Accretion Disks, Black Hole Physics, Galaxies: Active, Galaxies: Nuclei, Galaxies: Starburst, Galaxies: Quasars: General},
	month = aug,
	pages = {1038-1056},
	title = {{Radiative Feedback from Massive Black Holes in Elliptical Galaxies: AGN Flaring and Central Starburst Fueled by Recycled Gas}},
	volume = 665,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/519833}}

@article{condon92,
	adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1992ARA%26A..30..575C},
	author = {{Condon}, J.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1146/annurev.aa.30.090192.003043},
	journal = {\araa},
	pages = {575-611},
	title = {{Radio emission from normal galaxies}},
	volume = {30},
	year = {1992},
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.aa.30.090192.003043}}

@article{nesvadba06,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...650..693N},
	author = {{Nesvadba}, N.~P.~H. and {Lehnert}, M.~D. and {Eisenhauer}, F. and {Gilbert}, A. and {Tecza}, M. and {Abuter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/507266},
	eprint = {arXiv:astro-ph/0606530},
	journal = {\apj},
	keywords = {Cosmology: Observations, Galaxies: Evolution, Galaxies: Kinematics and Dynamics, Infrared: Galaxies},
	month = oct,
	pages = {693-705},
	title = {{Extreme Gas Kinematics in the z=2.2 Powerful Radio Galaxy MRC 1138-262: Evidence for Efficient Active Galactic Nucleus Feedback in the Early Universe?}},
	volume = 650,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/507266}}

@article{murray05,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...618..569M},
	author = {{Murray}, N. and {Quataert}, E. and {Thompson}, T.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/426067},
	eprint = {arXiv:astro-ph/0406070},
	journal = {\apj},
	keywords = {Galaxies: Formation, Galaxies: Fundamental Parameters, Galaxies: General, Galaxies: Starburst, Galaxies: Intergalactic Medium},
	month = jan,
	pages = {569-585},
	title = {{On the Maximum Luminosity of Galaxies and Their Central Black Holes: Feedback from Momentum-driven Winds}},
	volume = 618,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/426067}}

@article{Maiolino:1998,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...338..781M},
	author = {{Maiolino}, R. and {Salvati}, M. and {Bassani}, L. and {Dadina}, M. and {della Ceca}, R. and {Matt}, G. and {Risaliti}, G. and {Zamorani}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {arXiv:astro-ph/9806055},
	journal = {\aap},
	keywords = {X-RAYS: GALAXIES, GALAXIES: SEYFERT, GALAXIES: ACTIVE},
	month = oct,
	pages = {781-794},
	title = {{Heavy obscuration in X-ray weak AGNs}},
	volume = 338,
	year = 1998}

@article{Turner:1997,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...488..164T},
	author = {{Turner}, T.~J. and {George}, I.~M. and {Nandra}, K. and {Mushotzky}, R.~F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/304701},
	eprint = {arXiv:astro-ph/9705087},
	journal = {\apj},
	keywords = {GALAXIES: ACTIVE, GALAXIES: NUCLEI, LINE: FORMATION, X-RAYS: GALAXIES},
	month = oct,
	pages = {164-+},
	title = {{ASCA Observations of Type 2 Seyfert Galaxies. II. The Importance of X-Ray Scattering and Reflection}},
	volume = 488,
	year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/304701}}

@article{Smith:1996,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1996MNRAS.280..355S},
	author = {{Smith}, D.~A. and {Done}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\mnras},
	keywords = {ACCRETION, ACCRETION DISCS, GALAXIES: NUCLEI, GALAXIES: SEYFERT, X-RAYS: GALAXIES},
	month = may,
	pages = {355-377},
	title = {{Unified theories of active galactic nuclei: a hard X-ray sample of Seyfert 2 galaxies}},
	volume = 280,
	year = 1996}

@article{Sajina:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...683..659S},
	author = {{Sajina}, A. and {Yan}, L. and {Lutz}, D. and {Steffen}, A. and {Helou}, G. and {Huynh}, M. and {Frayer}, D. and {Choi}, P. and {Tacconi}, L. and {Dasyra}, K.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/589914},
	journal = {\apj},
	keywords = {Galaxies: Active, Infrared: Galaxies, Galaxies: Quasars: General, Radio Continuum: Galaxies},
	month = aug,
	pages = {659-682},
	title = {{Spitzer Mid-Infrared Spectroscopy of Infrared Luminous Galaxies at z \~{} 2. III. Far-IR to Radio Properties and Optical Spectral Diagnostics}},
	volume = 683,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/589914}}

@article{Kovacs:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...650..592K},
	author = {{Kov{\'a}cs}, A. and {Chapman}, S.~C. and {Dowell}, C.~D. and {Blain}, A.~W. and {Ivison}, R.~J. and {Smail}, I. and {Phillips}, T.~G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/506341},
	eprint = {arXiv:astro-ph/0604591},
	journal = {\apj},
	keywords = {Galaxies: Evolution, Galaxies: High-Redshift, Galaxies: ISM, Galaxies: Photometry, Galaxies: Starburst, Infrared: Galaxies, Submillimeter},
	month = oct,
	pages = {592-603},
	title = {{SHARC-2 350 {$\mu$}m Observations of Distant Submillimeter-selected Galaxies}},
	volume = 650,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/506341}}

@article{Yun:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...554..803Y},
	author = {{Yun}, M.~S. and {Reddy}, N.~A. and {Condon}, J.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/323145},
	eprint = {arXiv:astro-ph/0102154},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Luminosity Function, Mass Function, Galaxies: Starburst, Infrared: Galaxies, Radio Continuum: Galaxies, Surveys},
	month = jun,
	pages = {803-822},
	title = {{Radio Properties of Infrared-selected Galaxies in the IRAS 2 Jy Sample}},
	volume = 554,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/323145}}

@article{Strazzullo:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...714.1305S},
	archiveprefix = {arXiv},
	author = {{Strazzullo}, V. and {Pannella}, M. and {Owen}, F.~N. and {Bender}, R. and {Morrison}, G.~E. and {Wang}, {W.-H.} and {Shupe}, D.~L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/714/2/1305},
	eprint = {1003.4734},
	journal = {\apj},
	keywords = {cosmology: observations, galaxies: active, galaxies: evolution, galaxies: starburst, radio continuum: galaxies},
	month = may,
	pages = {1305-1323},
	primaryclass = {astro-ph.CO},
	title = {{The Deep Swire Field. IV. First Properties of the sub-mJy Galaxy Population: Redshift Distribution, AGN Activity, and Star Formation}},
	volume = 714,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/714/2/1305}}

@article{Ueda:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ApJS..179..124U},
	archiveprefix = {arXiv},
	author = {{Ueda}, Y. and {Watson}, M.~G. and {Stewart}, I.~M. and {Akiyama}, M. and {Schwope}, A.~D. and {Lamer}, G. and {Ebrero}, J. and {Carrera}, F.~J. and {Sekiguchi}, K. and {Yamada}, T. and {Simpson}, C. and {Hasinger}, G. and {Mateos}, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/591083},
	eprint = {0806.2846},
	journal = {\apjs},
	keywords = {Catalogs, Cosmology: Diffuse Radiation, Galaxies: Active, X-Rays: Galaxies, X-Rays: General},
	month = nov,
	pages = {124-141},
	title = {{The Subaru/XMM-Newton Deep Survey (SXDS). III. X-Ray Data}},
	volume = 179,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/591083}}

@article{Simpson:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.372..741S},
	author = {{Simpson}, C. and {Mart{\'{\i}}nez-Sansigre}, A. and {Rawlings}, S. and {Ivison}, R. and {Akiyama}, M. and {Sekiguchi}, K. and {Takata}, T. and {Ueda}, Y. and {Watson}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2006.10907.x},
	eprint = {arXiv:astro-ph/0609529},
	journal = {\mnras},
	keywords = {catalogues, surveys, galaxies: active, radio continuum: galaxies},
	month = oct,
	pages = {741-757},
	title = {{Radio imaging of the Subaru/XMM-Newton Deep Field - I. The 100-{$\mu$}Jy catalogue, optical identifications, and the nature of the faint radio source population}},
	volume = 372,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10907.x}}

@article{Fadda:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004AJ....128....1F},
	author = {{Fadda}, D. and {Jannuzi}, B.~T. and {Ford}, A. and {Storrie-Lombardi}, L.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/421366},
	eprint = {arXiv:astro-ph/0403490},
	journal = {\aj},
	keywords = {Catalogs, Galaxies: Photometry},
	month = jul,
	pages = {1-15},
	title = {{The Spitzer Space Telescope First-Look Survey: KPNO Mosaic-1 R-Band Images and Source Catalogs}},
	volume = 128,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/421366}}

@article{Georgakakis:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.354..127G},
	author = {{Georgakakis}, A. and {Hopkins}, A.~M. and {Afonso}, J. and {Sullivan}, M. and {Mobasher}, B. and {Cram}, L.~E.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2004.08174.x},
	eprint = {arXiv:astro-ph/0407078},
	journal = {\mnras},
	keywords = {surveys, galaxies: general, X-rays: galaxies, X-rays: general},
	month = oct,
	pages = {127-141},
	title = {{The Phoenix Deep Survey: the radio properties of the hard X-ray-selected sample}},
	volume = 354,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.08174.x}}

@article{Ciliegi:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.342..575C},
	author = {{Ciliegi}, P. and {Vignali}, C. and {Comastri}, A. and {Fiore}, F. and {La Franca}, F. and {Perola}, G.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2003.06573.x},
	eprint = {arXiv:astro-ph/0302556},
	journal = {\mnras},
	keywords = {surveys, quasars: general, radio continuum: galaxies},
	month = jun,
	pages = {575-586},
	title = {{The BeppoSAX High Energy Large Area Survey (HELLAS) - VI. The radio properties}},
	volume = 342,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2003.06573.x}}

@article{Barger:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001AJ....122.2177B},
	author = {{Barger}, A.~J. and {Cowie}, L.~L. and {Bautz}, M.~W. and {Brandt}, W.~N. and {Garmire}, G.~P. and {Hornschemeier}, A.~E. and {Ivison}, R.~J. and {Owen}, F.~N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/323454},
	eprint = {arXiv:astro-ph/0106219},
	journal = {\aj},
	keywords = {Cosmology: Observations, Galaxies: Active, Galaxies: Distances and Redshifts, Galaxies: Evolution, Galaxies: Formation},
	month = nov,
	pages = {2177-2189},
	title = {{Supermassive Black Hole Accretion History Inferred from a Large Sample of Chandra Hard X-Ray Sources}},
	volume = 122,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/323454}}

@article{Ibar:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386..953I},
	archiveprefix = {arXiv},
	author = {{Ibar}, E. and {Cirasuolo}, M. and {Ivison}, R. and {Best}, P. and {Smail}, I. and {Biggs}, A. and {Simpson}, C. and {Dunlop}, J. and {Almaini}, O. and {McLure}, R. and {Foucaud}, S. and {Rawlings}, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.13077.x},
	eprint = {0802.2694},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: fundamental parameters, galaxies: high-redshift, galaxies: starburst},
	month = may,
	pages = {953-962},
	title = {{Exploring the infrared/radio correlation at high redshift}},
	volume = 386,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13077.x}}

@article{Garn:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.394..105G},
	archiveprefix = {arXiv},
	author = {{Garn}, T. and {Alexander}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.14296.x},
	eprint = {0812.0281},
	journal = {\mnras},
	keywords = {infrared: galaxies , radio continuum: galaxies},
	month = mar,
	pages = {105-116},
	title = {{Radio source stacking and the infrared/radio correlation at {$\mu$}Jy flux densities}},
	volume = 394,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.14296.x}}

@article{Beswick:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.385.1143B},
	archiveprefix = {arXiv},
	author = {{Beswick}, R.~J. and {Muxlow}, T.~W.~B. and {Thrall}, H. and {Richards}, A.~M.~S. and {Garrington}, S.~T.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.12931.x},
	eprint = {0801.1035},
	journal = {\mnras},
	keywords = {galaxies: high-redshift , galaxies: starburst , infrared: galaxies , radio continuum: galaxies},
	month = apr,
	pages = {1143-1154},
	title = {{An evolution of the infrared-radio correlation at very low flux densities?}},
	volume = 385,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.12931.x}}

@article{ElBouchefry:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.396.2011E},
	archiveprefix = {arXiv},
	author = {{El Bouchefry}, K.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2009.14915.x},
	eprint = {0904.2586},
	journal = {\mnras},
	keywords = {galaxies: active , galaxies: high-redshift , X-rays: diffuse background , X-rays: galaxies},
	month = jul,
	pages = {2011-2037},
	primaryclass = {astro-ph.CO},
	title = {{X-ray identifications of FIRST radio sources in the XBo{\"o}tes field}},
	volume = 396,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.14915.x}}

@article{Brusa:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...409...65B},
	author = {{Brusa}, M. and {Comastri}, A. and {Mignoli}, M. and {Fiore}, F. and {Ciliegi}, P. and {Vignali}, C. and {Severgnini}, P. and {Cocchia}, F. and {La Franca}, F. and {Matt}, G. and {Perola}, G.~C. and {Maiolino}, R. and {Baldi}, A. and {Molendi}, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20031107},
	eprint = {arXiv:astro-ph/0307368},
	journal = {\aap},
	keywords = {surveys, galaxies: active, X-ray: galaxies, X-ray: diffuse background},
	month = oct,
	pages = {65-78},
	title = {{The HELLAS2XMM survey. III. Multiwavelength observations of hard X-ray selected sources in the PKS 0312-77 field}},
	volume = 409,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031107}}

@article{Smolcic:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ApJS..177...14S},
	archiveprefix = {arXiv},
	author = {{Smol{\v c}i{\'c}}, V. and {Schinnerer}, E. and {Scodeggio}, M. and {Franzetti}, P. and {Aussel}, H. and {Bondi}, M. and {Brusa}, M. and {Carilli}, C.~L. and {Capak}, P. and {Charlot}, S. and {Ciliegi}, P. and {Ilbert}, O. and {Ivezi{\'c}}, {\v Z}. and {Jahnke}, K. and {McCracken}, H.~J. and {Obri{\'c}}, M. and {Salvato}, M. and {Sanders}, D.~B. and {Scoville}, N. and {Trump}, J.~R. and {Tremonti}, C. and {Tasca}, L. and {Walcher}, C.~J. and {Zamorani}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/588028},
	eprint = {0803.0997},
	journal = {\apjs},
	keywords = {Cosmology: Observations, Radio Continuum: Galaxies, Surveys},
	month = jul,
	pages = {14-38},
	title = {{A New Method to Separate Star-forming from AGN Galaxies at Intermediate Redshift: The Submillijansky Radio Population in the VLA-COSMOS Survey}},
	volume = 177,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/588028}}

@inproceedings{vanBreugel:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999ldss.work..236V},
	author = {{van Breugel}, W. and {De Breuck}, C. and {R{\"o}ttgering}, H. and {Miley}, G. and {Stanford}, A.},
	booktitle = {Looking Deep in the Southern Sky},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{R.~Morganti; W.~J.~Couch}},
	eprint = {arXiv:astro-ph/9806135},
	pages = {236},
	title = {{Very High Redshift Radio Galaxies}},
	year = 1999}

@article{Lusso:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...512A..34L},
	archiveprefix = {arXiv},
	author = {{Lusso}, E. and {Comastri}, A. and {Vignali}, C. and {Zamorani}, G. and {Brusa}, M. and {Gilli}, R. and {Iwasawa}, K. and {Salvato}, M. and {Civano}, F. and {Elvis}, M. and {Merloni}, A. and {Bongiorno}, A. and {Trump}, J.~R. and {Koekemoer}, A.~M. and {Schinnerer}, E. and {Le Floc'h}, E. and {Cappelluti}, N. and {Jahnke}, K. and {Sargent}, M. and {Silverman}, J. and {Mainieri}, V. and {Fiore}, F. and {Bolzonella}, M. and {Le F{\`e}vre}, O. and {Garilli}, B. and {Iovino}, A. and {Kneib}, J.~P. and {Lamareille}, F. and {Lilly}, S. and {Mignoli}, M. and {Scodeggio}, M. and {Vergani}, D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361/200913298},
	eprint = {0912.4166},
	journal = {\aap},
	keywords = {galaxies: active, Galaxy: evolution, quasars: general, methods: statistical},
	month = mar,
	pages = {A34+},
	primaryclass = {astro-ph.CO},
	title = {{The X-ray to optical-UV luminosity ratio of X-ray selected type 1 AGN in XMM-COSMOS}},
	volume = 512,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200913298}}

@article{deBreuck:2000,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2000A%26AS..143..303D},
	author = {{De Breuck}, C. and {van Breugel}, W. and {R{\"o}ttgering}, H.~J.~A. and {Miley}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/aas:2000181},
	eprint = {arXiv:astro-ph/0002297},
	journal = {\aaps},
	keywords = {SURVEYS, GALAXIES: ACTIVE, RADIO CONTINUUM: GALAXIES},
	month = apr,
	pages = {303-333},
	title = {{A sample of 669 ultra steep spectrum radio sources to find high redshift radio galaxies}},
	volume = 143,
	year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/aas:2000181}}

@article{Nesvadba:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...491..407N},
	archiveprefix = {arXiv},
	author = {{Nesvadba}, N.~P.~H. and {Lehnert}, M.~D. and {De Breuck}, C. and {Gilbert}, A.~M. and {van Breugel}, W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:200810346},
	eprint = {0809.5171},
	journal = {\aap},
	keywords = {galaxies: high-redshift, galaxies: formation, galaxies: jets, infrared: galaxies, galaxies: kinematics and dynamics},
	month = nov,
	pages = {407-424},
	title = {{Evidence for powerful AGN winds at high redshift: dynamics of galactic outflows in radio galaxies during the ``Quasar Era''}},
	volume = 491,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200810346}}

@article{Nesvadba:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...475..145N},
	archiveprefix = {arXiv},
	author = {{Nesvadba}, N.~P.~H. and {Lehnert}, M.~D. and {De Breuck}, C. and {Gilbert}, A. and {van Breugel}, W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20078175},
	eprint = {0708.4150},
	journal = {\aap},
	keywords = {galaxies: high-redshift, galaxies: formation, galaxies: kinematics and dynamics, infrared: galaxies, galaxies: jets},
	month = nov,
	pages = {145-153},
	title = {{Compact radio sources and jet-driven AGN feedback in the early universe: constraints from integral-field spectroscopy}},
	volume = 475,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078175}}

@article{Komissarov:1994,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1994A%26A...285...27K},
	author = {{Komissarov}, S.~S. and {Gubanov}, A.~G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\aap},
	keywords = {GALAXIES: CLUSTERS OF, GALAXIES: ACTIVE, RADIATION MECHANISMS: NON THERMAL, RADIO CONTINUUM: GALAXIES},
	month = may,
	pages = {27-43},
	title = {{Relic radio galaxies: evolution of synchrotron spectrum}},
	volume = 285,
	year = 1994}

@article{Murgia:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1011.0567M},
	archiveprefix = {arXiv},
	author = {{Murgia}, M. and {Parma}, P. and {Mack}, {K.~-.} and {de Ruiter}, H.~R. and {Fanti}, R. and {Govoni}, F. and {Tarchi}, A. and {Giacintucci}, S. and {Markevitch}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {1011.0567},
	journal = {ArXiv e-prints},
	keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
	month = nov,
	primaryclass = {astro-ph.CO},
	title = {{Dying Radio Sources in Clusters}},
	year = 2010}

@book{Longair:1992,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1992hea..book.....L},
	author = {{Longair}, M.~S.},
	booktitle = {High Energy Astrophysics, by Malcolm S.~Longair, pp.~436.~ISBN 0521387736.~Cambridge, UK: Cambridge University Press, March 1992.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{Willcox, P.~J.}},
	month = mar,
	title = {{High energy astrophysics. Vol.1: Particles, photons and their detection}},
	year = 1992}

@article{Barger:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002AJ....124.1839B},
	author = {{Barger}, A.~J. and {Cowie}, L.~L. and {Brandt}, W.~N. and {Capak}, P. and {Garmire}, G.~P. and {Hornschemeier}, A.~E. and {Steffen}, A.~T. and {Wehner}, E.~H.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/342448},
	eprint = {arXiv:astro-ph/0206370},
	journal = {\aj},
	keywords = {Cosmology: Observations, Galaxies: Evolution, Galaxies: Formation},
	month = oct,
	pages = {1839-1885},
	title = {{X-Ray, Optical, and Infrared Imaging and Spectral Properties of the 1 Ms Chandra Deep Field North Sources}},
	volume = 124,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/342448}}

@article{Trouille:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...703.2160T},
	archiveprefix = {arXiv},
	author = {{Trouille}, L. and {Barger}, A.~J. and {Cowie}, L.~L. and {Yang}, Y. and {Mushotzky}, R.~F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/703/2/2160},
	eprint = {0908.0002},
	journal = {\apj},
	keywords = {cosmology: observations, galaxies: active},
	month = oct,
	pages = {2160-2170},
	primaryclass = {astro-ph.CO},
	title = {{The OPTX Project. III. X-ray Versus Optical Spectral Type for Active Galactic Nuclei}},
	volume = 703,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/703/2/2160}}

@inproceedings{Panessa:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007AIPC..924..830P},
	author = {{Panessa}, F. and {Barcons}, X. and {Bassani}, L. and {Cappi}, M. and {Carrera}, F.~J. and {Dadina}, M. and {Ho}, L.~C. and {Iwasawa}, K. and {Pellegrini}, S.},
	booktitle = {The Multicolored Landscape of Compact Objects and Their Explosive Origins},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1063/1.2774949},
	editor = {{T.~di Salvo, G.~L.~Israel, L.~Piersant, L.~Burderi, G.~Matt, A.~Tornambe, \&amp; M.~T.~Menna}},
	eprint = {arXiv:astro-ph/0612593},
	keywords = {Active and peculiar galaxies and related systems, X-ray sources; X-ray bursts, Galactic nuclei , circumnuclear matter, and bulges, Magnitudes and colors; luminosities},
	month = aug,
	pages = {830-835},
	series = {American Institute of Physics Conference Series},
	title = {{Multi-wavelength and black hole mass properties of Low Luminosity Active Nuclei}},
	volume = 924,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1063/1.2774949}}

@article{Sikora:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...658..815S},
	author = {{Sikora}, M. and {Stawarz}, {\L}. and {Lasota}, {J.-P.}},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/511972},
	eprint = {arXiv:astro-ph/0604095},
	journal = {\apj},
	keywords = {Galaxies: Jets, Magnetohydrodynamics: MHD, Radiation Mechanisms: Nonthermal},
	month = apr,
	pages = {815-828},
	title = {{Radio Loudness of Active Galactic Nuclei: Observational Facts and Theoretical Implications}},
	volume = 658,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/511972}}

@article{Ho:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...564..120H},
	author = {{Ho}, L.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/324399},
	eprint = {arXiv:astro-ph/0110440},
	journal = {\apj},
	keywords = {Black Hole Physics, Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, Galaxies: Quasars: General, Radio Continuum: Galaxies},
	month = jan,
	pages = {120-132},
	title = {{On the Relationship between Radio Emission and Black Hole Mass in Galactic Nuclei}},
	volume = 564,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/324399}}

@article{Ishibashi:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1010.5591I},
	archiveprefix = {arXiv},
	author = {{Ishibashi}, W. and {Courvoisier}, {T.~J.~-.}},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {1010.5591},
	journal = {ArXiv e-prints},
	keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Galaxy Astrophysics},
	month = oct,
	primaryclass = {astro-ph.HE},
	title = {{Synchrotron radio emission in radio-quiet AGNs}},
	year = 2010}

@article{Ulvestad:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...621..123U},
	author = {{Ulvestad}, J.~S. and {Antonucci}, R.~R.~J. and {Barvainis}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/427426},
	eprint = {arXiv:astro-ph/0411678},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Quasars: General, Radio Continuum: Galaxies},
	month = mar,
	pages = {123-129},
	title = {{VLBA Imaging of Central Engines in Radio-Quiet Quasars}},
	volume = 621,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/427426}}

@article{Debuhr:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1006.3312D},
	archiveprefix = {arXiv},
	author = {{DeBuhr}, J. and {Quataert}, E. and {Ma}, {C.-P.}},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {1006.3312},
	journal = {ArXiv e-prints},
	keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
	month = jun,
	primaryclass = {astro-ph.CO},
	title = {{The Growth of Massive Black Holes in Galaxy Merger Simulations with Feedback by Radiation Pressure}},
	year = 2010}

@article{Wilkes:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009ApJS..185..433W},
	archiveprefix = {arXiv},
	author = {{Wilkes}, B.~J. and {Kilgard}, R. and {Kim}, {D.-W.} and {Kim}, M. and {Polletta}, M. and {Lonsdale}, C. and {Smith}, H.~E. and {Surace}, J. and {Owen}, F.~N. and {Franceschini}, A. and {Siana}, B. and {Shupe}, D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0067-0049/185/2/433},
	eprint = {0910.2675},
	journal = {\apjs},
	keywords = {catalogs, quasars: general, surveys, X-rays: galaxies},
	month = dec,
	pages = {433-450},
	primaryclass = {astro-ph.HE},
	title = {{The SWIRE/Chandra Survey: The X-ray Sources}},
	volume = 185,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/185/2/433}}

@article{Page:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.369..156P},
	author = {{Page}, M.~J. and {Loaring}, N.~S. and {Dwelly}, T. and {Mason}, K.~O. and {McHardy}, I. and {Gunn}, K. and {Moss}, D. and {Sasseen}, T. and {Cordova}, F. and {Kennea}, J. and {Seymour}, N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2006.10278.x},
	eprint = {arXiv:astro-ph/0604015},
	journal = {\mnras},
	keywords = {surveys: galaxies: active: quasars: general: X-rays: galaxies, surveys, galaxies: active, quasars: general, X-rays: galaxies},
	month = jun,
	pages = {156-170},
	title = {{X-ray spectra of sources in the 13^{H} XMM-Newton/Chandra deep field}},
	volume = 369,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10278.x}}

@article{Jamrozy:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.378..581J},
	author = {{Jamrozy}, M. and {Konar}, C. and {Saikia}, D.~J. and {Stawarz}, {\L}. and {Mack}, {K.-H.} and {Siemiginowska}, A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2007.11782.x},
	eprint = {arXiv:astro-ph/0703723},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: individual: 4C29.30, galaxies: nuclei, radio continuum: galaxies},
	month = jun,
	pages = {581-593},
	title = {{Intermittent jet activity in the radio galaxy 4C29.30?}},
	volume = 378,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.11782.x}}

@article{Lal:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.374.1085L},
	author = {{Lal}, D.~V. and {Rao}, A.~P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2006.11225.x},
	eprint = {arXiv:astro-ph/0610678},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: formation, radio continuum: galaxies},
	month = jan,
	pages = {1085-1102},
	title = {{Giant Metrewave Radio Telescope observations of X-shaped radio sources}},
	volume = 374,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.11225.x}}

@article{Jamrozy:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...427...79J},
	author = {{Jamrozy}, M. and {Klein}, U. and {Mack}, {K.-H.} and {Gregorini}, L. and {Parma}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20048056},
	journal = {\aap},
	keywords = {radio continuum: galaxies, galaxies: active, galaxies: individual: B2 0924+30},
	month = nov,
	pages = {79-86},
	title = {{Spectral ageing in the relic radio galaxy B2 0924+30}},
	volume = 427,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20048056}}

@article{Parma:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...470..875P},
	archiveprefix = {arXiv},
	author = {{Parma}, P. and {Murgia}, M. and {de Ruiter}, H.~R. and {Fanti}, R. and {Mack}, {K.-H.} and {Govoni}, F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20077592},
	eprint = {0705.3209},
	journal = {\aap},
	keywords = {radio continuum: galaxies, galaxies: active},
	month = aug,
	pages = {875-888},
	title = {{In search of dying radio sources in the local universe}},
	volume = 470,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077592}}

@article{Fanti:1990,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1990A%26A...231..333F},
	author = {{Fanti}, R. and {Fanti}, C. and {Schilizzi}, R.~T. and {Spencer}, R.~E. and {Nan Rendong} and {Parma}, P. and {van Breugel}, W.~J.~M. and {Venturi}, T.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\aap},
	keywords = {QUASARS, RADIO JETS (ASTRONOMY), RADIO SOURCES (ASTRONOMY), RADIO SPECTRA, COSMOLOGY, VERY LARGE ARRAY (VLA), VERY LONG BASE INTERFEROMETRY},
	month = may,
	pages = {333-346},
	title = {{On the nature of compact steep spectrum radio sources}},
	volume = 231,
	year = 1990}

@article{Tajer:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...467...73T},
	author = {{Tajer}, M. and {Polletta}, M. and {Chiappetti}, L. and {Maraschi}, L. and {Trinchieri}, G. and {Maccagni}, D. and {Andreon}, S. and {Garcet}, O. and {Surdej}, J. and {Pierre}, M. and {Le F{\`e}vre}, O. and {Franceschini}, A. and {Lonsdale}, C.~J. and {Surace}, J.~A. and {Shupe}, D.~L. and {Fang}, F. and {Rowan-Robinson}, M. and {Smith}, H.~E. and {Tresse}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20066667},
	eprint = {arXiv:astro-ph/0703263},
	journal = {\aap},
	keywords = {X-rays: general, surveys, galaxies: active},
	month = may,
	pages = {73-91},
	title = {{Obscured and unobscured AGN populations in a hard-X-ray selected sample of the XMDS survey}},
	volume = 467,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20066667}}

@inproceedings{Prandoni:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009pra..confE..36P},
	author = {{Prandoni}, I. and {Morganti}, R. and {Mignano}, A.},
	booktitle = {Panoramic Radio Astronomy: Wide-field 1-2 GHz Research on Galaxy Evolution},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	title = {{The AGN component in radio deep fields: the First Look Survey}},
	year = 2009}

@article{allen06,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.372...21A},
	author = {{Allen}, S.~W. and {Dunn}, R.~J.~H. and {Fabian}, A.~C. and {Taylor}, G.~B. and {Reynolds}, C.~S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:49:32 +0200},
	doi = {10.1111/j.1365-2966.2006.10778.x},
	eprint = {arXiv:astro-ph/0602549},
	journal = {\mnras},
	keywords = {accretion, accretion discs: black hole physics: galaxies: active: galaxies: jets: X-rays: galaxies, accretion discs, black hole physics, galaxies: active, galaxies: jets, X-rays: galaxies},
	month = oct,
	pages = {21-30},
	title = {{The relation between accretion rate and jet power in X-ray luminous elliptical galaxies}},
	volume = 372,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10778.x}}

@article{Ogle:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...647..161O},
	author = {{Ogle}, P. and {Whysong}, D. and {Antonucci}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/505337},
	eprint = {arXiv:astro-ph/0601485},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Jets, Infrared: Galaxies, Galaxies: Quasars: General},
	month = aug,
	pages = {161-171},
	title = {{Spitzer Reveals Hidden Quasar Nuclei in Some Powerful FR II Radio Galaxies}},
	volume = 647,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/505337}}

@article{Hardcastle:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.396.1929H},
	archiveprefix = {arXiv},
	author = {{Hardcastle}, M.~J. and {Evans}, D.~A. and {Croston}, J.~H.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2009.14887.x},
	eprint = {0904.1323},
	journal = {\mnras},
	keywords = {galaxies: active , X-rays: galaxies},
	month = jul,
	pages = {1929-1952},
	title = {{The active nuclei of z {\lt} 1.0 3CRR radio sources}},
	volume = 396,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.14887.x}}

@article{Hardcastle:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.376.1849H},
	author = {{Hardcastle}, M.~J. and {Evans}, D.~A. and {Croston}, J.~H.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2007.11572.x},
	eprint = {arXiv:astro-ph/0701857},
	journal = {\mnras},
	keywords = {galaxies: active, X-rays: galaxies},
	month = apr,
	pages = {1849-1856},
	title = {{Hot and cold gas accretion and feedback in radio-loud active galaxies}},
	volume = 376,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.11572.x}}

@article{Deyoung:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...710..743D},
	archiveprefix = {arXiv},
	author = {{De Young}, D.~S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/710/1/743},
	eprint = {1001.1178},
	journal = {\apj},
	keywords = {galaxies: active, galaxies: evolution, galaxies: jets, radio continuum: galaxies, turbulence},
	month = feb,
	pages = {743-754},
	title = {{How Does Radio AGN Feedback Feed Back?}},
	volume = 710,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/710/1/743}}

@article{Fabian:2000,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.318L..65F},
	author = {{Fabian}, A.~C. and {Sanders}, J.~S. and {Ettori}, S. and {Taylor}, G.~B. and {Allen}, S.~W. and {Crawford}, C.~S. and {Iwasawa}, K. and {Johnstone}, R.~M. and {Ogle}, P.~M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2000.03904.x},
	eprint = {arXiv:astro-ph/0007456},
	journal = {\mnras},
	keywords = {GALAXIES: CLUSTERS: INDIVIDUAL: PERSEUS, COOLING FLOWS, GALAXIES: INDIVIDUAL: NGC 1275, X-RAYS: GALAXIES},
	month = nov,
	pages = {L65-L68},
	title = {{Chandra imaging of the complex X-ray core of the Perseus cluster}},
	volume = 318,
	year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2000.03904.x}}

@article{Dimatteo:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005Natur.433..604D},
	author = {{Di Matteo}, T. and {Springel}, V. and {Hernquist}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1038/nature03335},
	eprint = {arXiv:astro-ph/0502199},
	journal = {\nat},
	month = feb,
	pages = {604-607},
	title = {{Energy input from quasars regulates the growth and activity of black holes and their host galaxies}},
	volume = 433,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature03335}}

@article{Croton:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.365...11C},
	author = {{Croton}, D.~J. and {Springel}, V. and {White}, S.~D.~M. and {De Lucia}, G. and {Frenk}, C.~S. and {Gao}, L. and {Jenkins}, A. and {Kauffmann}, G. and {Navarro}, J.~F. and {Yoshida}, N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2005.09675.x},
	eprint = {arXiv:astro-ph/0508046},
	journal = {\mnras},
	keywords = {black hole physics, galaxies: active, cooling flows, galaxies: evolution, galaxies: formation, cosmology: theory},
	month = jan,
	pages = {11-28},
	title = {{The many lives of active galactic nuclei: cooling flows, black holes and the luminosities and colours of galaxies}},
	volume = 365,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09675.x}}

@article{Fabian:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.308L..39F},
	author = {{Fabian}, A.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.1999.03017.x},
	eprint = {arXiv:astro-ph/9908064},
	journal = {\mnras},
	month = oct,
	pages = {L39-L43},
	title = {{The obscured growth of massive black holes}},
	volume = 308,
	year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1999.03017.x}}

@article{merloni08,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.388.1011M},
	archiveprefix = {arXiv},
	author = {{Merloni}, A. and {Heinz}, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:48:42 +0200},
	doi = {10.1111/j.1365-2966.2008.13472.x},
	eprint = {0805.2499},
	journal = {\mnras},
	keywords = {accretion, accretion discs , black hole physics , galaxies: active , galaxies: evolution , quasars: general},
	month = aug,
	pages = {1011-1030},
	title = {{A synthesis model for AGN evolution: supermassive black holes growth and feedback modes}},
	volume = 388,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13472.x}}

@article{Hopkins:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...669...67H},
	archiveprefix = {arXiv},
	author = {{Hopkins}, P.~F. and {Hernquist}, L. and {Cox}, T.~J. and {Robertson}, B. and {Krause}, E.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/521601},
	eprint = {0707.4005},
	journal = {\apj},
	keywords = {Cosmology: Theory, Galaxies: Active, Galaxies: Evolution, Galaxies: Quasars: General},
	month = nov,
	pages = {67-73},
	title = {{An Observed Fundamental Plane Relation for Supermassive Black Holes}},
	volume = 669,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/521601}}

@article{Tremaine:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...574..740T},
	author = {{Tremaine}, S. and {Gebhardt}, K. and {Bender}, R. and {Bower}, G. and {Dressler}, A. and {Faber}, S.~M. and {Filippenko}, A.~V. and {Green}, R. and {Grillmair}, C. and {Ho}, L.~C. and {Kormendy}, J. and {Lauer}, T.~R. and {Magorrian}, J. and {Pinkney}, J. and {Richstone}, D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/341002},
	eprint = {arXiv:astro-ph/0203468},
	journal = {\apj},
	keywords = {Black Hole Physics, Galaxies: Bulges, Galaxies: Fundamental Parameters, Galaxies: Nuclei, Galaxy: Bulge, Galaxy: Kinematics and Dynamics},
	month = aug,
	pages = {740-753},
	title = {{The Slope of the Black Hole Mass versus Velocity Dispersion Correlation}},
	volume = 574,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/341002}}

@article{Zakamska:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003AJ....126.2125Z},
	author = {{Zakamska}, N.~L. and {Strauss}, M.~A. and {Krolik}, J.~H. and {Collinge}, M.~J. and {Hall}, P.~B. and {Hao}, L. and {Heckman}, T.~M. and {Ivezi{\'c}}, {\v Z}. and {Richards}, G.~T. and {Schlegel}, D.~J. and {Schneider}, D.~P. and {Strateva}, I. and {Vanden Berk}, D.~E. and {Anderson}, S.~F. and {Brinkmann}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/378610},
	eprint = {arXiv:astro-ph/0309551},
	journal = {\aj},
	keywords = {Galaxies: Active, Galaxies: Quasars: Emission Lines, Galaxies: Quasars: General, Surveys},
	month = nov,
	pages = {2125-2144},
	title = {{Candidate Type II Quasars from the Sloan Digital Sky Survey. I. Selection and Optical Properties of a Sample at 0.3{\lt}Z{\lt}0.83}},
	volume = 126,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/378610}}

@article{Roussel:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...646..841R},
	author = {{Roussel}, H. and {Helou}, G. and {Smith}, J.~D. and {Draine}, B.~T. and {Hollenbach}, D.~J. and {Moustakas}, J. and {Spoon}, H.~W. and {Kennicutt}, R.~C. and {Rieke}, G.~H. and {Walter}, F. and {Armus}, L. and {Dale}, D.~A. and {Sheth}, K. and {Bendo}, G.~J. and {Engelbracht}, C.~W. and {Gordon}, K.~D. and {Meyer}, M.~J. and {Regan}, M.~W. and {Murphy}, E.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/505038},
	eprint = {arXiv:astro-ph/0604267},
	journal = {\apj},
	keywords = {ISM: Dust, Extinction, Galaxies: Evolution, Galaxies: Individual: NGC Number: NGC 1377, Galaxies: ISM, Galaxies: Starburst, Infrared: Galaxies},
	month = aug,
	pages = {841-857},
	title = {{The Opaque Nascent Starburst in NGC 1377: Spitzer SINGS Observations}},
	volume = 646,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/505038}}

@article{Urry:1995,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1995PASP..107..803U},
	author = {{Urry}, C.~M. and {Padovani}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/133630},
	eprint = {arXiv:astro-ph/9506063},
	journal = {\pasp},
	keywords = {GALAXIES: ACTIVE, GALAXIES: FUNDAMENTAL PARAMETERS},
	month = sep,
	pages = {803-+},
	title = {{Unified Schemes for Radio-Loud Active Galactic Nuclei}},
	volume = 107,
	year = 1995,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/133630}}

@inproceedings{Wilson:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003SPIE.4841..451W},
	author = {{Wilson}, J.~C. and {Eikenberry}, S.~S. and {Henderson}, C.~P. and {Hayward}, T.~L. and {Carson}, J.~C. and {Pirger}, B. and {Barry}, D.~J. and {Brandl}, B.~R. and {Houck}, J.~R. and {Fitzgerald}, G.~J. and {Stolberg}, T.~M.},
	booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1117/12.460336},
	editor = {{M.~Iye \& A.~F.~M.~Moorwood}},
	month = mar,
	pages = {451-458},
	series = {Presented at the Society of Photo-Optical Instrumentation Engineers (SPIE) Conference},
	title = {{A Wide-Field Infrared Camera for the Palomar 200-inch Telescope}},
	volume = 4841,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.460336}}

@article{Tueller:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010ApJS..186..378T},
	archiveprefix = {arXiv},
	author = {{Tueller}, J. and {Baumgartner}, W.~H. and {Markwardt}, C.~B. and {Skinner}, G.~K. and {Mushotzky}, R.~F. and {Ajello}, M. and {Barthelmy}, S. and {Beardmore}, A. and {Brandt}, W.~N. and {Burrows}, D. and {Chincarini}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0067-0049/186/2/378},
	eprint = {0903.3037},
	journal = {\apjs},
	keywords = {catalogs, galaxies: active, gamma rays: observations, novae, cataclysmic variables, surveys, X-rays: binaries},
	month = feb,
	pages = {378-405},
	title = {{The 22 Month Swift-BAT All-Sky Hard X-ray Survey}},
	volume = 186,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/186/2/378}}

@article{bird10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010ApJS..186....1B},
	archiveprefix = {arXiv},
	author = {{Bird}, A.~J. and {Bazzano}, A. and {Bassani}, L. and {Capitanio}, F. and {Fiocchi}, M. and {Hill}, A.~B. and {Malizia}, A. and {McBride}, V.~A. and {Scaringi}, S. and {Sguera}, V. and {Stephen}, J.~B. and {Ubertini}, P. and {Dean}, A.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:50:27 +0200},
	doi = {10.1088/0067-0049/186/1/1},
	eprint = {0910.1704},
	journal = {\apjs},
	keywords = {Galaxy: general, gamma rays: observations, surveys},
	month = jan,
	pages = {1-9},
	title = {{The Fourth IBIS/ISGRI Soft Gamma-ray Survey Catalog}},
	volume = 186,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/186/1/1}}

@article{Malizia:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.399..944M},
	archiveprefix = {arXiv},
	author = {{Malizia}, A. and {Stephen}, J.~B. and {Bassani}, L. and {Bird}, A.~J. and {Panessa}, F. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2009.15330.x},
	eprint = {0906.5544},
	journal = {\mnras},
	keywords = {galaxies: active , galaxies: nuclei , X-rays: galaxies},
	month = oct,
	pages = {944-951},
	title = {{The fraction of Compton-thick sources in an INTEGRAL complete AGN sample}},
	volume = 399,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15330.x}}

@article{haardt1991,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...380L..51H},
	author = {{Haardt}, F. and {Maraschi}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:48:31 +0200},
	doi = {10.1086/186171},
	journal = {\apjl},
	keywords = {ACCRETION DISKS, ASTRONOMICAL MODELS, EMISSION SPECTRA, SEYFERT GALAXIES, X RAY SPECTRA, COMPUTATIONAL ASTROPHYSICS, GALACTIC NUCLEI, GRAVITATIONAL EFFECTS, INTERSTELLAR MAGNETIC FIELDS, MAGNETIC FIELD RECONNECTION},
	month = oct,
	pages = {L51-L54},
	title = {{A two-phase model for the X-ray emission from Seyfert galaxies}},
	volume = 380,
	year = 1991,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/186171}}

@article{Hardcastle:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.309..969H},
	author = {{Hardcastle}, M.~J. and {Worrall}, D.~M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.1999.02945.x},
	eprint = {arXiv:astro-ph/9907034},
	journal = {\mnras},
	month = nov,
	pages = {969-990},
	title = {{ROSAT X-ray observations of 3CRR radio sources}},
	volume = 309,
	year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1999.02945.x}}

@article{Ulvestad:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...562L.133U},
	author = {{Ulvestad}, J.~S. and {Ho}, L.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/338254},
	eprint = {arXiv:astro-ph/0110535},
	journal = {\apjl},
	keywords = {Accretion, Accretion Disks, Galaxies: Active, Galaxies: Individual: NGC Number: NGC 3147, Galaxies: Individual: NGC Number: NGC 4203, Galaxies: Individual: NGC Number: NGC 4579, Galaxies: Nuclei, Radio Continuum: Galaxies},
	month = dec,
	pages = {L133-L136},
	title = {{The Origin of Radio Emission in Low-Luminosity Active Galactic Nuclei: Jets, Accretion Flows, or Both?}},
	volume = 562,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/338254}}

@article{Lal:2010,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010AJ....139.1089V},
	archiveprefix = {arXiv},
	author = {{Vir Lal}, D. and {Ho}, L.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-6256/139/3/1089},
	eprint = {1001.1476},
	journal = {\aj},
	keywords = {galaxies: active, galaxies: jets, galaxies: nuclei, galaxies: Seyfert, galaxies: structure, radio continuum: galaxies},
	month = mar,
	pages = {1089-1105},
	title = {{The Radio Properties of Type 2 Quasars}},
	volume = 139,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/139/3/1089}}

@article{Trouille:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ApJS..179....1T},
	archiveprefix = {arXiv},
	author = {{Trouille}, L. and {Barger}, A.~J. and {Cowie}, L.~L. and {Yang}, Y. and {Mushotzky}, R.~F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/591648},
	eprint = {0811.0824},
	journal = {\apjs},
	keywords = {Cosmology: Observations, Galaxies: Active},
	month = nov,
	pages = {1-18},
	title = {{The OPTX Project. I. The Flux and Redshift Catalogs for the CLANS, CLASXS, and CDF-N Fields}},
	volume = 179,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/591648}}

@article{Vollmer:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...489...49V},
	archiveprefix = {arXiv},
	author = {{Vollmer}, B. and {Krichbaum}, T.~P. and {Angelakis}, E. and {Kovalev}, Y.~Y.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20078857},
	eprint = {0806.3694},
	journal = {\aap},
	keywords = {radio continuum: galaxies},
	month = oct,
	pages = {49-55},
	title = {{Quasi-simultaneous multi-frequency observations of inverted-spectrum GPS candidate sources}},
	volume = 489,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078857}}

@article{sopp91,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1991MNRAS.251P..14S},
	author = {{Sopp}, H.~M. and {Alexander}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\mnras},
	keywords = {FAR INFRARED RADIATION, LUMINOSITY, QUASARS, RADIO EMISSION, ACTIVE GALACTIC NUCLEI, RADIO GALAXIES, SEYFERT GALAXIES, STARBURST GALAXIES},
	month = jul,
	pages = {14P-16P},
	title = {{A composite plot of far-infrared versus radio luminosity, and the origin of far-infrared luminosity in quasars}},
	volume = 251,
	year = 1991}

@article{vanBreugel:1998,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...502..614V},
	author = {{van Breugel}, W.~J.~M. and {Stanford}, S.~A. and {Spinrad}, H. and {Stern}, D. and {Graham}, J.~R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/305925},
	eprint = {arXiv:astro-ph/9803019},
	journal = {\apj},
	keywords = {GALAXIES: ACTIVE, GALAXIES: ELLIPTICAL AND LENTICULAR, CD, RADIO CONTINUUM: GALAXIES, GALAXIES: PHOTOMETRY, GALAXIES: STRUCTURE},
	month = aug,
	pages = {614-+},
	title = {{Morphological Evolution in High-Redshift Radio Galaxies and the Formation of Giant Elliptical Galaxies}},
	volume = 502,
	year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/305925}}

@inproceedings{Surace:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005AAS...207.6301S},
	author = {{Surace}, J.~A. and {Shupe}, D.~L. and {Fang}, F. and {Evans}, T. and {Alexov}, A. and {Frayer}, D. and {Lonsdale}, C.~J. and {SWIRE Team}},
	booktitle = {Bulletin of the American Astronomical Society},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	month = dec,
	pages = {1246},
	series = {Bulletin of the American Astronomical Society},
	title = {{Data Processing and Validation of the SWIRE Survey}},
	volume = 37,
	year = 2005}

@article{Lonsdale:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003PASP..115..897L},
	author = {{Lonsdale}, C.~J. and {Smith}, H.~E. and {Rowan-Robinson}, M. and {Surace}, J. and {Shupe}, D. and {Xu}, C. and {Oliver}, S. and {Padgett}, D. and {Fang}, F. and {Conrow}, T. and {Franceschini}, A. and {Gautier}, N. and {Griffin}, M. and {Hacking}, P. and {Masci}, F. and {Morrison}, G. and {O'Linger}, J. and {Owen}, F. and {P{\'e}rez-Fournon}, I. and {Pierre}, M. and {Puetter}, R. and {Stacey}, G. and {Castro}, S. and {Polletta}, M.~d.~C. and {Farrah}, D. and {Jarrett}, T. and {Frayer}, D. and {Siana}, B. and {Babbedge}, T. and {Dye}, S. and {Fox}, M. and {Gonzalez-Solares}, E. and {Salaman}, M. and {Berta}, S. and {Condon}, J.~J. and {Dole}, H. and {Serjeant}, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/376850},
	eprint = {arXiv:astro-ph/0305375},
	journal = {\pasp},
	keywords = {Surveys, Galaxies: Evolution, Galaxies: Active, Cosmology: Large-Scale Structure of Universe, infrared: galaxies},
	month = aug,
	pages = {897-927},
	title = {{SWIRE: The SIRTF Wide-Area Infrared Extragalactic Survey}},
	volume = 115,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/376850}}

@article{Polletta:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...642..673D},
	author = {{Polletta}, M.~d.~C. and {Wilkes}, B.~J. and {Siana}, B. and {Lonsdale}, C.~J. and {Kilgard}, R. and {Smith}, H.~E. and {Kim}, {D.-W.} and {Owen}, F. and {Efstathiou}, A. and {Jarrett}, T. and {Stacey}, G. and {Franceschini}, A. and {Rowan-Robinson}, M. and {Babbedge}, T.~S.~R. and {Berta}, S. and {Fang}, F. and {Farrah}, D. and {Gonz{\'a}lez-Solares}, E. and {Morrison}, G. and {Surace}, J.~A. and {Shupe}, D.~L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/500821},
	eprint = {arXiv:astro-ph/0602228},
	journal = {\apj},
	keywords = {Galaxies: Active, Infrared: Galaxies, quasars: individual (SWIRE J104409.95+585224.8), quasars: individual (SWIRE J104406.30+583954.1), X-Rays: Galaxies},
	month = may,
	pages = {673-693},
	title = {{Chandra and Spitzer Unveil Heavily Obscured Quasars in the Chandra/SWIRE Survey}},
	volume = 642,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/500821}}

@article{McNamara:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...562L.149M},
	author = {{McNamara}, B.~R. and {Wise}, M.~W. and {Nulsen}, P.~E.~J. and {David}, L.~P. and {Carilli}, C.~L. and {Sarazin}, C.~L. and {O'Dea}, C.~P. and {Houck}, J. and {Donahue}, M. and {Baum}, S. and {Voit}, M. and {O'Connell}, R.~W. and {Koekemoer}, A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/338326},
	eprint = {arXiv:astro-ph/0110554},
	journal = {\apjl},
	keywords = {Galaxies: Cooling Flows, Galaxies: Clusters: General, Galaxies: Intergalactic Medium, Radio Continuum: Galaxies, X-Rays: Galaxies: Clusters},
	month = dec,
	pages = {L149-L152},
	title = {{Discovery of Ghost Cavities in the X-Ray Atmosphere of Abell 2597}},
	volume = 562,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/338326}}

@article{Gallimore:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...613..794G},
	author = {{Gallimore}, J.~F. and {Baum}, S.~A. and {O'Dea}, C.~P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/423167},
	eprint = {arXiv:astro-ph/0406062},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Individual: NGC Number: NGC 1068, Galaxies: Nuclei, Galaxies: Seyfert, Radio Continuum: Galaxies},
	month = oct,
	pages = {794-810},
	title = {{The Parsec-Scale Radio Structure of NGC 1068 and the Nature of the Nuclear Radio Source}},
	volume = 613,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/423167}}

@article{Gallimore:1996,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...464..198G},
	author = {{Gallimore}, J.~F. and {Baum}, S.~A. and {O'Dea}, C.~P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/177311},
	journal = {\apj},
	keywords = {GALAXIES: INDIVIDUAL NGC NUMBER: NGC 1068, GALAXIES: JETS, GALAXIES: NUCLEI, GALAXIES: SEYFERT, GALAXIES: STRUCTURE, RADIO CONTINUUM: GALAXIES},
	month = jun,
	pages = {198-+},
	title = {{The Subarcsecond Radio Structure in NGC 1068. II. Implications for the Central Engine and Unifying Schemes}},
	volume = 464,
	year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/177311}}

@article{Roy:1998,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...504..147R},
	author = {{Roy}, A.~L. and {Colbert}, E.~J.~M. and {Wilson}, A.~S. and {Ulvestad}, J.~S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/306071},
	journal = {\apj},
	keywords = {GALAXIES: INDIVIDUAL NGC NUMBER: NGC 1068, GALAXIES: ISM, GALAXIES: JETS, GALAXIES: NUCLEI, GALAXIES: SEYFERT, RADIO CONTINUUM: GALAXIES},
	month = sep,
	pages = {147-+},
	title = {{The Compact Radio Sources in the Nucleus of NGC 1068}},
	volume = 504,
	year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/306071}}

@article{Barvainis:1998,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1998AJ....115..885B},
	author = {{Barvainis}, R. and {Lonsdale}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/300262},
	eprint = {arXiv:astro-ph/9711247},
	journal = {\aj},
	keywords = {GALAXIES: ACTIVE, GALAXIES: ACTIVE},
	month = mar,
	pages = {885-889},
	title = {{Search for Free-Free Absorption Cutoffs from Tori in Three Type 2 Active Galactic Nuclei}},
	volume = 115,
	year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/300262}}

@article{Bassani:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...636L..65B},
	author = {{Bassani}, L. and {Molina}, M. and {Malizia}, A. and {Stephen}, J.~B. and {Bird}, A.~J. and {Bazzano}, A. and {B{\'e}langer}, G. and {Dean}, A.~J. and {De Rosa}, A. and {Laurent}, P. and {Lebrun}, F. and {Ubertini}, P. and {Walter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/500132},
	eprint = {arXiv:astro-ph/0512015},
	journal = {\apjl},
	keywords = {Galaxies: Active, Gamma Rays: Observations, Surveys},
	month = jan,
	pages = {L65-L68},
	title = {{INTEGRAL IBIS Extragalactic Survey: Active Galactic Nuclei Selected at 20-100 keV}},
	volume = 636,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/500132}}

@article{Ulvestad:1986,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1986MNRAS.218..711U},
	author = {{Ulvestad}, J.~S. and {Wilson}, A.~S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\mnras},
	keywords = {ASTRONOMICAL SPECTROSCOPY, EXTRAGALACTIC RADIO SOURCES, GALACTIC NUCLEI, GAMMA RAY SPECTRA, SEYFERT GALAXIES, CENTIMETER WAVES, DIFFUSE RADIATION, EMISSION SPECTRA, GALACTIC STRUCTURE, HIGH RESOLUTION, SPECTRAL RESOLUTION, VISIBLE SPECTRUM},
	month = feb,
	pages = {711-719},
	title = {{The radio source in the very luminous gamma-ray Seyfert galaxy MCG 8-11-11}},
	volume = 218,
	year = 1986}

@article{Ubertini:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411L.131U},
	author = {{Ubertini}, P. and {Lebrun}, F. and {Di Cocco}, G. and {Bazzano}, A. and {Bird}, A.~J. and {Broenstad}, K. and {Goldwurm}, A. and {La Rosa}, G. and {Labanti}, C. and {Laurent}, P. and {Mirabel}, I.~F. and {Quadrini}, E.~M. and {Ramsey}, B. and {Reglero}, V. and {Sabau}, L. and {Sacco}, B. and {Staubert}, R. and {Vigroux}, L. and {Weisskopf}, M.~C. and {Zdziarski}, A.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20031224},
	journal = {\aap},
	keywords = {INTEGRAL, IBIS, gamma-ray imaging},
	month = nov,
	pages = {L131-L139},
	title = {{IBIS: The Imager on-board INTEGRAL}},
	volume = 411,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031224}}

@article{Sambruna:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...665.1030S},
	archiveprefix = {arXiv},
	author = {{Sambruna}, R.~M. and {Reeves}, J.~N. and {Braito}, V.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/519306},
	eprint = {0704.3053},
	journal = {\apj},
	keywords = {Galaxies: Active, X-Rays: Galaxies},
	month = aug,
	pages = {1030-1037},
	title = {{The Remarkable X-Ray Spectrum of the Broad-Line Radio Galaxy 3C 445}},
	volume = 665,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/519306}}

@article{Risaliti:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...386..379R},
	author = {{Risaliti}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20020170},
	eprint = {arXiv:astro-ph/0202392},
	journal = {\aap},
	keywords = {Galaxies: Active, Galaxies: Seyfert, X-rays: Galaxies},
	month = may,
	pages = {379-398},
	title = {{The BeppoSAX view of bright Compton-thin Seyfert 2 galaxies}},
	volume = 386,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20020170}}

@article{Mushotzky:1993,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1993ARA%26A..31..717M},
	author = {{Mushotzky}, R.~F. and {Done}, C. and {Pounds}, K.~A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1146/annurev.aa.31.090193.003441},
	journal = {\araa},
	keywords = {ACTIVE GALACTIC NUCLEI, POWER SPECTRA, QUASARS, X RAY SPECTRA, SEYFERT GALAXIES, VARIABILITY},
	pages = {717-761},
	title = {{X-ray spectra and time variability of active galactic nuclei}},
	volume = 31,
	year = 1993,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.aa.31.090193.003441}}

@article{Miller:1990,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1990MNRAS.244..207M},
	author = {{Miller}, L. and {Peacock}, J.~A. and {Mead}, A.~R.~G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\mnras},
	keywords = {QUASARS, RADIO ASTRONOMY, RADIO EMISSION, ASTRONOMICAL SPECTROSCOPY, LUMINOSITY, RED SHIFT},
	month = may,
	pages = {207-213},
	title = {{The bimodal radio luminosity function of quasars}},
	volume = 244,
	year = 1990}

@article{Masetti:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...482..113M},
	archiveprefix = {arXiv},
	author = {{Masetti}, N. and {Mason}, E. and {Morelli}, L. and {Cellone}, S.~A. and {McBride}, V.~A. and {Palazzi}, E. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A.~J. and {Charles}, P.~A. and {Dean}, A.~J. and {Galaz}, G. and {Gehrels}, N. and {Landi}, R. and {Malizia}, A. and {Minniti}, D. and {Panessa}, F. and {Romero}, G.~E. and {Stephen}, J.~B. and {Ubertini}, P. and {Walter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20079332},
	eprint = {0802.0988},
	journal = {\aap},
	keywords = {galaxies: Seyfert, X-rays: binaries, stars: novae, , cataclysmic variables, techniques: spectroscopic, X-rays:, general},
	month = apr,
	pages = {113-132},
	title = {{Unveiling the nature of INTEGRAL objects through optical spectroscopy. VI. A multi-observatory identification campaign}},
	volume = 482,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20079332}}

@article{Lewis:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...622..816L},
	author = {{Lewis}, K.~T. and {Eracleous}, M. and {Gliozzi}, M. and {Sambruna}, R.~M. and {Mushotzky}, R.~F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/428380},
	eprint = {arXiv:astro-ph/0412537},
	journal = {\apj},
	keywords = {Accretion, Accretion Disks, Galaxies: Active, Galaxies: Individual: Alphanumeric: 3C 111, Galaxies: Nuclei, X-Rays: Galaxies},
	month = apr,
	pages = {816-829},
	title = {{A Simultaneous RXTE and XMM-Newton Observation of the Broad-Line Radio Galaxy 3C 111}},
	volume = 622,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/428380}}

@article{Larsson:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.388.1037L},
	archiveprefix = {arXiv},
	author = {{Larsson}, J. and {Fabian}, A.~C. and {Ballantyne}, D.~R. and {Miniutti}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.13497.x},
	eprint = {0805.3603},
	journal = {\mnras},
	keywords = {galaxies: active , galaxies: individual: 4C+74.26 , X-rays: galaxies},
	month = aug,
	pages = {1037-1046},
	title = {{Exploring the disc/jet interaction in the radio-loud quasar 4C+74.26 with Suzaku}},
	volume = 388,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13497.x}}

@article{Kharb:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...652..177K},
	author = {{Kharb}, P. and {O'Dea}, C.~P. and {Baum}, S.~A. and {Colbert}, E.~J.~M. and {Xu}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/507945},
	eprint = {arXiv:astro-ph/0607603},
	journal = {\apj},
	keywords = {galaxies: individual (Mrk 6), Galaxies: Seyfert, Radio Continuum: Galaxies},
	month = nov,
	pages = {177-188},
	title = {{A Radio Study of the Seyfert Galaxy Markarian 6: Implications for Seyfert Life Cycles}},
	volume = 652,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/507945}}

@article{Ishwara-Chandra:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.309..100I},
	author = {{Ishwara-Chandra}, C.~H. and {Saikia}, D.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.1999.02835.x},
	eprint = {arXiv:astro-ph/9902252},
	journal = {\mnras},
	month = oct,
	pages = {100-112},
	title = {{Giant radio sources}},
	volume = 309,
	year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1999.02835.x}}

@article{Hardcastle:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.363..649H},
	author = {{Hardcastle}, M.~J. and {Croston}, J.~H.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2005.09469.x},
	eprint = {arXiv:astro-ph/0507694},
	journal = {\mnras},
	keywords = {radiation mechanisms: non-thermal, galaxies: active, galaxies: individual: Pictor A, galaxies: jets, X-rays: galaxies},
	month = oct,
	pages = {649-660},
	title = {{The Chandra view of extended X-ray emission from Pictor A}},
	volume = 363,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09469.x}}

@article{Grandi:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...343...33G},
	author = {{Grandi}, P. and {Guainazzi}, M. and {Haardt}, F. and {Maraschi}, L. and {Massaro}, E. and {Matt}, G. and {Piro}, L. and {Urry}, C.~M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {arXiv:astro-ph/9810450},
	journal = {\aap},
	keywords = {GALAXIES: ACTIVE, GALAXIES: INDIVIDUAL: 3C 390.3, RADIO CONTINUUM: GALAXIES, X-RAYS: GALAXIES},
	month = mar,
	pages = {33-40},
	title = {{Reprocessing and variable cold absorption in the broad-line radio galaxy 3C 390.3}},
	volume = 343,
	year = 1999}

@article{Gliozzi:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...584..176G},
	author = {{Gliozzi}, M. and {Sambruna}, R.~M. and {Eracleous}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/345661},
	eprint = {arXiv:astro-ph/0210300},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Individual: Alphanumeric: 3C 120, Galaxies: Individual: Alphanumeric: 3C 390.3, Galaxies: Nuclei},
	month = feb,
	pages = {176-189},
	title = {{Long-Term Continuous Monitoring of the Broad-Line Radio Galaxies 3C 390.3 and 3C 120 with the Rossi X-Ray Timing Explorer}},
	volume = 584,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/345661}}

@article{Fan:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...407..899F},
	author = {{Fan}, J.~H. and {Zhang}, J.~S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20030896},
	journal = {\aap},
	keywords = {BL Lacertae objects: general, quasars: general, galaxies: Seyfert, galaxies: jets},
	month = sep,
	pages = {899-904},
	title = {{The core dominance parameter of extragalactic radio sources}},
	volume = 407,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20030896}}

@article{Evans:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...642...96E},
	author = {{Evans}, D.~A. and {Worrall}, D.~M. and {Hardcastle}, M.~J. and {Kraft}, R.~P. and {Birkinshaw}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/500658},
	eprint = {arXiv:astro-ph/0512600},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Jets, X-Rays: Galaxies},
	month = may,
	pages = {96-112},
	title = {{Chandra and XMM-Newton Observations of a Sample of Low-Redshift FR I and FR II Radio Galaxy Nuclei}},
	volume = 642,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/500658}}

@article{Dickey:1990,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1990ARA%26A..28..215D},
	author = {{Dickey}, J.~M. and {Lockman}, F.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1146/annurev.aa.28.090190.001243},
	journal = {\araa},
	keywords = {H I REGIONS, MILKY WAY GALAXY, ABSORPTION SPECTRA, LYMAN ALPHA RADIATION, MOLECULAR CLOUDS, RADIO EMISSION, ULTRAVIOLET ASTRONOMY, VERY LONG BASE INTERFEROMETRY},
	pages = {215-261},
	title = {{H I in the Galaxy}},
	volume = 28,
	year = 1990,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.aa.28.090190.001243}}

@article{Derosa:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...483..749D},
	archiveprefix = {arXiv},
	author = {{de Rosa}, A. and {Bassani}, L. and {Ubertini}, P. and {Panessa}, F. and {Malizia}, A. and {Dean}, A.~J. and {Walter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20078319},
	eprint = {0801.4675},
	journal = {\aap},
	keywords = {X-rays: galaxies, galaxies: Seyfert, galaxies: nuclei},
	month = jun,
	pages = {749-758},
	title = {{An X-ray view of absorbed INTEGRAL AGN}},
	volume = 483,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078319}}

@article{de-Bruyn:1989,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...226L..13D},
	author = {{de Bruyn}, A.~G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\aap},
	keywords = {EXTRAGALACTIC RADIO SOURCES, GALACTIC CLUSTERS, QUASARS, RADIO GALAXIES, ASTRONOMICAL SPECTROSCOPY, RADIO ASTRONOMY},
	month = dec,
	pages = {L13-L16},
	title = {{0309 + 411, an Mpc-sized core-dominated radio galaxy/quasar}},
	volume = 226,
	year = 1989}

@article{Ballantyne:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.336..867B},
	author = {{Ballantyne}, D.~R. and {Ross}, R.~R. and {Fabian}, A.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2002.05818.x},
	eprint = {arXiv:astro-ph/0202148},
	journal = {\mnras},
	keywords = {line: formation, radiative transfer, galaxies: active, galaxies: individual: MCG-6-30-15, X-rays: galaxies, X-rays: general},
	month = nov,
	pages = {867-872},
	title = {{Soft X-ray emission lines from photoionized accretion discs: constraints on their strength and width}},
	volume = 336,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2002.05818.x}}

@article{Ballantyne:2005b,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...622L..97B},
	author = {{Ballantyne}, D.~R. and {Fabian}, A.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/429691},
	eprint = {arXiv:astro-ph/0502461},
	journal = {\apjl},
	keywords = {Accretion, Accretion Disks, Galaxies: Active, Galaxies: Individual: Alphanumeric: 4C 74.26, Galaxies: Jets, X-Rays: Galaxies},
	month = apr,
	pages = {L97-L100},
	title = {{Evidence of an Untruncated Accretion Disk in the Broad-Line Radio Galaxy 4C 74.26}},
	volume = 622,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/429691}}

@article{Ballantyne:2005a,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.362.1183B},
	author = {{Ballantyne}, D.~R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2005.09345.x},
	eprint = {arXiv:astro-ph/0506673},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: individual: 4C +74.26, X-rays: galaxies},
	month = oct,
	pages = {1183-1188},
	title = {{A complete view of the broad-line radio galaxy 4C +74.26 with XMM-Newton}},
	volume = 362,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09345.x}}

@article{Brinkmann:2000,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...356..445B},
	author = {{Brinkmann}, W. and {Laurent-Muehleisen}, S.~A. and {Voges}, W. and {Siebert}, J. and {Becker}, R.~H. and {Brotherton}, M.~S. and {White}, R.~L. and {Gregg}, M.~D.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {\aap},
	keywords = {GALAXIES: ACTIVE, GALAXIES: QUASARS: GENERAL, X-RAYS: GENERAL, RADIO CONTINUUM: GENERAL},
	month = apr,
	pages = {445-462},
	title = {{Radio and X-ray bright AGN: the ROSAT - FIRST correlation}},
	volume = 356,
	year = 2000}

@article{Kellermann:1981,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1981ARA%26A..19..373K},
	author = {{Kellermann}, K.~I. and {Pauliny-Toth}, I.~I.~K.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1146/annurev.aa.19.090181.002105},
	journal = {\araa},
	keywords = {EXTRAGALACTIC RADIO SOURCES, RADIANT FLUX DENSITY, RADIATION DISTRIBUTION, RADIO SPECTRA, SPATIAL DISTRIBUTION, BRIGHTNESS TEMPERATURE, GALACTIC EVOLUTION, QUASARS, RADIO ASTRONOMY, RADIO GALAXIES},
	pages = {373-410},
	title = {{Compact radio sources}},
	volume = 19,
	year = 1981,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.aa.19.090181.002105}}

@article{Jackson:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.304..160J},
	author = {{Jackson}, C.~A. and {Wall}, J.~V.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.1999.02310.x},
	eprint = {arXiv:astro-ph/9808054},
	journal = {\mnras},
	keywords = {GALAXIES: EVOLUTION, GALAXIES: JETS, QUASARS: GENERAL, RADIO CONTINUUM: GALAXIES},
	month = mar,
	pages = {160-174},
	title = {{Extragalactic radio-source evolution under the dual-population unification scheme}},
	volume = 304,
	year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1999.02310.x}}

@article{Seymour:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386.1695S},
	archiveprefix = {arXiv},
	author = {{Seymour}, N. and {Dwelly}, T. and {Moss}, D. and {McHardy}, I. and {Zoghbi}, A. and {Rieke}, G. and {Page}, M. and {Hopkins}, A. and {Loaring}, N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.13166.x},
	eprint = {0802.4105},
	journal = {\mnras},
	keywords = {galaxies: evolution , galaxies: starburst , radio continuum: galaxies},
	month = may,
	pages = {1695-1708},
	title = {{The star formation history of the Universe as revealed by deep radio observations}},
	volume = 386,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13166.x}}

@article{White:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...654...99W},
	author = {{White}, R.~L. and {Helfand}, D.~J. and {Becker}, R.~H. and {Glikman}, E. and {de Vries}, W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/507700},
	eprint = {arXiv:astro-ph/0607335},
	journal = {\apj},
	keywords = {Catalogs, Galaxies: Quasars: Absorption Lines, Galaxies: Quasars: General, Radio Continuum: General, Surveys},
	month = jan,
	pages = {99-114},
	title = {{Signals from the Noise: Image Stacking for Quasars in the FIRST Survey}},
	volume = 654,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/507700}}

@article{Zamfir:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.387..856Z},
	archiveprefix = {arXiv},
	author = {{Zamfir}, S. and {Sulentic}, J.~W. and {Marziani}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.13290.x},
	eprint = {0804.0788},
	journal = {\mnras},
	keywords = {galaxies: active , quasars: emission lines , quasars: general},
	month = jun,
	pages = {856-870},
	title = {{New insights on the QSO radio-loud/radio-quiet dichotomy: SDSS spectra in the context of the 4D eigenvector1 parameter space}},
	volume = 387,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13290.x}}

@article{Kellermann:1989,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1989AJ.....98.1195K},
	author = {{Kellermann}, K.~I. and {Sramek}, R. and {Schmidt}, M. and {Shaffer}, D.~B. and {Green}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/115207},
	journal = {\aj},
	keywords = {ASTRONOMICAL CATALOGS, QUASARS, RADIO SOURCES (ASTRONOMY), VERY LARGE ARRAY (VLA), CENTIMETER WAVES, DATA SAMPLING, LUMINOSITY, RADIANT FLUX DENSITY},
	month = oct,
	pages = {1195-1207},
	title = {{VLA observations of objects in the Palomar Bright Quasar Survey}},
	volume = 98,
	year = 1989,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/115207}}

@article{Wilkes:1987,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1987ApJ...323..243W},
	author = {{Wilkes}, B.~J. and {Elvis}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/165822},
	journal = {\apj},
	keywords = {ASTRONOMICAL SPECTROSCOPY, QUASARS, SPECTRAL ENERGY DISTRIBUTION, X RAY SPECTRA, BL LACERTAE OBJECTS, RADIO SPECTRA, RED SHIFT, STELLAR LUMINOSITY},
	month = dec,
	pages = {243-262},
	title = {{Quasar energy distributions. I - Soft X-ray spectra of quasars}},
	volume = 323,
	year = 1987,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/165822}}

@article{Chiappetti:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...439..413C},
	author = {{Chiappetti}, L. and {Tajer}, M. and {Trinchieri}, G. and {Maccagni}, D. and {Maraschi}, L. and {Paioro}, L. and {Pierre}, M. and {Surdej}, J. and {Garcet}, O. and {Gosset}, E. and {Le F{\`e}vre}, O. and {Bertin}, E. and {McCracken}, H.~J. and {Mellier}, Y. and {Foucaud}, S. and {Radovich}, M. and {Ripepi}, V. and {Arnaboldi}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20042583},
	eprint = {arXiv:astro-ph/0505117},
	journal = {\aap},
	keywords = {X-ray: general, surveys, quasars: general, catalogs},
	month = aug,
	pages = {413-425},
	title = {{The XMM-LSS survey. The XMDS/VVDS 4{$\sigma$} catalogue}},
	volume = 439,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20042583}}

@article{baldi02,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...564..190B},
	author = {{Baldi}, A. and {Molendi}, S. and {Comastri}, A. and {Fiore}, F. and {Matt}, G. and {Vignali}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:50:04 +0200},
	doi = {10.1086/324261},
	eprint = {arXiv:astro-ph/0108514},
	journal = {\apj},
	keywords = {Galaxies: Active, X-Rays: Diffuse Background, X-Rays: Galaxies},
	month = jan,
	pages = {190-195},
	title = {{The HELLAS2XMM Survey. I. The X-Ray Data and the logN-logS Relation}},
	volume = 564,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/324261}}

@article{Rieke:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004ApJS..154...25R},
	author = {{Rieke}, G.~H. and {Young}, E.~T. and {Engelbracht}, C.~W. and {Kelly}, D.~M. and {Low}, F.~J. and {Haller}, E.~E. and {Beeman}, J.~W. and {Gordon}, K.~D. and {Stansberry}, J.~A. and {Misselt}, K.~A. and {Cadien}, J. and {Morrison}, J.~E. and {Rivlis}, G. and {Latter}, W.~B. and {Noriega-Crespo}, A. and {Padgett}, D.~L. and {Stapelfeldt}, K.~R. and {Hines}, D.~C. and {Egami}, E. and {Muzerolle}, J. and {Alonso-Herrero}, A. and {Blaylock}, M. and {Dole}, H. and {Hinz}, J.~L. and {Le Floc'h}, E. and {Papovich}, C. and {P{\'e}rez-Gonz{\'a}lez}, P.~G. and {Smith}, P.~S. and {Su}, K.~Y.~L. and {Bennett}, L. and {Frayer}, D.~T. and {Henderson}, D. and {Lu}, N. and {Masci}, F. and {Pesenson}, M. and {Rebull}, L. and {Rho}, J. and {Keene}, J. and {Stolovy}, S. and {Wachter}, S. and {Wheaton}, W. and {Werner}, M.~W. and {Richards}, P.~L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/422717},
	journal = {\apjs},
	keywords = {Infrared: General, Space Vehicles: Instruments},
	month = sep,
	pages = {25-29},
	title = {{The Multiband Imaging Photometer for Spitzer (MIPS)}},
	volume = 154,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422717}}

@article{Fazio:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004ApJS..154...10F},
	author = {{Fazio}, G.~G. and {Hora}, J.~L. and {Allen}, L.~E. and {Ashby}, M.~L.~N. and {Barmby}, P. and {Deutsch}, L.~K. and {Huang}, {J.-S.} and {Kleiner}, S. and {Marengo}, M. and {Megeath}, S.~T. and {Melnick}, G.~J. and {Pahre}, M.~A. and {Patten}, B.~M. and {Polizotti}, J. and {Smith}, H.~A. and {Taylor}, R.~S. and {Wang}, Z. and {Willner}, S.~P. and {Hoffmann}, W.~F. and {Pipher}, J.~L. and {Forrest}, W.~J. and {McMurty}, C.~W. and {McCreight}, C.~R. and {McKelvey}, M.~E. and {McMurray}, R.~E. and {Koch}, D.~G. and {Moseley}, S.~H. and {Arendt}, R.~G. and {Mentzell}, J.~E. and {Marx}, C.~T. and {Losch}, P. and {Mayman}, P. and {Eichhorn}, W. and {Krebs}, D. and {Jhabvala}, M. and {Gezari}, D.~Y. and {Fixsen}, D.~J. and {Flores}, J. and {Shakoorzadeh}, K. and {Jungo}, R. and {Hakun}, C. and {Workman}, L. and {Karpati}, G. and {Kichak}, R. and {Whitley}, R. and {Mann}, S. and {Tollestrup}, E.~V. and {Eisenhardt}, P. and {Stern}, D. and {Gorjian}, V. and {Bhattacharya}, B. and {Carey}, S. and {Nelson}, B.~O. and {Glaccum}, W.~J. and {Lacy}, M. and {Lowrance}, P.~J. and {Laine}, S. and {Reach}, W.~T. and {Stauffer}, J.~A. and {Surace}, J.~A. and {Wilson}, G. and {Wright}, E.~L. and {Hoffman}, A. and {Domingo}, G. and {Cohen}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/422843},
	eprint = {arXiv:astro-ph/0405616},
	journal = {\apjs},
	keywords = {Infrared: General, Instrumentation: Detectors, Space Vehicles: Instruments},
	month = sep,
	pages = {10-17},
	title = {{The Infrared Array Camera (IRAC) for the Spitzer Space Telescope}},
	volume = 154,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422843}}

@article{Polletta:2000,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...362...75P},
	author = {{Polletta}, M. and {Courvoisier}, {T.~J.-L.} and {Hooper}, E.~J. and {Wilkes}, B.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {arXiv:astro-ph/0006315},
	journal = {\aap},
	keywords = {GALAXIES: QUASARS: GENERAL, INFRARED: GALAXIES, RADIO CONTINUUM: GALAXIES},
	month = oct,
	pages = {75-96},
	title = {{The far-infrared emission of radio loud and radio quiet quasars}},
	volume = 362,
	year = 2000}

@article{Polletta:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...663...81P},
	author = {{Polletta}, M. and {Tajer}, M. and {Maraschi}, L. and {Trinchieri}, G. and {Lonsdale}, C.~J. and {Chiappetti}, L. and {Andreon}, S. and {Pierre}, M. and {Le F{\`e}vre}, O. and {Zamorani}, G. and {Maccagni}, D. and {Garcet}, O. and {Surdej}, J. and {Franceschini}, A. and {Alloin}, D. and {Shupe}, D.~L. and {Surace}, J.~A. and {Fang}, F. and {Rowan-Robinson}, M. and {Smith}, H.~E. and {Tresse}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/518113},
	journal = {\apj},
	keywords = {Galaxies: Active, Infrared: Galaxies, Galaxies: Quasars: General, X-Rays: Galaxies},
	month = jul,
	pages = {81-102},
	title = {{Spectral Energy Distributions of Hard X-Ray Selected Active Galactic Nuclei in the XMM-Newton Medium Deep Survey}},
	volume = 663,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/518113}}

@article{Polletta:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...492...81P},
	archiveprefix = {arXiv},
	author = {{Polletta}, M. and {Omont}, A. and {Berta}, S. and {Bergeron}, J. and {Stalin}, C.~S. and {Petitjean}, P. and {Giorgetti}, M. and {Trinchieri}, G. and {Srianand}, R. and {McCracken}, H.~J. and {Pei}, Y. and {Dannerbauer}, H.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:200810345},
	eprint = {0810.2518},
	journal = {\aap},
	keywords = {galaxies: active, galaxies: evolution, galaxies: high-redshift, quasars: general, infrared: galaxies},
	month = dec,
	pages = {81-92},
	title = {{Obscured and powerful AGN and starburst activities at z \~{} 3.5}},
	volume = 492,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200810345}}

@article{Owen:2009b,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009ApJS..182..625O},
	archiveprefix = {arXiv},
	author = {{Owen}, F.~N. and {Morrison}, G.~E.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0067-0049/182/2/625},
	eprint = {0904.4651},
	journal = {\apjs},
	keywords = {cosmology: observations, galaxies: active, galaxies: starburst, infrared: galaxies},
	month = jun,
	pages = {625-627},
	title = {{The Deep Swire Field. III. Wiyn Spectroscopy}},
	volume = 182,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/182/2/625}}

@article{Owen:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008AJ....136.1889O},
	archiveprefix = {arXiv},
	author = {{Owen}, F.~N. and {Morrison}, G.~E.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-6256/136/5/1889},
	eprint = {0809.0314},
	journal = {\aj},
	keywords = {cosmology: observations, galaxies: evolution, galaxies: starburst, infrared: galaxies},
	month = nov,
	pages = {1889-1900},
	title = {{The Deep Swire Field. I. 20 cm Continuum Radio Observations: A Crowded Sky}},
	volume = 136,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/136/5/1889}}

@article{Owen:2009a,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009AJ....137.4846O},
	archiveprefix = {arXiv},
	author = {{Owen}, F.~N. and {Morrison}, G.~E. and {Klimek}, M.~D. and {Greisen}, E.~W.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-6256/137/6/4846},
	eprint = {0904.2011},
	journal = {\aj},
	keywords = {cosmology: observations, galaxies: active, galaxies: evolution, galaxies: general, galaxies: starburst},
	month = jun,
	pages = {4846-4853},
	title = {{The Deep SWIRE Field. II. 90 cm Continuum Observations and 20 cm-90 cm Spectra}},
	volume = 137,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/137/6/4846}}

@inproceedings{Norris:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009ASPC..408..334N},
	author = {{Norris}, R.~P.},
	booktitle = {Astronomical Society of the Pacific Conference Series},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{W.~Wang, Z.~Yang, Z.~Luo, \& Z.~Chen}},
	month = oct,
	pages = {334},
	series = {Astronomical Society of the Pacific Conference Series},
	title = {{Co-Evolution of AGN and Star-Forming Galaxies in the Australia Telescope Large Area Survey}},
	volume = 408,
	year = 2009}

@article{Boyle:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.376.1182B},
	author = {{Boyle}, B.~J. and {Cornwell}, T.~J. and {Middelberg}, E. and {Norris}, R.~P. and {Appleton}, P.~N. and {Smail}, I.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2007.11509.x},
	eprint = {arXiv:astro-ph/0701602},
	journal = {\mnras},
	keywords = {galaxies: starburst , infrared: galaxies , radio continuum: general},
	month = apr,
	pages = {1182-1188},
	title = {{Extending the infrared radio correlation}},
	volume = 376,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.11509.x}}

@article{appleton04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004ApJS..154..147A},
	author = {{Appleton}, P.~N. and {Fadda}, D.~T. and {Marleau}, F.~R. and {Frayer}, D.~T. and {Helou}, G. and {Condon}, J.~J. and {Choi}, P.~I. and {Yan}, L. and {Lacy}, M. and {Wilson}, G. and {Armus}, L. and {Chapman}, S.~C. and {Fang}, F. and {Heinrichson}, I. and {Im}, M. and {Jannuzi}, B.~T. and {Storrie-Lombardi}, L.~J. and {Shupe}, D. and {Soifer}, B.~T. and {Squires}, G. and {Teplitz}, H.~I.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:49:41 +0200},
	doi = {10.1086/422425},
	eprint = {arXiv:astro-ph/0406030},
	journal = {\apjs},
	keywords = {Cosmology: Observations, Galaxies: Evolution, Galaxies: High-Redshift, Infrared: Galaxies},
	month = sep,
	pages = {147-150},
	title = {{The Far- and Mid-Infrared/Radio Correlations in the Spitzer Extragalactic First Look Survey}},
	volume = 154,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422425}}

@article{zdziarski98,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.301..435Z},
	author = {{Zdziarski}, A.~A. and {Poutanen}, J. and {Mikolajewska}, J. and {Gierlinski}, M. and {Ebisawa}, K. and {Johnson}, W.~N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:48:51 +0200},
	doi = {10.1046/j.1365-8711.1998.02021.x},
	eprint = {arXiv:astro-ph/9807300},
	journal = {\mnras},
	keywords = {ACCRETION, ACCRETION DISCS, BINARIES: GENERAL, STARS: INDIVIDUAL: GX 339-4, GAMMA-RAYS: OBSERVATIONS, GAMMA-RAYS: THEORY, X-RAYS: STARS},
	month = dec,
	pages = {435-450},
	title = {{Broad-band X-ray/gamma-ray spectra and binary parameters of GX 339-4 and their astrophysical implications}},
	volume = 301,
	year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1998.02021.x}}

@article{Zdziarski:1990,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1990ApJ...363L...1Z},
	author = {{Zdziarski}, A.~A. and {Ghisellini}, G. and {George}, I.~M. and {Fabian}, A.~C. and {Svensson}, R. and {Done}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/185851},
	journal = {\apjl},
	keywords = {ACTIVE GALACTIC NUCLEI, COMPTON EFFECT, ELECTRON-POSITRON PAIRS, X RAY SPECTRA, ACCRETION DISKS, ASTRONOMICAL SPECTROSCOPY, BACKGROUND RADIATION, GAMMA RAY SPECTRA},
	month = nov,
	pages = {L1-L4},
	title = {{Electron-positron pairs, Compton reflection, and the X-ray spectra of active galactic nuclei}},
	volume = 363,
	year = 1990,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/185851}}

@article{Winter:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...690.1322W},
	archiveprefix = {arXiv},
	author = {{Winter}, L.~M. and {Mushotzky}, R.~F. and {Reynolds}, C.~S. and {Tueller}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/690/2/1322},
	eprint = {0808.0461},
	journal = {\apj},
	keywords = {galaxies: active, surveys, X-rays: galaxies},
	month = jan,
	pages = {1322-1349},
	title = {{X-Ray Spectral Properties of the BAT AGN Sample}},
	volume = 690,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/690/2/1322}}

@article{Winter:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...674..686W},
	archiveprefix = {arXiv},
	author = {{Winter}, L.~M. and {Mushotzky}, R.~F. and {Tueller}, J. and {Markwardt}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/525274},
	eprint = {0711.0019},
	journal = {\apj},
	keywords = {Galaxies: Active, Surveys, X-Rays: Galaxies},
	month = feb,
	pages = {686-710},
	title = {{X-Ray Properties of an Unbiased Hard X-Ray-detected Sample of Active Galactic Nuclei}},
	volume = 674,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/525274}}

@article{Vaughan:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.348.1415V},
	author = {{Vaughan}, S. and {Fabian}, A.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2004.07456.x},
	eprint = {arXiv:astro-ph/0311473},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: individual: MCG, 6-30-15, galaxies: Seyfert, X-rays: galaxies},
	month = mar,
	pages = {1415-1438},
	title = {{A long hard look at MCG-6-30-15 with XMM-Newton- II. Detailed EPIC analysis and modelling}},
	volume = 348,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.07456.x}}

@article{Turner:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...365L.110T},
	author = {{Turner}, M.~J.~L. and {Reeves}, J.~N. and {Ponman}, T.~J. and {Arnaud}, M. and {Barbera}, M. and {Bennie}, P.~J. and {Boer}, M. and {Briel}, U. and {Butler}, I. and {Clavel}, J. and {Dhez}, P. and {Cordova}, F. and {Dos Santos}, S. and {Ferrando}, P. and {Ghizzardi}, S. and {Goodall}, C.~V. and {Griffiths}, R.~G. and {Hochedez}, J.~F. and {Holland}, A.~D. and {Jansen}, F. and {Kendziorra}, E. and {Lagostina}, A. and {Laine}, R. and {La Palombara}, N. and {Lortholary}, M. and {Mason}, K.~O. and {Molendi}, S. and {Pigot}, C. and {Priedhorsky}, W. and {Reppin}, C. and {Rothenflug}, R. and {Salvetat}, P. and {Sauvageot}, J. and {Schmitt}, D. and {Sembay}, S. and {Short}, A. and {Str{\"u}der}, L. and {Trifoglio}, M. and {Tr{\"u}mper}, J. and {Vercellone}, S. and {Vigroux}, L. and {Villa}, G. and {Ward}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20000070},
	eprint = {arXiv:astro-ph/0010612},
	journal = {\aap},
	keywords = {GALAXIES: ACTIVE, GALAXIES: STARBURST, X-RAYS: GALAXIES},
	month = jan,
	pages = {L110-L115},
	title = {{XMM-Newton first-light observations of the Hickson galaxy group 16}},
	volume = 365,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20000070}}

@article{Tueller:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...681..113T},
	archiveprefix = {arXiv},
	author = {{Tueller}, J. and {Mushotzky}, R.~F. and {Barthelmy}, S. and {Cannizzo}, J.~K. and {Gehrels}, N. and {Markwardt}, C.~B. and {Skinner}, G.~K. and {Winter}, L.~M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/588458},
	eprint = {0711.4130},
	journal = {\apj},
	keywords = {Galaxies: Active, Gamma Rays: Observations, Surveys},
	month = jul,
	pages = {113-127},
	title = {{Swift BAT Survey of AGNs}},
	volume = 681,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/588458}}

@article{Treister:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...696..110T},
	archiveprefix = {arXiv},
	author = {{Treister}, E. and {Urry}, C.~M. and {Virani}, S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/696/1/110},
	eprint = {0902.0608},
	journal = {\apj},
	keywords = {galaxies: active, galaxies: Seyfert, X-rays: diffuse background, X-rays: galaxies},
	month = may,
	pages = {110-120},
	title = {{The Space Density of Compton-Thick Active Galactic Nucleus and the X-Ray Background}},
	volume = 696,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/696/1/110}}

@article{Struder:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...365L..18S},
	author = {{Str{\"u}der}, L. and {Briel}, U. and {Dennerl}, K. and {Hartmann}, R. and {Kendziorra}, E. and {Meidinger}, N. and {Pfeffermann}, E. and {Reppin}, C. and {Aschenbach}, B. and {Bornemann}, W. and {Br{\"a}uninger}, H. and {Burkert}, W. and {Elender}, M. and {Freyberg}, M. and {Haberl}, F. and {Hartner}, G. and {Heuschmann}, F. and {Hippmann}, H. and {Kastelic}, E. and {Kemmer}, S. and {Kettenring}, G. and {Kink}, W. and {Krause}, N. and {M{\"u}ller}, S. and {Oppitz}, A. and {Pietsch}, W. and {Popp}, M. and {Predehl}, P. and {Read}, A. and {Stephan}, K.~H. and {St{\"o}tter}, D. and {Tr{\"u}mper}, J. and {Holl}, P. and {Kemmer}, J. and {Soltau}, H. and {St{\"o}tter}, R. and {Weber}, U. and {Weichert}, U. and {von Zanthier}, C. and {Carathanassis}, D. and {Lutz}, G. and {Richter}, R.~H. and {Solc}, P. and {B{\"o}ttcher}, H. and {Kuster}, M. and {Staubert}, R. and {Abbey}, A. and {Holland}, A. and {Turner}, M. and {Balasini}, M. and {Bignami}, G.~F. and {La Palombara}, N. and {Villa}, G. and {Buttler}, W. and {Gianini}, F. and {Lain{\'e}}, R. and {Lumb}, D. and {Dhez}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20000066},
	journal = {\aap},
	keywords = {XMM-NEWTON, BACK ILLUMINATED PN-CCDS, RADIATION HARDNESS, ENERGY RESOLUTION, QUANTUM EFFICIENCY, PARTICLE AND FLOURESCENCE BACKGROUND},
	month = jan,
	pages = {L18-L26},
	title = {{The European Photon Imaging Camera on XMM-Newton: The pn-CCD camera}},
	volume = 365,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20000066}}

@article{Spergel:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003ApJS..148..175S},
	author = {{Spergel}, D.~N. and {Verde}, L. and {Peiris}, H.~V. and {Komatsu}, E. and {Nolta}, M.~R. and {Bennett}, C.~L. and {Halpern}, M. and {Hinshaw}, G. and {Jarosik}, N. and {Kogut}, A. and {Limon}, M. and {Meyer}, S.~S. and {Page}, L. and {Tucker}, G.~S. and {Weiland}, J.~L. and {Wollack}, E. and {Wright}, E.~L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/377226},
	eprint = {arXiv:astro-ph/0302209},
	journal = {\apjs},
	keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Cosmological Parameters- Cosmology: Observations, Cosmology: Early Universe},
	month = sep,
	pages = {175-194},
	title = {{First-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Determination of Cosmological Parameters}},
	volume = 148,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/377226}}

@article{Sazonov:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...482..517S},
	archiveprefix = {arXiv},
	author = {{Sazonov}, S. and {Krivonos}, R. and {Revnivtsev}, M. and {Churazov}, E. and {Sunyaev}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20078537},
	eprint = {0708.3215},
	journal = {\aap},
	keywords = {surveys, galaxies: active, galaxies: evolution, galaxies: Seyfert, X-rays: diffuse background},
	month = may,
	pages = {517-527},
	title = {{Cumulative hard X-ray spectrum of local AGN: a link to the cosmic X-ray background}},
	volume = 482,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078537}}

@article{Sambruna:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...526...60S},
	author = {{Sambruna}, R.~M. and {Eracleous}, M. and {Mushotzky}, R.~F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/307981},
	eprint = {arXiv:astro-ph/9905365},
	journal = {\apj},
	keywords = {GALAXIES: ACTIVE, RADIATION MECHANISMS: NONTHERMAL, SURVEYS, X-RAYS: GALAXIES},
	month = nov,
	pages = {60-96},
	title = {{An X-Ray Spectral Survey of Radio-loud Active Galactic Nuclei with ASCA}},
	volume = 526,
	year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/307981}}

@article{Reeves:2000,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.316..234R},
	author = {{Reeves}, J.~N. and {Turner}, M.~J.~L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2000.03510.x},
	eprint = {arXiv:astro-ph/0003080},
	journal = {\mnras},
	keywords = {SURVEYS, GALAXIES: ACTIVE, QUASARS: GENERAL, X-RAYS: GENERAL},
	month = aug,
	pages = {234-248},
	title = {{X-ray spectra of a large sample of quasars with ASCA}},
	volume = 316,
	year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2000.03510.x}}

@article{Piro:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999AN....320..236P},
	author = {{Piro}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	journal = {Astronomische Nachrichten},
	pages = {236-+},
	title = {{Probing the AGN environment with X-ray measurements}},
	volume = 320,
	year = 1999}

@article{Piconcelli:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...432..835P},
	author = {{Piconcelli}, E. and {Guainazzi}, M. and {Cappi}, M. and {Jimenez-Bailon}, E. and {Schartel}, N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20041804},
	eprint = {arXiv:astro-ph/0412360},
	journal = {\aap},
	keywords = {galaxies: individual: RX J1343.4+0001, galaxies: active, galaxies: quasars: general, X-ray: galaxies},
	month = mar,
	pages = {835-839},
	title = {{The XMM-Newton spectrum of the high-z optically-obscured QSO RX J1343.4+0001: a classic radio quiet QSO}},
	volume = 432,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20041804}}

@article{Petrucci:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...556..716P},
	author = {{Petrucci}, P.~O. and {Haardt}, F. and {Maraschi}, L. and {Grandi}, P. and {Malzac}, J. and {Matt}, G. and {Nicastro}, F. and {Piro}, L. and {Perola}, G.~C. and {De Rosa}, A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/321629},
	eprint = {arXiv:astro-ph/0101219},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Seyfert, X-Rays: Galaxies},
	month = aug,
	pages = {716-726},
	title = {{Testing Comptonization Models Using BeppoSAX Observations of Seyfert 1 Galaxies}},
	volume = 556,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/321629}}

@article{Perola:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...389..802P},
	author = {{Perola}, G.~C. and {Matt}, G. and {Cappi}, M. and {Fiore}, F. and {Guainazzi}, M. and {Maraschi}, L. and {Petrucci}, P.~O. and {Piro}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20020658},
	eprint = {arXiv:astro-ph/0205045},
	journal = {\aap},
	keywords = {galaxies: Seyfert, X-rays: galaxies},
	month = jul,
	pages = {802-811},
	title = {{Compton reflection and iron fluorescence in BeppoSAX observations of Seyfert type 1 galaxies}},
	volume = 389,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20020658}}

@article{Panessa:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...483..151P},
	archiveprefix = {arXiv},
	author = {{Panessa}, F. and {Bassani}, L. and {de Rosa}, A. and {Bird}, A.~J. and {Dean}, A.~J. and {Fiocchi}, M. and {Malizia}, A. and {Molina}, M. and {Ubertini}, P. and {Walter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20078657},
	eprint = {0803.0896},
	journal = {\aap},
	keywords = {galaxies: Seyfert, X-rays: galaxies},
	month = may,
	pages = {151-160},
	title = {{The broad-band XMM-Newton and INTEGRAL spectra of bright type 1 Seyfert galaxies}},
	volume = 483,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078657}}

@article{Mushotzky:1984,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1984AdSpR...3..157M},
	author = {{Mushotzky}, R.~F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1016/0273-1177(84)90081-4},
	journal = {Advances in Space Research},
	keywords = {ACTIVE GALACTIC NUCLEI, HEAO, PERIODIC VARIATIONS, X RAY SOURCES, X RAY SPECTRA, ASTRONOMICAL MODELS, BL LACERTAE OBJECTS, QUASARS, RADIO GALAXIES, SEYFERT GALAXIES, SPECTRAL ENERGY DISTRIBUTION, SPECTRAL LINE WIDTH},
	pages = {157-165},
	title = {{X-ray spectra and time variability of active galactic nuclei}},
	volume = 3,
	year = 1984,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/0273-1177(84)90081-4}}

@article{Molina:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.371..821M},
	author = {{Molina}, M. and {Malizia}, A. and {Bassani}, L. and {Bird}, A.~J. and {Dean}, A.~J. and {Landi}, R. and {de Rosa}, A. and {Walter}, R. and {Barlow}, E.~J. and {Clark}, D.~J. and {Hill}, A.~B. and {Sguera}, V.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2006.10715.x},
	eprint = {arXiv:astro-ph/0606488},
	journal = {\mnras},
	keywords = {galaxies: active: galaxies: Seyfert, galaxies: active, galaxies: Seyfert},
	month = sep,
	pages = {821-828},
	title = {{INTEGRAL observations of active galactic nuclei obscured by the Galactic plane}},
	volume = 371,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10715.x}}

@article{Molina:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.382..937M},
	archiveprefix = {arXiv},
	author = {{Molina}, M. and {Giroletti}, M. and {Malizia}, A. and {Landi}, R. and {Bassani}, L. and {Bird}, A.~J. and {Dean}, A.~J. and {de Rosa}, A. and {Fiocchi}, M. and {Panessa}, F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2007.12464.x},
	eprint = {0709.1895},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: Seyfert, X-rays: galaxies},
	month = dec,
	pages = {937-943},
	title = {{Broad-band X-ray spectrum of the newly discovered broad-line radio galaxy IGR J21247+5058}},
	volume = 382,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12464.x}}

@article{Molina:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.390.1217M},
	archiveprefix = {arXiv},
	author = {{Molina}, M. and {Bassani}, L. and {Malizia}, A. and {Bird}, A.~J. and {Dean}, A.~J. and {Fiocchi}, M. and {Panessa}, F. and {de Rosa}, A. and {Landi}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.13824.x},
	eprint = {0809.0255},
	journal = {\mnras},
	keywords = {galaxies: active , X-rays: galaxies},
	month = nov,
	pages = {1217-1228},
	title = {{A broad-band spectral analysis of eight radio-loud type 1 active galactic nuclei selected in the hard X-ray band}},
	volume = 390,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13824.x}}

@article{Molina:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.399.1293M},
	archiveprefix = {arXiv},
	author = {{Molina}, M. and {Bassani}, L. and {Malizia}, A. and {Stephen}, J.~B. and {Bird}, A.~J. and {Dean}, A.~J. and {Panessa}, F. and {de Rosa}, A. and {Landi}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2009.15257.x},
	eprint = {0906.2909},
	journal = {\mnras},
	keywords = {galaxies: active , gamma-rays: observations , X-rays: galaxies},
	month = nov,
	pages = {1293-1306},
	title = {{The INTEGRAL complete sample of type 1 AGN}},
	volume = 399,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15257.x}}

@article{Miniutti:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007PASJ...59S.315M},
	author = {{Miniutti}, G. and {Fabian}, A.~C. and {Anabuki}, N. and {Crummy}, J. and {Fukazawa}, Y. and {Gallo}, L. and {Haba}, Y. and {Hayashida}, K. and {Holt}, S. and {Kunieda}, H. and {Larsson}, J. and {Markowitz}, A. and {Matsumoto}, C. and {Ohno}, M. and {Reeves}, J.~N. and {Takahashi}, T. and {Tanaka}, Y. and {Terashima}, Y. and {Torii}, K. and {Ueda}, Y. and {Ushio}, M. and {Watanabe}, S. and {Yamauchi}, M. and {Yaqoob}, T.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {arXiv:astro-ph/0609521},
	journal = {\pasj},
	keywords = {galaxies: active, galaxies: individual (MCG -6-30-15), galaxies: Seyfert, X-rays: galaxies},
	month = jan,
	pages = {315-325},
	title = {{Suzaku Observations of the Hard X-Ray Variability of MCG -6-30-15: the Effects of Strong Gravity around a Kerr Black Hole}},
	volume = 59,
	year = 2007}

@article{Miniutti:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.349.1435M},
	author = {{Miniutti}, G. and {Fabian}, A.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2004.07611.x},
	eprint = {arXiv:astro-ph/0309064},
	journal = {\mnras},
	keywords = {accretion, accretion discs, black hole physics, relativity, galaxies: active, X-rays: galaxies, X-rays: stars},
	month = apr,
	pages = {1435-1448},
	title = {{A light bending model for the X-ray temporal and spectral properties of accreting black holes}},
	volume = 349,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.07611.x}}

@article{Merloni:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.370.1699M},
	author = {{Merloni}, A. and {Malzac}, J. and {Fabian}, A.~C. and {Ross}, R.~R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2006.10676.x},
	eprint = {arXiv:astro-ph/0606262},
	journal = {\mnras},
	keywords = {accretion, accretion discs: black hole physics, accretion discs, black hole physics},
	month = aug,
	pages = {1699-1712},
	title = {{On the X-ray spectra of luminous, inhomogeneous accretion flows}},
	volume = 370,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10676.x}}

@article{Mattson:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...664..101M},
	archiveprefix = {arXiv},
	author = {{Mattson}, B.~J. and {Weaver}, K.~A. and {Reynolds}, C.~S.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/518783},
	eprint = {0704.1587},
	journal = {\apj},
	keywords = {Galaxies: Seyfert, X-Rays: Galaxies},
	month = jul,
	pages = {101-105},
	title = {{Possible X-Ray Diagnostic for Jet/Disk Dominance in Type 1 AGNs}},
	volume = 664,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/518783}}

@article{Matt:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...445..451M},
	author = {{Matt}, G. and {Bianchi}, S. and {de Rosa}, A. and {Grandi}, P. and {Perola}, G.~C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20054013},
	eprint = {arXiv:astro-ph/0509017},
	journal = {\aap},
	keywords = {galaxies: active, X-rays: galaxies, galaxies: individual: MCG+8-11-11},
	month = jan,
	pages = {451-456},
	title = {{XMM-Newton observation of the bright Seyfert 1 galaxy, MCG+8-11-11}},
	volume = 445,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20054013}}

@inproceedings{Matt:2001,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001AIPC..599..209M},
	author = {{Matt}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1063/1.1434634},
	eprint = {arXiv:astro-ph/0007105},
	journal = {X-ray Astronomy: Stellar Endpoints, AGN, and the Diffuse X-ray Background},
	keywords = {Active and peculiar galaxies and related systems, X-ray sources; X-ray bursts},
	month = dec,
	pages = {209-218},
	title = {{The broad band spectrum and variability of Seyfert 1}},
	volume = 599,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1063/1.1434634}}

@article{Masetti:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...470..331M},
	archiveprefix = {arXiv},
	author = {{Masetti}, N. and {Landi}, R. and {Pretorius}, M.~L. and {Sguera}, V. and {Bird}, A.~J. and {Perri}, M. and {Charles}, P.~A. and {Kennea}, J.~A. and {Malizia}, A. and {Ubertini}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20077509},
	eprint = {0704.3682},
	journal = {\aap},
	keywords = {astrometry, stars: binaries: general, X-rays: binaries, stars: neutron, stars: individual: IGR J16194-2810},
	month = jul,
	pages = {331-337},
	title = {{IGR J16194-2810: a new symbiotic X-ray binary}},
	volume = 470,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077509}}

@article{Markowitz:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...646..783M},
	author = {{Markowitz}, A. and {Reeves}, J.~N. and {Braito}, V.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/505107},
	eprint = {arXiv:astro-ph/0604353},
	journal = {\apj},
	keywords = {Galaxies: Active, galaxies: individual (IC 4329a), Galaxies: Seyfert, X-Rays: Galaxies},
	month = aug,
	pages = {783-800},
	title = {{Fe K Emission and Absorption in the XMM-EPIC Spectrum of the Seyfert Galaxy IC 4329a}},
	volume = 646,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/505107}}

@inproceedings{Maraschi:1997,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1997ASPC..121..101M},
	author = {{Maraschi}, L. and {Haardt}, F.},
	booktitle = {IAU Colloq. 163: Accretion Phenomena and Related Outflows},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	editor = {{D.~T.~Wickramasinghe, G.~V.~Bicknell, \& L.~Ferrario}},
	pages = {101-+},
	series = {Astronomical Society of the Pacific Conference Series},
	title = {{Disk-Corona Models and X-Ray Emission from Seyfert Galaxies}},
	volume = 121,
	year = 1997}

@article{malzac02,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.336.1209M},
	author = {{Malzac}, J. and {Petrucci}, {P.-O.}},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:49:08 +0200},
	doi = {10.1046/j.1365-8711.2002.05851.x},
	eprint = {arXiv:astro-ph/0109339},
	journal = {\mnras},
	keywords = {accretion, accretion discs, black hole physics, radiative transfer, galaxies: Seyfert, gamma-rays: theory, X-rays: general},
	month = nov,
	pages = {1209-1216},
	title = {{Reflection at large distance from the central engine in Seyferts}},
	volume = 336,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2002.05851.x}}

@article{Malzac:2001a,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.326..417M},
	author = {{Malzac}, J. and {Beloborodov}, A.~M. and {Poutanen}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2001.04450.x},
	eprint = {arXiv:astro-ph/0102490},
	journal = {\mnras},
	keywords = {ACCRETION, ACCRETION DISCS, RADIATIVE TRANSFER, STARS: INDIVIDUAL: CYG X-1, GALAXIES: SEYFERT, GAMMA-RAYS: THEORY, X-RAYS: GENERAL},
	month = sep,
	pages = {417-427},
	title = {{X-ray spectra of accretion discs with dynamic coronae}},
	volume = 326,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2001.04450.x}}

@article{malzac01b,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.325.1625M},
	author = {{Malzac}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:49:00 +0200},
	doi = {10.1046/j.1365-8711.2001.04567.x},
	eprint = {arXiv:astro-ph/0104273},
	journal = {\mnras},
	keywords = {ACCRETION, ACCRETION DISCS, BLACK HOLE PHYSICS, RADIATIVE TRANSFER, GALAXIES: SEYFERT, GAMMA-RAYS: THEORY, X-RAYS: GENERAL},
	month = aug,
	pages = {1625-1636},
	title = {{A quasi-spherical inner accretion flow in Seyfert galaxies?}},
	volume = 325,
	year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2001.04567.x}}

@article{Malizia:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.389.1360M},
	archiveprefix = {arXiv},
	author = {{Malizia}, A. and {Bassani}, L. and {Bird}, A.~J. and {Landi}, R. and {Masetti}, N. and {de Rosa}, A. and {Panessa}, F. and {Molina}, M. and {Dean}, A.~J. and {Perri}, M. and {Tueller}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2008.13657.x},
	eprint = {0806.4824},
	journal = {\mnras},
	keywords = {galaxies: active , galaxies: Seyfert , X-rays: galaxies},
	month = sep,
	pages = {1360-1366},
	title = {{First high-energy observations of narrow-line Seyfert 1s with INTEGRAL/IBIS}},
	volume = 389,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13657.x}}

@article{Malizia:2003a,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...406..105M},
	author = {{Malizia}, A. and {Bassani}, L. and {Capalbi}, M. and {Fabian}, A.~C. and {Fiore}, F. and {Nicastro}, F.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20030743},
	eprint = {arXiv:astro-ph/0305329},
	journal = {\aap},
	keywords = {X-rays: galaxies, galaxies: Seyfert, galaxies: individual: MKN6},
	month = jul,
	pages = {105-109},
	title = {{A BeppoSAX observation of MKN6}},
	volume = 406,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20030743}}

@article{Malizia:2003b,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...589L..17M},
	author = {{Malizia}, A. and {Bassani}, L. and {Stephen}, J.~B. and {Di Cocco}, G. and {Fiore}, F. and {Dean}, A.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/375712},
	eprint = {arXiv:astro-ph/0304133},
	journal = {\apjl},
	keywords = {Galaxies: Active, Galaxies: Seyfert},
	month = may,
	pages = {L17-L20},
	title = {{BeppoSAX Average Spectra of Seyfert Galaxies}},
	volume = 589,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/375712}}

@article{Lebrun:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411L.141L},
	author = {{Lebrun}, F. and {Leray}, J.~P. and {Lavocat}, P. and {Cr{\'e}tolle}, J. and {Arqu{\`e}s}, M. and {Blondel}, C. and {Bonnin}, C. and {Bou{\`e}re}, A. and {Cara}, C. and {Chaleil}, T. and {Daly}, F. and {Desages}, F. and {Dzitko}, H. and {Horeau}, B. and {Laurent}, P. and {Limousin}, O. and {Mathy}, F. and {Mauguen}, V. and {Meignier}, F. and {Molini{\'e}}, F. and {Poindron}, E. and {Rouger}, M. and {Sauvageon}, A. and {Tourrette}, T.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20031367},
	eprint = {arXiv:astro-ph/0310362},
	journal = {\aap},
	keywords = {space telescope, cadmium telluride detectors, gamma-ray astronomy, calibration, INTEGRAL},
	month = nov,
	pages = {L141-L148},
	title = {{ISGRI: The INTEGRAL Soft Gamma-Ray Imager}},
	volume = 411,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031367}}

@article{Landi:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.380..926L},
	archiveprefix = {arXiv},
	author = {{Landi}, R. and {de Rosa}, A. and {Dean}, A.~J. and {Bassani}, L. and {Ubertini}, P. and {Bird}, A.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2007.12168.x},
	eprint = {0707.0832},
	journal = {\mnras},
	keywords = {gamma-rays: observations, X-rays: individual: PSR J1617-5055},
	month = sep,
	pages = {926-932},
	title = {{HESS J1616-508: likely to be powered by PSR J1617-5055}},
	volume = 380,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12168.x}}

@inproceedings{Hill:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004SPIE.5165..217H},
	author = {{Hill}, J.~E. and {Burrows}, D.~N. and {Nousek}, J.~A. and {Abbey}, A.~F. and {Ambrosi}, R.~M. and {Br{\"a}uninger}, H.~W. and {Burkert}, W. and {Campana}, S. and {Cheruvu}, C. and {Cusumano}, G. and {Freyberg}, M.~J. and {Hartner}, G.~D. and {Klar}, R. and {Mangels}, C. and {Moretti}, A. and {Mori}, K. and {Morris}, D.~C. and {Short}, A.~D.~T. and {Tagliaferri}, G. and {Watson}, D.~J. and {Wood}, P. and {Wells}, A.~A.},
	booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1117/12.505728},
	editor = {{K.~A.~Flanagan \& O.~H.~W.~Siegmund}},
	month = feb,
	pages = {217-231},
	series = {Presented at the Society of Photo-Optical Instrumentation Engineers (SPIE) Conference},
	title = {{Readout modes and automated operation of the Swift X-ray Telescope}},
	volume = 5165,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.505728}}

@article{Hickox:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...645...95H},
	author = {{Hickox}, R.~C. and {Markevitch}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/504070},
	eprint = {arXiv:astro-ph/0512542},
	journal = {\apj},
	keywords = {Galaxies: Active, Methods: Data Analysis, X-Rays: Diffuse Background, X-Rays: Galaxies},
	month = jul,
	pages = {95-114},
	title = {{Absolute Measurement of the Unresolved Cosmic X-Ray Background in the 0.5-8 keV Band with Chandra}},
	volume = 645,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/504070}}

@article{Guainazzi:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006AN....327.1032G},
	author = {{Guainazzi}, M. and {Bianchi}, S. and {Dov{\v c}iak}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1002/asna.200610687},
	eprint = {arXiv:astro-ph/0610151},
	journal = {Astronomische Nachrichten},
	keywords = {quasars: emission lines, galaxies: nuclei, galaxies: active, X-ray: galaxies, line: profiles},
	pages = {1032-+},
	title = {{Statistics of relativistically broadened Fe K{$\alpha$} lines in AGN}},
	volume = 327,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1002/asna.200610687}}

@article{Guainazzi:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...346..407G},
	author = {{Guainazzi}, M. and {Perola}, G.~C. and {Matt}, G. and {Nicastro}, F. and {Bassani}, L. and {Fiore}, F. and {dal Fiume}, D. and {Piro}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {arXiv:astro-ph/9903449},
	journal = {\aap},
	keywords = {GALAXIES: INDIVIDUAL: NGC 4593, GALAXIES: NUCLEI, GALAXIES: SEYFERT, X-RAYS: GALAXIES},
	month = jun,
	pages = {407-414},
	title = {{The complex 0.1-200 keV spectrum of the Seyfert 1 Galaxy NGC 4593}},
	volume = 346,
	year = 1999}

@article{Gruber:1999,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...520..124G},
	author = {{Gruber}, D.~E. and {Matteson}, J.~L. and {Peterson}, L.~E. and {Jung}, G.~V.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/307450},
	eprint = {arXiv:astro-ph/9903492},
	journal = {\apj},
	keywords = {COSMOLOGY: DIFFUSE RADIATION, INSTRUMENTATION: DETECTORS, X-RAYS: GENERAL},
	month = jul,
	pages = {124-129},
	title = {{The Spectrum of Diffuse Cosmic Hard X-Rays Measured with HEAO 1}},
	volume = 520,
	year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/307450}}

@article{Grandi:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...642..113G},
	author = {{Grandi}, P. and {Malaguti}, G. and {Fiocchi}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/500100},
	eprint = {arXiv:astro-ph/0511784},
	journal = {\apj},
	keywords = {Galaxies: Active, Galaxies: Nuclei, Surveys, X-Rays: Galaxies},
	month = may,
	pages = {113-125},
	title = {{BeppoSAX View of Radio-loud Active Galactic Nuclei}},
	volume = 642,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/500100}}

@article{Goldwurm:2003,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411L.223G},
	author = {{Goldwurm}, A. and {David}, P. and {Foschini}, L. and {Gros}, A. and {Laurent}, P. and {Sauvageon}, A. and {Bird}, A.~J. and {Lerusse}, L. and {Produit}, N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20031395},
	eprint = {arXiv:astro-ph/0311172},
	journal = {\aap},
	keywords = {coded masks, imaging, gamma-rays},
	month = nov,
	pages = {L223-L229},
	title = {{The INTEGRAL/IBIS scientific data analysis}},
	volume = 411,
	year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031395}}

@article{Gilli:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...463...79G},
	author = {{Gilli}, R. and {Comastri}, A. and {Hasinger}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20066334},
	eprint = {arXiv:astro-ph/0610939},
	journal = {\aap},
	keywords = {X-rays: galaxies, galaxies: active, X-rays: general, cosmology: diffuse radiation, X-rays: diffuse background},
	month = feb,
	pages = {79-96},
	title = {{The synthesis of the cosmic X-ray background in the Chandra and XMM-Newton era}},
	volume = 463,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20066334}}

@article{Gandhi:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.382.1005G},
	archiveprefix = {arXiv},
	author = {{Gandhi}, P. and {Fabian}, A.~C. and {Suebsuwong}, T. and {Malzac}, J. and {Miniutti}, G. and {Wilman}, R.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2007.12462.x},
	eprint = {0709.1984},
	journal = {\mnras},
	keywords = {galaxies: active, X-rays: galaxies},
	month = dec,
	pages = {1005-1018},
	title = {{Constraints on light bending and reflection from the hard X-ray background}},
	volume = 382,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12462.x}}

@article{Fabian:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.335L...1F},
	author = {{Fabian}, A.~C. and {Vaughan}, S. and {Nandra}, K. and {Iwasawa}, K. and {Ballantyne}, D.~R. and {Lee}, J.~C. and {De Rosa}, A. and {Turner}, A. and {Young}, A.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1046/j.1365-8711.2002.05740.x},
	eprint = {arXiv:astro-ph/0206095},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: general, galaxies: individual: MCG, 6-30-15, galaxies: Seyfert, X-rays: galaxies},
	month = sep,
	pages = {L1-L5},
	title = {{A long hard look at MCG-6-30-15 with XMM-Newton}},
	volume = 335,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2002.05740.x}}

@article{Fabian:2004,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.353.1071F},
	author = {{Fabian}, A.~C. and {Miniutti}, G. and {Gallo}, L. and {Boller}, T. and {Tanaka}, Y. and {Vaughan}, S. and {Ross}, R.~R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2004.08036.x},
	eprint = {arXiv:astro-ph/0405160},
	journal = {\mnras},
	keywords = {line: formation, galaxies: active, galaxies: individual: 1H 0707-495, X-rays: galaxies, X-rays: general},
	month = oct,
	pages = {1071-1077},
	title = {{X-ray reflection in the narrow-line Seyfert 1 galaxy 1H 0707-495}},
	volume = 353,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.08036.x}}

@article{Fabian:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.361..795F},
	author = {{Fabian}, A.~C. and {Miniutti}, G. and {Iwasawa}, K. and {Ross}, R.~R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2005.09148.x},
	eprint = {arXiv:astro-ph/0504472},
	journal = {\mnras},
	keywords = {line: formation, galaxies: active, galaxies: individual: 1H 0419-577, X-rays: galaxies, X-rays: general},
	month = aug,
	pages = {795-802},
	title = {{X-ray reflection in the Seyfert galaxy 1H 0419-577 revealing strong relativistic effects in the vicinity of a Kerr black hole}},
	volume = 361,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09148.x}}

@article{Elitzur:2006,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...648L.101E},
	author = {{Elitzur}, M. and {Shlosman}, I.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/508158},
	eprint = {arXiv:astro-ph/0605686},
	journal = {\apjl},
	keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, Infrared: Galaxies, Galaxies: Quasars: General},
	month = sep,
	pages = {L101-L104},
	title = {{The AGN-obscuring Torus: The End of the ``Doughnut'' Paradigm?}},
	volume = 648,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/508158}}

@article{Derosa:2002,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...387..838D},
	author = {{De Rosa}, A. and {Piro}, L. and {Fiore}, F. and {Grandi}, P. and {Maraschi}, L. and {Matt}, G. and {Nicastro}, F. and {Petrucci}, P.~O.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20020444},
	eprint = {arXiv:astro-ph/0203344},
	journal = {\aap},
	keywords = {galaxies: individual: NGC 3783, galaxies: Seyfert, X-rays: galaxies},
	month = jun,
	pages = {838-849},
	title = {{The BeppoSAX broad-band spectrum and variability of the Seyfert 1 NGC 3783}},
	volume = 387,
	year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20020444}}

@article{Derosa:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...463..903D},
	author = {{de Rosa}, A. and {Piro}, L. and {Perola}, G.~C. and {Capalbi}, M. and {Cappi}, M. and {Grandi}, P. and {Maraschi}, L. and {Petrucci}, P.~O.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20065028},
	eprint = {arXiv:astro-ph/0611470},
	journal = {\aap},
	keywords = {galaxies: Seyfert, X-rays: galaxies, galaxies: individual: NGC 4151},
	month = mar,
	pages = {903-912},
	title = {{The broad band spectrum and variability of NGC 4151 observed by BeppoSAX}},
	volume = 463,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20065028}}

@article{Dadina:2008,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...485..417D},
	archiveprefix = {arXiv},
	author = {{Dadina}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20077569},
	eprint = {0801.4338},
	journal = {\aap},
	keywords = {X-rays: galaxies, galaxies: Seyfert:, galaxies: active},
	month = jul,
	pages = {417-424},
	title = {{Seyfert galaxies in the local Universe (z {\le} 0.1): the average X-ray spectrum as seen by BeppoSAX}},
	volume = 485,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077569}}

@article{Dadina:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...461.1209D},
	author = {{Dadina}, M.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20065734},
	journal = {\aap},
	keywords = {catalogs, galaxies: active, galaxies: Seyfert, X-ray: galaxies},
	month = jan,
	pages = {1209-1252},
	title = {{BeppoSAX observations in the 2-100 keV band of the nearby Seyfert galaxies: an atlas of spectra}},
	volume = 461,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20065734}}

@article{Comastri:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007PThPS.169..274C},
	archiveprefix = {arXiv},
	author = {{Comastri}, A. and {Gilli}, R. and {Vignali}, C. and {Matt}, G. and {Fiore}, F. and {Iwasawa}, K.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {0704.1253},
	journal = {Progress of Theoretical Physics Supplement},
	pages = {274-277},
	title = {{Compton Thick AGN in the Suzaku Era}},
	volume = 169,
	year = 2007}

@article{Comastri:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005ExA....20...41C},
	author = {{Comastri}, A. and {Gilli}, R. and {Hasinger}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1007/s10686-006-9041-6},
	eprint = {arXiv:astro-ph/0604523},
	journal = {Experimental Astronomy},
	keywords = {X-rays, Background radiation, AGN},
	month = dec,
	pages = {41-47},
	title = {{Rolling down from the 30 keV peak: Modelling the Hard X-Ray and {$\gamma$}-Ray Backgrounds}},
	volume = 20,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10686-006-9041-6}}

@article{Comastri:1995,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...296....1C},
	author = {{Comastri}, A. and {Setti}, G. and {Zamorani}, G. and {Hasinger}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	eprint = {arXiv:astro-ph/9409067},
	journal = {\aap},
	keywords = {X-RAYS: GENERAL, X-RAYS: GALAXIES, COSMOLOGY: DIFFUSE RADIATION, GALAXIES:NUCLEI, QUASARS:GENERAL},
	month = apr,
	pages = {1-+},
	title = {{The contribution of AGNs to the X-ray background.}},
	volume = 296,
	year = 1995}

@article{Cappi:1996,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...458..149C},
	author = {{Cappi}, M. and {Mihara}, T. and {Matsuoka}, M. and {Hayashida}, K. and {Weaver}, K.~A. and {Otani}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/176799},
	eprint = {arXiv:astro-ph/9510065},
	journal = {\apj},
	keywords = {GALAXIES: INDIVIDUAL ALPHANUMERIC: IC 4329A, GALAXIES: SEYFERT, X-RAYS: GALAXIES},
	month = feb,
	pages = {149-+},
	title = {{Warm Absorber, Reflection, and Fe K Line in the X-Ray Spectrum of IC 4329A}},
	volume = 458,
	year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/176799}}

@article{bird04,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...607L..33B},
	author = {{Bird}, A.~J. and {Barlow}, E.~J. and {Bassani}, L. and {Bazzano}, A. and {Bodaghee}, A. and {Capitanio}, F. and {Cocchi}, M. and {Del Santo}, M. and {Dean}, A.~J. and {Hill}, A.~B. and {Lebrun}, F. and {Malaguti}, G. and {Malizia}, A. and {Much}, R. and {Shaw}, S.~E. and {Stephen}, J.~B. and {Terrier}, R. and {Ubertini}, P. and {Walter}, R.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:50:36 +0200},
	doi = {10.1086/421772},
	journal = {\apjl},
	keywords = {Galaxy: General, Gamma Rays: Observations, Surveys},
	month = may,
	pages = {L33-L37},
	title = {{The First IBIS/ISGRI Soft Gamma-Ray Galactic Plane Survey Catalog}},
	volume = 607,
	year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/421772}}

@article{bird06,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...636..765B},
	author = {{Bird}, A.~J. and {Barlow}, E.~J. and {Bassani}, L. and {Bazzano}, A. and {B{\'e}langer}, G. and {Bodaghee}, A. and {Capitanio}, F. and {Dean}, A.~J. and {Fiocchi}, M. and {Hill}, A.~B. and {Lebrun}, F. and {Malizia}, A. and {Mas-Hesse}, J.~M. and {Molina}, M. and {Moran}, L. and {Renaud}, M. and {Sguera}, V. and {Shaw}, S.~E. and {Stephen}, J.~B. and {Terrier}, R. and {Ubertini}, P. and {Walter}, R. and {Willis}, D.~R. and {Winkler}, C.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:50:53 +0200},
	doi = {10.1086/498090},
	journal = {\apj},
	keywords = {Galaxy: General, Gamma Rays: Observations, Surveys},
	month = jan,
	pages = {765-776},
	title = {{The Second IBIS/ISGRI Soft Gamma-Ray Survey Catalog}},
	volume = 636,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/498090}}

@article{bird07,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..170..175B},
	author = {{Bird}, A.~J. and {Malizia}, A. and {Bazzano}, A. and {Barlow}, E.~J. and {Bassani}, L. and {Hill}, A.~B. and {B{\'e}langer}, G. and {Capitanio}, F. and {Clark}, D.~J. and {Dean}, A.~J. and {Fiocchi}, M. and {G{\"o}tz}, D. and {Lebrun}, F. and {Molina}, M. and {Produit}, N. and {Renaud}, M. and {Sguera}, V. and {Stephen}, J.~B. and {Terrier}, R. and {Ubertini}, P. and {Walter}, R. and {Winkler}, C. and {Zurita}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:50:44 +0200},
	doi = {10.1086/513148},
	eprint = {arXiv:astro-ph/0611493},
	journal = {\apjs},
	keywords = {Galaxy: General, Gamma Rays: Observations, Surveys},
	month = may,
	pages = {175-186},
	title = {{The Third IBIS/ISGRI Soft Gamma-Ray Survey Catalog}},
	volume = 170,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/513148}}

@article{Bianchi:2009,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...495..421B},
	archiveprefix = {arXiv},
	author = {{Bianchi}, S. and {Guainazzi}, M. and {Matt}, G. and {Fonseca Bonilla}, N. and {Ponti}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:200810620},
	eprint = {0811.1126},
	journal = {\aap},
	keywords = {galaxies: active, galaxies: Seyfert, quasars: general, X-rays: general},
	month = feb,
	pages = {421-430},
	title = {{CAIXA: a catalogue of AGN in the XMM-Newton archive. I. Spectral analysis}},
	volume = 495,
	year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200810620}}

@article{Bianchi:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...467L..19B},
	author = {{Bianchi}, S. and {Guainazzi}, M. and {Matt}, G. and {Fonseca Bonilla}, N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20077331},
	eprint = {arXiv:astro-ph/0703433},
	journal = {\aap},
	keywords = {galaxies: active, galaxies: Seyfert, quasars: general, X-rays: general},
	month = may,
	pages = {L19-L22},
	title = {{On the Iwasawa-Taniguchi effect of radio-quiet AGN}},
	volume = 467,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077331}}

@article{Beckmann:2007,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...475..827B},
	author = {{Beckmann}, V. and {Barthelmy}, S.~D. and {Courvoisier}, {T.~J.-L.} and {Gehrels}, N. and {Soldi}, S. and {Tueller}, J. and {Wendt}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1051/0004-6361:20078355},
	journal = {\aap},
	keywords = {galaxies: active, galaxies: Seyfert , X-rays:, galaxies, surveys},
	month = dec,
	pages = {827-835},
	title = {{Hard X-ray variability of active galactic nuclei}},
	volume = 475,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078355}}

@article{baumgartner08,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ATel.1429....1B},
	author = {{Baumgartner}, W. and {Tueller}, J. and {Mushotzky}, R. and {Barthelmy}, S. and {Cannizzo}, J. and {Gehrels}, N. and {Markwardt}, C. and {Skinner}, G. and {Winter}, L.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:50:16 +0200},
	journal = {The Astronomer's Telegram},
	keywords = {X-ray, Gamma Ray, AGN, Black Holes, Quasars},
	month = mar,
	pages = {1-+},
	title = {{Swift/BAT teams announces website with catalog of AGN from the first 9}},
	volume = 1429,
	year = 2008}

@article{Barger:2005,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2005AJ....129..578B},
	author = {{Barger}, A.~J. and {Cowie}, L.~L. and {Mushotzky}, R.~F. and {Yang}, Y. and {Wang}, {W.-H.} and {Steffen}, A.~T. and {Capak}, P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/426915},
	eprint = {arXiv:astro-ph/0410527},
	journal = {\aj},
	keywords = {Cosmology: Observations, Galaxies: Active, Galaxies: Distances and Redshifts, Galaxies: Evolution, Galaxies: Formation},
	month = feb,
	pages = {578-609},
	title = {{The Cosmic Evolution of Hard X-Ray-selected Active Galactic Nuclei}},
	volume = 129,
	year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/426915}}

@article{Avni:1980,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1980ApJ...235..694A},
	author = {{Avni}, Y. and {Bahcall}, J.~N.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/157673},
	journal = {\apj},
	keywords = {COSMOLOGY, DATA SAMPLING, QUASARS, STELLAR EVOLUTION, ASTROPHYSICS, POISSON DENSITY FUNCTIONS, STELLAR LUMINOSITY},
	month = feb,
	pages = {694-716},
	title = {{On the simultaneous analysis of several complete samples - The V/Vmax and Ve/Va variables, with applications to quasars}},
	volume = 235,
	year = 1980,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/157673}}

@inproceedings{arnaud96,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/1996ASPC..101...17A},
	author = {{Arnaud}, K.~A.},
	booktitle = {Astronomical Data Analysis Software and Systems V},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:49:53 +0200},
	editor = {{G.~H.~Jacoby \& J.~Barnes}},
	pages = {17},
	series = {Astronomical Society of the Pacific Conference Series},
	title = {{XSPEC: The First Ten Years}},
	volume = 101,
	year = 1996}

@article{ajello08,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...673...96A},
	archiveprefix = {arXiv},
	author = {{Ajello}, M. and {Rau}, A. and {Greiner}, J. and {Kanbach}, G. and {Salvato}, M. and {Strong}, A.~W. and {Barthelmy}, S.~D. and {Gehrels}, N. and {Markwardt}, C.~B. and {Tueller}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:49:24 +0200},
	doi = {10.1086/524104},
	eprint = {0709.4333},
	journal = {\apj},
	keywords = {Galaxies: Active, Surveys, X-Rays: Binaries, X-Rays: Galaxies},
	month = jan,
	pages = {96-113},
	title = {{The Swift BAT X-Ray Survey. III. X-Ray Spectra and Statistical Properties}},
	volume = 673,
	year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/524104}}

@article{croton06a,
	adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006MNRAS.369.1808C&db_key=AST},
	author = {{Croton}, D.~J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2006.10429.x},
	eprint = {arXiv:0512375},
	journal = {\mnras},
	month = jul,
	pages = {1808-1812},
	title = {{Evolution in the black hole mass-bulge mass relation: a theoretical perspective}},
	volume = {369},
	year = {2006},
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10429.x}}

@article{norris11,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...736...55N},
	archiveprefix = {arXiv},
	author = {{Norris}, R.~P. and {Afonso}, J. and {Cava}, A. and {Farrah}, D. and {Huynh}, M.~T. and {Ivison}, R.~J. and {Jarvis}, M. and {Lacy}, M. and {Mao}, M. and {Maraston}, C. and {Mauduit}, J.-C. and {Middelberg}, E. and {Oliver}, S. and {Seymour}, N. and {Surace}, J.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1088/0004-637X/736/1/55},
	eprint = {1105.0960},
	journal = {\apj},
	keywords = {galaxies: evolution, galaxies: formation, galaxies: starburst},
	month = jul,
	pages = {55-+},
	primaryclass = {astro-ph.CO},
	title = {{Deep Spitzer Observations of Infrared-faint Radio Sources: High-redshift Radio-loud Active Galactic Nuclei?}},
	volume = 736,
	year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/736/1/55}}

@article{sikora07,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...658..815S},
	author = {{Sikora}, M. and {Stawarz}, {\L}. and {Lasota}, J.-P.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1086/511972},
	eprint = {arXiv:astro-ph/0604095},
	journal = {\apj},
	keywords = {Galaxies: Jets, Magnetohydrodynamics: MHD, Radiation Mechanisms: Nonthermal},
	month = apr,
	pages = {815-828},
	title = {{Radio Loudness of Active Galactic Nuclei: Observational Facts and Theoretical Implications}},
	volume = 658,
	year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/511972}}

@article{best06,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.368L..67B},
	author = {{Best}, P.~N. and {Kaiser}, C.~R. and {Heckman}, T.~M. and {Kauffmann}, G.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1745-3933.2006.00159.x},
	eprint = {arXiv:astro-ph/0602171},
	journal = {\mnras},
	keywords = {galaxies: active, galaxies: evolution, galaxies: stellar content, accretion, radio continuum: galaxies},
	month = may,
	pages = {L67-L71},
	title = {{AGN-controlled cooling in elliptical galaxies}},
	volume = 368,
	year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2006.00159.x}}

@article{clemens10,
	adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.405..887C},
	archiveprefix = {arXiv},
	author = {{Clemens}, M.~S. and {Scaife}, A. and {Vega}, O. and {Bressan}, A.},
	date-added = {2021-04-22 17:45:04 +0200},
	date-modified = {2021-04-22 17:45:04 +0200},
	doi = {10.1111/j.1365-2966.2010.16534.x},
	eprint = {1002.3334},
	journal = {\mnras},
	keywords = {galaxies: active, infrared: galaxies, radio continuum: galaxies},
	month = jun,
	pages = {887-897},
	primaryclass = {astro-ph.GA},
	title = {{Starburst evolution: free-free absorption in the radio spectra of luminous IRAS galaxies}},
	volume = 405,
	year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.16534.x}}

